Network Inspection for Detecting Strategic Attacks

This article studies a problem of strategic network inspection, in which a defender (agency) is tasked with detecting the presence of multiple attacks in the network. An inspection strategy entails monitoring the network components, possibly in a randomized manner, using a given number of detectors. We formulate the network inspection problem $(\mathcal{P})$ as a large-scale bilevel optimization problem, in which the defender seeks to determine an inspection strategy with minimum number of detectors that ensures a target expected detection rate under worst-case attacks. We show that optimal solutions of $(\mathcal{P})$ can be obtained from the equilibria of a large-scale zero-sum game. Our equilibrium analysis involves both game-theoretic and combinatorial arguments, and leads to a computationally tractable approach to solve $(\mathcal{P})$. Firstly, we construct an approximate solution by utilizing solutions of minimum set cover (MSC) and maximum set packing (MSP) problems, and evaluate its detection performance. In fact, this construction generalizes some of the known results in network security games. Secondly, we leverage properties of the optimal detection rate to iteratively refine our MSC/MSP-based solution through a column generation procedure. Computational results on benchmark water networks demonstrate the scalability, performance, and operational feasibility of our approach. The results indicate that utilities can achieve a high level of protection in large-scale networks by strategically positioning a small number of detectors.

==> E-Companion_v22.tex <==
%!TEX root = OR Manuscript V23.tex



%% Here starts the e-companion (EC)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ECSwitch

%\ECDisclaimer
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Main head for the e-companion
\ECHead{Proofs of Statements}

%\tr{Notation $\rho$ (maybe node basis)}



\section{Preliminary Results}
 
 
First, we define the following quantities: 
%For a given \defender's sensing strategy, the following quantities enable us to represent the nodes that are sensed, along with the probabilities of being sensed.
For a strategy $\sigma^1\in \Delta(\mathcal{A}_1)$ of \defender, the \emph{inspection probability} of node $i \in \nodes$, denoted $\nprob$, is the probability with which $i$ is inspected, i.e.:
%the probability with which $i$ is sensed by $\sigma^1$, i.e.:
\begin{align}
&\forall \sigma^1 \in \Delta(\mathcal{A}_1), \ \forall i \in \nodes,  \ \quad \nprob := \mathbb{E}_{\sigma^1}\left[\mathds{1}_{\{i \in \Def\}}\right] = \sum_{\{\Def \in \mathcal{A}_1 \, | \, i \in \Def\}}\sigma^1_{\Def} .\label{rho_sigma1}
\end{align}
%\item[--] The \emph{node basis} of a strategy $\sigma^1 \in \Delta(\mathcal{A}_1)$, denoted  $\nbasis{\sigma^1}$, is the set of nodes  with non-zero sensing probability, i.e.:
%\begin{align}
%\forall \sigma^1 \in \Delta(\mathcal{A}_1), \ \quad \nbasis{\sigma^1} := \{i \in \nodes \ | \ \nprob >0\}.\label{node basis}
%\end{align}
%\end{itemize}
%\end{definition}


%In other words, if \defender chooses a strategy $\sigma^1 \in \Delta(\mathcal{A}_1)$, then $\rho_{\sigma^1}(i)$ gives the probability with which the node $i \in \nodes$ is sensed, and $\nbasis{\sigma^1}$ represents the set of nodes that are sensed with positive probability. 

%\tb{Recall that \defender assigns a probability distributions over subsets of nodes, some of which may overlap. The sensing probability enables to translate \defender's strategy to individual node probabilities (or to shift the point of view from subset of nodes towards individual nodes...).}

%We can define analogous quantities for a given attack strategy of \attacker:
%Analogously, for a given \attacker's strategy, we can represent the components that are targeted by \attacker, along with the probabilities of being targeted.

%\begin{definition}[Attack Probability]\label{main_def_p2}\
%\begin{itemize}
%\item[--] 
Given a strategy $\sigma^2 \in \Delta(\mathcal{A}_2)$, the \emph{attack probability} of component $e \in \edges$, denoted $\eprob$, is the probability with which $e$ is targeted by $\sigma^2$, i.e.:
\begin{align}
&\forall \sigma^2 \in \Delta(\mathcal{A}_2), \ \forall e \in \edges, \ \quad \eprob := \mathbb{E}_{\sigma^2}\left[\mathds{1}_{\{e \in \att\}}\right]  = \sum_{\{\att \in \mathcal{A}_2 \, | \, e \in \att\}}\sigma^2_{\att} .\label{rho_sigma2}
\end{align}
%\item[--] The \emph{edge basis} of a strategy $\sigma^2 \in \Delta(\mathcal{A}_2)$, denoted $\ebasis{\sigma^2}$, is the set of components with non-zero attack probability, i.e.:
%\begin{align*}
%&\forall \sigma^2 \in \Delta(\mathcal{A}_2), \ \quad \ebasis{\sigma^2} := \{e \in \edges \ | \ \eprob >0\}.
%\end{align*}
%\end{itemize}
%\end{definition}
%\begin{align}
%\begin{array}{ccc}
%\text{minimize} & \displaystyle \sum_{i \in \nodes}x_i&\\
%\text{subject to} & \bs{F}^T\bs{x} \geq \bs{1}&\\
%& x_i \in \{0,1\}, & \forall i \in \nodes.
%\end{array}%\label{IP1}
%\end{align}
%or


%\begin{align}
%\begin{array}{ccc}
%\text{maximize} & \displaystyle \sum_{e \in \edges}y_e&\\
%\text{subject to} & \bs{F}\bs{y} \leq \bs{1}&\\
%& y_e \in \{0,1\}, & \forall e \in \edges.
%\end{array}%\label{IP2}
%\end{align}
%or

%\begin{lemma}\label{evil intersection}
%The monitoring sets satisfy the following properties:
%\begin{align}
%\forall (\Def,\Def^\prime) \in (2^\nodes)^2, \quad &\set{\Def\cup\Def^\prime} = \set{\Def} \cup \set{\Def^\prime},\label{nice union}\\
%&\set{\Def\cap\Def^\prime} \subseteq \set{\Def} \cap \set{\Def^\prime}, \label{bad intersection}
%%&\Def \subseteq \Def^{\prime} \ \Longrightarrow \ \set{\Def} \subseteq \set{\Def^\prime}. \label{nice inclusion}
%\end{align}
%\end{lemma}

%\proof{Proof of Lemma~\ref{evil intersection}.}\
%\begin{enumerate}
%\item
%Trivially, we have: $\forall  (\Def,\Def^\prime) \in (2^\nodes)^2, \ \set{\Def\cup\Def^\prime} = \bigcup_{i \in \Def\cup\Def^\prime}\set{i} = \left(\bigcup_{i \in \Def}\set{i}\right) \bigcup \left(\bigcup_{i \in \Def^\prime}\set{i} \right) = \set{\Def} \cup \set{\Def^\prime}.$
%
%\item
%Now, consider two sensor placements $\Def, \Def^\prime \in 2^\nodes$, and consider a component $e \in \edges$. \\
%If $e \in \set{\Def\cap\Def^\prime} = \cup_{i \in \Def\cap\Def^\prime}\set{i}$, then $\exists \, i \in \Def\cap\Def^\prime \ | \ e \in \set{i}$. Since $i \in \Def\cap\Def^\prime$, we deduce that $\set{i} \subseteq \set{\Def}$ and $\set{i} \subseteq \set{\Def^\prime}$. Therefore, $e \in \set{\Def}\cap\set{\Def^\prime}$. Since this is true for any $e \in \set{\Def\cap\Def^\prime}$, we showed that $\set{\Def\cap\Def^\prime} \subseteq \set{\Def}\cap\set{\Def^\prime}$.
%
%%\item Consider $(\Def,\Def^{\prime}) \in (2^\nodes)^2 \ | \ \Def \subseteq \Def^{\prime}$. Then: $\set{\Def} = \bigcup_{i \in \Def}\set{i} \subseteq \bigcup_{i \in \Def^\prime}\set{i} = \set{\Def^{\prime}}.$
%\end{enumerate}
%\vspace{-0.5cm}
%\hfill \Halmos
%\endproof

\ifadditional
Note that the reversed inclusion $\set{\Def\cap\Def^\prime} \supseteq \set{\Def} \cap \set{\Def^\prime}$ does not hold in general (which is the main reason why $\valdet{\cdot}{\att}$ is submodular and not modular). Next, we use the properties of the monitoring sets to derive the properties of the sensing function $\detect$.

\else
\fi

%\vspace{-0.1cm}
%\color{blue}
\begin{lemma}\label{Submodularity}
The detection function defined in \eqref{detect_sets} satisfies the following properties:
\begin{enumerate}
\item For any subset of components $\att \in 2^\edges$, $\valdet{\cdot}{\att}$ is submodular and monotone:
\vspace{-0.1cm}
\begin{align}
\forall \att \in 2^\edges, \ \forall (\Def,\Def^\prime) \in (2^\nodes)^2, \
&\valdet{\Def \cup \Def^\prime}{\att} + \valdet{\Def \cap \Def^\prime}{\att} \leq \valdet{\Def}{\att} + \valdet{\Def^\prime}{\att},\label{submodular_inequality}\\
&\Def \subseteq \Def^\prime \ \Longrightarrow\ \valdet{\Def }{\att} \leq \valdet{\Def^\prime}{\att}.\label{monotonicity_detection}
\end{align}
%\begin{align*}
%\forall \att \in 2^\edges, \ \forall (\Def,\Def^\prime) \in (2^\nodes)^2 \ | \ 
%\end{align*}

\item For any detector positioning $\Def \in 2^\nodes$, $\valdet{\Def}{\cdot}$ is finitely additive:
\vspace{-0.1cm}
\begin{align}
\forall \Def \in 2^\nodes,\ \forall (\att,\att^\prime) \in (2^\edges)^2 \ | \ \att \cap \att^\prime = \emptyset, \quad \valdet{\Def}{\att \cup \att^\prime} = \valdet{\Def}{\att} + \valdet{\Def}{\att^\prime}.\label{additive_equality}
\end{align}
%\item Since $\detect$ is nonnegative, then we can also deduce that $\valdet{\cdot}{\att}$ is fractionally subadditive:
%\begin{align*}
%\forall \att \in 2^\edges, \ 
%\end{align*}
\end{enumerate}
\end{lemma}
%\color{black}
\proof{Proof of Lemma~\ref{Submodularity}.}\
\begin{enumerate}
\item %Let us show the submodularity and the monotonicity of $\detect$ with respect to the first variable. 
Consider a subset of components $\att \in 2^\edges$, and a pair of detector positionings $(\Def,\Def^\prime) \in (2^\nodes)^2$. Then, $\set{\Def\cup\Def^\prime} =\set{\Def} \cup \set{\Def^\prime}$ and $\set{\Def\cap\Def^\prime} \subseteq \set{\Def}\cap\set{\Def^\prime}$, and we obtain:
%
%
%
%Trivially, we have: $\forall  (\Def,\Def^\prime) \in (2^\nodes)^2, \ \set{\Def\cup\Def^\prime} = \bigcup_{i \in \Def\cup\Def^\prime}\set{i} = \left(\bigcup_{i \in \Def}\set{i}\right) \bigcup \left(\bigcup_{i \in \Def^\prime}\set{i} \right) = \set{\Def} \cup \set{\Def^\prime}.$
%
%%\item
%Now, consider two sensor placements $\Def, \Def^\prime \in 2^\nodes$, and consider a component $e \in \edges$. \\
%If $e \in \set{\Def\cap\Def^\prime} = \cup_{i \in \Def\cap\Def^\prime}\set{i}$, then $\exists \, i \in \Def\cap\Def^\prime \ | \ e \in \set{i}$. Since $i \in \Def\cap\Def^\prime$, we deduce that $\set{i} \subseteq \set{\Def}$ and $\set{i} \subseteq \set{\Def^\prime}$. Therefore, $e \in \set{\Def}\cap\set{\Def^\prime}$. Since this is true for any $e \in \set{\Def\cap\Def^\prime}$, we showed that $\set{\Def\cap\Def^\prime} \subseteq \set{\Def}\cap\set{\Def^\prime}$.
%
%
\vspace{-0.1cm}
\begin{align*}
&\valdet{\Def \cup \Def^\prime}{\att} + \valdet{\Def \cap \Def^\prime}{\att} \overset{\eqref{detect_sets}}{=} |\set{\Def \cup \Def^\prime} \cap \att| + |\set{\Def \cap \Def^\prime} \cap \att| = |(\set{\Def} \cap \att) \cup (\set{\Def^\prime} \cap \att)| + |\set{\Def \cap \Def^\prime} \cap \att|\nonumber\\
& = |\set{\Def} \cap \att| + |\set{\Def^\prime} \cap \att| - |\set{\Def} \cap \set{\Def^\prime}\cap \att| + |\set{\Def \cap \Def^\prime} \cap \att| \leq|\set{\Def} \cap \att| + |\set{\Def^\prime} \cap \att| \overset{\eqref{detect_sets}}{=} \valdet{\Def}{\att} + \valdet{\Def^\prime}{\att}.
\end{align*}


%\item
Furthermore, if $\Def \subseteq \Def^\prime$, then: $\valdet{\Def}{\att} \overset{\eqref{detect_sets}}{=} |\set{\Def} \cap \att| \leq  |\set{\Def^\prime} \cap \att| \overset{\eqref{detect_sets}}{=}\valdet{\Def^{\prime}}{\att}.$


\item %Now, let us show the additivity of $\detect$ with respect to the second variable. 
Consider a detector positioning $\Def \in 2^\nodes$. Then: $\forall (\att,\att^\prime) \in (2^\edges)^2 \ | \ \att \cap \att^\prime = \emptyset, \quad \valdet{\Def}{\att \cup \att^\prime} \overset{\eqref{detect_sets}}{=} |\set{\Def}\cap (\att \cup \att^\prime)| = |\set{\Def} \cap \att| +|\set{\Def} \cap \att^\prime| - |\set{\Def} \cap \att \cap \att^\prime|  \overset{\eqref{detect_sets}}{=} \valdet{\Def}{\att} + \valdet{\Def}{\att^\prime}.$\hfill \Halmos
%\begin{align*}
%\forall (\att,\att^\prime) \in (2^\edges)^2 \ | \ \att \cap \att^\prime = \emptyset, \quad \valdet{\Def}{\att \cup \att^\prime} &\overset{\eqref{detect_sets}}{=} |\set{\Def}\cap (\att \cup \att^\prime)| = |\set{\Def} \cap \att| +|\set{\Def} \cap \att^\prime| - \underset{=0}{\underbrace{|\set{\Def} \cap \att \cap \att^\prime| }}\nonumber \\[-0.1cm]
%&\overset{\eqref{detect_sets}}{=} \valdet{\Def}{\att} + \valdet{\Def}{\att^\prime}.
%\end{align*}
\end{enumerate}
%\vspace{-1.05cm}
%\hfill \Halmos
\endproof

%We now derive additional properties of the detection function that will be used in our analysis.

\begin{corollary}\label{useful_(in)equalities}
The detection function defined in \eqref{detect_sets} satisfies the following properties:
%\begin{enumerate}[(i)]
%\item S
%\item
%\item
%\begin{align*}
%\forall (\Def,\att) \in 2^\nodes \times 2^\edges, \ \valdet{\Def}{\att} \overset{\eqref{detect_sets}}{=}\sum_{e \in \att} \mathds{1}_{\{e \in \set{\Def}\}} =  \sum_{e \in \att} \valdet{\Def}{e}.
%\end{align*}
%\end{enumerate}
\begin{align}
\forall (\Def,\att) \in 2^{\nodes} \times 2^\edges, \ \valdet{\Def}{\att} \leq \sum_{i\in \Def}\valdet{i}{\att}, \label{redundant_nodes}\\
\forall (\Def,\att) \in 2^\nodes \times 2^\edges, \ \valdet{\Def}{\att} = \sum_{e \in \att} \valdet{\Def}{e}. \label{detection_disruptions}
%\forall \att \in 2^\edges, \ \forall (\Def,\Def^{\prime}) \in (2^\nodes)^2 \ | \  \Def \subseteq \Def^{\prime}, \ \valdet{\Def}{\att} \leq \valdet{\Def^{\prime}}{\att}. \label{monotonicity_detection}
\end{align}
\end{corollary}
\vspace{-0.0cm}
\proof{Proof of Corollary~\ref{useful_(in)equalities}.}\
\begin{enumerate}
\item  
Consider $\att \in 2^\edges$. Since $\valdet{\cdot}{\att}$ is a submodular and nonnegative function, then $\valdet{\cdot}{\att}$ is subadditive, i.e., $\forall (\Def,\Def^\prime) \in (2^\nodes)^2, \ \valdet{\Def\cup\Def^\prime}{\att} \leq \valdet{\Def}{\att} + \valdet{\Def^{\prime}}{\att}$. 

%
%First, note that $\valdet{\cdot}{\att}$ is normalized, i.e., $\valdet{\emptyset}{\att} = |\cup_{i \in \emptyset}\set{i} \cap \att| = 0$. Besides, since $\valdet{\cdot}{\att}$ is submodular (Lemma~\ref{Submodularity}), we have:
%\begin{align*}
%\forall (\Def,\Def^\prime) \in (2^\nodes)^2 \ | \ \Def \cap \Def^\prime = \emptyset, \ \valdet{\Def\cup\Def^\prime}{\att} = \valdet{\Def\cup\Def^\prime}{\att} + \underset{= 0}{\underbrace{\valdet{\Def\cap\Def^\prime}{\att}}} \overset{\eqref{submodular_inequality}}{\leq} \valdet{\Def}{\att} + \valdet{\Def^{\prime}}{\att}.
%\end{align*}

Therefore, by induction, we obtain: $\forall \Def \in 2^\nodes, \ \valdet{\Def}{\att} = \valdet{\cup_{i \in \Def}\{i\}}{\att} \leq \sum_{i \in \Def}\valdet{i}{\att}.$

\item Consider $\Def \in 2^\nodes$. Since $\valdet{\Def}{\cdot}$ is additive (Lemma~\ref{Submodularity}), we obtain by induction that $\forall \att \in 2^\edges, \ \valdet{\Def}{\att} = \valdet{\Def}{\cup_{e \in \att}\{e\}} \overset{\eqref{additive_equality}}{=} \sum_{e \in \att}\valdet{\Def}{e}$. \hfill \Halmos
%\begin{align*}
%\forall \att \in 2^\edges, \ \valdet{\Def}{\att} = \valdet{\Def}{\cup_{e \in \att}\{e\}} \overset{\eqref{additive_equality}}{=} \sum_{e \in \att}\valdet{\Def}{e}. 
%\end{align*}
%Consider $(\Def,e) \in 2^{\nodes} \times \edges$. Recall that $\valdet{\Def}{e} \overset{\eqref{detect_sets}}{=} \mathds{1}_{\{e \in \set{\Def}\}}$, and $\set{\Def} = \cup_{i \in \Def}\,\set{i}$. We consider two cases. If $e \in \set{\Def}$, then $\valdet{\Def}{e} = 1$ and $\exists \, i \in \Def \ | \ e \in \set{i}$, which implies that $\sum_{i \in \Def}\valdet{i}{e} \geq 1 = \valdet{\Def}{e}$. If $e \notin \set{\Def}$, then we have $ e \notin \set{i}, \ \forall i \in \Def$, which implies that $\valdet{\Def}{e} = 0 = \sum_{i \in \Def}\valdet{i}{e}$.
%\begin{enumitemize}
%\item[--]  If $e \in \set{\Def}$, then $\valdet{\Def}{e} = 1$ and $\exists \, i \in \Def \ | \ e \in \set{i}$, which implies that $$\sum_{i \in \Def}\valdet{i}{e} \geq 1 = \valdet{\Def}{e}$$. 
%\item[--] Case 2: If $e \notin \set{\Def}$, then we have $ e \notin \set{i}, \ \forall i \in \Def$, which implies that $\valdet{\Def}{e} = 0 = \sum_{i \in \Def}\valdet{i}{e}$.
%\end{enumitemize}
%since $\set{\Def} \subseteq \set{\Def^{\prime}}$.
\end{enumerate}
%\vspace{-0.8cm}
\endproof




\begin{lemma}\label{weights_in_bags}
Given an inspection strategy $\sigma^{1} \in \Delta(\mathcal{A}_1)$, let $\{i_1,\dots,i_n\} \in 2^\nodes$ denote a set that contains its node basis $\nbasis{\sigma^1}$ and such that $\rho_{\sigma^1}(i_1) \leq \dots \leq \rho_{\sigma^1}(i_n)$. Then, we have the following inequality:
\vspace{-0.5cm}
\begin{align}
\forall b \in \llbracket 1,n\rrbracket, \ \sum_{k=1}^{b} \rho_{\sigma^1}(i_k) \leq \frac{b}{n}\mathbb{E}_{\sigma^1}[|\Def|]. \label{worst_bags}
\end{align}

Similarly, given an attack strategy $\sigma^{2} \in \Delta(\mathcal{A}_2)$, let $\{e_1,\dots,e_m\} \in 2^\edges$ denote a set that contains its component basis $\ebasis{\sigma^2}$, and such that $\rho_{\sigma^2}(e_1) \geq \dots \geq \rho_{\sigma^2}(e_m)$. Then, we have the following inequality:
%\vspace{-0.5cm}
\begin{align}
\forall b \in \llbracket 1,m\rrbracket, \ \sum_{l=1}^{b} \rho_{\sigma^2}(e_l) \geq \frac{b}{m}\mathbb{E}_{\sigma^2}[|\att|]. \label{best_bags}
\end{align}
\end{lemma}
\proof{Proof of Lemma \ref{weights_in_bags}.}\
%\begin{enumerate}[i)]
%\item
Consider an inspection strategy $\sigma^1 \in \Delta(\mathcal{A}_1)$, and a set of nodes $\{i_1,\dots,i_n\} \in 2^\nodes$ such that $\nbasis{\sigma^1} \subseteq \{i_1,\dots,i_n\}$ and $\rho_{\sigma^1}(i_1) \leq \dots \leq \rho_{\sigma^1}(i_n)$. We show the result by contradiction: let us assume that $\exists\, b \in \llbracket 1,n\rrbracket \ | \ \sum_{k=1}^{b} \rho_{\sigma^1}(i_k) > \frac{b}{n}\mathbb{E}_{\sigma^1}[|\Def|]$. 

First, we can deduce the following inequality:
\begin{align}
\rho_{\sigma^1}(i_{b}) = \frac{1}{b}\sum_{k=1}^b\rho_{\sigma^1}(i_b) \geq \frac{1}{b}\sum_{k=1}^{b} \rho_{\sigma^1}(i_k) > \frac{b\mathbb{E}_{\sigma^1}[|\Def|]}{b n} = \frac{\mathbb{E}_{\sigma^1}[|\Def|]}{n}.\label{1st step to contradiction}
\end{align}

Besides, since $\nbasis{\sigma^1} \subseteq \{i_1,\dots,i_n\}$, then $\forall\Def \in \supp(\sigma^1), \ \Def \subseteq \{i_1,\dots,i_n\}$ and we have the following equality: $\forall \Def \in \supp(\sigma^1), \ |\Def| = \sum_{k=1}^n \mathds{1}_{\{i_k \in \Def \}}$. This enables us to obtain the following contradiction:
%\vspace{-0.5cm}
%\begin{align}
%\forall \Def \in \supp(\sigma^1), \ |\Def| = \sum_{k=1}^n \mathds{1}_{\{i_k \in \Def \}}.\label{2nd step to contradiction}
%\end{align}
%
%Then, we obtain the following contradiction:
%\begin{align*}
%\mathbb{E}_{\sigma^1}[|\Def|]& = \sum_{\Def \in \mathcal{A}_1} \sigma_{\Def}^1 |\Def| \overset{\eqref{2nd step to contradiction}}{=} \sum_{\Def \in \mathcal{A}_1} \sigma_{\Def}^1 \sum_{k=1}^n \mathds{1}_{\{i_k \in \Def\}} = \sum_{k=1}^n\sum_{\Def \in \mathcal{A}_1} \sigma_{\Def}^1\mathds{1}_{\{i_k \in \Def\}} \overset{\eqref{rho_sigma1}}{=} \sum_{k=1}^n \rho_{\sigma^1}(i_k) \\
%&=  \sum_{k=1}^{b} \rho_{\sigma^1}(i_k) + \sum_{b+1}^n  \rho_{\sigma^1}(i_k) > \frac{b\mathbb{E}_{\sigma^1}[|\Def|]}{n} +  \sum_{b+1}^n  \rho_{\sigma^1}(i_{b}) = \frac{b \mathbb{E}_{\sigma^1}[|\Def|]}{n} + (n-b) \rho_{\sigma^1}(i_{b})  \\
%&\overset{\eqref{1st step to contradiction}}{>} \frac{b\mathbb{E}_{\sigma^1}[|\Def|]}{n}+(n-b) \frac{\mathbb{E}_{\sigma^1}[|\Def|]}{n} = \mathbb{E}_{\sigma^1}[|\Def|].
%\end{align*}
\begin{align*}
\mathbb{E}_{\sigma^1}[|\Def|]& = \sum_{k=1}^n  \mathbb{E}_{\sigma^1}[ \mathds{1}_{\{i_k \in \Def \}}] \overset{\eqref{rho_sigma1}}{=}  \sum_{k=1}^{b} \rho_{\sigma^1}(i_k) + \sum_{b+1}^n  \rho_{\sigma^1}(i_k) > \frac{b \mathbb{E}_{\sigma^1}[|\Def|]}{n} + (n-b) \rho_{\sigma^1}(i_{b})  \overset{\eqref{1st step to contradiction}}{>} \mathbb{E}_{\sigma^1}[|\Def|].
\end{align*}

Therefore, $\forall b \in \llbracket 1,n \rrbracket, \ \sum_{k=1}^{b} \rho_{\sigma^1}(i_k) \leq \frac{b}{n}\mathbb{E}_{\sigma^1}[|\Def|]$.
\eqref{best_bags} can be analogously proved.
%\item \tr{[Remove since it is the very similar to i)]}
%Now, let us show that $\forall b \in \llbracket 1,m\rrbracket, \ \sum_{l=1}^{b} \rho_{\sigma^2}(e_l) \geq \frac{b}{m}\mathbb{E}_{\sigma^2}[|\att|]$. Instead, assume that $\exists \, b \in \llbracket 1,m\rrbracket \ | \ \sum_{l=1}^{b} \rho_{\sigma^2}(e_k) < \frac{b}{m}\mathbb{E}_{\sigma^2}[|\att|]$. Similarly, we deduce the following inequality:
%\begin{align}
%\rho_{\sigma^2}(e_{b})= \frac{1}{b}\sum_{l=1}^{b} \rho_{\sigma^2}(e_b)\leq \frac{1}{b}\sum_{l=1}^{b} \rho_{\sigma^2}(e_l) < \frac{b\mathbb{E}_{\sigma^2}[|\att|]}{b m} = \frac{\mathbb{E}_{\sigma^2}[|\att|]}{m}.\label{1st step again}
%\end{align}
%
%Moreover, since $\ebasis{\sigma^2} \subseteq \{e_1,\dots,e_m\}$, we have:
%\begin{align}
%\forall \att \in \supp(\sigma^2), \ |\att| = \sum_{l=1}^m \mathds{1}_{\{e_l \in \att\}}. \label{2nd step again}
%\end{align}
%
%Then, we obtain the following contradiction:
%\begin{align*}
%\mathbb{E}_{\sigma^2}[|\att|]& = \sum_{\att\in \mathcal{A}_2} \sigma_{\att}^2 |\att|  \overset{\eqref{2nd step again}}{=} \sum_{\att \in \mathcal{A}_2} \sigma_{\att}^2 \sum_{l=1}^m \mathds{1}_{\{e_l \in \att\}} = \sum_{l=1}^m\sum_{\att \in \mathcal{A}_2} \sigma_{\att}^2\mathds{1}_{\{e_l \in \att\}} \\
%&\overset{\eqref{rho_sigma2}}{=} \sum_{l=1}^m \rho_{\sigma^2}(e_l) =  \sum_{l=1}^{b} \rho_{\sigma^2}(e_l) + \sum_{b+1}^m  \rho_{\sigma^2}(e_l) \\
%&< \frac{b\mathbb{E}_{\sigma^2}[|\att|]}{m} +  \sum_{b+1}^m  \rho_{\sigma^2}(e_{b}) = \frac{b\mathbb{E}_{\sigma^2}[|\att|]}{m} + (m-b) \rho_{\sigma^2}(e_{b})  \\
%&\overset{\eqref{1st step again}}{<} \frac{b\mathbb{E}_{\sigma^2}[|\att|]}{m}+(m-b) \frac{\mathbb{E}_{\sigma^2}[|\att|]}{m} \\
%&=\mathbb{E}_{\sigma^2}[|\att|].
%\end{align*}
%%which is a contradiction.
%
%Therefore, $\forall b \in \llbracket 1,m \rrbracket, \ \sum_{l=1}^{b} \rho_{\sigma^2}(e_l) \geq \frac{b}{m}\mathbb{E}_{\sigma^2}[|\att|]$.
%\end{enumerate}
\hfill \Halmos
\endproof


\begin{lemma}\label{strategic_eq}
$\Gamma$ is strategically equivalent to the game $\widetilde{\Gamma} := \langle \{1,2\}, (\mathcal{A}_1, \mathcal{A}_2), (-u_2,u_2) \rangle$.
%where the payoff of \defender is the opposite of the number of undetected failure events, i.e.:
%\begin{align}
%\forall (\Def,\att) \in \mathcal{A}_1 \times \mathcal{A}_2, \ \widetilde{u}_1(\Def,\att) := \valdet{\Def}{\att} - |\att| = - u_2(\Def,\att).
%\label{u1_tilde}
%\end{align}
%Therefore, the NE of $\Gamma$ can be obtained by solving the following two linear programming problems:
%\begin{align*}\begin{array}{llcr}(\text{LP}_1) &\text{maximize}  & z &\mcr&\text{subject to} & \widetilde{U}_1(\sigma^1,\att) \geq z, & \forall \att \in \mathcal{A}_2 \mcr && \sigma^1 \in \Delta(\mathcal{A}_1) &\end{array}
%\quad
%\vrule{} \quad
%\begin{array}{llcr}(\text{LP}_2) &\text{maximize} & z^{\prime} &\mcr&\text{subject to} & \widetilde{U}_2(\Def,\sigma^2) \geq z^{\prime}, & \forall \Def \in \mathcal{A}_1 \mcr && \sigma^2 \in \Delta(\mathcal{A}_2) &\end{array}
%\end{align*}
%\begin{align*}
%(\text{LP}_1)  \quad \displaystyle \max_{\sigma^1 \in \Delta(\mathcal{A}_1)} \min_{\att \in \mathcal{A}_2} -{U}_2(\sigma^1,\att) \quad\quad \quad  \vrule{} \quad \quad \quad (\text{LP}_2) \quad \displaystyle \max_{\sigma^2 \in \Delta(\mathcal{A}_2)} \min_{\Def \in \mathcal{A}_1} {U}_2(\Def,\sigma^2).
%\end{align*}
%where ${U}_2$ is given by \eqref{payoff2}.
\end{lemma}

%\section{Proofs of Section \ref{sec:form}}
\proof{Proof of Lemma~\ref{strategic_eq}.}
Adding a term to \defender's payoff that only depends on \attacker's action does not change the NE of the game. Thus, the following transformation preserves the set of NE:
\begin{align}
&\forall (\Def,\att) \in \mathcal{A}_1 \times \mathcal{A}_2, \ u_1(\Def,\att) - |\att|  = \valdet{\Def}{\att} - |\att| = -u_2(\Def,\att). \label{transform1}
\end{align}



So $\Gamma(b_1,b_2)$ and $\widetilde{\Gamma}(b_1,b_2)$ are strategically equivalent, and have the same set of NE $\nash(b_1,b_2)$.
\hfill
\Halmos
\endproof

%\ifadditional
%From the interchangeability of NE in zero-sum games, if $({\sigma^1}^*,{\sigma^2}^*) \in \Sigma$ and $({\sigma^1}^{\dag},{\sigma^2}^{\dag})\in \Sigma$, then $({\sigma^1}^*,{\sigma^2}^{\dag})\in \Sigma$ and $({\sigma^1}^{\dag},{\sigma^2}^{*})\in \Sigma$; furthermore, $\Sigma$ is a convex set.
%\else
%\fi
%\section{Proofs of Section \ref{preliminaries}}

\begin{lemma}\label{MM<MSC}
The size of MSPs is no greater than the size of MSCs, i.e., $\semm \leq \smsc$.
\end{lemma}

\proof{Proof of Lemma~\ref{MM<MSC}.}
Consider an MSP $T^{max} = \{e_1,\dots,e_{\semm}\} \in \emm$ and an MSC $S^{min} = \{i_1,\dots,i_{\smsc}\} \in \msc$. Then, we have the desired inequality:
\begin{align*}
\semm &\overset{\eqref{def_minimum_set_cover}}{=} \sum_{l=1}^{\semm}\valdet{S^{min}}{e_l} \overset{\eqref{redundant_nodes}}{\leq} \sum_{l=1}^{\semm}\sum_{k=1}^{\smsc} \valdet{i_k}{e_l} =\sum_{k=1}^{\smsc} \sum_{l=1}^{\semm} \valdet{i_k}{e_l} \overset{\eqref{detection_disruptions}}{=}  \sum_{k=1}^{\smsc}\valdet{i_k}{T^{max}} \overset{\eqref{def_extended_matching}}{\leq} \smsc.%\hfill\Halmos
\end{align*}
%Consider an MSP $T^{max} \in \emm$ and an MSC $S^{min} \in \msc$. Then, we have the desired inequality:
%\begin{align*}
%\semm &\overset{\eqref{def_minimum_set_cover}}{=} \sum_{e \in \att^{max}}\valdet{S^{min}}{e} \overset{\eqref{redundant_nodes}}{\leq} \sum_{e \in \att^{max}}\sum_{i \in \Def^{min}} \valdet{i}{e} =\sum_{i \in \Def^{min}} \sum_{e \in \att^{max}} \valdet{i}{e} \overset{\eqref{detection_disruptions}}{=}  \sum_{i \in \Def^{min}}\valdet{i}{T^{max}} \overset{\eqref{def_extended_matching}}{\leq} \smsc.
%\end{align*}
%where the first inequality comes from $\{i_1,\dots,i_{\smsc}\}$ covering the whole network and the second inequality comes from $\{e_1,\dots,e_{\semm}\}$ being a maximum matching.

\vspace{-0.8cm}
\hfill\Halmos
\endproof


%\section{Integer Programming Formulations}\label{IPs}
%
%
%To concisely represent the sensing model $\mathcal{G} = (\nodes,\edges,\{\set{i}, \ i \in \nodes\})$ defined in Section~\ref{sec:detect}, we define the \emph{influence matrix} $\boldsymbol{F} = (\valdet{i}{e})_{(i,e) \in \nodes \times \edges}$. $\boldsymbol{F}$ is a $|\nodes| \times |\edges|$ binary matrix whose rows (resp. columns) are indexed by the nodes (resp. components) in the network. Thus, a given row of $\bs{F}$ indicates the components of the network that a sensor placed at the corresponding node monitors. Similarly, a given column of $\bs{F}$ indicates the locations from where a sensor is capable of monitoring the corresponding component.
%
%Then, solving (\hyperlink{(MSC)}{$\mathcal{I}_{\text{MSC}}$}) is equivalent to selecting a subset of rows of the influence matrix $\bs{F}$ of minimum cardinality such that each column of $\bs{F}$ is covered, i.e., it has at least one 1 entry in the selected subset of rows. This problem can be formulated as the following integer program:
%\begin{align}
%\def \arraystretch{\spacingarray}
%\begin{array}{ccc}
%\text{minimize} & \displaystyle \bs{1}_{|\nodes|}^T\,x&\\
%\text{subject to} & \bs{F}^Tx \geq \bs{1}_{|\edges|}&\\
%& x \in \{0,1\}^{|\nodes|}, &
%\end{array}\label{IP1}
%\end{align}
%where $\bs{1}_{|\nodes|}$ (resp. $\bs{1}_{|\edges|}$) represents the vector of length $|\nodes|$ (resp. $|\edges|$) filled with ones.
%
%%Besides, note that solving (\hyperlink{(MSC)}{MSC}) is equivalent to selecting a subset of rows of the influence matrix $\bs{F}$ of minimum cardinality such that each column of $\bs{F}$ is covered, i.e., it has at least one 1 entry in the selected subset of rows.
%
%
%Similarly, solving (\hyperlink{(MSP)}{$\mathcal{I}_{\text{MSP}}$}) is equivalent to selecting a subset of columns of $\bs{F}$ of maximum cardinality such that each row of $\bs{F}$ has at most one 1 entry in the selected subset of columns:
%\begin{align}
%\def \arraystretch{\spacingarray}
%\begin{array}{ccc}
%\text{maximize} & \displaystyle \bs{1}_{|\edges|}^T\,y&\\
%\text{subject to} & \bs{F}y \leq \bs{1}_{|\nodes|}&\\
%& y \in \{0,1\}^{|\edges|}. &
%\end{array}\label{IP2}
%\end{align}
%
%From \eqref{IP1} and \eqref{IP2}, it is easy to see that these integer programming formulations of (\hyperlink{(MSC)}{$\mathcal{I}_{\text{MSC}}$}) and (\hyperlink{(MSP)}{$\mathcal{I}_{\text{MSP}}$}) have linear programming relaxations that are dual of each other.


\ifadditional
\begin{example}

Consider the network shown in Fig.~\ref{Example1}. Assume a sensing model in which a sensor placed at any node can monitor edges at one-hop vertically, and at two hops horizontally. Thus, $\set{i_1} = \{e_1,e_2,e_3\}$, $\set{i_2} = \{e_1,e_2,e_4\}$, $\set{i_3} = \{e_1,e_2,e_5\}$, $\set{i_4} = \{e_4,e_6,e_7\}$, $\set{i_5} = \{e_5,e_6,e_8\}$, $\set{i_6} = \{e_3,e_9,e_{10}\}$, $\set{i_7} = \{e_7,e_9,e_{10}\}$, $\set{i_8} = \{e_8,e_9,e_{10}\}$.

\def \sizefig {1.4cm}
\def \scalefig {\small}
\def \innersepfig {0.07cm}
%%%---------------------------------------------------------------------------------------------------

\begin{figure}[ht]
\centering
{\scalefig
\begin{tikzpicture}[-,auto,x=\sizefig, y=\sizefig,
  thick,main node/.style={circle,draw,inner sep = \innersepfig,black},main node2/.style={circle,black,draw,fill=blue!60,inner sep = \innersepfig},flow_a/.style ={gray!100}]
\tikzstyle{edge} = [draw,thick,-,black]
\tikzstyle{cut} = [draw,very thick,-]
\tikzstyle{match} = [draw,very thick,black,-, dashed]
\tikzstyle{flow} = [draw,line width = 1.5pt,->,gray!100]

%\begin{scope}[yshift=0, xshift =-110]
	\node[main node] (1) at (0,2) {$i_1$};
	\node[main node] (2) at (1,2) {$i_2$};
	\node[main node2] (3) at (2,2) {$i_3$};
	\node[main node] (4) at (1,1) {$i_4$};
	\node[main node] (5) at (2,1) {$i_5$};
	\node[main node] (6) at (0,0) {$i_6$};
	\node[main node] (7) at (1,0) {$i_7$};
	\node[main node] (8) at (2,0) {$i_8$};
	%\node[main node, draw=white] (7) at (3.5,-0.5) {\textbf{a}};
	
	\path[edge]	
	%(2) edge (5)
	%(1) edge  (2)
	(1) edge node[left]{$e_3$} (6)
	(4) edge node {$e_6$} (5)
	(2) edge[double,blue!80]  node {$e_2$} (3)
	(2) edge node[left] {$e_4$} (4)
	(6) edge node[below] {$e_9$} (7)
	(7) edge node[below] {$e_{10}$} (8)
	%(3) edge  (5)	
	%(4) edge  (6)
	(5) edge node {$e_8$} (8);

	\path[edge]
	(1) edge[double,blue!80] node {$e_1$} (2)
	(3) edge[double,blue!80] node {$e_5$} (5)
	(4) edge node[left] {$e_7$} (7);
%\end{scope}

\end{tikzpicture}}

\caption{Example network. The monitoring set $\set{i_3} = \{e_1,e_2,e_5\}$ is represented by the double blue edges.} \label{Example1}
\end{figure}

\tr{Consider the example network in Section~\ref{example_detection_sensing}. Then, the corresponding influence matrix is given by:}
\begin{align*}
\bs{F} = \begin{array}{cc} & {\arraycolsep=3pt\begin{array}{cccccccccc} e_1 & e_2 & e_3 &e_4&e_5&e_6 & e_7 & e_8 &e_9 &e_{10}\end{array}}\vspace{0.1cm}\\
{\def\arraystretch{\spacinginfluence}\begin{array}{c}
i_1\\i_2\\i_3\\i_4\\i_5\\i_6\\i_7\\i_8\end{array}}&{\arraycolsep=5pt\def\arraystretch{\spacinginfluence}
  \left({\begin{array}{cccccccccc}
	1 & 1 & 1 & 0 & 0 & 0 &0 &0 &0 &0 \\
	1 & 1 & 0 & 1 & 0 & 0&0 &0  &0 &0\\
	 1 &  1 &  0 &  0 &  1 &  0 & 0 & 0&0 &0\\
	 0 &  0 &  0 &  1 &  0 &  1 & 1 & 0&0 &0\\
	 0 &  0 &  0 &  0 &  1 &  1 & 0 & 1&0 &0 \\
	0 & 0 & 1 & 0 & 0 & 0&0 &0&1 &1\\
	0 & 0 & 0 & 0 & 0 & 0&1 &0&1 &1\\
	0 & 0 & 0 & 0 & 0 & 0&0 &1&1 &1
  \end{array}}\right)}\end{array}
\end{align*}

As mentioned in Section~\ref{example_detection_sensing}, a solution of (\hyperlink{(MSC)}{$\mathcal{I}_{\text{MSC}}$}) is given by $\{i_3,i_4,i_6,i_8\}$ and a solution of (\hyperlink{(MSP)}{$\mathcal{I}_{\text{MSP}}$}) is given by $\{e_3,e_4,e_8\}$. They are illustrated in Fig.~\ref{influence_matrices}.
%The MSC (resp. MSP) solutions can also be obtained by choosing appropriate rows (resp. columns) of the influence matrix $\bs{F}$ (see Fig.~\ref{influence_matrices}).
\begin{figure}[ht]
\vspace{\spacingfigure}
\centering
%\renewcommand{\arraystretch}{0.4}
\begin{align*}
\begin{array}{cc} & {\arraycolsep=3pt\begin{array}{cccccccccc} e_1 & e_2 & e_3 &e_4&e_5&e_6 & e_7 & e_8 &e_9 &e_{10}\end{array}}\vspace{0.1cm}\\
{\def\arraystretch{\spacinginfluence}\begin{array}{c}
i_1\\i_2\\i_3\\i_4\\i_5\\i_6\\i_7\\i_8\end{array}}&{\arraycolsep=5pt\def\arraystretch{\spacinginfluence}
  \left({\begin{array}{cccccccccc}
	1 & 1 & 1 & 0 & 0 & 0 &0 &0 &0 &0 \\
	1 & 1 & 0 & 1 & 0 & 0&0 &0  &0 &0\\
	 \cellcolor{Green}1 &  \cellcolor{Green}1 &  \cellcolor{Green}0 &\cellcolor{Green}  0 &\cellcolor{Green}  1 &\cellcolor{Green}  0 &\cellcolor{Green} 0 &\cellcolor{Green} 0&\cellcolor{Green}0 &\cellcolor{Green}0\\
	 \cellcolor{Green}0 &\cellcolor{Green}  0 &\cellcolor{Green}  0 &\cellcolor{Green}  1 &\cellcolor{Green}  0 &\cellcolor{Green}  1 &\cellcolor{Green} 1 &\cellcolor{Green} 0&\cellcolor{Green}0 &\cellcolor{Green}0\\
	 0 &  0 &  0 &  0 &  1 &  1 & 0 & 1&0 &0 \\
	\cellcolor{Green}0 &\cellcolor{Green} 0 &\cellcolor{Green} 1 &\cellcolor{Green} 0 &\cellcolor{Green} 0 &\cellcolor{Green} 0&\cellcolor{Green}0 &\cellcolor{Green}0&\cellcolor{Green}1 &\cellcolor{Green}1\\
	0 & 0 & 0 & 0 & 0 & 0&1 &0&1 &1\\
	\cellcolor{Green}0 &\cellcolor{Green} 0 &\cellcolor{Green} 0 &\cellcolor{Green} 0 &\cellcolor{Green} 0 &\cellcolor{Green} 0&\cellcolor{Green}0 &\cellcolor{Green}1&\cellcolor{Green}1 &\cellcolor{Green}1
  \end{array}}\right)}\end{array}
  \quad \quad \quad
\begin{array}{cc} & {\arraycolsep=3pt\begin{array}{cccccccccc} e_1 & e_2 & e_3 &e_4&e_5&e_6 & e_7 & e_8 &e_9 &e_{10}\end{array}}\vspace{0.1cm}\\
{\def\arraystretch{\spacinginfluence}\begin{array}{c}
i_1\\i_2\\i_3\\i_4\\i_5\\i_6\\i_7\\i_8\end{array}}&{\arraycolsep=5pt\def\arraystretch{\spacinginfluence}
  \left({\begin{array}{cc>{\columncolor{red!50}}c>{\columncolor{red!50}}cccc>{\columncolor{red!50}}ccc}
	1 & 1 & 1 & 0 & 0 & 0 &0 &0 &0 &0 \\
	1 & 1 & 0 & 1 & 0 & 0&0 &0  &0 &0\\
	 1 &  1 &  0 &  0 &  1 &  0 & 0 & 0&0 &0\\
	 0 &  0 &  0 &  1 &  0 &  1 & 1 & 0&0 &0\\
	 0 &  0 &  0 &  0 &  1 &  1 & 0 & 1&0 &0 \\
	0 & 0 & 1 & 0 & 0 & 0&0 &0&1 &1\\
	0 & 0 & 0 & 0 & 0 & 0&1 &0&1 &1\\
	0 & 0 & 0 & 0 & 0 & 0&0 &1&1 &1
  \end{array}}\right)}\end{array}
\end{align*}
\caption{Illustration of an MSC (left) and an MSP (right) for the influence matrix $\bs{F}$ corresponding to the example network in Section~\ref{example_detection_sensing}.}
\label{influence_matrices}
\end{figure}

\end{example}
\else
\fi

\section{Proofs of Section \ref{general}}\label{Main Proofs}
%\subsection{Proofs of Section \ref{general}}


%We now show how to construct a strategy profile that satisfies the conditions in Lemma~\ref{algebra1}: 
%Consider a set of nodes $\Def \in 2^\nodes$ of size at least $b_1$. Then, to construct the support of the sensing strategy $\sold{\Def}{b_1}{}$, one can ``cycle'' over size-$b_1$ subsets of $\Def$: Given any arbitrary ordering of the nodes in $\Def$, we consider the first, second, up to the $b_1$'th nodes of $\Def$ and define the first pure action (sensor placement) $\Def^1$. Then, we take the second $b_1$ nodes of $\Def$, and define the second sensor placement $\Def^2$, and so on, until there are $k < b_1$ nodes of $\Def$ remaining. If $k=0$, i.e., there is no node remaining (meaning that the size of $\Def$ is divisible by $b_1$), then we stop. Otherwise, we take the remaining $k$ nodes, and complete with the first $b_1 - k$ nodes of $\Def$ to create another sensor placement. We repeat the procedure until $k=0$. Once all these sensor placements are defined, $\sold{\Def}{b_1}{}$ is obtained by uniformly randomizing over them. A similar construction is obtained for $\sola{\att}{b_2}{}$. The following lemma formally constructs this strategy profile.


%The following lemma is an extended version of Lemma~\ref{algebra1}.
\begin{lemma}\label{algebra2}
Consider a set of nodes $\Def = \{i_1,\dots,i_{n}\} \in 2^{\nodes}$ of size $n \geq b_1$, and a set of  components $\att = \{e_1,\dots,e_{m}\} \in 2^{\edges}$ of size $m \geq b_2$. We define the following pure actions:
%Then $\forall k \in \llbracket 1,n_1 \rrbracket,$ let $\Def^k$ be the defense defined as follows:
%\begin{align}
%\forall k \in \llbracket 1,n\rrbracket, \ &\Def^k= \{i_{\tau_{n}((k-1)b_1 +1)},\dots,i_{\tau_{n}(kb_1)}\},\label{S^k}\\
%\forall l \in \llbracket 1,m \rrbracket, \ &\att^l = \{e_{\tau_{m}((l-1)b_2 +1)},\dots,e_{\tau_{m}(lb_2)}\},\label{att^k}
%\end{align}
\vspace{-0.0cm}
\begin{align}
\forall k \in \llbracket 1,n\rrbracket, \ &\Def^k= \left\{\begin{array}{ll}
      \{i_{k},\dots,i_{k+b_1 -1}\}& \quad \text{ if }\ k\leq n-b_1+1, \mcr
    \{i_k,\dots,i_n,i_1,\dots,i_{k+ b_1 -n- 1}\}  & \quad \text{ if }\ k \geq n-b_1 +2,
\end{array}\right. 
%\begin{cases}
%      \{i_{k},\dots,i_{k+b_1 -1}\}& \text{ if }\ k\leq n-b_1+1, \\
%    \{i_k,\dots,i_n,i_1,\dots,i_{k+ b_1 -n- 1}\}  & \text{ if }\ k \geq n-b_1 +2,
%\end{cases}
\label{S^k}\\
\forall l \in \llbracket 1,m \rrbracket, \ &\att^l = \left\{\begin{array}{ll}
      \{e_{l},\dots,e_{l+b_2 -1}\}& \quad \text{ if }\ l\leq m-b_2+1, \mcr
    \{e_l,\dots,e_m,e_1,\dots,e_{l+ b_2 -m- 1}\}  & \quad \text{ if }\ l \geq m-b_2 +2,
\end{array}\right.\label{att^k}
\end{align}
and a strategy profile  $(\sold{\Def}{b_1}{},\sola{\att}{b_2}{}) \in \Delta(\mathcal{A}_1)\times\Delta(\mathcal{A}_2)$ supported over $\{\Def^1,\dots,\Def^{n}\}$ and $\{\att^1,\dots,\att^{m}\}$, where:
\vspace{-0.6cm}
\begin{align}
\forall k \in \llbracket 1,n \rrbracket, \ &\sold{\Def}{b_1}{\Def^k} := \frac{1}{n},\label{sigma^S}\\
\forall l \in \llbracket 1,m \rrbracket, \ &\sola{\att}{b_2}{\att^l} := \frac{1}{m}.\label{sigma^T}
\end{align}

Then,  the strategy profile $(\sold{\Def}{b_1}{},\sola{\att}{b_2}{})$ has the following properties:
\begin{enumerate}
\item Each node in $\Def$ (resp. each component in $\att$) is inspected (resp. targeted) with an identical probability given by:
\vspace{-0.4cm}
\begin{align}
&\forall i \in \Def, \ \rho_{\sold{\Def}{b_1}{}}(i) = \frac{b_1}{n}, \label{set_sensing_prob_comp}\\
&\forall e \in \att, \ \rho_{\sola{\att}{b_2}{}}(e) = \frac{b_2}{m}.\label{set_disruption_prob_comp}
\end{align}

%Let $(q_1,q_2) \in (\mathbb{N}^*)^2$ that satisfy $p_1b_1 = q_1 n$ and $p_2 b_2 = q_2 m$. Then:
\item Each node in $\Def$ (resp. each component in $\att$) belongs to $\antiorder{n}{b_1}$ actions (resp. $\antiorder{m}{b_2}$ actions) in the support of $\sold{\Def}{b_1}{}$ (resp. $\sola{\att}{b_2}{}$):
%\vspace{-0.5cm}
\begin{align}
&\forall i \in \Def, \ |\{k \in \llbracket 1,\order{n}{b_1}\rrbracket \ | \ i \in \Def^k\}| = \antiorder{n}{b_1}, \label{q1}\\
&\forall e \in \att, \ |\{l \in \llbracket 1,\order{m}{b_2}\rrbracket \ | \ e \in \att^l\}| = \antiorder{m}{b_2}.\label{q2}
\end{align}


\item The following inequality is satisfied:
\begin{align}
\forall e \in \edges, \ \valdet{\Def}{e} \leq \frac{1}{\antiorder{n}{b_1}}\sum_{k=1}^{\order{n}{b_1}}\valdet{\Def^k}{e}.\label{nice_detection_inequality}
\end{align}
\end{enumerate}
\end{lemma}



\proof{Proof of Lemma~\ref{algebra2}.}
We show the result for a set of nodes $\Def = \{i_1,\dots,i_n\} \in 2^\nodes$ of size $n \geq b_1$.

First we note, by construction, that each node $i_l$, $l \in \llbracket 1,n\rrbracket$ belongs to the same number of detector positionings $S^k$, $k \in \llbracket 1,\order{n}{b_1}\rrbracket$. Thus, \eqref{q1} follows from the following calculations:
%\begin{align*}
%\order{n}{b_1}b_1 &= \sum_{k=1}^{\order{n}{b_1}}b_1 \overset{\eqref{S^k}}{=} \sum_{k=1}^{\order{n}{b_1}}|\Def^k| =  \sum_{k=1}^{\order{n}{b_1}}\sum_{ i \in \nodes} \mathds{1}_{\{i \in \Def^k\}} = \sum_{ i \in \nodes}  \sum_{k=1}^{\order{n}{b_1}} \mathds{1}_{\{i \in \Def^k\}} \\
%& = \sum_{ i \in \nodes} |\{k \in \llbracket 1,\order{n}{b_1}\rrbracket \ | \ i \in \Def^k\}  =  \sum_{i \in \Def} |\{k \in \llbracket 1,\order{n}{b_1}\rrbracket \ | \ i \in \Def^k\}|\\
%& = n \times |\{k \in \llbracket 1,\order{n}{b_1}\rrbracket \ | \ i \in \Def^k\}|, \quad \forall i \in \Def,
%\end{align*}
\begin{align*}
\order{n}{b_1}b_1 & \overset{\eqref{S^k}}{=}   \sum_{k=1}^{\order{n}{b_1}}\sum_{ i \in \nodes} \mathds{1}_{\{i \in \Def^k\}}  = \sum_{ i \in \nodes} |\{k \in \llbracket 1,\order{n}{b_1}\rrbracket \ | \ i \in \Def^k\}  = n \times |\{k \in \llbracket 1,\order{n}{b_1}\rrbracket \ | \ i \in \Def^k\}|, \quad \forall i \in \Def.
\end{align*}
%\begin{align*}
%\order{n}{b_1}b_1 & \overset{\eqref{S^k}}{=} \sum_{k=1}^{\order{n}{b_1}}|\Def^k| =  \sum_{k=1}^{\order{n}{b_1}}\sum_{ i \in \nodes} \mathds{1}_{\{i \in \Def^k\}} = \sum_{ i \in \nodes}  \sum_{k=1}^{\order{n}{b_1}} \mathds{1}_{\{i \in \Def^k\}} = \sum_{ i \in \nodes} |\{k \in \llbracket 1,\order{n}{b_1}\rrbracket \ | \ i \in \Def^k\}  \\
%&=  \sum_{i \in \Def} |\{k \in \llbracket 1,\order{n}{b_1}\rrbracket \ | \ i \in \Def^k\}|= n \times |\{k \in \llbracket 1,\order{n}{b_1}\rrbracket \ | \ i \in \Def^k\}|, \quad \forall i \in \Def,
%\end{align*}
%which proves \eqref{q1}.
%\begin{align}
%\tr{\forall i \in \Def, \ |\{k \in \llbracket 1,\order{n}{b_1}\rrbracket \ | \ i \in \Def^k\}| = \frac{\order{n}{b_1}b_1}{n} {=} \antiorder{n}{b_1}.} \label{introducing_q1}
%\end{align}

%\tr{In other words, every node in $\Def$ is sensed by $\antiorder{n}{b_1}$ pure actions in the support of $\sold{\Def}{b_1}{}$.}
Then, we can show \eqref{set_sensing_prob_comp}. For every node $i \in \Def$, we have:
%\begin{align*}
%\forall i \in \Def, \ \rho_{\sold{\Def}{b_1}{}}(i) &\overset{\eqref{rho_sigma1}}{=} \sum_{\Def^{\prime} \in \mathcal{A}_2} \sold{\Def}{b_1}{\Def^{\prime}} \mathds{1}_{\{i \in \Def^{\prime}\}} = \sum_{k=1}^{\order{n}{b_1}}  \sold{\Def}{b_1}{\Def^{k}}\mathds{1}_{\{i \in \Def^{k}\}} \overset{\eqref{sigma^S}}{=} \frac{1}{\order{n}{b_1}}\sum_{k=1}^{\order{n}{b_1}}  \mathds{1}_{\{i \in \Def^{k}\}}  \\
%&= \frac{1}{\order{n}{b_1}}|\{k \in \llbracket 1,\order{n}{b_1}\rrbracket \ | \ i \in \Def^k\}| \overset{\eqref{q1}}{=}  \frac{b_1}{n}.
%\end{align*}
\begin{align*}
\rho_{\sold{\Def}{b_1}{}}(i) &\overset{\eqref{rho_sigma1}}{=}  \sum_{k=1}^{\order{n}{b_1}}  \sold{\Def}{b_1}{\Def^{k}}\mathds{1}_{\{i \in \Def^{k}\}} \overset{\eqref{sigma^S}}{=} \frac{1}{\order{n}{b_1}}\sum_{k=1}^{\order{n}{b_1}}  \mathds{1}_{\{i \in \Def^{k}\}}  = \frac{1}{\order{n}{b_1}}|\{k \in \llbracket 1,\order{n}{b_1}\rrbracket \ | \ i \in \Def^k\}| \overset{\eqref{q1}}{=}  \frac{b_1}{n}.
\end{align*}

An analogous proof can be applied to $\att  \in 2^\edges$ of size  $m \geq b_2$ to show \eqref{set_disruption_prob_comp} and \eqref{q2}.

Finally, let us show \eqref{nice_detection_inequality}. Consider $e \in \edges$. If $\valdet{\Def}{e} = 1$, then $\exists \,i_0 \in \Def \ | \ \valdet{i_0}{e} = 1$. Since there are $\antiorder{n}{b_1}$ detector positionings in $\{\Def^k, \ k \in \llbracket 1,\order{n}{b_1}\rrbracket\}$ that contain $i_0$, then $\frac{1}{\antiorder{n}{b_1}}\sum_{k=1}^{\order{n}{b_1}}\valdet{\Def^k}{e} \geq 1 = \valdet{\Def}{e}$. If $\valdet{\Def}{e}=0$, then $\forall i \in \Def$, $\valdet{i}{e} = 0$ and $\frac{1}{\antiorder{n}{b_1}}\sum_{k=1}^{\order{n}{b_1}}\valdet{\Def^k}{e} = 0$. 
%Note that the inequality \eqref{nice_detection_inequality} can also be derived from a property of the sensing function. Since $\forall \att \in 2^\edges$, $\valdet{\cdot}{\att}$ is submodular, monotone and nonnegative (Lemma~\ref{Submodularity}), then it is fractionally subadditive. \eqref{nice_detection_inequality} is then a direct application of this property combined with \eqref{q1}.
%Due to Proposition~\ref{minimum_set_cov} we only need to show that $\forall k \in \llbracket 1,\smsc\rrbracket, \ \rho_{\tilde{\sigma}^{1}}(i_k) = \frac{b_1}{\smsc}$ and $\forall l \in \llbracket 1,\smsc\rrbracket, \ \rho_{\tilde{\sigma}^{2}}(e_l) = \frac{b_2}{\smsc}$.
%$n_1$ is the order of $b_1$ in $\mathbb{Z}/\smsc\mathbb{Z}$, which means that $n_1 = \min\{m \in \mathbb{N}^* \ | \ \exists \, p \in \mathbb{N}^* \ | \ mb_1 = p\smsc\}$. Let us denote $q_1$ the positive integer such that $n_1b_1 = q_1\smsc$.
%Then $\frac{b_1}{\smsc} = \frac{}{n_1}$. Thus, we need to show that for every node $i_k$ of the MSC, there are exactly $$ defenses in the support of $\sigma^{1^*}$ that sense node $i_k$.
\hfill \Halmos
\endproof


We illustrate this construction with an example:
\begin{example}\label{algebra_for_game_theory}
Consider a set of three nodes $\Def = \{i_1,i_2,i_3\}$ and suppose that \defender has two detectors ($b_1 = 2$). First, we define three pure actions $\Def^1 = \{i_1,i_2\}$, $\Def^2 = \{i_2,i_3\}$, and $\Def^3 = \{i_3,i_1\}$; see Fig.~\ref{example_S^k}. The strategy $\sold{\Def}{b_1}{}$ is then obtained by assigning uniform probability (i.e., $\frac{1}{3}$) to each pure action. One can check that each node in $\Def$  is inspected with probability $\frac{2}{3} = \frac{b_1}{|\Def|}$.
\begin{figure}[ht]
\centering
\small
\begin{tikzpicture}[-,auto,x=1.3cm, y=0.9cm,
  thick,main node/.style={circle,black,draw,inner sep = 0.07cm},main node2/.style={circle,black,draw,fill=blue!50,inner sep = 0.07cm},flow_a/.style ={gray!100}]
\tikzstyle{edge} = [draw,thick,-,black]
\tikzstyle{detect} = [draw,very thick,Green,-]
\tikzstyle{match} = [draw,very thick,black,-, dashed]
\tikzstyle{flow} = [draw,line width = 1.5pt,->,gray!100]

%\begin{scope}[yshift=0, xshift =-110]
	\node[main node] (1) at (0,2) {$i_1$};
	\node[main node] (2) at (0,1) {$i_2$};
	\node[main node] (3) at (0,0) {$i_3$};
%	\node[main node] (4) at (4,0) {$i_4$};
%	\node[main node] (5) at (5,0) {$i_5$};
%	\node[main node] (6) at (6,0) {$i_6$};
	
	\node[main node2] (1) at (1,2) {$i_1$};
	\node[main node2] (2) at (1,1) {$i_2$};
	\node[main node] (3) at (1,0) {$i_3$};
%	\node[main node2] (4) at (4,-1) {$i_4$};
%	\node[main node] (5) at (5,-1) {$i_5$};
%	\node[main node] (6) at (6,-1) {$i_6$};
	
	
	\node[main node] (1) at (2,2) {$i_1$};
	\node[main node2] (2) at (2,1) {$i_2$};
	\node[main node2] (3) at (2,0) {$i_3$};
%	\node[main node] (4) at (4,-2) {$i_4$};
%	\node[main node2] (5) at (5,-2) {$i_5$};
%	\node[main node2] (6) at (6,-2) {$i_6$};
	
	\node[main node2] (1) at (3,2) {$i_1$};
	\node[main node] (2) at (3,1) {$i_2$};
	\node[main node2] (3) at (3,0) {$i_3$};
%	\node[main node2] (4) at (4,-3) {$i_4$};
%	\node[main node2] (5) at (5,-3) {$i_5$};
%	\node[main node2] (6) at (6,-3) {$i_6$};
	%\node[main node, draw=white] (7) at (3.5,-0.5) {\textbf{a}};
\draw[black] (0.5,-0.5) -- (0.5,2.5);
%\node{1} at (1,1);

\node[black] (10) at (0,2.9) {$\Def$ };
\node[black] (10) at (1,2.9) {$\Def^1$ };
\node[black] (10) at (2,2.9) {$\Def^2$ };
\node[black] (10) at (3,2.9) {$\Def^3$ };
%	\path[edge]	
%	%(2) edge (5)
%	%(1) edge  (2)
%	(2) edge  node{$e_3$} (3)
%	%(3) edge  (5)	
%	%(4) edge  (6)
%	(5) edge[dashed] node[below right] {$e_8$} (6);
	
%	\path[detect]
%	(1) edge[double] node {$e_1$} (2)
%	(3) edge[double] node {$e_5$} (5)
%	(2) edge[double,dashed] node {$e_4$} (4)
%	(1) edge[double,dashed]  node[below left] {$e_2$} (3)
%	(5) edge[double] node {$e_6$} (4)
%	(6) edge[double] node[above right] {$e_7$} (4);
%	\path[edge]
	
	
%\end{scope}
\normalsize
\end{tikzpicture}
\caption{Support of $\sold{\Def}{b_1}{}$ when $\Def$ is composed of three nodes and $b_1 = 2$.} \label{example_S^k}
\end{figure}

\vspace{-1cm}
\hfill $\triangle$


%The same construction applies to subsets of edges for \attacker.
\end{example}




%
%\begin{lemma}
%
%\end{lemma}





\proof{Proof of Proposition~\ref{best_set_cover}.} We show that (i) given a minimal set cover $\Def^{\prime} \in 2^\nodes$, the optimal value of \rlpo{\Def^{\prime}} is $b_2\left(\frac{b_1}{|\Def^\prime|}-1\right)$, and an optimal solution is given by $\sold{\Def^\prime}{b_1}{}$. Then, we show that (ii) given a set packing $\att^{\prime} \in 2^\edges$ of size at least $b_2$, the optimal value of \rlpt{\att^{\prime}} is $\max\left\{0,b_2\left(1 - \frac{b_1}{|\att^\prime|}\right)\right\}$, and an optimal solution is given by $\sola{\att^{\prime}}{b_2}{}$.
\begin{enumerate}
\item
Consider a minimal set cover $\Def^{\prime} = \{i_1,\dots,i_n\} \in 2^\nodes$ of size $n$. Necessarily, $\Def^{\prime}$ is such that:
%\vspace{-0.5cm}
\begin{align}
\forall k \in \llbracket 1,n \rrbracket, \ \exists \, e_k \in \edges \ | \ \valdet{i_k}{e_k} = 1 \text{ and } \valdet{i_j}{e_k} = 0, \quad \forall j \neq k. \label{minimal_set_cover}
\end{align}

%Indeed, if $\exists \, k \in \llbracket 1,n\rrbracket \ | \ \forall e \in \edges: \ \valdet{i_k}{e} = 0$ or $\exists \, j \neq k \ | \ \valdet{i_j}{e}=1$, then any component that is monitored by $i_k$ is also monitored by another node of $\Def^{\prime}$. Therefore, removing $i_k$ from $\Def^{\prime}$ will still produce a set cover, which contradicts $\Def^\prime$ being a minimal set cover.
\begin{itemize}
\item[--]First, let us show that $\max_{\{\sigma^1 \in  \Delta(\mathcal{A}_1) \, | \, \nbasis{\sigma^1} \subseteq \Def^{\prime}\}} \min_{\att \in \mathcal{A}_2} -U_2(\sigma^1,\att) \geq b_2\left(\frac{b_1}{n}-1\right)$.  Consider $\sold{\Def^{\prime}}{b_1}{} \in \Delta(\mathcal{A}_1)$ defined in \eqref{sigma^S}.
 Recall that $\sold{\Def^{\prime}}{b_1}{}$ is such that $\nbasis{\sold{\Def^{\prime}}{b_1}{}} = \Def^{\prime}$ and $\forall k \in \llbracket 1,n \rrbracket, \ \rho_{\sold{\Def^{\prime}}{b_1}{}}(i_k) = \frac{b_1}{n}$. Also, recall that we are in the case when $b_1 < \smsc$, implying that $b_1 < \smsc \leq n$.

Since $\Def^{\prime}$ is a set cover, then $\forall e \in \edges, \ \exists\, k_e \in \llbracket 1,n\rrbracket \ | \ \valdet{i_{k_e}}{e} = 1$. Furthermore, $\detect$ is a nonnegative function. Therefore:
%Then, by partitioning the set of actions $\mathcal{A}_1$ into the set of detector positionings that contain $i_{k_e}$ and the set of detector positionings that do not, we obtain:
%\begin{align}
%\forall e \in \edges, \ \sum_{\Def \in \mathcal{A}_1} \sold{\Def^{\prime}}{b_1}{\Def} \valdet{\Def}{e} &= \sum_{\{\Def \in \mathcal{A}_1 \, | \, i_{k_e} \in \Def\}}\sold{\Def^{\prime}}{b_1}{\Def}\valdet{\Def}{e} + \sum_{\{\Def \in \mathcal{A}_1 \, | \, i_{k_e} \notin \Def\}} \sold{\Def^{\prime}}{b_1}{\Def}  \underset{\geq 0}{\underbrace{\valdet{\Def}{e}}} \nonumber\\
%& \geq \sum_{\{\Def \in \mathcal{A}_1 \, | \, i_{k_e} \in \Def\}}\sold{\Def^{\prime}}{b_1}{\Def}\valdet{\Def}{e}\overset{\eqref{monotonicity_detection}}{\geq}  \sum_{\{\Def \in \mathcal{A}_1 \, | \, i_{k_e} \in \Def\}}\sold{\Def^{\prime}}{b_1}{\Def}\valdet{i_{k_e}}{e} \nonumber\\
%&=\sum_{\{\Def \in \mathcal{A}_1 \, | \, i_{k_e} \in \Def\}} \sold{\Def^{\prime}}{b_1}{\Def}\overset{\eqref{rho_sigma1}}{=} \rho_{\sold{\Def^{\prime}}{b_1}{}}(i_{k_e})\overset{\eqref{set_sensing_prob_comp}}{=} \frac{b_1}{n}.\label{ineq1}
%\end{align}
%\begin{align}
%\forall e \in \edges, \ &\sum_{\Def \in \mathcal{A}_1} \sold{\Def^{\prime}}{b_1}{\Def} \valdet{\Def}{e} = \sum_{\{\Def \in \mathcal{A}_1 \, | \, i_{k_e} \in \Def\}}\sold{\Def^{\prime}}{b_1}{\Def}\valdet{\Def}{e} + \sum_{\{\Def \in \mathcal{A}_1 \, | \, i_{k_e} \notin \Def\}} \sold{\Def^{\prime}}{b_1}{\Def}  \underset{\geq 0}{\underbrace{\valdet{\Def}{e}}} \nonumber\\
%& \overset{\eqref{monotonicity_detection}}{\geq}  \sum_{\{\Def \in \mathcal{A}_1 \, | \, i_{k_e} \in \Def\}}\sold{\Def^{\prime}}{b_1}{\Def}\underset{=1}{\underbrace{\valdet{i_{k_e}}{e} }}\overset{\eqref{rho_sigma1}}{=} \rho_{\sold{\Def^{\prime}}{b_1}{}}(i_{k_e})\overset{\eqref{set_sensing_prob_comp}}{=} \frac{b_1}{n}.\label{ineq1}
%\end{align}
%\vspace{-0.3cm}
\begin{align}
\forall e \in \edges, \ &\sum_{\Def \in \mathcal{A}_1} \sold{\Def^{\prime}}{b_1}{\Def} \valdet{\Def}{e} \overset{\eqref{monotonicity_detection}}{\geq}  \sum_{\{\Def \in \mathcal{A}_1 \, | \, i_{k_e} \in \Def\}}\sold{\Def^{\prime}}{b_1}{\Def}\overset{\eqref{rho_sigma1}}{=} \rho_{\sold{\Def^{\prime}}{b_1}{}}(i_{k_e})\overset{\eqref{set_sensing_prob_comp}}{=} \frac{b_1}{n}.\label{ineq1}
\end{align}

Thus, we obtain:
\begin{align}
\forall \att \in \mathcal{A}_2, \ -{U}_2(\sold{\Def^{\prime}}{b_1}{},\att) &\overset{\eqref{payoff2}}{=} \sum_{\Def \in \mathcal{A}_1} \sold{\Def^{\prime}}{b_1}{\Def} \valdet{\Def}{\att} - |\att| \overset{\eqref{detection_disruptions}}{=} \sum_{e \in \att}\sum_{\Def \in \mathcal{A}_1} \sold{\Def^{\prime}}{b_1}{\Def} \valdet{\Def}{e} - |\att| \nonumber\\
& \overset{\eqref{ineq1}}{\geq} \sum_{e \in \att}\frac{b_1}{n} - |\att|= \underset{<0}{\underbrace{\left(\frac{b_1}{n}-1\right)}}\underset{\leq b_2}{\underbrace{|\att|}}  \geq b_2 \left(\frac{b_1}{n}-1\right). \label{for later}
\end{align}

%\vspace{-2cm}
Therefore, %$\min_{\att \in \mathcal{A}_2}-{U}_2(\sold{\Def^{\prime}}{b_1}{},\att) \geq b_2 \left(\frac{b_1}{n}-1\right)$, which implies:
%\vspace{-0.5cm}
%\begin{align}
$\max_{\{\sigma^1 \in \Delta(\mathcal{A}_1) \, | \, \nbasis{\sigma^1} \subseteq \Def^{\prime}\}} \min_{\att \in \mathcal{A}_2} -{U}_2(\sigma^1,\att) \geq \min_{\att \in \mathcal{A}_2}-{U}_2(\sold{\Def^{\prime}}{b_1}{},\att) \geq b_2 \left(\frac{b_1}{n}-1\right).$ %\label{1st_ineq_max-min}
%\end{align}

%Note that the only property of $\sold{\Def^\prime}{b_1}{}$ that was used to show \eqref{1st_ineq_max-min} is that its node basis is $\Def^\prime$ and that $\forall i \in \Def^\prime, \ \rho_{\sold{\Def^\prime}{b_1}{}}(i) = \frac{b_1}{n}$.

\item[--]
Now, let us show the reverse inequality. Consider any $\sigma^1 \in \Delta(\mathcal{A}_1) $ such that $\nbasis{\sigma^1} \subseteq \Def^{\prime} =  \{i_1,\dots,i_n\}$. Let us reorder the indices such that $\rho_{\sigma^1}(i_1) \leq \dots \leq \rho_{\sigma^1}(i_n)$. 
%Then, thanks to Lemma~\ref{weights_in_bags}, we have $\sum_{k=1}^{b_2} \rho_{\sigma^1}(i_k) \leq \frac{b_2}{n} \mathbb{E}_{\sigma^1}[|\Def|]$.

Consider $\att^\prime = \{e_1,\dots,e_{b_2}\}$ (where the $e_k$'s are defined in \eqref{minimal_set_cover}). Then, for every $k \in \llbracket 1,b_2 \rrbracket$:  
%partitioning $\mathcal{A}_1$ into the set of detector positionings that contain $i_{k}$ and the ones that do not gives us:
%\begin{align}
%\forall k \in \llbracket 1,b_2 \rrbracket, \ \sum_{\Def \in \mathcal{A}_1} \sigma_{\Def}^1 \valdet{\Def}{e_k} &\overset{\eqref{minimal_set_cover}}{=} \sum_{\{\Def \in \mathcal{A}_1 \, | \, i_{k} \in \Def\}} \sigma_{\Def}^1\underset{=1}{\underbrace{\valdet{\Def}{e_k}}} + \sum_{\{\Def \in \mathcal{A}_1 \, | \, i_{k} \notin \Def\}} \underset{=0}{\underbrace{\sigma_{\Def}^1 \valdet{\Def}{e_k}}}\nonumber\\
%&\overset{\eqref{rho_sigma1}}{=} \rho_{\sigma^1}(i_{k}), \label{to be used soon}
%\end{align}
\begin{align}
\mathbb{E}_{\sigma^1}[\valdet{\Def}{e_k}] &\overset{\eqref{minimal_set_cover}}{=} \sum_{\{\Def \in \mathcal{A}_1 \, | \, i_{k} \in \Def\}} \sigma_{\Def}^1\underset{=1}{\underbrace{\valdet{\Def}{e_k}}} + \sum_{\{\Def \in \mathcal{A}_1 \, | \, i_{k} \notin \Def\}} \underset{=0}{\underbrace{\sigma_{\Def}^1 \valdet{\Def}{e_k}}}\overset{\eqref{rho_sigma1}}{=} \rho_{\sigma^1}(i_{k}), \label{to be used soon}
\end{align}
where we combined the fact that the node basis of $\sigma^1$ is a subset of $\Def^\prime$ and that $i_k$ is the only node from $\Def^{\prime}$ that monitors component $e_k$ (by construction). This implies that:
%\begin{align*}
%-{U}_2(\sigma^1,\att^\prime)  &\overset{\eqref{payoff2}}{=}  \sum_{\Def \in \mathcal{A}_1}\sigma_{\Def}^1 \valdet{\Def}{\att^\prime} - |\att^\prime| \overset{\eqref{detection_disruptions}}{=} \sum_{k=1}^{b_2}\sum_{\Def \in \mathcal{A}_1}\sigma_{\Def}^1 \valdet{\Def}{e_k} - b_2  \overset{\eqref{to be used soon}}{=} \sum_{k=1}^{b_2}\rho_{\sigma^1}(i_{k}) - b_2\\
%& \overset{\eqref{worst_bags}}{\leq} \frac{b_2}{n}\mathbb{E}_{\sigma^1}[|\Def|] -b_2 \overset{\eqref{p1's set}}{\leq} b_2 \left(\frac{b_1}{n}  - 1\right).
%\end{align*}
\begin{align*}
\min_{\att \in \mathcal{A}_2} -{U}_2(\sigma^1,\att)  \leq-{U}_2(\sigma^1,\att^\prime)  &\overset{\eqref{payoff2}}{=}  
 \mathbb{E}_{\sigma^1}[\valdet{\Def}{\att^\prime}] - |\att^\prime|   \overset{\eqref{detection_disruptions},\eqref{to be used soon}}{=} \sum_{k=1}^{b_2}\rho_{\sigma^1}(i_{k}) - b_2 \overset{\eqref{worst_bags}}{\leq} b_2 \left(\frac{b_1}{n}  - 1\right).
\end{align*}
%Thus, $\min_{\att \in \mathcal{A}_2} -{U}_2(\sigma^1,\att)  \leq b_2 \left(\frac{b_1}{n}  - 1\right)$. 
This upper bound holds for any $\sigma^1 \in \Delta(\mathcal{A}_1)$ such that  $\nbasis{\sigma^1} \subseteq \Def^{\prime}$, and does not depend on $\sigma^1$. Therefore,
%\begin{align}
$\max_{\{\sigma^1 \in \Delta(\mathcal{A}_1) \, | \, \nbasis{\sigma^1} \subseteq\Def^{\prime}\}} \min_{\att \in \mathcal{A}_2} -U_2(\sigma^1,\att) \leq b_2 \left(\frac{b_1}{n}-1\right)$, and %\label{2nd_ineq_max-min}
%\end{align}
%
%
%By combining \eqref{1st_ineq_max-min} and \eqref{2nd_ineq_max-min}, 
we can conclude that:
\begin{align*}
\max_{\{\sigma^1 \in \Delta(\mathcal{A}_1) \, | \, \nbasis{\sigma^1} \subseteq \Def^{\prime}\}} \min_{\att \in \mathcal{A}_2} -U_2(\sigma^1,\att) = \min_{\att \in \mathcal{A}_2} - U_2(\sold{\Def^\prime}{b_1}{},\att) = b_2 \left(\frac{b_1}{n}-1\right).
\end{align*}
%
%\item[--] Now, let us show that $\sold{\Def^\prime}{b_1}{}$ is an optimal solution of \rlpo{\Def^{\prime}}, i.e., $\min_{\att \in \mathcal{A}_2} - U_2(\sold{\Def^\prime}{b_1}{},\att) = b_2 \left(\frac{b_1}{n}-1\right)$.
%
%We already showed in \eqref{1st_ineq_max-min} that $\min_{\att \in \mathcal{A}_2} - U_2(\sold{\Def^\prime}{b_1}{},\att) \geq b_2 \left(\frac{b_1}{n}-1\right)$. Now, consider $\att^\prime = \{e_1,\dots,e_{b_2}\}$, where the $e_k$'s are defined in \eqref{minimal_set_cover} (note that $b_2 < \semm \leq \smsc \leq n$). Then we can show that the inequality is tight:
%\begin{align*}
%-{U}_2( \sold{\Def^\prime}{b_1}{},\att^\prime) &\overset{\eqref{payoff2}}{=}   \sum_{\Def \in \mathcal{A}_1} \sold{\Def^\prime}{b_1}{\Def} \valdet{\Def}{\att^\prime} - |\att^\prime| \overset{\eqref{detection_disruptions}}{=} \sum_{k=1}^{b_2} \sum_{\Def \in \mathcal{A}_1} \sold{\Def^\prime}{b_1}{\Def} \valdet{\Def}{e_k} - |\att^\prime|\\
%& = \sum_{k=1}^{b_2}\left(\sum_{\{\Def \in \mathcal{A}_1 \, | \, i_{k} \in \Def\}}\sold{\Def^\prime}{b_1}{\Def}\valdet{\Def}{e_k} + \sum_{\{\Def \in \mathcal{A}_1 \, | \, i_{k} \notin \Def\}} \sold{\Def^\prime}{b_1}{\Def}  \valdet{\Def}{e_k}\right) - |\att^\prime|\\
%& \overset{\eqref{minimal_set_cover}}{=} \sum_{k=1}^{b_2} \sum_{\{\Def \in \mathcal{A}_1 \, | \, i_{k} \in \Def\}}\sold{\Def^\prime}{b_1}{\Def} - |\att^{\prime}|\\
%& \overset{\eqref{rho_sigma1}}{=} \sum_{k=1}^{b_2}\rho_{\sold{\Def^\prime}{b_1}{}}(i_k) - |\att^\prime|\\
%&\overset{\eqref{set_sensing_prob_comp}}{=} \sum_{k=1}^{b_2}\frac{b_1}{n} - \underset{=b_2}{\underbrace{|\att^\prime|}}\\
%& = b_2\left(\frac{b_1}{n}-1 \right)
%\end{align*}
%
The optimal value of \rlpo{\Def^\prime} is $b_2 \left(\frac{b_1}{n}-1\right)$, and an optimal solution is given by $\sold{\Def^\prime}{b_1}{}$.
\end{itemize}

%\hfill \Halmos
%\endproof


%\proof{Proof of Proposition~\ref{best_set_cover}.}
\item
Consider a set packing $\att^{\prime} = \{e_1,\dots,e_m\} \in 2^\edges$ of size $m \geq b_2$. %We separately consider the cases when $b_1 \geq m$ and $b_1 < m$.

\textbf{Case 1:} If $b_1 \geq m$, then \defender can monitor all the components of $\att^\prime$ with a single detector positioning $\Def^\prime$. Therefore,  the optimal value of \rlpt{\att^\prime} in this case is equal to $0 = \max\{0,b_2(1 - \frac{b_1}{m})\}$.
% no matter which strategy supported over $\att^\prime$ \attacker chooses, her attacks will always be detected by $\Def^\prime$.

\textbf{Case 2:} Consider $b_1 < m$. In this case, note that $ \max\{0,b_2(1 - \frac{b_1}{m})\} = b_2(1 - \frac{b_1}{m})$.
\begin{itemize}
\item[--] First, we show that $\max_{\{\sigma^2 \in \Delta(\mathcal{A}_2) \, | \, \ebasis{\sigma^2} \subseteq \att^\prime\}} \min_{\Def \in \mathcal{A}_1} {U}_2(\Def,\sigma^2) \geq b_2 \left(1 - \frac{b_1}{m}\right)$. Consider $\sola{\att^{\prime}}{b_2}{} \in \Delta(\mathcal{A}_2)$ defined in \eqref{sigma^T}. 
%Recall that $\sola{\att^{\prime}}{b_2}{}$ is such that its component basis is $\ebasis{\sola{\att^{\prime}}{b_2}{}} = \att^\prime$ and $\forall l \in \llbracket 1,m \rrbracket, \ \rho_{\sola{\att^{\prime}}{b_2}{}}(e_l) = \frac{b_2}{m}$.
%
Since $\att^\prime$ is a set packing, then $\forall i \in \nodes, \ \valdet{i}{\att^\prime} \leq 1$. This implies that:
%\begin{align*}
%\forall i \in \nodes, \ \sum_{\att \in \mathcal{A}_2} \sigma^{\att^{\prime}}_{\att} \valdet{i}{\att} = \sum_{\{\att \in \mathcal{A}_2 \, | \, e_{k} \in \Def\}} \hat{\sigma}_{\Def}^1 + \sum_{\{\Def \in \mathcal{A}_1 \, | \, i_{k_e} \notin \Def\}} \hat{\sigma}_{\Def}^1  \valdet{\Def}{e} \geq \sum_{\{\Def \in \mathcal{A}_1 \, | \, i_{k_e} \in \Def\}} \hat{\sigma}_{\Def}^1 = \rho_{\hat{\sigma}^1}(i_{k_e}) = \frac{b_1}{n}
%\end{align*}
%Thus, we obtain:
%\begin{align*}
%\forall \Def \in \mathcal{A}_1, \ &U_2(\Def, \sola{\att^{\prime}}{b_2}{}) \overset{\eqref{payoff2}}{=} \sum_{\att \in \mathcal{A}_2} \sola{\att^{\prime}}{b_2}{\att} (|\att| - \valdet{\Def}{\att})  \overset{\eqref{redundant_nodes}}{\geq} \sum_{\att \in \mathcal{A}_2} \sola{\att^{\prime}}{b_2}{\att} (|\att| - \sum_{i \in \Def}\valdet{i}{\att}) \\
%& \overset{\eqref{detection_disruptions}}{=}\sum_{\att \in \mathcal{A}_2} \sola{\att^{\prime}}{b_2}{\att} \sum_{e \in \att}(1 - \sum_{i \in \Def}\valdet{i}{e})  = \sum_{e \in \edges}(1 - \sum_{i \in \Def}\valdet{i}{e})\sum_{\att \in \mathcal{A}_2} \sola{\att^{\prime}}{b_2}{\att} \mathds{1}_{\{e \in \att\}}\\
%&\overset{\eqref{rho_sigma2}}{=} \sum_{e \in \edges}(1 - \sum_{i \in \Def}\valdet{i}{e})  \rho_{\sola{\att^{\prime}}{b_2}{}}(e)  \overset{\eqref{set_disruption_prob_comp}}{=} \sum_{l=1}^m(1 - \sum_{i \in \Def}\valdet{i}{e_l})  \frac{b_2}{m}  \overset{\eqref{detection_disruptions}}{=} b_2 - \frac{b_2}{m}\sum_{i \in \Def}\valdet{i}{\att^\prime} \\
%& \geq b_2 - \frac{b_2}{m}\sum_{i \in \Def}1 \overset{\eqref{p1's set}}{\geq}  b_2\left( 1 - \frac{b_1}{m} \right).
%\end{align*}
%\begin{align*}
%\forall \Def \in \mathcal{A}_1, \ &U_2(\Def, \sola{\att^{\prime}}{b_2}{}) \overset{\eqref{payoff2}}{=} \mathbb{E}_{\sola{\att^{\prime}}{b_2}{}}[|\att| - \valdet{\Def}{\att}] \overset{\eqref{redundant_nodes},\eqref{att^k}}{\geq} b_2 - \sum_{i \in \Def}\mathbb{E}_{\sola{\att^{\prime}}{b_2}{}}[\valdet{i}{\att}]\\
%& \overset{\eqref{detection_disruptions}}{=} b_2 - \sum_{i \in \Def}\sum_{e \in \edges} \mathbb{E}_{\sola{\att^{\prime}}{b_2}{}}[\valdet{i}{e}\mathds{1}_{\{e \in \att\}}]   \overset{\eqref{rho_sigma2}}{=} b_2 - \sum_{i \in\Def} \sum_{e \in \edges} \valdet{i}{e}\rho_{\sola{\att^{\prime}}{b_2}{}}(e) \\
%&\overset{\eqref{set_disruption_prob_comp}}{=} b_2 -  \frac{b_2}{m}\sum_{i \in\Def} \sum_{e \in \att^\prime}\valdet{i}{e}  \overset{\eqref{detection_disruptions}}{=} b_2 -  \frac{b_2}{m}\sum_{i \in\Def} \underset{\leq 1}{\underbrace{\valdet{i}{\att^\prime}}} \geq b_2 -  \frac{b_2}{m}\underset{\leq b_1}{\underbrace{|\Def|}} \geq b_2\left( 1 - \frac{b_1}{m} \right).
%%& \overset{\eqref{detection_disruptions}}{=}\sum_{\att \in \mathcal{A}_2} \sola{\att^{\prime}}{b_2}{\att} \sum_{e \in \att}(1 - \sum_{i \in \Def}\valdet{i}{e})  = \sum_{e \in \edges}(1 - \sum_{i \in \Def}\valdet{i}{e})\sum_{\att \in \mathcal{A}_2} \sola{\att^{\prime}}{b_2}{\att} \mathds{1}_{\{e \in \att\}}\\
%%&\overset{\eqref{rho_sigma2}}{=} \sum_{e \in \edges}(1 - \sum_{i \in \Def}\valdet{i}{e})  \rho_{\sola{\att^{\prime}}{b_2}{}}(e)  \overset{\eqref{set_disruption_prob_comp}}{=} \sum_{l=1}^m(1 - \sum_{i \in \Def}\valdet{i}{e_l})  \frac{b_2}{m}  \overset{\eqref{detection_disruptions}}{=} b_2 - \frac{b_2}{m}\sum_{i \in \Def}\valdet{i}{\att^\prime} \\
%%& \geq b_2 - \frac{b_2}{m}\sum_{i \in \Def}1 \overset{\eqref{p1's set}}{\geq}  b_2\left( 1 - \frac{b_1}{m} \right).
%\end{align*}
\begin{align*}
\forall \Def \in \mathcal{A}_1, \ &U_2(\Def, \sola{\att^{\prime}}{b_2}{}) \overset{\eqref{payoff2}}{=} \mathbb{E}_{\sola{\att^{\prime}}{b_2}{}}[|\att| - \valdet{\Def}{\att}] \overset{\eqref{redundant_nodes},\eqref{att^k}}{\geq} b_2 - \sum_{i \in \Def}\mathbb{E}_{\sola{\att^{\prime}}{b_2}{}}[\valdet{i}{\att}]\\
&  \overset{\eqref{detection_disruptions},\eqref{rho_sigma2}}{=} b_2 - \sum_{i \in\Def} \sum_{e \in \edges} \valdet{i}{e}\rho_{\sola{\att^{\prime}}{b_2}{}}(e)  \overset{\eqref{set_disruption_prob_comp},\eqref{detection_disruptions}}{=} b_2 -  \frac{b_2}{m}\sum_{i \in\Def} \underset{\leq 1}{\underbrace{\valdet{i}{\att^\prime}}}  \geq b_2\left( 1 - \frac{b_1}{m} \right).
\end{align*}


Therefore, $\max_{\{\sigma^2 \in \Delta(\mathcal{A}_2) \, | \, \ebasis{\sigma^2} \subseteq \att^\prime\}} \min_{\Def \in \mathcal{A}_1} {U}_2(\Def,\sigma^2) \geq \min_{\Def \in \mathcal{A}_1}U_2(\Def,\sola{\att^{\prime}}{b_2}{}) \geq b_2 \left(1 - \frac{b_1}{m}\right).$
%\vspace{-0.5cm}
%\begin{align}
%\max_{\{\sigma^2 \in \Delta(\mathcal{A}_2) \, | \, \ebasis{\sigma^2} \subseteq \att^\prime\}} \min_{\Def \in \mathcal{A}_1} {U}_2(\Def,\sigma^2) \geq \min_{\Def \in \mathcal{A}_1}U_2(\Def,\sola{\att^{\prime}}{b_2}{}) \geq b_2 \left(1 - \frac{b_1}{m}\right). \label{1st_inteq_max-min_bis}
%\end{align}

%Similarly, note that the only property of $\sola{\att^\prime}{b_2}{}$ that was used to show \eqref{1st_inteq_max-min_bis} is that its component basis is $\att^\prime$ and that $\forall e \in \att^\prime, \ \rho_{\sola{\att^\prime}{b_2}{}}(e) = \frac{b_2}{m}$.
\item[--]
Now, let us show the reverse inequality. Consider any $\sigma^2 \in \Delta(\mathcal{A}_2) \ | \ \ebasis{\sigma^2} \subseteq \att^{\prime} = \{e_1,\dots,e_m\}$. Let us reorder the indices such that $\rho_{\sigma^2}(e_1) \geq \dots \geq \rho_{\sigma^2}(e_m)$. 
%Then, thanks to Lemma~\ref{weights_in_bags}, we have $\sum_{l=1}^{b_1} \rho_{\sigma^2}(e_l) \geq \frac{b_1}{m}\mathbb{E}_{\sigma^2}[|\att|]$.
In Section \ref{sec:detect}, we assumed that each component can be monitored from at least one node. Therefore $\forall l \in \llbracket 1,m \rrbracket, \ \exists \, i_l \in \nodes \ | \ \valdet{i_l}{e_l} = 1$ (note that the $i_l$'s are distinct since $\att^\prime$ is a set packing).  Now, consider the detector positioning $\Def^\prime = \{i_1,\dots,i_{b_1}\}$. $\Def^\prime$ monitors $\{e_1,\dots,e_{b_1}\}$, which enables us to show:
%\begin{align*}
%U_2(\Def^\prime, \sigma^{2}) &\overset{\eqref{payoff2}}{=} \sum_{\att \in \mathcal{A}_2} \sigma^{2}_{\att} (|\att| - \valdet{\Def^\prime}{\att})  \overset{\eqref{detection_disruptions}}{=} \mathbb{E}_{\sigma^2}[|\att|] - \sum_{\att \in \mathcal{A}_2} \sigma^{2}_{\att}\sum_{e \in \att}\valdet{\Def^\prime}{e} \\
%& =  \mathbb{E}_{\sigma^2}[|\att|]  - \sum_{e \in \edges} \valdet{\Def^\prime}{e}\sum_{\att \in \mathcal{A}_2} \sigma^{2}_{\att}\mathds{1}_{\{e \in \att\}}  \overset{\eqref{rho_sigma2}}{=}  \mathbb{E}_{\sigma^2}[|\att|]  - \sum_{e \in \edges} \valdet{\Def^\prime}{e}\rho_{\sigma^2}(e)\\
%& =  \mathbb{E}_{\sigma^2}[|\att|]  - \sum_{e \in \att^\prime} \valdet{\Def^\prime}{e}\rho_{\sigma^2}(e) =  \mathbb{E}_{\sigma^2}[|\att|]  - \sum_{l=1}^{b_1} \valdet{\Def^\prime}{e_l}\rho_{\sigma^2}(e_l) - \sum_{l=b_1+1}^{m} \valdet{\Def^\prime}{e_l}\rho_{\sigma^2}(e_l)\\
%& \leq  \mathbb{E}_{\sigma^2}[|\att|]  - \sum_{l=1}^{b_1} \valdet{\Def^\prime}{e_l}\rho_{\sigma^2}(e_l)  =  \mathbb{E}_{\sigma^2}[|\att|]  - \sum_{l=1}^{b_1} \rho_{\sigma^2}(e_l) \\
%& \overset{\eqref{best_bags}}{\leq}  \mathbb{E}_{\sigma^2}[|\att|]  - \frac{b_1\mathbb{E}_{\sigma^2}[|\att|]}{m} = \underset{>0}{\underbrace{\left( 1 - \frac{b_1}{m}\right)}}  \mathbb{E}_{\sigma^2}[|\att|]\\
%& \overset{\eqref{p2's set}}{\leq}\left( 1 - \frac{b_1}{m}\right)b_2.
%\end{align*}
%\begin{align*}
%U_2(\Def^\prime, \sigma^{2}) &\overset{\eqref{payoff2},\eqref{detection_disruptions}}{=} \mathbb{E}_{\sigma^2}[|\att|] - \mathbb{E}_{\sigma^2}[\sum_{e \in \att}\valdet{\Def^\prime}{e}] = \mathbb{E}_{\sigma^2}[|\att|] - \sum_{e \in \edges}\valdet{\Def^\prime}{e}\mathbb{E}_{\sigma^2}[\mathds{1}_{\{e \in \att\}}]  \\
%& \overset{\eqref{rho_sigma2}}{=} \mathbb{E}_{\sigma^2}[|\att|] - \sum_{e \in \edges}\valdet{\Def^\prime}{e}\rho_{\sigma^2}(e) =  \mathbb{E}_{\sigma^2}[|\att|]  - \sum_{l=1}^{b_1} \underset{=1}{\underbrace{\valdet{\Def^\prime}{e_l}}}\rho_{\sigma^2}(e_l) - \sum_{l=b_1+1}^{m} \underset{\geq 0}{\underbrace{\valdet{\Def^\prime}{e_l}\rho_{\sigma^2}(e_l)}}\\
%& \leq   \mathbb{E}_{\sigma^2}[|\att|]  - \sum_{l=1}^{b_1} \rho_{\sigma^2}(e_l)  \overset{\eqref{best_bags}}{\leq}  \underset{>0}{\underbrace{\left( 1 - \frac{b_1}{m}\right)}}  \underset{\leq b_2}{\underbrace{\mathbb{E}_{\sigma^2}[|\att|]}}\leq \left( 1 - \frac{b_1}{m}\right)b_2.
%\end{align*}
\begin{align*}
&\min_{\Def \in \mathcal{A}_1} U_2(\Def,\sigma^2)  \leq U_2(\Def^\prime, \sigma^{2}) \overset{\eqref{payoff2},\eqref{detection_disruptions}}{=} \mathbb{E}_{\sigma^2}[|\att|] - \mathbb{E}_{\sigma^2}[\sum_{e \in \att}\valdet{\Def^\prime}{e}]  \overset{\eqref{rho_sigma2}}{=} \mathbb{E}_{\sigma^2}[|\att|] - \sum_{e \in \edges}\valdet{\Def^\prime}{e}\rho_{\sigma^2}(e) \\
&=  \mathbb{E}_{\sigma^2}[|\att|]  - \sum_{l=1}^{b_1} \underset{=1}{\underbrace{\valdet{\Def^\prime}{e_l}}}\rho_{\sigma^2}(e_l) - \sum_{l=b_1+1}^{m} \underset{\geq 0}{\underbrace{\valdet{\Def^\prime}{e_l}\rho_{\sigma^2}(e_l)}} \overset{\eqref{best_bags}}{\leq}  \underset{>0}{\underbrace{\left( 1 - \frac{b_1}{m}\right)}}  \underset{\leq b_2}{\underbrace{\mathbb{E}_{\sigma^2}[|\att|]}}\leq \left( 1 - \frac{b_1}{m}\right)b_2.
\end{align*}


%\begin{align*}
%\widetilde{U}_2(\Def, \sigma^{2}) &= \sum_{\att \in \mathcal{A}_2} \sigma^{2}_{\att} (|\att| - \valdet{\Def}{\att})  = \sum_{\att \in \mathcal{A}_2} \sigma^{2}_{\att} (|\att| - \sum_{i \in \Def}\valdet{i}{\att}) \\
%& =\sum_{\att \in \mathcal{A}_2} \sigma^{2}_{\att} \sum_{e \in \att}(1 - \sum_{i \in \Def}\valdet{i}{e}) \\
%& = \sum_{e \in \edges}\sum_{\att \in \mathcal{A}_2} \sigma^{2}_{\att}(1 - \sum_{i \in \Def}\valdet{i}{e}) \mathds{1}_{\{e \in \att\}}\\
%& = \sum_{e \in \edges}(1 - \sum_{i \in \Def}\valdet{i}{e})  \rho_{\sigma^{2}}(e) \\
%& = \sum_{k=1}^m(1 - \sum_{i \in \Def}\valdet{i}{e_k})  \frac{b_2}{m}\\
%& = b_2 - \frac{b_2}{m}\sum_{i \in \Def}\valdet{i}{\att^\prime} \\
%& \geq b_2 - \frac{b_2}{m}\sum_{i \in \Def}1 \\
%& \geq  b_2\left( 1 - \frac{b_1}{m} \right)
%%& = \sum_{e \in \edges}\rho_{\hat{\sigma}^2}(e) - \sum_{\att \in \mathcal{A}_2} \hat{\sigma}^2_{\att}\sum_{i \in \Def}\valdet{i}{e} \mathds{1}_{e \in \att}\\
%%& \geq \sum_{\att \in \mathcal{A}_2} \hat{\sigma}^2_{\att} (|\att| - \sum_{i \in \Def}1) \\
%%& \geq \sum_{\att \in \mathcal{A}_2} \hat{\sigma}^2_{\att} (|\att| - \sum_{i \in \Def}1) \\
%%&\geq  \sum_{e \in \att}\sum_{\Def \in \mathcal{A}_1}\hat{\sigma}_{\Def}^1 \valdet{\Def}{e} - |\att| \\
%%& \geq \sum_{e \in \att}\frac{b_1}{n} - |\att| = \underset{<0}{\underbrace{\left(\frac{b_1}{n}-1\right)}}|\att|\\
%%& \geq b_2 \left(\frac{b_1}{n}-1\right)
%\end{align*}
%
%
%
%\begin{align*}
%\forall k \in \llbracket 1,b_2 \rrbracket, \ \sum_{\Def \in \mathcal{A}_1} \sigma_{\Def}^1 \valdet{\Def}{e_k} = \sum_{\{\Def \in \mathcal{A}_1 \, | \, i_{k} \in \Def\}} \sigma_{\Def}^1 + \sum_{\{\Def \in \mathcal{A}_1 \, | \, i_{k} \notin \Def\}} \sigma_{\Def}^1  \times 0 = \sum_{\{\Def \in \mathcal{A}_1 \, | \, i_{k} \in \Def\}} \sigma_{\Def}^1 = \rho_{\sigma^1}(i_{k})
%\end{align*}
%
%Therefore, we obtain:
%\begin{align*}
%\widetilde{U}_1(\sigma^1,\att)  &=  \sum_{\Def \in \mathcal{A}_1}\sigma_{\Def}^1 \valdet{\Def}{\att} - |\att| = \sum_{k=1}^{b_2}\sum_{\Def \in \mathcal{A}_1}\sigma_{\Def}^1 \valdet{\Def}{e_k} - b_2 \\
%& = \sum_{k=1}^{b_2}\rho_{\sigma^1}(i_{k}) - b_2\\
%& \leq b_2 \left(\frac{b_1}{n}  - 1\right)
%\end{align*}

%Thus, $\min_{\Def \in \mathcal{A}_1} U_2(\Def,\sigma^2)  \leq b_2 \left(1 - \frac{b_1}{m} \right)$. 
This upper bound is valid for any $\sigma^2 \in \Delta(\mathcal{A}_2)$ such that $\ebasis{\sigma^2} \subseteq \att^\prime$, and does not depend on $\sigma^2$. Therefore,
%\begin{align}
$\max_{\{\sigma^2 \in \Delta(\mathcal{A}_2) \, | \, \ebasis{\sigma^2} \subseteq \att^{\prime}\}} \min_{\Def \in \mathcal{A}_1} U_2(\Def,\sigma^2) \leq b_2 \left(1 - \frac{b_1}{m}\right)$, %\label{2nd_inteq_max-min_bis}
%\end{align}
 and we can conclude that:
\begin{align*}
\max_{\{\sigma^2 \in \Delta(\mathcal{A}_2) \, | \, \ebasis{\sigma^2} \subseteq \att^\prime\}} \min_{\Def \in \mathcal{A}_1} U_2(\Def,\sigma^2) =  \min_{\Def \in \mathcal{A}_1} U_2(\Def,\sola{\att^\prime}{b_2}{}) = b_2 \left(1 - \frac{b_1}{m}\right).
\end{align*}

The optimal value of \rlpt{\att^\prime} in this case ($b_1 < m$) is $b_2 \left(1 - \frac{b_1}{m}\right) =  \max\left\{0, b_2 \left(1 - \frac{b_1}{m}\right) \right\}$, and an optimal solution is given by $\sola{\att^{\prime}}{b_2}{}$.\hfill \Halmos
\end{itemize}
\end{enumerate}
%If we consider a sensor placement $\Def^\prime$ of size $b_1$ that detects events occurring on $b_1$ edges of $\att^{\prime}$ (recall that we are in the case where $b_1<m=|\att^\prime|$). Then the inequality becomes tight:  
%
%First, we need to show that $\forall e \in \att^\prime$, $\valdet{\Def^\prime}{e} = \sum_{i \in \Def^\prime}\valdet{i}{e}$. There are two cases to consider.
%\begin{enumerate}
%\item[1)] Given $e \in \att^\prime$, if $\valdet{\Def^\prime}{e}=0$, then: 
%$$\forall i \in \Def^\prime, \ 0 \leq\valdet{i}{e}\overset{\eqref{monotonicity_detection}}{\leq} \valdet{\Def^\prime}{e}=0,$$ 
%which implies that $\sum_{i \in \Def^\prime}\valdet{i}{e} = \valdet{\Def^\prime}{e}$. 
%\item[2)] Given $e \in \att^\prime$, if $\valdet{\Def^\prime}{e}=1$, then we need to show that there exists a unique node $i \in \Def^\prime$ such that $\valdet{i}{e} = 1$. 
%
%Since $\valdet{\Def^\prime}{e}=1$, then we know from \eqref{redundant_nodes} that $\exists \, i \in \Def^\prime \ | \ \valdet{i}{e} = 1$. 
%
%Now, let us assume that $\exists \, i \neq i^{\prime} \in \Def^\prime \ | \ \valdet{i}{e} = \valdet{i^{\prime}}{e} = 1$. Then, this contradicts $\Def^\prime$ detecting events on $b_1$ edges of $\att^{\prime}$: in order to detect events on $b_1$ edges of the set packing $\att^{\prime}$, each node of $\Def^\prime$ must monitor a different edge of $\att^{\prime}$ (since we have $b_1$ sensors and a single sensor can monitor at most one edge of $\att^{\prime}$). Therefore, if $\valdet{i}{e} = \valdet{i^{\prime}}{e} = 1$, then $\Def^\prime$ monitors strictly less than $b_1$ edges of $\att^{\prime}$, which is a contradiction. \note{Do you prefer a mathematical proof of this argument?}
%
%Thus, $\exists \, !\, i \in \Def^\prime, \ | \ \valdet{i}{e} = 1$, which implies that $\valdet{\Def^\prime}{e} = \sum_{i \in \Def^\prime}\valdet{i}{e}$.
%\end{enumerate}
%
%Then, we get:
%\begin{align}
%{U}_2(\Def^\prime, \sigma^{\att^{\prime}}) &\overset{\eqref{payoff2}}{=} \sum_{\att \in \mathcal{A}_2} \sigma^{\att^{\prime}}_{\att} (|\att| - \valdet{\Def^\prime}{\att}) \nonumber \\
%& \overset{\eqref{detection_disruptions}}{=} \sum_{\att \in \mathcal{A}_2} \sigma^{\att^{\prime}}_{\att} \sum_{e \in \att}(1 - \valdet{\Def^\prime}{e}) \nonumber\\
%& = \sum_{e \in \edges}(1 - \valdet{\Def^\prime}{e})\sum_{\att \in \mathcal{A}_2} \sigma^{\att^{\prime}}_{\att}\mathds{1}_{\{e \in \att\}} \nonumber\\
%&\overset{\eqref{rho_sigma2}}{=} \sum_{e \in \edges}(1 - \valdet{\Def^\prime}{e})\rho_{\sigma^{\att^{\prime}}}(e)\nonumber\\
%&\overset{\eqref{set_disruption_prob}}{=} \sum_{e \in \att^\prime}(1 - \valdet{\Def^\prime}{e})  \frac{b_2}{m}\nonumber\\
%& = \frac{mb_2}{m} - \frac{b_2}{m}\sum_{e \in \att^\prime}\sum_{i \in \Def^\prime}\valdet{i}{e}\nonumber\\
%& \overset{\eqref{detection_disruptions}}{=} b_2 - \frac{b_2}{m}\sum_{i \in \Def^\prime}\valdet{i}{\att^\prime}\label{intermediate_1_2}
%%& \overset{\eqref{redundant_nodes}}{\geq} \sum_{\att \in \mathcal{A}_2} \sigma^{\att^{\prime}}_{\att} (|\att| - \sum_{i \in \Def}\valdet{i}{\att}) \\
%%& \overset{\eqref{detection_disruptions}}{=}\sum_{\att \in \mathcal{A}_2} \sigma^{\att^{\prime}}_{\att} \sum_{e \in \att}(1 - \sum_{i \in \Def}\valdet{i}{e}) \\
%%& = \sum_{e \in \edges}\sum_{\att \in \mathcal{A}_2} \sigma^{\att^{\prime}}_{\att}(1 - \sum_{i \in \Def}\valdet{i}{e}) \mathds{1}_{\{e \in \att\}}\\
%%& \overset{\eqref{rho_sigma2}}{=} \sum_{e \in \edges}(1 - \sum_{i \in \Def}\valdet{i}{e})  \rho_{\sigma^{\att^{\prime}}}(e) \\
%%& \overset{\eqref{set_disruption_prob}}{=} \sum_{l=1}^m(1 - \sum_{i \in \Def}\valdet{i}{e_l})  \frac{b_2}{m}\\
%%&  \overset{\eqref{detection_disruptions}}{=} b_2 - \frac{b_2}{m}\sum_{i \in \Def}\valdet{i}{\att^\prime} \\
%%& \geq b_2 - \frac{b_2}{m}\sum_{i \in \Def}1 \\
%%& \overset{\eqref{p1's set}}{\geq}  b_2\left( 1 - \frac{b_1}{m} \right)
%\end{align}
%
%Besides, we have:
%\begin{align*}
%b_1 = \valdet{\Def^\prime}{\att^\prime} \leq \sum_{i \in \Def^\prime} \valdet{i}{\att^\prime} \leq\sum_{i \in \Def^{\prime}}1 = |\Def^{\prime}| = b_1
%\end{align*}
%
%It implies that $\forall i \in \Def^{\prime}, \ \valdet{i}{\att^\prime} = 1$, which combined with \eqref{intermediate_1_2}, gives:
%\begin{align*}
%\widetilde{U}_2(\Def^\prime,\sigma^{\att^\prime}) &\overset{\eqref{intermediate_1_2}}{=} b_2 - \frac{b_2}{m}\sum_{i \in \Def^\prime}\valdet{i}{\att^\prime}\\
%& = b_2 - \frac{b_2}{m}\sum_{i \in \Def^\prime}1\\
%& = b_2 - \frac{b_2}{m}|\Def^{\prime}|\\
%& = b_2\left( 1 - \frac{b_1}{m}\right)
%\end{align*}
%
%%The second equality comes from the fact that each targeted edge is part of the extended matching $\att^{\prime}$, and the fact that $\Def$ detects events on $b_1$ edges of $\att^{\prime}$. There are two subcases to consider. 
%
%%Given $\att \in \supp(\sigma^{\att^{\prime}})$ and $e \in \att$, if $\valdet{\Def}{e}=0$, then $\forall i \in \Def, \ \valdet{i}{e}=0$, so $\sum_{i \in \Def}\valdet{i}{e} = \valdet{\Def}{e}$. 
%%
%%
%%
%%Indeed, we have:
%%\begin{align*}
%%\forall \att \in \supp(\sigma^{\att^{\prime}}), \ \sum_{i \in \Def} \valdet{i}{\att} \overset{\eqref{detection_disruptions}}{=} \sum_{e \in \att} \sum_{i \in \Def} \valdet{i}{e} = \sum_{e \in \att} \valdet{\Def}{e}  \overset{\eqref{detection_disruptions}}{=} \valdet{\Def}{\att}  
%%\end{align*}
%%
%%
%%The penultimate inequality becomes an equality since each node of $\Def$ detects exactly one event on $\att^{\prime}$. This is the same argument as previously: since $\Def$ detects $b_1$ events on $\att^{\prime}$, is composed of $b_1$ sensors, and each sensor can detect at most one event on the extended matching $\att^{\prime}$, then necessarily, each sensor placed in $\Def$ detects exactly one event on $\att^{\prime}$.
%
%
%%The last inequality becomes an equality since $|\Def| = b_1$. 
%
%Therefore $\min_{\Def \in \mathcal{A}_1}\widetilde{U}_2(\Def,\sigma^{\att^{\prime}})  = b_2 \left(1 -\frac{b_1}{m}\right)$, and we deduce that:
%\vspace{-0.5cm}
\endproof




\proof{Proof of Proposition \ref{all_resources}.}\ 

%\tb{Eq.~\eqref{res2} is shown by contraposition: If \attacker assigns positive probability on an attack $\att$ that does not use all resources, then we can find another attack (by enlarging $\att$), that improves \attacker's payoff, which can only happen if there is a component outside of $\att$ that is not monitored with probability 1 by $\defender$. If we were to assume that such a component does not exist, we would obtain a contradiction regarding the expected number of components that are not monitored by \defender, which is now \attacker's payoff. From Proposition~\ref{best_set_cover} and the duality between \lpo and \lpt, we know that this quantity is upper bounded by $\frac{b_2}{\smsc}(\smsc - b_1) < \smsc - b_1$ since $b_2 < \semm \leq \smsc$ (from weak duality between MSC and MSP). However, this cannot be, because with a sensor placement of $b_1$ sensors, the number of unmonitored components cannot be less than $\smsc - b_1$, otherwise, we could generate a set cover of size strictly less than $\smsc$. Therefore, the expected number of unmonitored components is also at least $\smsc - b_1$, and we obtain a contradiction.
%}
%Outline of the proof.
%\tb{The main idea to prove \eqref{res1} is the following: suppose that \defender assigns positive probability on a defense $\Def$ that does not use the whole budget. At equilibrium we can prove that \attacker disrupts edges that are out of range of $\Def$ because otherwise \defender would always choose $\Def$ and \attacker would change her strategy. Because of Assumption \ref{A2}, we know that there are edges out of range of $\Def$, and if we note $e \in \edges$ an edge disrupted with positive probability and that is out of range of $\Def$, then \defender would get a better payoff by transferring the probability of $\Def$ to another defense $\Def^{\prime}$ that senses the same nodes as $\Def$ plus one of the end nodes of $e$, which is a contradiction.}
%
%\tb{Similarly, at equilibrium, Prop. \ref{all_edges} tells us that \defender must randomize over defenses such that every edge is detected with positive probability. Then, Assumption \ref{A2} says that every edge in the network is not sensed by at least one of these defenses. Therefore, for every edge $e$ in the network, the probability with which an attack at $e$ is not detected is strictly positive and induces an increase in \attacker's utility. Thus \attacker has an incentive to use all her budget, and hence we obtain~\eqref{res2}.}
%
\begin{enumerate}
\item[(i.a)] First, let us show by contradiction that \defender uses all her resources in equilibrium. Suppose that $\exists \, ({\sigma^1}^*,{\sigma^2}^*) \in \nash, \ \exists\, \Def^0 \in \supp({\sigma^1}^*) \ | \ |\Def^0| <   b_1$. 
%\tr{We show first that necessarily, \attacker's attack strategy $\sigma^{2^*}$ targets with positive probability an edge that is not monitored by $\Def^0$. Then we deduce that \defender has an incentive to use her remaining sensing resources to detect that failure event and increase her payoff, leading to a contradiction.}
\begin{enumitemize}
\item[--] The first step is to show that \attacker's strategy $\sigma^{2^*}$ necessarily targets with positive probability at least one component  that is not monitored by $\Def^0$. On the contrary, assume that $\forall e \in \edges: \ \rho_{\sigma^{2^*}}(e) > 0\ \Longrightarrow\ \valdet{\Def^0}{e}=1$. Then, \defender can detect all the attacks of $\sigma^{2^*}$ with the detector positioning $\Def^0$. Thus, $\Def^0$ is a best response for \defender to $\sigma^{2^*}$, and \attacker's  payoff in equilibrium is 0. Since \attacker's  payoff is identical for any NE (direct consequence of Lemma~\ref{strategic_eq}), then \attacker's payoff for the initial NE we considered, $(\sigma^{1^*},\sigma^{2^*})$, is also 0. However, since $b_1 < \smsc$, we know that $\exists \, e^\prime \in \edges \ | \ \valdet{\Def^0}{e^\prime} = 0$, i.e., $e^\prime$ is not monitored by $\Def^0$. Since $\Def^0 \in \supp(\sigma^{1^*})$, then $e^\prime$ is not monitored with positive probability. Therefore, if \attacker targets $e^\prime$, she will get a positive payoff,
%\begin{align*}
%U_2(\sigma^{1^*},e^\prime) &\overset{\eqref{payoff2}}{=} |\{e^\prime\}| - \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def}\valdet{\Def}{e^\prime} = 1 - \sigma^{1^*}_{\Def^0}\,\underset{=0}{\underbrace{\valdet{\Def^0}{e^\prime}}} - \sum_{\Def \in \mathcal{A}_1 \backslash\{\Def^0\}}\sigma^{1^*}_{\Def}\underset{\leq 1}{\underbrace{\valdet{\Def}{e^\prime}}}\\
%& \geq 1- \sum_{\Def \in \mathcal{A}_1 \backslash\{\Def^0\}}\sigma^{1^*}_{\Def}= \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def} - \sum_{\Def \in \mathcal{A}_1 \backslash\{\Def^0\}}\sigma^{1^*}_{\Def} = \underset{>0}{\underbrace{\sigma^{1^*}_{\Def^0}}}> U_2(\sigma^{1^*},\sigma^{2^*}),
%\end{align*} 
which contradicts the equilibrium condition \eqref{best2} for $(\sigma^{1^*},\sigma^{2^*})$. Therefore, $\exists \, e_0 \in \edges \ | \ \rho_{\sigma^{2^*}}(e_0) >0$ and $\valdet{\Def^0}{e_0} = 0$. 

\item[--] Now, we can show that \defender can increase her payoff by placing one more detector. Let us denote $i_0 \in \nodes \backslash S^0$ that satisfies $\valdet{i_0}{e_0} = 1$. Then, by considering the detector positioning $\Def^{\prime} = \Def^0 \cup \{i_0\} \in \mathcal{A}_1$, we obtain that $U_1(\Def^{\prime},\sigma^{2^*}) \geq \rho_{\sigma^{2^*}}(e_0) + U_1(\Def^{0},\sigma^{2^*}) > U_1(\Def^{0},\sigma^{2^*})$%(by combining \eqref{payoff1},\eqref{rho_sigma2},\eqref{monotonicity_detection}, and \eqref{detection_disruptions}),
%\begin{align*}
%U_1(\Def^{\prime},\sigma^{2^*}) & \overset{\eqref{payoff1}}{=} \sum_{\att \in \mathcal{A}_2} \sigma^{2^*}_{\att} \valdet{\Def^{\prime}}{\att}\overset{\eqref{detection_disruptions}}{=} \sum_{\att \in \mathcal{A}_2} \sigma^{2^*}_{\att} \sum_{e \in \att} \valdet{\Def^{\prime}}{e} = \sum_{\att \in \mathcal{A}_2} \sigma^{2^*}_{\att} \sum_{e \in \edges} \valdet{\Def^{\prime}}{e} \mathds{1}_{\{e \in \att\}}\\
%&=\sum_{e \in \edges} \valdet{\Def^{\prime}}{e} \sum_{\att \in \mathcal{A}_2} \sigma^{2^*}_{\att} \mathds{1}_{\{e \in \att\}} \overset{\eqref{rho_sigma2}}{=}\sum_{e \in \edges} \valdet{\Def^{\prime}}{e} \rho_{\sigma^{2^*}}(e)\\
%& =\rho_{\sigma^{2^*}}(e_0) + \sum_{e \in \edges\backslash\{e_0\}} \valdet{\Def^{\prime}}{e} \rho_{\sigma^{2^*}}(e)\overset{\eqref{monotonicity_detection}}{\geq} \rho_{\sigma^{2^*}}(e_0) + \sum_{e \in \edges\backslash\{e_0\}} \valdet{\Def^{0}}{e} \rho_{\sigma^{2^*}}(e)\\
%& = \rho_{\sigma^{2^*}}(e_0) + \sum_{e \in \edges} \valdet{\Def^{0}}{e} \rho_{\sigma^{2^*}}(e)  \overset{\eqref{payoff1}}{=} \underset{>0}{\underbrace{\rho_{\sigma^{2^*}}(e_0)}}  + U_1(\Def^{0},\sigma^{2^*})\\
%& > U_1(\Def^{0},\sigma^{2^*}),
%\end{align*}
%\begin{align*}
%U_1(\Def^{\prime},\sigma^{2^*}) & \overset{\eqref{payoff1}}{=} \mathbb{E}_{\sigma^{2^*}}[\valdet{\Def^\prime}{\att}] \overset{\eqref{detection_disruptions}}{=} \mathbb{E}_{\sigma^{2^*}}[\sum_{e \in \edges}\valdet{\Def^\prime}{e}\mathds{1}_{\{e \in \att\}}]  \overset{\eqref{rho_sigma2}}{=}\sum_{e \in \edges} \valdet{\Def^{\prime}}{e} \rho_{\sigma^{2^*}}(e)\\
%& =\rho_{\sigma^{2^*}}(e_0) + \sum_{e \in \edges\backslash\{e_0\}} \valdet{\Def^{\prime}}{e} \rho_{\sigma^{2^*}}(e)\overset{\eqref{monotonicity_detection}}{\geq} \rho_{\sigma^{2^*}}(e_0) + \sum_{e \in \edges\backslash\{e_0\}} \valdet{\Def^{0}}{e} \rho_{\sigma^{2^*}}(e)\\
%& = \rho_{\sigma^{2^*}}(e_0) + \sum_{e \in \edges} \valdet{\Def^{0}}{e} \rho_{\sigma^{2^*}}(e)  \overset{\eqref{payoff1}}{=} \underset{>0}{\underbrace{\rho_{\sigma^{2^*}}(e_0)}}  + U_1(\Def^{0},\sigma^{2^*}) > U_1(\Def^{0},\sigma^{2^*}),
%\end{align*}
%\begin{align*}
%U_1(\Def^{\prime},\sigma^{2^*}) & \overset{\eqref{payoff1},\eqref{detection_disruptions},\eqref{rho_sigma2}}{=} \rho_{\sigma^{2^*}}(e_0) + \sum_{e \in \edges\backslash\{e_0\}} \valdet{\Def^{\prime}}{e} \rho_{\sigma^{2^*}}(e)\overset{\eqref{monotonicity_detection}}{\geq} \rho_{\sigma^{2^*}}(e_0) + \sum_{e \in \edges\backslash\{e_0\}} \valdet{\Def^{0}}{e} \rho_{\sigma^{2^*}}(e)\\
%& = \rho_{\sigma^{2^*}}(e_0) + \sum_{e \in \edges} \valdet{\Def^{0}}{e} \rho_{\sigma^{2^*}}(e)  \overset{\eqref{payoff1}}{=} \underset{>0}{\underbrace{\rho_{\sigma^{2^*}}(e_0)}}  + U_1(\Def^{0},\sigma^{2^*}) > U_1(\Def^{0},\sigma^{2^*}),
%\end{align*}
, which violates the equilibrium condition \eqref{best1} for $({\sigma^1}^*,{\sigma^2}^*)$. Therefore, $\forall \Def \in \supp(\sigma^{1^*}), \ |\Def| = b_1$.

\end{enumitemize}

\item[(i.b)] Now, let us show that \attacker uses all her resources  in equilibrium. By contradiction, suppose that $\exists \, (\sigma^{1^*},\sigma^{2^*}) \in \nash,\ \exists \, \att^0 \in \supp(\sigma^{2^*}) \ | \ |\att^0| <b_2$. 
%\tr{If we manage to show that there exists an edge  not in $\att^0$ that is unmonitored with positive probability by \defender's sensing strategy $\sigma^{1^*}$, then \attacker would increase her payoff by targeting that edge as well, and this would prevent $\att^0$ from being part of an equilibrium strategy.}
\begin{enumitemize}
\item[--] The first step is to show that there exists a component $e^{\prime}$ not in $\att^0$ that is not monitored by every detector positioning in the support of $\sigma^{1^*}$.
%; this would imply that \attacker can improve her payoff by using her remaining attack resources to target that component. 
Let us assume the contrary, i.e., that $
\forall \Def \in \supp(\sigma^{1^*}), \ \forall e \notin \att^0, \ \valdet{\Def}{e} = 1.$
%all the components not in $\att^0$ are monitored by every detector positioning in the support of $\sigma^{1^*}$: 
First, let us denote $\att^1 \subseteq \att^0$ the subset of components of $\att^0$ that are unmonitored by at least one detector positioning $\Def \in \supp(\sigma^{1^*})$, i.e.,  $\att^1 \coloneqq  \bigcup_{\Def \in \supp(\sigma^{1^*})} (\edges\backslash\set{\Def}) \subseteq \att^0.$

For all $S \in \supp(\sigma^{1^*})$, let $k_S$ denote the number of components of $T^1$ that are not monitored by $S$. 
Since every component outside of $\att^{1}$ is monitored by every detector positioning in the support of $\sigma^{1^*}$, then \attacker's best response to $\sigma^{1^*}$ is any attack plan $\att \in \mathcal{A}_2$ such that $\att^1 \subseteq \att$ (note that $|\att^1| \leq  b_2$), and \attacker's equilibrium  payoff is equal to $k^* \coloneqq \mathbb{E}_{\sigma^{1^*}}[k_S]$. %This is shown in the following steps:
%\begin{align*}
%\forall \att \in \mathcal{A}_2 \ | \ \att^1 \subseteq \att, \ U_2(\sigma^{1^*},\att) &\overset{\eqref{payoff2}}{=} |\att| - \sum_{\Def \in \mathcal{A}_1} \sigma^{1^*}_{\Def} \valdet{\Def}{\att} \overset{\eqref{detection_disruptions}}{=} |\att| - \sum_{\Def \in \mathcal{A}_1} \sigma^{1^*}_{\Def} \sum_{e \in \att}\valdet{\Def}{e}\\
%& = |\att| - \sum_{e \in \att^1}\sum_{\Def \in \mathcal{A}_1} \sigma^{1^*}_{\Def} \valdet{\Def}{e} - \sum_{e \in \att \backslash \att^1}\sum_{\Def \in \mathcal{A}_1} \sigma^{1^*}_{\Def} \underset{=1}{\underbrace{\valdet{\Def}{e}}}\\
%& = |\att| -\sum_{\Def \in \mathcal{A}_1} \sigma^{1^*}_{\Def}  \sum_{e \in \att^1}\valdet{\Def}{e} - \sum_{e \in \att \backslash \att^1}\underset{=1}{\underbrace{\sum_{\Def \in \mathcal{A}_1} \sigma^{1^*}_{\Def}}}\\
%&  \overset{\eqref{detection_disruptions}}{=} |\att| - \sum_{\Def \in \mathcal{A}_1} \sigma^{1^*}_{\Def} \valdet{\Def}{\att^1} - |\att\backslash\att^1|\\
%%& = |\att^1| - \sum_{e \in \att^1}\sum_{\Def \in \mathcal{A}_1} \sigma^{1^*}_{\Def} \valdet{\Def}{e}\\
%& = |\att^1| - \sum_{\Def \in \mathcal{A}_1} \sigma^{1^*}_{\Def} \valdet{\Def}{\att^1} = |\att^1| - \sum_{\Def \in \mathcal{A}_1} \sigma^{1^*}_{\Def} (|\att^1|-k_\Def)\\
%& = |\att^1|\left(1 -  \sum_{\Def \in \mathcal{A}_1} \sigma^{1^*}_{\Def}\right)  + \sum_{\Def \in \mathcal{A}_1} \sigma^{1^*}_{\Def}k_\Def\\
%& = \mathbb{E}_{\sigma^{1^*}}[k_S].
%\end{align*}
%\begin{align*}
%\forall \att \in \mathcal{A}_2 &\ | \ \att^1 \subseteq \att, \ U_2(\sigma^{1^*},\att) \overset{\eqref{payoff2}}{=} |\att| - \mathbb{E}_{\sigma^{1^*}}[\valdet{\Def}{\att}] \overset{\eqref{additive_equality}}{=} |\att| - \mathbb{E}_{\sigma^{1^*}}[\valdet{\Def}{\att^1}] - \mathbb{E}_{\sigma^{1^*}}[\valdet{\Def}{\att\backslash\att^1}]\\
%& = |\att| - \mathbb{E}_{\sigma^{1^*}}[|\att^1| - k_\Def] - \mathbb{E}_{\sigma^{1^*}}[|\att\backslash\att^1|] =\mathbb{E}_{\sigma^{1^*}}[k_\Def].
%&  =|\att| - \sum_{e \in \att^1}\mathbb{E}_{\sigma^{1^*}}[\valdet{\Def}{e}] - \sum_{e \in \att\backslash\att^1}\mathbb{E}_{\sigma^{1^*}}[\valdet{\Def}{e}] \\
%& = |\att| - \sum_{e \in \att^1}\sum_{\Def \in \mathcal{A}_1} \sigma^{1^*}_{\Def} \valdet{\Def}{e} - \sum_{e \in \att \backslash \att^1}\sum_{\Def \in \mathcal{A}_1} \sigma^{1^*}_{\Def} \underset{=1}{\underbrace{\valdet{\Def}{e}}}\\
%& = |\att| -\sum_{\Def \in \mathcal{A}_1} \sigma^{1^*}_{\Def}  \sum_{e \in \att^1}\valdet{\Def}{e} - \sum_{e \in \att \backslash \att^1}\underset{=1}{\underbrace{\sum_{\Def \in \mathcal{A}_1} \sigma^{1^*}_{\Def}}}\\
%&  \overset{\eqref{detection_disruptions}}{=} |\att| - \sum_{\Def \in \mathcal{A}_1} \sigma^{1^*}_{\Def} \valdet{\Def}{\att^1} - |\att\backslash\att^1|\\
%%& = |\att^1| - \sum_{e \in \att^1}\sum_{\Def \in \mathcal{A}_1} \sigma^{1^*}_{\Def} \valdet{\Def}{e}\\
%& = |\att^1| - \sum_{\Def \in \mathcal{A}_1} \sigma^{1^*}_{\Def} \valdet{\Def}{\att^1} = |\att^1| - \sum_{\Def \in \mathcal{A}_1} \sigma^{1^*}_{\Def} (|\att^1|-k_\Def)\\
%& = |\att^1|\left(1 -  \sum_{\Def \in \mathcal{A}_1} \sigma^{1^*}_{\Def}\right)  + \sum_{\Def \in \mathcal{A}_1} \sigma^{1^*}_{\Def}k_\Def\\
%& = \mathbb{E}_{\sigma^{1^*}}[k_S].
%\end{align*}
%
%Then, $\sigma^{2^*} \in \Delta(\mathcal{A}_2)$ is an equilibrium strategy only if $\forall \att \in \supp(\sigma^{2^*}), \ \att^1 \subseteq \att$.
%
%Recall that our original $\sigma^{1^*}$
Thus, \defender's equilibrium payoff in the zero-sum game $\widetilde{\Gamma}$ is equal to $-k^*$. From Proposition~\ref{best_set_cover}, we know that $-k^* \geq b_2\left(\frac{b_1}{\smsc}- 1 \right)$. Since we are in the case when $b_2 < \semm$, and we have $\semm \leq \smsc$ (Lemma~\ref{MM<MSC}), then we obtain:
\begin{align}
k^* \leq \frac{b_2}{\smsc }\left(\smsc  - b_1\right) <\frac{\semm}{\smsc }\left(\smsc  - b_1\right)\leq \smsc  - b_1. \label{too_many_detections}
\end{align}
%because $b_2 < m^* \leq n^*$ due to \aref{b1<MSC}.

Consider $\Def \in \supp(\sigma^{1^*})$. We know that $\Def$ leaves $k_\Def$ network components unmonitored, that we denote $e_1,\dots,e_{k_\Def}$. For $l \in \llbracket 1,k_{\Def}\rrbracket$, let  $i_l$ be a node from where a detector can monitor component $e_l$. Then, $
\Def \cup\{i_1,\dots,i_{k_{\Def}}\}$ is a set cover (of size at most $b_1+k_\Def$). By definition of $\smsc$, we deduce that $b_1 + k_S \geq \smsc$. Therefore, $\forall S \in \supp(\sigma^{1^*}), \ k_S \geq \smsc - b_1$.
%Since the MSCs have a size equal to $\smsc$, then necessarily $b_1 + k_S \geq \smsc$. Indeed, if we had instead $b_1 + k_S < \smsc$, we would be able to monitor all the edges of the network by adding $k_S$ sensors to the sensor placement $S$ of size $b_1$ and it would contradict $\smsc$ being the size of the minimum set covers. Therefore $\forall S \in \supp(\sigma^{1^*}), \ k_S \geq \smsc - b_1$.
This last result implies that $k^* =  \mathbb{E}_{\sigma^{1^*}}[k_S] \geq \smsc - b_1$, which contradicts \eqref{too_many_detections}.
Thus, $\exists \, (e^\prime,\Def^\prime) \in \edges\backslash\att^0 \times \supp(\sigma^{1^*}) \ | \  \valdet{\Def^\prime}{e^\prime} = 0$. 
%there exists a component $e^{\prime}$ not in $\att^0$ that is  not monitored by at least one detector positioning, denoted $\Def^\prime$, in the support of $\sigma^{1^*}$.



%Consider a defense $\Def$ in the support of $\sigma^{1^*}$. \tb{Because of \aref{b1<MSC}, we know that there exists an attack $\att$ that is not detected by $\Def$ and that uses all \attacker's resources. In other words, there exist $b_2$ edges that are not detected by $\Def$. Since $\att^0$ disrupts less than $b_2$ edges, then there exists an edge $e^{\prime}$ that is not detected by $\Def$. Therefore there exists an edge $e^{\prime}$ not attacked by $\att^0$ that is not detected by every defense in the support of $\sigma^{1^*}$.}

\item[--] Now, we can show that \attacker can increase her payoff by targeting component $e^{\prime}$ and the components in $\att^0$.  Let $\att^{\prime} = \att^0 \cup \{e^{\prime}\} \in \mathcal{A}_2$ (since $|T^0| <b_2$). Then, we get $U_2(\sigma^{1^*},\att^{\prime}) \geq  \sigma^{1^*}_{\Def^\prime} + U_2(\sigma^{1^*},\att^{0}) > U_2(\sigma^{1^*},\att^{0})$, 
%\begin{align*}
%U_2(\sigma^{1^*},\att^{\prime})  & \overset{\eqref{payoff2}}{=}  |\att^{\prime}| - \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def}\valdet{\Def}{\att^{\prime}}   \overset{\eqref{detection_disruptions}}{=}|\att^{\prime}| - \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def}\sum_{e \in \att^{\prime} }\valdet{\Def}{e} \\
%& =  \sum_{e \in \att^{\prime}}\left(1 - \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def}\valdet{\Def}{e}\right) \\
% &=  1 - \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def}\valdet{\Def}{e^{\prime}} +\sum_{e \in \att^{\prime}\backslash\{e^{\prime}\}}\left(1 - \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def}\valdet{\Def}{e}\right) \\
%  &=  \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def}\left(1 - \valdet{\Def}{e^{\prime}}\right) +\sum_{e \in \att^{\prime}\backslash\{e^{\prime}\}}\left(1 - \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def}\valdet{\Def}{e}\right) \\
%    &=  \sigma^{1^*}_{\Def^\prime}(1 - \underset{=0}{\underbrace{\valdet{\Def^\prime}{e^\prime}}}) + \underset{\geq0}{\underbrace{\sum_{\Def \in \mathcal{A}_1\backslash\{\Def^\prime\}}\sigma^{1^*}_{\Def}\left(1 - \valdet{\Def}{e^{\prime}}\right)}}+\sum_{e \in \att^{\prime}\backslash\{e^{\prime}\}}\left(1 - \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def}\valdet{\Def}{e}\right) \\
%  & \geq  \underset{>0}{\underbrace{\sigma^{1^*}_{\Def^\prime}}} + \sum_{e \in \att^{\prime}\backslash\{e^{\prime}\}}\left(1 - \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def}\valdet{\Def}{e}\right) \\
%&>   \sum_{e \in \att^{\prime}\backslash\{e^{\prime}\}}\left(1 - \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def}\valdet{\Def}{e}\right) =  \sum_{e \in \att^0}\left(1 - \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def}\valdet{\Def}{e}\right) \\
%&\overset{\eqref{detection_disruptions}}{=}|\att^{0}| - \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def}\valdet{\Def}{\att^0}  \overset{\eqref{payoff2}}{=}   U_2(\sigma^{1^*},\att^{0}),
%\end{align*}
%\begin{align*}
%U_2(\sigma^{1^*},\att^{\prime})-  U_2(\sigma^{1^*},\att^{0})& \overset{\eqref{payoff2}}{=}  |\att^{\prime}| - \mathbb{E}_{\sigma^{1^*}}[\valdet{\Def}{\att^\prime}] - |\att^0|  + \mathbb{E}_{\sigma^{1^*}}[\valdet{\Def}{\att^0}]\overset{\eqref{additive_equality}}{=}1 -\mathbb{E}_{\sigma^{1^*}}[\valdet{\Def}{e^\prime}] \\
%& = \mathbb{E}_{\sigma^{1^*}}[\underset{\geq 0}{\underbrace{1 - \valdet{\Def}{e^\prime}}}]  \geq \underset{>0}{\underbrace{\sigma^{1^*}_{\Def^\prime}}}(1 - \underset{=0}{\underbrace{\valdet{\Def}{e^\prime}}}) > 0, 
%& =  \sum_{e \in \att^{\prime}}\left(1 - \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def}\valdet{\Def}{e}\right) \\
% &=  1 - \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def}\valdet{\Def}{e^{\prime}} +\sum_{e \in \att^{\prime}\backslash\{e^{\prime}\}}\left(1 - \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def}\valdet{\Def}{e}\right) \\
%  &=  \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def}\left(1 - \valdet{\Def}{e^{\prime}}\right) +\sum_{e \in \att^{\prime}\backslash\{e^{\prime}\}}\left(1 - \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def}\valdet{\Def}{e}\right) \\
%    &=  \sigma^{1^*}_{\Def^\prime}(1 - \underset{=0}{\underbrace{\valdet{\Def^\prime}{e^\prime}}}) + \underset{\geq0}{\underbrace{\sum_{\Def \in \mathcal{A}_1\backslash\{\Def^\prime\}}\sigma^{1^*}_{\Def}\left(1 - \valdet{\Def}{e^{\prime}}\right)}}+\sum_{e \in \att^{\prime}\backslash\{e^{\prime}\}}\left(1 - \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def}\valdet{\Def}{e}\right) \\
%  & \geq  \underset{>0}{\underbrace{\sigma^{1^*}_{\Def^\prime}}} + \sum_{e \in \att^{\prime}\backslash\{e^{\prime}\}}\left(1 - \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def}\valdet{\Def}{e}\right) \\
%&>   \sum_{e \in \att^{\prime}\backslash\{e^{\prime}\}}\left(1 - \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def}\valdet{\Def}{e}\right) =  \sum_{e \in \att^0}\left(1 - \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def}\valdet{\Def}{e}\right) \\
%&\overset{\eqref{detection_disruptions}}{=}|\att^{0}| - \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def}\valdet{\Def}{\att^0}  \overset{\eqref{payoff2}}{=}   U_2(\sigma^{1^*},\att^{0}),
%\end{align*}
which is a contradiction. Therefore, $\forall \att \in \supp(\sigma^{2^*}), \ |\att|= b_2$.
\end{enumitemize}
%\end{enumerate}
%\hfill \Halmos
%\endproof
%
%
%\proof{Proof of Proposition~\ref{all_resources}.}\
%\begin{enumerate}
\item[(ii)] Finally, we show that \defender's strategies in equilibrium are the optimal solutions of \lpob. First, from (i), we can deduce that the set of optimal solutions of \lpo is a subset of $\Delta(\overline{\mathcal{A}_1})$. 
%
%Indeed, if there exists an optimal solution $\sigma^{1^*}$ of \lpo that is not in $\Delta(\overline{\mathcal{A}_1})$, then $\exists \, \Def \in \supp(\sigma^{1^*}) \ | \ |\Def| < b_1$, which is a contradiction since optimal solutions of \lpo are the sensing strategies in equilibrium, and should satisfy \eqref{res1} in Proposition~\ref{all_resources}. 
Therefore, the equilibrium inspection strategies are the optimal solutions of $\max_{\sigma^1 \in \Delta(\overline{\mathcal{A}_1})} \min_{\att \in \mathcal{A}_2} -{U}_2(\sigma^1,\att).$

Now, consider an inspection strategy $\sigma^1 \in \Delta(\overline{\mathcal{A}_1})$. Since $\overline{\mathcal{A}_2} \subseteq \mathcal{A}_2$, then we trivially have $\min_{\att \in \mathcal{A}_2} -U_2(\sigma^1,\att) \leq \min_{\att \in \overline{\mathcal{A}_2}} -U_2(\sigma^1,\att)$. To obtain the reverse inequality, 
%\begin{align}
%.\label{(in)equality}
%\end{align}
let $\att^0 \in \mathcal{A}_2$ be an attack plan that satisfies $
\att^0 \in \argmin_{\att \in \mathcal{A}_2} - U_2(\sigma^1,\att).$ Then, consider $\att^\prime \in \overline{\mathcal{A}_2} \ | \ \att^0 \subseteq \att^\prime$. We can deduce that $\min_{\att \in \mathcal{A}_2}-U_2(\sigma^1,\att)=  -U_2(\sigma^1,\att^0)  \geq -U_2(\sigma^1,\att^{\prime}) \geq \min_{\att \in \overline{A_2}} -U_2(\sigma^1,\att)$.
%\begin{align}
%\min_{\att \in \mathcal{A}_2}-U_2(\sigma^1,\att) =  -U_2(\sigma^1,\att^0) &\overset{\eqref{payoff2}}{=} \sum_{\Def \in \mathcal{A}_1}\sigma^1_{\Def} \valdet{\Def}{\att^0} - |\att^0| \overset{\eqref{detection_disruptions}}{=} \sum_{e \in \att^0} \left( \sum_{\Def \in \mathcal{A}_1}\sigma^1_{\Def}\valdet{\Def}{e} - 1  \right)\nonumber\\
%& = \sum_{e \in \att^{\prime}} \left( \sum_{\Def \in \mathcal{A}_1}\sigma^1_{\Def}\valdet{\Def}{e} - 1  \right) - \sum_{e \in \att^{\prime}\backslash\att^0} \underset{\leq 0}{\underbrace{\left( \sum_{\Def \in \mathcal{A}_1}\sigma^1_{\Def}\valdet{\Def}{e} - 1  \right) }}\nonumber\\
%& \geq \sum_{e \in \att^{\prime}} \left( \sum_{\Def \in \mathcal{A}_1}\sigma^1_{\Def}\valdet{\Def}{e} - 1  \right) \overset{\eqref{payoff2}}{=} -U_2(\sigma^1,\att^{\prime})\nonumber\\
%& \geq \min_{\att \in \overline{A_2}} -U_2(\sigma^1,\att).\label{une equation}
%\end{align}
%\begin{align}
%\min_{\att \in \mathcal{A}_2}-U_2(\sigma^1,\att) &=  -U_2(\sigma^1,\att^0) \overset{\eqref{payoff2}}{=} 
%\mathbb{E}_{\sigma^1}[\valdet{\Def}{\att^0}] - |\att^0| \nonumber\\
%&\overset{\eqref{additive_equality}}{=} \mathbb{E}_{\sigma^1}[\valdet{\Def}{\att^\prime}]  - |\att^\prime| - \mathbb{E}_{\sigma^1}[\underset{\leq |\att^\prime\backslash\att^0|}{\underbrace{\valdet{\Def}{\att^\prime\backslash\att^0}}}] + |\att^\prime \backslash \att^0|    \nonumber\\&\overset{\eqref{payoff2}}{\geq} -U_2(\sigma^1,\att^{\prime})
%%& = \sum_{e \in \att^{\prime}} \left( \sum_{\Def \in \mathcal{A}_1}\sigma^1_{\Def}\valdet{\Def}{e} - 1  \right) - \sum_{e \in \att^{\prime}\backslash\att^0} \underset{\leq 0}{\underbrace{\left( \sum_{\Def \in \mathcal{A}_1}\sigma^1_{\Def}\valdet{\Def}{e} - 1  \right) }}\nonumber\\
%%& \geq \sum_{e \in \att^{\prime}} \left( \sum_{\Def \in \mathcal{A}_1}\sigma^1_{\Def}\valdet{\Def}{e} - 1  \right) \overset{\eqref{payoff2}}{=} -U_2(\sigma^1,\att^{\prime})\nonumber\\
% \geq \min_{\att \in \overline{A_2}} -U_2(\sigma^1,\att).\label{une equation}
%\end{align}


Therefore,  $\forall \sigma^1 \in \Delta(\overline{\mathcal{A}_1}), \ \min_{\att \in \mathcal{A}_2} -U_2(\sigma^1,\att) = \min_{\att \in \overline{\mathcal{A}_2}} -U_2(\sigma^1,\att)$, which implies that 
%Then, we show that for any sensing strategy $\sigma^1 \in \Delta(\mathcal{A}_1)$, we have:
%\begin{align*}
%\min_{\att \in \mathcal{A}_2} -U_2(\sigma^1,\att) = \min_{\att \in \overline{\mathcal{A}_2}} -U_2(\sigma^1,\att).
%\end{align*}
%Since $\overline{\mathcal{A}_2} \subset \mathcal{A}_2$, this is equivalent to showing that:
%\begin{align}
%\min_{\att \in \mathcal{A}_2} -U_2(\sigma^1,\att) \geq \min_{\att \in \overline{\mathcal{A}_2}} -U_2(\sigma^1,\att).\label{(in)equality}
%\end{align}
%Consider a sensing strategy $\sigma^1 \in \Delta(\mathcal{A}_1)$, and $(\att,\att^{\prime}) \in \mathcal{A}_2\times \overline{\mathcal{A}_2} \ | \ \att \subseteq \att^{\prime}$. Then we have:
%\begin{align*}
%-U_2(\sigma^1,\att) &\overset{\eqref{payoff2}}{=} \sum_{\Def \in \mathcal{A}_1}\sigma^1_{\Def} \valdet{\Def}{\att} - |\att| \overset{\eqref{detection_disruptions}}{=} \sum_{e \in \att} \left( \sum_{\Def \in \mathcal{A}_1}\sigma^1_{\Def}\valdet{\Def}{e} - 1  \right)\\
%& = \sum_{e \in \att^{\prime}} \left( \sum_{\Def \in \mathcal{A}_1}\sigma^1_{\Def}\valdet{\Def}{e} - 1  \right) - \sum_{e \in \att^{\prime}\backslash\att} \underset{\leq 0}{\underbrace{\left( \sum_{\Def \in \mathcal{A}_1}\sigma^1_{\Def}\valdet{\Def}{e} - 1  \right) }}\\
%& \geq \sum_{e \in \att^{\prime}} \left( \sum_{\Def \in \mathcal{A}_1}\sigma^1_{\Def}\valdet{\Def}{e} - 1  \right)\\
%& \overset{\eqref{payoff2}}{=} -U_2(\sigma^1,\att^{\prime})
%\end{align*}
%
%Therefore, for any $\att \in \mathcal{A}_2$, we can find an attack $\att^\prime \in \overline{\mathcal{A}_2}$ such that $-U_2(\sigma^1,\att) \geq - U_2(\sigma^1,\att^\prime)$, which shows \eqref{(in)equality}.
%Since this is true for any sensing strategy $\sigma^1 \in \Delta(\overline{\mathcal{A}_1})$, we can conclude that 
$
\max_{\sigma^1 \in \Delta(\overline{\mathcal{A}_1})} \min_{\att \in \mathcal{A}_2} -{U}_2(\sigma^1,\att) = \max_{\sigma^1 \in \Delta(\overline{\mathcal{A}_1})} \min_{\att \in \overline{\mathcal{A}_2}} -{U}_2(\sigma^1,\att).$ Furthermore,  $\forall (\sigma^1,\att) \in \Delta(\overline{\mathcal{A}_1}) \times\overline{\mathcal{A}_2}, -U_2(\sigma^1,\att) \overset{\eqref{transform1}}{=} U_1(\sigma^1,\att) - b_2$. Thus, the equilibrium inspection strategies are the optimal solutions of \lpob.
An analogous proof can be applied to show that the equilibrium attack strategies are the optimal solutions of \lptb.\hfill \Halmos
%Therefore, $(\sigma^1,z)$ is also a feasible solution of $(\widetilde{\text{LP}_1})$.
%
%Thus, $(\widetilde{\text{LP}_1})$ and $(\overline{\text{LP}_1})$ have the same set of feasible solutions and are then equal.
%
%Therefore, $(\text{LP}_1) = (\overline{\text{LP}_1})$.
%\item[(ii.b)] \tr{Again, from \eqref{res2} in Prop.~\ref{all_resources}, we can deduce that the set of optimal solutions of \lpt is a subset of $\Delta(\overline{\mathcal{A}_2})$, and the attack strategies in equilibrium are the optimal solutions of the following linear program:}\hypertarget{LP2tilde}{}
%\begin{align*}
%(\widetilde{\text{LP}_2})  \quad \displaystyle \max_{\sigma^2 \in \Delta(\overline{\mathcal{A}_2})} \min_{\Def \in \mathcal{A}_1} {U}_2(\Def,\sigma^2).
%\end{align*}
%
%
%
%
%%The same arguments prove that $(\text{LP}_2) = (\widetilde{\text{LP}_2})$, and that the set of feasible solutions of $(\widetilde{\text{LP}_2})$ is included in the set of feasible solutions of $(\overline{\text{LP}_2})$.
%%
%%Now, we argue that any feasible solution of $(\overline{\text{LP}_2})$ is a feasible solution of $(\widetilde{\text{LP}_2}) $. Consider $(\sigma^2,z^{\prime}) \in \Delta(\overline{\mathcal{A}_2}) \times \mathbb{R} \ | \ \forall \Def \in \overline{\mathcal{A}_1}, \ \widetilde{U}_2(\Def,\sigma^2) \geq z^{\prime}$, and let us show that $\forall \Def \in \mathcal{A}_1, \ \widetilde{U}_2(\Def,\sigma^2) \geq z^{\prime}$.
%
%Now, consider an attack strategy $\sigma^2 \in \Delta(\overline{\mathcal{A}_2})$, and let $\Def^0 \in \mathcal{A}_1$ be a  sensor placement that satisfies: $
%\Def^0 \in \argmin_{\Def \in \mathcal{A}_1} U_2(\Def,\sigma^2).$ Then, consider $\Def^{\prime} \in \overline{\mathcal{A}_1}$   such that  $\Def^0 \subseteq \Def^{\prime}$. We can deduce that:
%\begin{align}
%\min_{\Def \in \mathcal{A}_1} U_2(\Def,\sigma^2) &= U_2(\Def^0,\sigma^2) \overset{\eqref{payoff2}}{=} \sum_{\att \in \mathcal{A}_2}\sigma^2_{\att}\left(|\att| - \valdet{\Def^0}{\att} \right) \nonumber\\
%&\overset{\eqref{monotonicity_detection}}{\geq} \sum_{\att \in \mathcal{A}_2}\sigma^2_{\att}\left(|\att| - \valdet{\Def^{\prime}}{\att} \right)\overset{\eqref{payoff2}}{=}  U_2(\Def^{\prime},\sigma^2)\geq \min_{\Def \in \overline{\mathcal{A}_1}} U_2(\Def,\sigma^2).\nonumber%\label{(in)equality2}
%\end{align}
%%(since $\Def^{\prime} \in \overline{\mathcal{A}_1}$).
%
%%Therefore:
%%\begin{align}
%%\forall \sigma^2 \in \Delta(\mathcal{A}_2), \ \min_{\Def \in \mathcal{A}_2} U_2(\Def,\sigma^2) \geq \min_{\Def \in \overline{\mathcal{A}_2}} U_2(\Def,\sigma^2).
%%\end{align} 
%
%Since $\overline{\mathcal{A}_2} \subset \mathcal{A}_2$, then the reverse inequality is also true, which implies that:
%\begin{align}
%\min_{\Def \in \mathcal{A}_2} U_2(\Def,\sigma^2) = \min_{\Def \in \overline{\mathcal{A}_2}} U_2(\Def,\sigma^2). \label{Almosst}
%\end{align}
%
%Since \eqref{Almosst} holds for any attack strategy $\sigma^{2} \in \Delta(\overline{\mathcal{A}_2})$, this implies that:
%\begin{align*}
%\max_{\sigma^2 \in \Delta(\overline{\mathcal{A}_2})}\min_{\Def \in \mathcal{A}_2} U_2(\Def,\sigma^2) = \max_{\sigma^2 \in \Delta(\overline{\mathcal{A}_2})}\min_{\Def \in \overline{\mathcal{A}_2}} U_2(\Def,\sigma^2),
%\end{align*}
%and the attack strategies in equilibrium are the optimal solutions of \lptb.
%
%Therefore, $(\sigma^2,z)$ is also a feasible solution of $(\widetilde{\text{LP}_2})$.
%
%Thus, $(\widetilde{\text{LP}_2})$ and $(\overline{\text{LP}_2})$ have the same set of feasible solutions and are then equal.
%
%Therefore, $(\text{LP}_2) = (\overline{\text{LP}_2})$.
\end{enumerate}
%\vspace{-0.5cm}
\endproof


\proof{Proof of Proposition~\ref{all_edges}.}\
\begin{enumerate}
\item
We show the result by contradiction, that is, suppose that $\exists \, ({\sigma^1}^*,{\sigma^2}^*) \in \nash$ such that $\nbasis{\sigma^{1^*}}$ is not a set cover. For simplicity, we introduce the following notation:
\begin{align}
\forall e \in \edges, \ \eta_{\sigma^{1^*}}(e) := \mathbb{E}_{\sigma^{1^*}}[\valdet{\Def}{e}].\label{eta_detection}
\end{align}
%which is the probability with which component $e$ is monitored by $\sigma^{1^*}$.
Let us sort the components in nondecreasing order of monitoring probability: $
\eta_{\sigma^{1^*}}(e_1) \leq \eta_{\sigma^{1^*}}(e_2) \leq \dots \leq \eta_{\sigma^{1^*}}(e_{|\edges|}).$ Then,  $\att^{\prime} = \{e_1,\dots,e_{b_2}\}$ is a best response to $\sigma^{1^*}$ for \attacker  (recall that \attacker uses all her resources; see Proposition~\ref{all_resources}).
%
%
%since \attacker maximizes her payoff when targeting components that are monitored with the smallest probability, it is easy to see that $\att^{\prime} = \{e_1,\dots,e_{b_2}\}$ is a best response for \attacker (recall that \attacker uses all her resources; see Proposition~\ref{all_resources}). 
%\begin{align*}
%0 =  \eta_{\sigma^{1^*}}(e_1) = \dots = \eta_{\sigma^{1^*}}(e_k) <   \eta_{\sigma^{1^*}}(e_{k+1}) \leq \eta_{\sigma^{1^*}}(e_{k+2}) \leq \dots \leq \eta_{\sigma^{1^*}}(e_{|\edges|}).
%\end{align*}
Let  $\att^0 = \{e_1,\dots,e_{k}\} \in 2^{\edges}$ denote the components that are not monitored by any detector positioning $\Def \in \supp(\sigma^{1^*})$. Then,  $\eta_{\sigma^{1^*}}(e_1) = \dots = \eta_{\sigma^{1^*}}(e_k) = 0$, and  \attacker's equilibrium payoff is:
%\begin{align}
%U_2(\sigma^{1^*},\att^{\prime}) & = |\att^{\prime}| - \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def} \valdet{\Def}{\att^{\prime}} \overset{\eqref{detection_disruptions}}{=} b_2 - \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def} \sum_{e \in \att^{\prime}}\valdet{\Def}{e} \overset{\eqref{eta_detection}}{=}  b_2 - \sum_{e \in \att^{\prime}}\eta_{\sigma^{1^*}}(e)\nonumber\\
%& =   b_2 - \sum_{i=k+1}^{b_2}\eta_{\sigma^{1^*}}(e_i).\label{inequality_useful_later}
%\end{align}
\begin{align}
U_2(\sigma^{1^*},\att^{\prime}) & \overset{\eqref{payoff2}}{=} |\att^{\prime}| - \mathbb{E}_{\sigma^{1^*}}[\valdet{\Def}{\att^\prime}]\overset{\eqref{detection_disruptions},\eqref{eta_detection}}{=}  b_2 - \sum_{e \in \att^{\prime}}\eta_{\sigma^{1^*}}(e) =   b_2 - \sum_{i=k+1}^{b_2}\eta_{\sigma^{1^*}}(e_i).\label{inequality_useful_later}
\end{align}

Thus, \defender's equilibrium payoff in the game $\widetilde{\Gamma}$ is $-b_2 + \sum_{i=k+1}^{b_2}\eta_{\sigma^{1^*}}(e_i)$.
Now, to show the contradiction, we construct another strategy $\widehat{\sigma}^1$ that will provide a better payoff than $\sigma^{1^*}$ to \defender.




\begin{itemize}
\item[--] \textbf{Case 1:} $k \geq b_2$. Then \defender's equilibrium payoff in $\widetilde{\Gamma}$ is $-b_2$ (it corresponds to zero detections). However, she has an incentive to switch her strategy, and by randomizing over the nodes that can monitor the $k$ components in $\att^0$, she will increase her payoff; which is a contradiction.
\item[--] \textbf{Case 2:} $k < b_2$. Then \attacker will randomize over attack plans that contain $\att^0$. % (i.e. $\rho_{\sigma^{2^*}}(e_1) = \dots = \rho_{\sigma^{2^*}}(e_k) = 1$).
\begin{itemize}
\item[-] \textbf{Case 2.1:} $k\geq b_1$. Then \defender's equilibrium payoff in $\widetilde{\Gamma}$ is at least equal to $b_1 - b_2$ (since she can monitor $b_1$ components in $\att^0$ that are always targeted). This implies that \attacker's equilibrium payoff  is at most $b_2 - b_1$. However, thanks to Proposition~\ref{best_set_cover}, we know that \attacker's equilibrium payoff is larger than or equal to $b_2 - \frac{b_1b_2}{\semm}> b_2 - b_1$ (since $b_2 < m^*$). Therefore there is a contradiction.

\item[-] \textbf{Case 2.2:} $k < b_1$. Then, the idea is to construct another strategy that position $k$ detectors to monitor the components in $\att^0$ (that were previously unmonitored), and that randomizes the positioning of the remaining $b_1 - k$ detectors over the node basis of $\sigma^{1^*}$.

For now, assume that \defender has $b_1 - k$ detectors. For any detector positioning $\Def \in \supp(\sigma^{1^*})$ (viewed as a set of nodes), we consider $\sold{\Def}{b_1-k}{}$ defined in \eqref{sigma^S} (in this case, we randomize the placement of $b_1 - k$ detectors over the set $\Def$ of size $b_1$). Recall that $\supp(\sold{\Def}{b_1-k}{}) = \{S^1,\dots,S^{\order{b_1}{b_1-k}}\}$, and that $\forall l \in \llbracket 1,\order{b_1}{b_1-k} \rrbracket, \ \sold{\Def}{b_1-k}{\Def^l} = \frac{1}{\order{b_1}{b_1-k}}$.
Now, let us construct the following inspection strategy:
\begin{align}
\sigma^{1^{\prime}} = \sum_{\Def \in \supp(\sigma^{1^*})}\sigma^{1^*}_{\Def}\sold{\Def}{b_1-k}{}.\label{sigma1'}
\end{align}

One can check that $\sigma^\prime \in \Delta(\mathcal{A}_1)$, and is such that 
$\supp(\sigma^{1^{\prime}}) = \cup_{\Def \in \supp(\sigma^{1^*})}\{\Def^1,\dots,\Def^{\order{b_1}{b_1-k}}\}$. 
%Notice that it is indeed a probability distribution:
%\begin{align*}
%\sum_{\Def^{\prime} \in \mathcal{A}_1} \sigma^{1^{\prime}}_{\Def^{\prime}} &\overset{\eqref{sigma1'}}{=} \sum_{\Def^{\prime} \in \mathcal{A}_1} \sum_{\Def \in \supp(\sigma^{1^*})}\sigma^{1^*}_{\Def} \sold{\Def}{b_1-k}{\Def^\prime} =  \sum_{\Def \in \supp(\sigma^{1^*})}\sigma^{1^*}_{\Def}\sum_{\Def^{\prime} \in \mathcal{A}_1} \sold{\Def}{b_1-k}{\Def^\prime} \\
%&= \sum_{\Def \in \supp(\sigma^{1^*})}\sigma^{1^*}_{\Def} = 1,
%\end{align*}
%where we first used the fact that $\forall \Def \in \supp(\sigma^{1^*}), \ \sold{\Def}{b_1-k}{}$ is a probability distribution, and then that $\sigma^{1^*}$ is a probability distribution.
Thus, $\sigma^{1^{\prime}}$ is a probability distribution that randomizes over detector positionings of size $b_1 - k$. Then, $\forall \Def \in \supp(\sigma^{1^{\prime}})$, we augment $\Def$ by placing $k$ additional detectors to monitor the subset of  components  $\att^0$ that was previously unmonitored and that is always targeted in equilibrium by \attacker. We denote $\{i_1,\dots,i_k\}$ the placement of such additional detectors, and we denote $\widehat{\Def} = \Def \cup \{i_1,\dots,i_k\}, \ \forall \Def \in \supp(\sigma^{1^\prime})$ the augmented detector positioning. Then, we consider the probability distribution $\widehat{\sigma}^1$ with support equal to $\cup_{\Def \in \supp(\sigma^{1^*})}\{\widehat{\Def}^1,\dots,\widehat{\Def}^{\order{b_1}{b_1-k}}\}$ and such that:
\begin{align}
\forall \Def \in \supp(\sigma^{1^{\prime}}), \ \sigma^{1^{\prime}}_{\Def} = \widehat{\sigma}^1_{\widehat{\Def}},\label{S=Shat}
\end{align}
i.e., $\widehat{\sigma}^1$ is the same probability distribution as $\sigma^{1^\prime}$ except that it randomizes over the augmented detector positionings present in the support of $\sigma^{1^\prime}$.

%\tb{Now, note the following inequality \tb{(it can go in Lemma~\ref{algebra2} if you prefer)} :
%\begin{align}
%\forall \Def \in \supp(\sigma^{1^*}), \ \valdet{\Def}{e} \leq \frac{1}{q_1}\sum_{l=1}^{p_1}\valdet{\Def^l}{e},\label{nice_detection_inequality}
%\end{align}
%where $q_1$ is the number of sensor placements $\Def^l$ that contain a given node of $\Def$ (see Lemma~\ref{algebra2}). Indeed, if $\valdet{\Def}{e} = 1$, then $\exists \,i_0 \in \Def \ | \ \valdet{i_0}{e} = 1$. Since there are $q_1$ sensor placements in $\{\Def^l\}_{l \in \llbracket 1,p_1\rrbracket}$ that contain $i_0$, then $\frac{1}{q_1}\sum_{l=1}^{p_1}\valdet{\Def^l}{e} \geq 1$. The case when $\valdet{\Def}{e}=0$ is trivial since the sensing function is nonnegative. }

Then, we can derive the following calculations which combine the previous construction of $\widehat{\sigma}^1$ with a property of the detection function derived in \eqref{nice_detection_inequality}, and which will lead to a contradiction:
%\begin{align}
%\forall \att \in \mathcal{A}_2 \ &| \ \{e_1,\dots,e_k\} \subset \att \text{ and } |\att| = b_2, \ -U_2(\widehat{\sigma}^1,\att)  \overset{\eqref{payoff2}}{=} -b_2 + \sum_{\Def \in \mathcal{A}_1} \widehat{\sigma}^1_{\Def} \valdet{\Def}{\att}\nonumber\\
%& \overset{\eqref{detection_disruptions}}{=} -b_2 +\sum_{l=1}^k\underset{=1}{\underbrace{\sum_{\Def \in \mathcal{A}_1} \widehat{\sigma}^1_{\Def} \valdet{\Def}{e_l}}} + \sum_{e \in \att\backslash\{e_1,\dots,e_k\}} \sum_{\Def \in \mathcal{A}_1} \widehat{\sigma}^1_{\Def} \valdet{\Def}{e}\nonumber\\
%& = -b_2 +k + \sum_{e \in \att\backslash\{e_1,\dots,e_k\}} \sum_{\Def \in \supp(\sigma^{1^*})} \sum_{l=1}^{\order{b_1}{b_1-k}}\widehat{\sigma}^1_{\widehat{\Def}^l} \valdet{\widehat{\Def}^l}{e}\nonumber\\
%& \overset{\eqref{S=Shat}}{=} -b_2 +k + \sum_{e \in \att\backslash\{e_1,\dots,e_k\}} \sum_{\Def \in \supp(\sigma^{1^*})} \sum_{l=1}^{\order{b_1}{b_1-k}}\sigma^{1^{\prime}}_{\Def^l} \valdet{\widehat{\Def}^l}{e}\nonumber\\
%& \overset{\eqref{monotonicity_detection}}{\geq} -b_2 +k + \sum_{e \in \att\backslash\{e_1,\dots,e_k\}} \sum_{\Def \in \supp(\sigma^{1^*})} \sum_{l=1}^{\order{b_1}{b_1-k}}\sigma^{1^{\prime}}_{\Def^l} \valdet{\Def^l}{e}\nonumber\\
%&\overset{\eqref{sigma^S},\eqref{sigma1'}}{=} -b_2 +k + \sum_{e \in \att\backslash\{e_1,\dots,e_k\}} \sum_{\Def \in \supp(\sigma^{1^*})} \sum_{l=1}^{\order{b_1}{b_1-k}}\frac{1}{\order{b_1}{b_1-k}}\sigma^{1^{*}}_{\Def} \valdet{\Def^l}{e}\nonumber\\
%&= -b_2 +k + \sum_{e \in \att\backslash\{e_1,\dots,e_k\}} \sum_{\Def \in \supp(\sigma^{1^*})} \frac{1}{\order{b_1}{b_1-k}}\sigma^{1^{*}}_{\Def}\sum_{l=1}^{\order{b_1}{b_1-k}} \valdet{\Def^l}{e}\nonumber\\
%&\overset{\eqref{nice_detection_inequality}}{\geq} -b_2 +k + \sum_{e \in \att\backslash\{e_1,\dots,e_k\}} \sum_{\Def \in \supp(\sigma^{1^*})} \frac{\antiorder{b_1}{b_1-k}}{\order{b_1}{b_1-k}}\sigma^{1^{*}}_{\Def}\valdet{\Def}{e}\nonumber\\
%&\overset{\eqref{arithmetic equality},\eqref{eta_detection}}{=} -b_2 +k + \underset{>0}{\underbrace{\frac{b_1 - k}{b_1}}}\sum_{e \in \att\backslash\{e_1,\dots,e_k\}}\eta_{\sigma^{1^*}}(e)\nonumber\\
%& \geq -b_2 +k + \frac{b_1 - k}{b_1}\sum_{i=k+1}^{b_2}\eta_{\sigma^{1^*}}(e_i)\label{need for explanation}\\
%& = -b_2 +\sum_{i=k+1}^{b_2}\eta_{\sigma^{1^*}}(e_i) + k\left(1 - \frac{1}{b_1}\sum_{i=k+1}^{b_2}\eta_{\sigma^{1^*}}(e_i)  \right).\label{big_calculation!}
%\end{align} 
\begin{align}
&\forall \att \in \mathcal{A}_2 \ | \ \att^0 \subset \att \text{ and } |\att| = b_2, \ \mathbb{E}_{\widehat{\sigma}^1}[\valdet{\Def}{\att}] \overset{\eqref{additive_equality}}{=} \mathbb{E}_{\widehat{\sigma}^1}[\underset{=k}{\underbrace{\valdet{\Def}{\att^0}}}] + \mathbb{E}_{\widehat{\sigma}^1}[\valdet{\Def}{\att\backslash\att^0}] \nonumber\\
%& \overset{\eqref{detection_disruptions}}{=} -b_2 +\sum_{l=1}^k\underset{=1}{\underbrace{\sum_{\Def \in \mathcal{A}_1} \widehat{\sigma}^1_{\Def} \valdet{\Def}{e_l}}} + \sum_{e \in \att\backslash\{e_1,\dots,e_k\}} \sum_{\Def \in \mathcal{A}_1} \widehat{\sigma}^1_{\Def} \valdet{\Def}{e}\nonumber\\
& = k +\sum_{\Def \in \supp(\sigma^{1^*})} \sum_{l=1}^{\order{b_1}{b_1-k}}\widehat{\sigma}^1_{\widehat{\Def}^l} \valdet{\widehat{\Def}^l}{\att\backslash\att^0} \overset{\eqref{monotonicity_detection},\eqref{S=Shat}}{\geq} k +  \sum_{\Def \in \supp(\sigma^{1^*})} \sum_{l=1}^{\order{b_1}{b_1-k}}\sigma^{1^{\prime}}_{\Def^l} \valdet{\Def^l}{\att\backslash\att^0}\nonumber\\
&\overset{\eqref{sigma^S},\eqref{sigma1'}}{=} k +\sum_{\Def \in \supp(\sigma^{1^*})} \sum_{l=1}^{\order{b_1}{b_1-k}}\frac{1}{\order{b_1}{b_1-k}}\sigma^{1^{*}}_{\Def} \valdet{\Def^l}{\att\backslash\att^0} \overset{\eqref{nice_detection_inequality}}{\geq} k + \sum_{\Def \in \supp(\sigma^{1^*})} \frac{\antiorder{b_1}{b_1-k}}{\order{b_1}{b_1-k}}\sigma^{1^{*}}_{\Def}\valdet{\Def}{\att\backslash\att^0} \nonumber\\
&\overset{\eqref{detection_disruptions},\eqref{eta_detection}}{=} k + \underset{>0}{\underbrace{\frac{b_1 - k}{b_1}}}\sum_{e \in \att\backslash\att^0}\eta_{\sigma^{1^*}}(e) \geq  k + \frac{b_1 - k}{b_1}\sum_{i=k+1}^{b_2}\eta_{\sigma^{1^*}}(e_i)\nonumber\\%\label{need for explanation}\\
& = \sum_{i=k+1}^{b_2}\eta_{\sigma^{1^*}}(e_i) + k\left(1 - \frac{1}{b_1}\sum_{i=k+1}^{b_2}\eta_{\sigma^{1^*}}(e_i)  \right).\label{big_calculation!}
\end{align}

%In the third equality, we used the fact that events on each $e_l$ ($l \in \llbracket 1,k\rrbracket$) are always detected by $\widehat{\sigma}_{\Def}^1$ (by construction). 
%In inequality \eqref{need for explanation}, we used the fact that the size of $\att\backslash\att^0$ is $b_2-k$, and no matter what these $b_2-k$ components are, the sum of the $\eta_{\sigma^{1^*}}(e)$ is always larger than or equal to $\sum_{i=k+1}^{b_2} \eta_{\sigma^{1^*}}(e_i)$ (since we sorted the components in nondecreasing order of monitoring).


From Proposition~\ref{best_set_cover}, we know that the equilibrium payoff of \attacker is at least $b_2 - \frac{b_1b_2}{m^*}$. Therefore:
\begin{align*}
U_2(\sigma^{1^*},\sigma^{2^*}) \overset{\eqref{inequality_useful_later}}{=}b_2 - \sum_{i=k+1}^{b_2}\eta_{\sigma^{1^*}}(e_i)  \geq b_2 - \frac{b_1b_2}{m^*} \Longleftrightarrow \frac{1}{b_1}\sum_{i=k+1}^{b_2}\eta_{\sigma^{1^*}}(e_i)  \leq \frac{b_2}{m^*}  < 1,
\end{align*}

since $b_2 < m^*$. Then, by combining the previous inequality with \eqref{big_calculation!}, we obtain:
\begin{align*}
\forall \att \in \mathcal{A}_2 \ | \ \att^0 \subset \att \text{ and } |\att| = b_2, \ -U_2(\widehat{\sigma}^1,\att) \overset{\eqref{payoff2},\eqref{big_calculation!}}{>} -b_2 +\sum_{i=k+1}^{b_2}\eta_{\sigma^{1^*}}(e_i) \overset{\eqref{inequality_useful_later}}{=} - U_2(\sigma^{1^*},\sigma^{2^*}).
\end{align*}

Since each attack plan in the support of an equilibrium strategy uses all the resources (Proposition~\ref{all_resources}), and must contain $\att^0$ (beginning of Case 2), then: $-U_2(\widehat{\sigma}^1,\sigma^{2^*}) = \mathbb{E}_{\sigma^{2^*}}[-U_2(\widehat{\sigma}^1,\att)]> -U_2(\sigma^{1^*},\sigma^{2^*}),$ which violates the equilibrium condition \eqref{best1} in the strategic equivalent game $\widetilde{\Gamma}$.\end{itemize}
\end{itemize}

Therefore, $\forall ({\sigma^1}^*,{\sigma^2}^*) \in \nash, \ \nbasis{\sigma^{1^*}}$ is a set cover.
%\begin{align*}
%\forall ({\sigma^1}^*,{\sigma^2}^*) \in \nash, \ &\forall e \in \edges, \ \exists \, \Def \in \supp({\sigma^1}^*) \ \text{s.t.} \ \valdet{\Def}{e} = 1.%\\
%%\forall ({\sigma^1}^*,{\sigma^2}^*) \in \nash, \ &\forall e \in \edges, \ \exists \, \Def \in \supp({\sigma^1}^*) \ \text{s.t.} \ e \in \set{\Def}.
%\end{align*}

%\hfill \Halmos
%\endproof
%
%\proof{Proof of Proposition~\ref{all_edges}.}
\item From Proposition~\ref{all_edges} and the fact that $b_1<n^*$, \defender must randomize her detector positionings in equilibrium so the node basis is a set cover.
Now, assume that there exists a NE $(\sigma^{1^*},\att) \in \nash$ such that \attacker chooses a pure strategy $\att$ (of size $b_2$ from Proposition~\ref{all_resources}). %There are two cases to consider.
\begin{enumitemize}
\item[--] If $b_1 \geq b_2$, then \defender can detect all the attacks in $\att$ by placing $b_2$ detectors at the nodes that can monitor the  components of $\att$, and \attacker's equilibrium payoff would be 0. Again, since \attacker's payoff is identical for any NE, then $U_2(\sigma^{1^*},\att) = 0$. However, we showed in the proof of Proposition~\ref{all_resources} that there exists a component outside of $\att$ that is not monitored with positive probability by $\sigma^{1^*}$. Therefore, \attacker can increase her payoff by targeting that component, thus leading to a contradiction.

\item[--] If $b_1 < b_2$, then \defender can detect at least $b_1$ attacks in $\att$ by placing  detectors on $b_1$ nodes that can collectively monitor $b_1$ components of $\att$. The resulting payoff for \defender in the game $\widetilde{\Gamma}$ is at least $b_1 - b_2$. However, from Proposition~\ref{best_set_cover}, we know that \attacker's equilibrium payoff is at least $\max\{0,b_2(1 - \frac{b_1}{\semm})\} \geq b_2(1 - \frac{b_1}{\semm}) > b_2 - b_1$ (since $b_2 < \semm$). Therefore, \defender's equilibrium payoff in $\widetilde{\Gamma}$ is strictly upper bounded by $b_1 - b_2$, thus leading to a contradiction.
\end{enumitemize}

Therefore, in equilibrium, both players must randomize their actions.\hfill \Halmos
\end{enumerate}
%\vspace{-0.5cm}
%
\endproof

\proof{Proof of Theorem~\ref{bounds_game}.}\
\begin{enumerate}
\item Since \attacker's expected payoff in the game $\Gamma$ is also her expected payoff in $\widetilde{\Gamma}$, we know that \attacker's equilibrium payoff is constant. From Proposition~\ref{best_set_cover}, we can directly obtain:
\begin{align}
\forall (\sigma^{1^*},\sigma^{2^*}) \in \nash, \ \max\left\{0,b_2\left(1 -  \frac{b_1}{\semm}\right) \right\} \leq U_2(\sigma^{1^*},\sigma^{2^*}) \leq b_2\left(1 - \frac{b_1}{\smsc}\right). \label{bounds Lipton}
\end{align}

By combining  \eqref{transform1} and Proposition~\ref{all_resources}, we deduce that \defender's payoff in equilibrium of $\Gamma$ is also constant, and can be bounded as follows:
\begin{align}
\forall (\sigma^{1^*},\sigma^{2^*}) \in \Sigma, \ & \frac{b_1b_2}{\smsc} \leq U_1(\sigma^{1^*},\sigma^{2^*}) \leq \min\left\{\frac{b_1b_2}{\semm},b_2\right\}.\label{bounds Lipton2}
%&  \max\left\{0,b_2 \left(1 - \frac{b_1}{\semm} \right) \right\}\leq U_2(\sigma^{1^*},\sigma^{2^*}) \leq  b_2 \left(1 - \frac{b_1}{n^{*}} \right)
\end{align}


\item
Again, thanks to Proposition~\ref{all_resources}, we have $\forall \sigma^* \in \nash, \ r(\sigma^*) \overset{\eqref{Exp_detection_rate}}{=} \mathbb{E}_{\sigma^*}\left[\frac{\valdet{\Def}{\att}}{|\att|}\right] = \frac{1}{b_2}\mathbb{E}_{\sigma^*}[\valdet{\Def}{\att}] \overset{\eqref{payoff1}}{=} \frac{1}{b_2}U_1(\sigma^{1^*},\sigma^{2^*})$. Therefore, from \eqref{bounds Lipton2}, we obtain that the expected detection rate in equilibrium is constant and bounded as follows: $\forall \sigma^* \in \nash, \ \frac{b_1}{\smsc} \leq r(\sigma^*) \leq  \min\left\{\frac{b_1}{\semm},1\right\}.$\hfill \Halmos
%\begin{align}
%\forall \sigma^* \in \nash, \ r(\sigma^*) \overset{\eqref{Exp_detection_rate}}{=} \mathbb{E}_{\sigma^*}\left[\frac{\valdet{\Def}{\att}}{|\att|}\right] = \frac{1}{b_2}\mathbb{E}_{\sigma^*}[\valdet{\Def}{\att}] \overset{\eqref{payoff1}}{=} \frac{1}{b_2}U_1(\sigma^{1^*},\sigma^{2^*}). \label{easyy}
%\end{align}
%Therefore, from \eqref{bounds Lipton2} and \eqref{easyy}, we obtain that the expected detection rate in equilibrium is constant and bounded as follows: $\forall \sigma^* \in \nash, \ \frac{b_1}{\smsc} \leq r(\sigma^*) \leq  \min\left\{\frac{b_1}{\semm},1\right\}.$\hfill \Halmos
%\begin{align*}
%\forall \sigma^* \in \nash, \ \frac{b_1}{\smsc} \leq r(\sigma^*) \leq  \min\left\{\frac{b_1}{\semm},1\right\}.
%\end{align*}
\end{enumerate}
%\vspace{-0.9cm}

\endproof

\proof{Proof of Theorem~\ref{MSC-MSP-eNE}} \ 
\begin{enumerate}
\item[(i.a)] Let $\Def^{min} \in \msc$ be an MSC and $\att^{max} \in \emm$ be an MSP. Then, let us show that $(\sold{\Def^{min}}{b_1}{},\sola{\att^{max}}{b_2}{})$ is an $\epsilon-$NE where $\epsilon =  b_1 b_2\left( \frac{1}{\max\{b_1,\semm\}} - \frac{1}{\smsc}\right)$. First, note that $- \epsilon = \max\left\{0,b_2\left(1 -\frac{b_1}{\semm}  \right)\right\}+ b_2\left(\frac{b_1}{\smsc} - 1 \right).$ Then, we have:
%\begin{align}
%- \epsilon = \max\left\{0,b_2\left(1 -\frac{b_1}{\semm}  \right)\right\}+ b_2\left(\frac{b_1}{\smsc} - 1 \right). \label{epsilon difference}
%\end{align}
%
%
\begin{align}
\forall \sigma^1 \in \Delta(\mathcal{A}_1), & \ -U_2(\sold{\Def^{min}}{b_1}{},\sola{\att^{max}}{b_2}{}) \geq \min_{\sigma^2 \in \Delta(\mathcal{A}_2)} -U_2(\sold{\Def^{min}}{b_1}{},\sigma^{2})  \nonumber\\
&\overset{\text{Prop.}~\ref{best_set_cover}}{=} b_2\left(\frac{b_1}{\smsc} - 1 \right) =  -\max\left\{0,b_2\left(1 -\frac{b_1}{\semm}  \right)\right\} - \epsilon \nonumber\\
& \overset{\text{Prop.}~\ref{best_set_cover}}{=} -\min_{\sigma^{1^{\prime}} \in \Delta(\mathcal{A}_1)}U_2(\sigma^{1^{\prime}},\sola{\att^{max}}{b_2}{}) - \epsilon \geq  -U_2(\sigma^{1},\sola{\att^{max}}{b_2}{}) - \epsilon.\label{epsilon_u1_tilde}
\end{align}

Therefore, $\forall \sigma^1 \in \Delta(\mathcal{A}_1)$, $U_1(\sold{\Def^{min}}{b_1}{},\sola{\att^{max}}{b_2}{})  - U_1(\sigma^1,\sola{\att^{max}}{b_2}{}) \overset{\eqref{epsilon_u1_tilde},\eqref{transform1}}{\geq} - \epsilon$.
%\begin{align}
%&U_1(\sold{\Def^{min}}{b_1}{},\sola{\att^{max}}{b_2}{})  - U_1(\sigma^1,\sola{\att^{max}}{b_2}{})  \overset{\eqref{transform1}}{=} -U_2(\sold{\Def^{min}}{b_1}{},\sola{\att^{max}}{b_2}{}) + \mathbb{E}_{\sola{\att^{max}}{b_2}{}}[|\att|]  \nonumber\\
%& \overset{\eqref{epsilon_u1_tilde}}{\geq}  -U_2(\sigma^{1},\sola{\att^{max}}{b_2}{})  - \epsilon + \mathbb{E}_{\sola{\att^{max}}{b_2}{}}[|\att|] \overset{\eqref{transform1}}{=}  - \epsilon. \label{epsilon_u1_}%\\
%%& \geq  U_1(\sigma^1,\sigma^{2^*})  - \max\{,\}\epsilon
%\end{align}

%\begin{align*}
%\forall \sigma^1 \in \Delta(\mathcal{A}_1), \ \widetilde{U}_1(\hat{\sigma}^1,\sigma^{2^*}) \geq \min_{\sigma^2 \in \Delta(\mathcal{A}_2)} \widetilde{U}_1(\hat{\sigma}^1,\sigma^{2}) = \opt{n} = \opt{\smsc} - \epsilon = \widetilde{U}_1(\sigma^{1^*},\sigma^{2^*}) - \epsilon \geq  \widetilde{U}_1(\sigma^{1},\sigma^{2^*}) - \epsilon 
%\end{align*}

Analogous calculations show that ${U}_2(\sold{\Def^{min}}{b_1}{},\sola{\att^{max}}{b_2}{}) \geq U_2(\sold{\Def^{min}}{b_1}{},\sigma^{2}) - \epsilon, \ \forall \sigma^2 \in \Delta(\mathcal{A}_2).$
%Similarly, we have:
%\begin{align}
%\forall \sigma^2 \in \Delta(\mathcal{A}_2), & \ {U}_2(\sold{\Def^{min}}{b_1}{},\sola{\att^{max}}{b_2}{}) \geq \min_{\sigma^1 \in \Delta(\mathcal{A}_1)} U_2(\sigma^{1},\sola{\att^{max}}{b_2}{}) \nonumber \\
%& \overset{\text{Prop.}~\ref{best_set_cover}}{=} \max\left\{0,\left(1 - \frac{b_1}{\semm} \right)b_2\right\}  = - b_2\left(\frac{b_1}{\smsc} - 1 \right) - \epsilon  \label{Lipton lower bound}\\
%& \overset{\text{Prop.}~\ref{best_set_cover}}{=}  -\min_{\sigma^{2^{\prime}} \in \Delta(\mathcal{A}_2)}-U_2(\sold{\Def^{min}}{b_1}{},\sigma^{2^{\prime}}) - \epsilon \geq  U_2(\sold{\Def^{min}}{b_1}{},\sigma^{2}) - \epsilon.\nonumber
%\end{align}
%\begin{align*}
%\forall \sigma^2 \in \Delta(\mathcal{A}_2), \ \widetilde{U}_2(\hat{\sigma}^1,\sigma^{2^*}) &= -\widetilde{U}_1(\hat{\sigma}^1,\sigma^{2^*})  \geq - \widetilde{U}_1(\sigma^{1^*},\sigma^{2^*})  = - \opt{\smsc} = - \opt{n} - \epsilon \\
%&=- \min_{{\sigma^2}^{\prime} \in \Delta(\mathcal{A}_2)} \widetilde{U}_1(\hat{\sigma}^1,{\sigma^2}^{\prime}) - \epsilon \geq - \widetilde{U}_1(\hat{\sigma}^1,\sigma^2) - \epsilon \\
%&= \widetilde{U}_2(\hat{\sigma}^1,\sigma^2) - \epsilon
%\end{align*}
%Therefore, $(\sold{\Def^{min}}{b_1}{},\sola{\att^{max}}{b_2}{})$ is an $\epsilon-$NE of the game $\widetilde{\Gamma}$.
%Now, let us show that $(\sold{\Def^{min}}{b_1}{},\sola{\att^{max}}{b_2}{}) \in \nash_{\epsilon}$.
%Since $U_2 = \widetilde{U}_2$, then:
%\begin{align*}
%\forall \sigma^2 \in \Delta(\mathcal{A}_2), \ U_2(\sigma^{\Def^{\text{min}}},\sigma^{\att^{\text{max}}}) =\widetilde{U}_2(\sigma^{\Def^{\text{min}}},\sigma^{\att^{\text{max}}})   \overset{\eqref{epsilon_u2_tilde}}{\geq}\widetilde{U}_2(\sigma^{\Def^{\text{min}}}, \sigma^{2})   - \epsilon =  U_2(\sigma^{\Def^{\text{min}}}, \sigma^{2})   - \epsilon 
%\end{align*}
Therefore, we conclude that $(\sold{\Def^{min}}{b_1}{},\sola{\att^{max}}{b_2}{}) \in \nash_{\epsilon}(b_1,b_2)$.

\item[(i.b)]
Again, from Proposition~\ref{best_set_cover}, we deduce that: 
\begin{align*}
\max\left\{0,\left(1 - \frac{b_1}{\semm} \right)b_2\right\} \leq U_2(\sold{\Def^{min}}{b_1}{},\sola{\att^{max}}{b_2}{}) \leq b_2\left(1 - \frac{b_1}{\smsc}\right).
\end{align*}

By combining it with \eqref{bounds Lipton}, we obtain for any NE $(\sigma^{1^*},\sigma^{2^*}) \in \nash$:
\begin{align}
|U_2(\sold{\Def^{min}}{b_1}{},\sola{\att^{max}}{b_2}{}) - U_2(\sigma^{1^*},\sigma^{2^*})| &\leq b_2\left(1 - \frac{b_1}{\smsc}\right) - \max\left\{0,\left(1 - \frac{b_1}{\semm} \right)b_2\right\} = \epsilon.\nonumber
\end{align}

Furthermore, from \eqref{transform1}, \eqref{res2}, and \eqref{att^k}, we also deduce that for any NE $(\sigma^{1^*},\sigma^{2^*}) \in \nash$:
\begin{align*}
|U_1(\sold{\Def^{min}}{b_1}{},\sola{\att^{max}}{b_2}{}) - U_1(\sigma^{1^*},\sigma^{2^*})| &= |U_2(\sold{\Def^{min}}{b_1}{},\sola{\att^{max}}{b_2}{}) - U_2(\sigma^{1^*},\sigma^{2^*})|  \leq \epsilon.
\end{align*}


\item[(ii)] %Let us now show the detection guarantee of our MSC-based inspection strategy. 
Consider an MSC $\Def^{min} \in \msc$. Then we have:
\begin{align}
\forall \att \in \mathcal{A}_2, \ \frac{U_1(\sold{\Def^{min}}{b_1}{},\att)}{|\att|}&\overset{\eqref{transform1}}{=}\frac{-U_2(\sold{\Def^{min}}{b_1}{},\att)}{|\att|} + \frac{|\att|}{|\att|} \overset{\eqref{for later}}{\geq} \frac{b_1}{\smsc}.\label{allmost}
\end{align}

Thus, by linearity of the expectation, we obtain:
\begin{align*}
\forall \sigma^2 \in \Delta(\mathcal{A}_2), \ r{(\sold{\Def^{min}}{b_1}{},\sigma^2)} &\overset{\eqref{Exp_detection_rate},\eqref{payoff1}}{=} \mathbb{E}_{\sigma^2}\left[ \frac{U_1(\sold{\Def^{min}}{b_1}{},\att)}{|\att|}\right]  \overset{\eqref{allmost}}{\geq} \frac{b_1}{\smsc}.
\end{align*}
%(when $|\att| = 0$, we can let the detection rate be equal to 1 since there is no attack). 
Therefore, $\min_{\sigma^2 \in \Delta(\mathcal{A}_2)} r{(\sold{\Def^{min}}{b_1}{},\sigma^2)} \geq \frac{b_1}{\smsc}$. Now, consider $i^\prime \in \Def^{min}$. Recall from \eqref{minimal_set_cover} that $\exists \, e^\prime \in \edges \ | \ \valdet{i^\prime}{e^\prime} = 1 \ \text{and} \ \valdet{i}{e^\prime} = 0, \ \forall i \in \Def^{min} \backslash\{i^\prime\}$. Then, it is easy to see that $r(\sold{\Def^{min}}{b_1}{},e^\prime)\overset{\eqref{Exp_detection_rate},\eqref{rho_sigma1}}{=}   \rho_{\sold{\Def^{min}}{b_1}{}}(i^\prime) \overset{\eqref{set_sensing_prob_comp}}{=} \frac{b_1}{\smsc}.$ Therefore, $\min_{\sigma^2 \in \Delta(\mathcal{A}_2)}r(\sold{\Def^{min}}{b_1}{},\sigma^2) = \frac{b_1}{\smsc}$.
%
%
%\begin{align*}
%r(\sold{\Def^{min}}{b_1}{},e^\prime) &\overset{\eqref{Exp_detection_rate}}{=} \mathbb{E}_{\sold{\Def^{min}}{b_1}{}}[\valdet{\Def}{e^\prime}] = \sum_{\Def \in \mathcal{A}_1} \sold{\Def^{min}}{b_1}{\Def} \valdet{\Def}{e^\prime} \\
%&= \sum_{\{\Def \in \mathcal{A}_1 \, | \, i^\prime \in \Def\}} \sold{\Def^{min}}{b_1}{\Def} \underset{=1}{\underbrace{\valdet{\Def}{e^\prime}}} + \sum_{\{\Def \in \mathcal{A}_1 \, | \, i^\prime \notin \Def\}} \underset{=0}{\underbrace{\sold{\Def^{min}}{b_1}{\Def} \valdet{\Def}{e^\prime}}}\\
%& = \sum_{\{\Def \in \mathcal{A}_1 \, | \, i^\prime \in \Def\}} \sold{\Def^{min}}{b_1}{\Def}  \overset{\eqref{rho_sigma1}}{=} \rho_{\sold{\Def^{min}}{b_1}{}}(i^\prime) \overset{\eqref{set_sensing_prob_comp}}{=} \frac{b_1}{\smsc}.
%%& \overset{\eqref{sigma^S}}{=} \frac{1}{\order{\smsc}{b_1}}\sum_{k=1}^{\order{\smsc}{b_1}} \mathds{1}_{\{i^\prime \in \Def^k\}}\\
%%& = \frac{1}{\order{\smsc}{b_1}}|\{k \in \llbracket 1,\order{\smsc}{b_1}\rrbracket \ | \ i^\prime \in \Def^k\}|\\
%%& \overset{\eqref{q1}}{=} \frac{\antiorder{\smsc}{b_1}}{\order{\smsc}{b_1}}\\
%%& \overset{\eqref{arithmetic equality}}{=} \frac{b_1}{\smsc}.
%\end{align*}

Finally, from Theorem~\ref{bounds_game}, we have $\forall (\sigma^{1^*},\sigma^{2^*}) \in \nash, \ r(\sigma^{1^*},\sigma^{2^*}) \leq \frac{b_1}{\max\{b_1,\semm\}}$, and we can deduce that: $\frac{\max\{b_1,\semm\}}{\smsc} r(\sigma^{1^*},\sigma^{2^*}) \leq \frac{b_1}{\smsc} = \min_{\sigma^2 \in \Delta(\mathcal{A}_2)} r{(\sold{\Def^{min}}{b_1}{},\sigma^2)}.$ \hfill
\Halmos
%\vspace{-0.5cm}
%\begin{align*}
%\frac{\max\{b_1,\semm\}}{\smsc} r(\sigma^{1^*},\sigma^{2^*}) \leq \frac{b_1}{\smsc} = \min_{\sigma^2 \in \Delta(\mathcal{A}_2)} r{(\sold{\Def^{min}}{b_1}{},\sigma^2)}.
%\end{align*}

\end{enumerate}

%\end{enumerate}
%\vspace{-0.5cm}

\endproof

%\section{Proofs of Section \ref{sec:strong_duality}}

%\tb{In this section, we consider the case when $b_1 < \smsc$, $b_2 < \semm$, and $\smsc = \semm$.}

\ifadditional
\begin{corollary}[of Theorem~\ref{bounds_game}]\label{Cor1}
Consider a network $\mathcal{G}$, a sensing model $\{\set{i}, \ i \in \nodes\}$, and  the players' resources $b_1 < \smsc$ and $b_2 < \semm$. If $\smsc = \semm$, then the game $\Gamma(b_1,b_2)$ has the following properties:
\begin{enumerate}
\item
The equilibrium payoffs of both players are constant and are given by:
\begin{align}
\forall (\sigma^{1^*},\sigma^{2^*}) \in \nash(b_1,b_2), \quad \begin{cases} U_1 ({\sigma^1}^*,{\sigma^2}^*) = \dfrac{  b_1  b_2}{\smsc},  \\
U_2 ({\sigma^1}^*,{\sigma^2}^*) =   b_2  \left(1 - \dfrac{  b_1  }{\smsc}\right).\end{cases}\label{eq_payoff_EC}
\end{align}
%\item
%\begin{align*}
%\Expone[*]{\valdet{\Def}{\att}} = \frac{b_1b_2}{\smsc}
%\end{align*}
\item In any equilibrium, the expected detection rate is constant and is given by:
\begin{align}
\forall \sigma^* \in \nash(b_1,b_2), \quad \sdet{*} = \dfrac{b_1}{\smsc}.\label{eq_srate_EC}
\end{align}
%\item All actions in the support of $\sigma^*$ use all the resources:
%\begin{align*}
%\forall \Def \in \supp(\sigma^{1^*}), \ |\Def| = b_1,\\
%\forall \att \in \supp(\sigma^{2^*}), \ |\att| = b_2.
%\end{align*}
\end{enumerate}
\end{corollary}

\proof{Proof of Corollary~\ref{Cor1}.}
By rewriting Thm.~\ref{bounds_game} when $\smsc = \semm$, we obtain $\forall (\sigma^{1^*},\sigma^{2^*}) \in \nash(b_1,b_2):$
\begin{align*}
& \frac{b_1b_2}{\smsc }\leq  U_1(\sigma^{1^*},\sigma^{2^*})  \leq \min\left\{\frac{b_1b_2}{\semm },b_2\right\} = \min\left\{\frac{b_1b_2}{\smsc },b_2\right\} =\frac{b_1b_2}{\smsc },\\
& b_2\left(1 - \frac{b_1}{\smsc }\right) = \max\left\{0,b_2\left(1 - \frac{b_1}{\smsc }\right)\right\} = \max\left\{0,b_2\left(1 - \frac{b_1}{\semm }\right)\right\}\leq  U_2(\sigma^{1^*},\sigma^{2^*})  \leq b_2\left(1 - \frac{b_1}{\smsc }\right),
\end{align*}
since $b_1 <\smsc$.

Similarly, for the expected detection rate in equilibrium, we obtain:
\begin{align*}
\forall \sigma^* \in \nash(b_1,b_2), \ \frac{b_1}{\smsc} \leq r(\sigma^*) \leq \min\left\{\frac{b_1}{\semm},1\right\}= \min\left\{\frac{b_1}{\smsc},1\right\} = \frac{b_1}{\smsc}.
\end{align*}
\hfill \Halmos
\endproof
\else
\fi



\ifadditional
\begin{lemma}\label{permutation}
For any MSC $\Def^{\text{min}} \in \mathcal{S}$ and any MSP $\att^{\text{max}} \in \mathcal{M}$ such that $\smsc = \semm$, each component in $\att^{\text{max}}$ is monitored by only one node in $\Def^{\text{min}}$, and each node in $\Def^{\text{min}}$ monitors only one component in $\att^{\text{max}}$.
%
%In other words, $\forall \{i_1,\dots,i_{\smsc}\} \in \msc, \ \forall \{e_1,\dots,e_{\smsc}\} \in \emm$,
%there exists a permutation $\psi$ of $\llbracket1,\smsc\rrbracket$ such that:
%\begin{align*}
%\forall (k,l) \in \llbracket 1,\smsc \rrbracket^2, \ \valdet{i_k}{e_l} = \delta_{\psi(k),l}. 
%\end{align*}
\end{lemma}
\proof{Proof of Lemma~\ref{permutation}.}
Consider an MSC $\Def^{min} \in \msc$ and an MSP $\att^{max} \in \emm$. Since $\att^{max}$ is an MSP, each node in $\Def^{min}$ monitors at most one component in $\att^{max}$. Now, assume that at least one node in $\Def^{min}$ does not monitor any component in $\att^{max}$. Since $\Def^{min}$ is an MSC, then the $\smsc$ components in $\att^{max}$ are monitored by at most $\smsc-1$ nodes. From Dirichlet's principle, there exists a node in $\Def^{min}$ that monitors at least two components in $\att^{max}$, which is a contradiction. Therefore, each node in $\Def^{min}$ monitors exactly one component in $\att^{max}$. 

Thus, we can define a mapping $\psi: \Def^{min} \longrightarrow \att^{max}$ such that $\forall i \in \Def^{min}, \ \psi(i)$ is the component in $\att^{max}$ that is monitored by node $i$. Now, since $\Def^{min}$ is an MSC, for every component $e \in \att^{max}, \ \exists \, i \in \Def^{min}$ such that $e$ is monitored by $i$. Therefore, $\psi$ is surjective which is equivalent to $\psi$ being injective since its domain and codomain have the same number of elements.
%Thus, we can define a mapping $\psi: \llbracket 1,\smsc \rrbracket \longrightarrow \llbracket 1,\smsc \rrbracket$ such that $\forall k \in \llbracket 1,\smsc \rrbracket, \ e_{\psi(k)}$ is the component of the MSP that is monitored by node $i_k$ of the MSC. Now, since $\{i_1,\dots,i_{\smsc}\}$ is an MSC, for every $l \in \llbracket 1,\smsc \rrbracket, \ \exists \, k \in \llbracket 1,\smsc \rrbracket \ | \ e_l$ is detected by $i_k$. Therefore, $\psi$ is surjective which is equivalent to $\psi$ being injective since its domain and codomain have the same number of elements.
%Therefore, each node of the MSC is uniquely mapped to the edge of the MSP it monitors.
%Now, suppose that there is an edge of the MM that is detected by at least two nodes of the MSC. Then the remaining $\smsc-1$ edges are detected by less than or equal to $\smsc -2$ nodes of the MSC.
%Since $\{i_1,\dots,i_{\smsc}\}$ is a MSC, then each component of the MM is detected by at least one node of the MSC. However, since $\{e_1,\dots,e_{\smsc}\}$ is a MM, then each component of the MM is detected by at most one node of the MSC. 
Therefore, each component in $\att^{max}$ is monitored by only one node in $\Def^{min}$.
\hfill
\Halmos
\endproof

This lemma tells us that no matter which MSC and which MSP we consider, there is a one-to-one correspondence between a node in the MSC and the component in the MSP in monitors.



In fact, we can obtain a sufficient \emph{and} necessary condition for a strategy profile constructed over an MSC and MSP to be a NE when $\smsc = \semm$.



%\subsection{Additional Nash Equilibrium Characterization

%\begin{proposition}\label{MSC/EMM-NE}
%Under \aref{b1<MSC} and \aref{MM=MSC}, for any MSC $\{i_1,\dots,i_{\smsc}\} \in \msc$ and any EMM $\{e_1,\dots,e_{\smsc}\} \in \emm$, a strategy profile  whose node basis is $\{i_1,\dots,i_{\smsc}\}$, whose component basis is $\{e_1,\dots,e_{\smsc}\}$ is a NE if and only if:
%\begin{align*}
%\forall k \in \llbracket 1,\smsc \rrbracket, \rho_{\sigma^{1^*}}(i_k) = \frac{b_1}{\smsc} \ \text{and} \ \rho_{\sigma^{2^*}}(e_k) = \frac{b_2}{\smsc}.
%\end{align*}
%
%If $\smsc = \semm$, $b_1 <\smsc$, and $b_2 < \semm$, then for any MSC $\Def^{min} \in \msc$ and any MSP $\att^{max} \in \emm$, a strategy profile $(\sigma^{1^*},\sigma^{2^*}) \in \Delta(\mathcal{A}_1) \times \Delta(\mathcal{A}_2) $ whose node basis is $\Def^{min}$ and whose component basis is $\att^{max}$ is a NE if and only if:
%\begin{align}
%\forall i \in \Def^{min}, \quad  \rho_{\sigma^{1^*}}(i) = \frac{b_1}{\smsc}, \quad \text{and} \quad \forall e \in \att^{max},\quad \rho_{\sigma^{2^*}}(e) = \frac{b_2}{\smsc}. \label{if and only if}
%\end{align}
%\end{proposition}

\begin{proposition}\label{MSC/EMM-NE}
%Under \aref{b1<MSC} and \aref{MM=MSC}, for any MSC $\{i_1,\dots,i_{\smsc}\} \in \msc$ and any EMM $\{e_1,\dots,e_{\smsc}\} \in \emm$, a strategy profile  whose node basis is $\{i_1,\dots,i_{\smsc}\}$, whose edge basis is $\{e_1,\dots,e_{\smsc}\}$ is a NE if and only if:
%\begin{align*}
%\forall k \in \llbracket 1,\smsc \rrbracket, \rho_{\sigma^{1^*}}(i_k) = \frac{b_1}{\smsc} \ \text{and} \ \rho_{\sigma^{2^*}}(e_k) = \frac{b_2}{\smsc}.
%\end{align*}
%
If $\smsc = \semm$, $b_1 <\smsc$, and $b_2 < \semm$, then for any MSC $\Def^{min} \in \msc$ and any MSP $\att^{max} \in \emm$, a strategy profile $(\sigma^{1^*},\sigma^{2^*}) \in \Delta(\mathcal{A}_1) \times \Delta(\mathcal{A}_2) $ whose node basis is $\Def^{min}$ and whose component basis is $\att^{max}$ is a NE if and only if:
\begin{align}
\forall i \in \Def^{min}, \quad  \mathbb{P}_{\sigma^{1^*}}(i \text{ is monitored}) = \frac{b_1}{\smsc}, \quad \text{and} \quad \forall e \in \att^{max},\quad \mathbb{P}_{\sigma^{2^*}}(e \text{ is targeted}) = \frac{b_2}{\smsc}. \label{if and only if}
\end{align}
\end{proposition}

\proof{Proof of Proposition~\ref{MSC/EMM-NE}.}
For simplicity, given an optimization problem $(\mathcal{Q})$, we denote $\OPT{(\mathcal{Q})}$ its objective value. Let $\Def^{min} \in \msc$ be an MSC and  $\att^{max} \in \emm$ be an MSP, and assume that they are of same size. Recall that from Proposition~\ref{best_set_cover}, we have  $\OPT{\rlpom{\Def^{min}}} \leq  \OPT{\lpom} =- \OPT{\lptm }\leq - \OPT{\rlptm{\att^{max}}}$. Since $\smsc = \semm$ (and $b_1 < \smsc$), then we also have:
\begin{align*}
\OPT{\rlpom{\Def^{min}}} = b_2 \left(\frac{b_1}{\smsc} - 1 \right)  = - b_2 \left(1 - \frac{b_1}{\semm}  \right)  = - \max\left\{0,b_2 \left(1 - \frac{b_1}{\semm}  \right) \right\} =  - \OPT{\rlptm{\att^{max}}}.
\end{align*}

Therefore, $\OPT{\rlpom{\Def^{min}}} = \OPT{\lpom}$ and  $\OPT{\rlptm{\att^{max}}} = \OPT{\lptm }$. Since \rlpo{\Def^{min}} (resp. \rlpt{\att^{max}}) is a restriction of \lpo (resp. \lpt), then any sensing strategy $\sigma^{1^*}$ (resp. attack strategy $\sigma^{2^*}$) that is optimal for  \rlpo{\Def^{min}} (resp. \rlpt{\att^{max}}) is optimal for \lpo (resp. \lpt). Thus, any strategy profile $(\sigma^{1^*},\sigma^{2^*})$ such that $\sigma^{1^*}$ and $\sigma^{2^*}$ are optimal solutions of \rlpo{\Def^{min}}  and \rlpt{\att^{max}} respectively is a NE. 

To show that a sensing strategy $\sigma^{1^*}$ (whose node basis is $\Def^{min}$) is an optimal solution of \rlpo{\Def^{min}}, it is sufficient to show that $\min_{\sigma^2 \in \Delta(\mathcal{A}_2)}-U_2(\sigma^{1^*},\sigma^2) \geq b_2\left(\frac{b_1}{\smsc} - 1\right) = \OPT{\rlpom{\Def^{min}}}$. By applying \eqref{1st_ineq_max-min} for $\Def^{min}$ (which is a minimal set cover), we know that $\min_{\sigma^2 \in \Delta(\mathcal{A}_2)}-U_2(\sold{\Def^{min}}{b_1}{},\sigma^2) \geq b_2\left(\frac{b_1}{\smsc} - 1\right)$. However, recall that to show this inequality, the only property from $\sold{\Def^{min}}{b_1}{}$ that we used was that its node basis is $\Def^{min}$ and that $\forall i \in \Def^{min}$, $\rho_{\sold{\Def^{min}}{b_1}{}}(i) = \frac{b_1}{\smsc}$. Therefore, any sensing strategy that satisfies the same conditions also satisfies the same inequality and is an optimal solution of \rlpo{\Def^{min}}.

Similarly, we can easily deduce from \eqref{1st_inteq_max-min_bis} that any attack strategy $\sigma^{2^*}$ whose component basis is $\att^{max}$ and which satisfies $\forall e \in \att^{max}, \ \rho_{\sigma^{2^*}}(e) = \frac{b_2}{\smsc}$ also satisfies the inequality $\min_{\sigma^1 \in \Delta(\mathcal{A}_1)} U_2(\sigma^1,\sigma^{2^*}) \geq b_2\left(1 - \frac{b_1}{\smsc} \right)$ and is an optimal solution of \rlpt{\att^{max}}.

%Recall that in the proof of Prop.~\ref{best_set_cover}, when we showed (in \eqref{1st_ineq_max-min}) that for any minimal set cover $\Def^{\prime}$, $\min_{\sigma^2 \in \Delta(\mathcal{A}_2)}-U_2(\sold{\Def^\prime}{b_1}{},\sigma^2) \geq b_2\left(\frac{b_1}{|\Def^\prime|} - 1\right)$, the only property from $\sold{\Def^\prime}{b_1}{}$ that we used was that its node basis is $\Def^\prime$ and that $\forall i \in \Def^\prime$, $\rho_{\sold{\Def^\prime}{b_1}{}}(i) = \frac{b_1}{|\Def^\prime|}$. Therefore, any sensing strategy that satisfies the same conditions also satisfies the same inequality. By applying this argument for $\Def^{min}$, we deduce that any sensing strategy that sati
%
%Recall from the proof of Prop.~\ref{best_set_cover} that to show \eqref{1st_ineq_max-min}, the only property from 



%If we look closely at the proofs of Props.~\ref{best_set_cover}-\ref{best_set_cover}, when we proved that $\sold{\Def^{min}}{b_1}{}$ (resp. $\sola{\att^{max}}{b_2}{}$) is an optimal solution of \rlpo{\Def^{min}} (resp. \rlpt{\att^{max}}), we can see that the only information we used regarding $\sold{\Def^{min}}{b_1}{}$ (resp $\sola{\att^{max}}{b_2}{}$) is the sensing probability of the nodes in its node basis (resp. the attack probability of the components in its component basis). Therefore, any strategy profile that satisfies the same conditions on the sensing and disruption probabilities will also be an optimal solution of \lpo and \lpt. 

Thus, any strategy profile $(\sigma^{1^*},\sigma^{2^*})$ whose node basis is $\Def^{min}$, whose component basis is $\att^{max}$, and that satisfies $\rho_{\sigma^{1^*}}(i) = \frac{b_1}{\smsc}, \forall i \in \Def^{min}, \ \text{and} \ \rho_{\sigma^{2^*}}(e) = \frac{b_2}{\smsc}, \ \forall e \in \att^{max},$ is a NE (it is a sufficient condition).

Now, let us show (by contradiction) that this is also a necessary condition.
\begin{enumerate}
\item Consider a NE $(\sigma^{1^*},\sigma^{2^*}) \in \nash$ whose node basis is an MSC $\Def^{min} = \{i_1,\dots,i_{\smsc}\} \in \msc$, and assume that the sensing probability is not identical among the nodes in $\Def^{min}$. Without loss of generality (by reordering the indices), assume that $\rho_{\sigma^{1^*}}(i_1) < \rho_{\sigma^{1^*}}(i_{b_2+1})$. 



Consider an MSP $\att^{max} = \{e_1,\dots,e_{\smsc}\} \in \emm$. Thanks to Lemma~\ref{permutation}, and without loss of generality, we can rearrange the indices such that $\forall k \in \llbracket 1,\smsc\rrbracket, \ e_k$ is only monitored by node $i_k$  in $\Def^{min}$. Now consider $\sola{\att^{max}}{b_2}{}$ defined in Lemma~\ref{algebra2}. Since $\sola{\att^{max}}{b_2}{}$ satisfies the above-mentioned sufficient conditions, i.e., its component basis is $\att^{max}$ and each component of $\att^{max}$ is targeted with probability $\frac{b_2}{\smsc}$, then $\sola{\att^{max}}{b_2}{}$ is an optimal solution of \rlpt{\att^{max}}. This implies that $(\sigma^{1^*},\sola{\att^{max}}{b_2}{})$ is a NE. Furthermore, the support of $\sola{\att^{max}}{b_2}{}$ contains $\att^1 = \{e_1\}\cup\{e_2,\dots,e_{b_2}\}$ and $\att^{2} = \{e_{b_2+1}\} \cup \{e_2,\dots,e_{b_2}\}$ (which are different since $b_2 < \semm = \smsc$). Therefore, $\att^1$ and $\att^{2}$ should give the same payoff to \attacker. However, we have the following contradiction:
\begin{align}
& U_2(\sigma^{1^*},\att^1)  \overset{\eqref{payoff2},\eqref{additive_equality}}{=}  |\att^1| - \mathbb{E}_{\sigma^{1^*}}[\valdet{\Def}{e_1}] - \mathbb{E}_{\sigma^{1^*}}[\valdet{\Def}{\att^1\backslash\{e_1\}}]\nonumber\\
& = \underset{= |\att^2|}{\underbrace{|\att^{1}|}} - \mathbb{E}_{\sigma^{1^*}}[\mathds{1}_{\{i_1 \in \Def\}}]  - \mathbb{E}_{\sigma^{1^*}}[\valdet{\Def}{\underset{=\att^{2}\backslash\{e_{b_2+1}\}}{\underbrace{\att^1\backslash\{e_1\}}}}]\label{needs some explanation}\\
 &\overset{\eqref{rho_sigma1}}{=} |\att^{2}| - \rho_{\sigma^{1^*}}(i_{1}) - \mathbb{E}_{\sigma^{1^*}}[\valdet{\Def}{\att^{2}\backslash\{e_{b_2+1}\}}] >  |\att^{2}| - \rho_{\sigma^{1^*}}(i_{b_2+1}) - \mathbb{E}_{\sigma^{1^*}}[\valdet{\Def}{\att^{2}\backslash\{e_{b_2+1}\}}]\nonumber\\
&\overset{\eqref{rho_sigma1}}{=}  |\att^{2}| - \mathbb{E}_{\sigma^{1^*}}[\valdet{\Def}{e_{b_2+1}}] - \mathbb{E}_{\sigma^{1^*}}[\valdet{\Def}{\att^{2}\backslash\{e_{b_2+1}\}}] \overset{\eqref{payoff2},\eqref{additive_equality}}{=}  U_2(\sigma^{1^*},\att^{2}).\label{needs some explanation2}
\end{align}
Note that in \eqref{needs some explanation} (resp. \eqref{needs some explanation2}), we used the fact that the node basis of $\sigma^{1^*}$ is $\Def^{min}$ and that $e_1$ (resp. $e_{b_2+1}$) is only monitored by $i_1$ (resp. $i_{b_2+1}$) in $\Def^{min}$. 

Thus, the sensing probability is necessarily identical among the nodes of $\Def^{min}$: $\exists \, \gamma \in \mathbb{R} \ | \ \forall i \in \Def^{min}, \ \rho_{\sigma^{1^*}}(i) \overset{\eqref{rho_sigma1}}{=} \sum_{\{\Def \in \mathcal{A}_1 \, | \, i \in \Def\}} \sigma^{1^*}_{\Def} = \gamma$. By summing over the nodes of $\Def^{min}$, and by combining Proposition~\ref{all_resources} with the fact that the node basis of $\sigma^{1^*}$ is $\Def^{min}$, we obtain:
\begin{align*}
\smsc\gamma &= \sum_{i \in \Def^{min}}\sum_{\{\Def \in \mathcal{A}_1 \, | \, i \in \Def\}} \sigma^{1^*}_{\Def} =   \sum_{i \in \Def^{min}}\sum_{\Def \in \mathcal{A}_1} \sigma^{1^*}_{\Def}\mathds{1}_{\{i \in \Def\}} =  \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def} \sum_{i \in \Def^{min}} \mathds{1}_{\{i \in \Def\}} \overset{\eqref{res1}}{=} b_1\sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def} = b_1.
\end{align*}
Therefore, $\gamma = \frac{b_1}{\smsc}$, meaning that in any NE $(\sigma^{1^*},\sigma^{2^*})$ whose node basis is an MSC, the sensing probability must be equal to $\frac{b_1}{\smsc}$ for all the nodes of the MSC, which proves the necessary condition on the sensing strategy.




\item Similarly, consider a NE $(\sigma^{1^*},\sigma^{2^*}) \in \nash$ whose component basis is an MSP $\att^{max} = \{e_1,\dots,e_{\smsc}\} \in \emm$, and assume that the attack probability is not identical among the components of $\att^{max}$. Again, without loss of generality, we assume that $\rho_{\sigma^{2^*}}(e_{1}) < \rho_{\sigma^{2^*}}(e_{b_1+1})$. 

Consider now an MSC $\Def^{min} = \{i_1,\dots,i_{\smsc}\} \in \msc$. Again, we reorder the indices such that $\forall l \in \llbracket 1,\smsc\rrbracket$, node $i_l$ only monitors component $e_l$ in $\att^{max}$. Analogously, consider the sensing strategy $\sold{\Def^{min}}{b_1}{}$. From the sufficient conditions, we know that $\sold{\Def^{min}}{b_1}{}$ is an optimal solution of \rlpo{\Def^{min}} and that $(\sold{\Def^{min}}{b_1}{},\sigma^{2^*})$ is a NE. Since $\sold{\Def^{min}}{b_1}{}$ assigns positive probabilities on the sensor placements $\Def^1:=\{i_1\}\cup\{i_2,\dots,i_{b_1}\}$ and  $\Def^{2} := \{i_{b_1+1}\} \cup\{i_2,\dots,i_{b_1}\}$, $\Def^{1}$ and $\Def^{2}$ should provide \defender with the same payoff. However, we have the following contradiction:
%
%
%
%Analogously, $(\sold{\Def^{min}}{b_1}{},\sigma^{2^*})$ is a NE, and $\sold{\Def^{min}}{b_1}{}$  assigns positive probabilities on the sensor placements $\Def^1:=\{i_1\}\cup\{i_2,\dots,i_{b_1}\}$ and  $\Def^{2} := \{i_{b_1+1}\} \cup\{i_2,\dots,i_{b_1}\}$. From the sufficient conditions, we know that $\sigma^{1^\prime}$ is an optimal solution of \rlpo{\Def^{min}} and that $(\sigma^{1^\prime},\sigma^{2^*})$ is a NE. Therefore $\Def^{1}$ and $\Def^{1^\prime}$ should provide \defender with the same payoff. However, we have the following contradiction:
\begin{align}
&U_1(\Def^1,\sigma^{2^*})  \overset{\eqref{payoff1}}{=} \mathbb{E}_{\sigma^{2^*}}[\valdet{\Def^1}{\att}] \overset{\eqref{detection_disruptions}}{=} \sum_{e \in \edges} \mathbb{E}_{\sigma^{2^*}}[\valdet{\Def^1}{e}\mathds{1}_{\{e \in \att\}}]  \overset{\eqref{rho_sigma2}}{=} \sum_{e\in \edges} \valdet{\Def^1}{e} \rho_{\sigma^{2^*}}(e)\nonumber\\
&=   \rho_{\sigma^{2^*}}(e_{1}) +  \sum_{e\in \att^{max} \backslash\{e_{1}\}} \valdet{\Def^1}{e} \rho_{\sigma^{2^*}}(e) <  \rho_{\sigma^{2^*}}(e_{b_1+1})+  \sum_{e\in \att^{max} \backslash\{e_{1}\}} \valdet{\Def^1}{e} \rho_{\sigma^{2^*}}(e)\label{oneee} \\
& =  \rho_{\sigma^{2^*}}(e_{b_1+1})+  \sum_{e\in  \{e_2,\dots,e_{b_1}\}} \valdet{\Def^1}{e} \rho_{\sigma^{2^*}}(e)  =  \rho_{\sigma^{2^*}}(e_{b_1+1})+  \sum_{e\in  \{e_2,\dots,e_{b_1}\}} \valdet{\Def^{2}}{e} \rho_{\sigma^{2^*}}(e)\label{three}\\
& =  \rho_{\sigma^{2^*}}(e_{b_1+1})+  \sum_{e\in \att^{max} \backslash\{e_{b_1+1}\}} \valdet{\Def^{2}}{e} \rho_{\sigma^{2^*}}(e) =  \sum_{e\in \edges} \valdet{\Def^{2}}{e} \rho_{\sigma^{2^*}}(e)  \overset{\eqref{payoff1},\eqref{detection_disruptions}}{=} U_1(\Def^{2},\sigma^{2^*}).\nonumber
\end{align}
In \eqref{oneee}, we used the fact that the component basis of $\sigma^{2^*}$ is $\att^{max}$. In \eqref{three}, we used the fact that $\Def^1$ only monitors components $\{e_1\}\cup\{e_2,\dots,e_{b_1}\}$ of $\att^{max}$, and that $\Def^1\backslash\{i_1\} = \Def^{2}\backslash\{i_{b_1+1}\}$.

Thus, the attack probability is identical among the components of $\att^{max}$: $\exists \, \gamma^{\prime} \in \mathbb{R} \ | \ \forall e \in \att^{max}, \ \rho_{\sigma^{2^*}}(e) \overset{\eqref{rho_sigma2}}{=} \sum_{\{\att \in \mathcal{A}_2 \, | \, e \in \att\}} \sigma^{2^*}_{\att} = \gamma^{\prime}$. By summing over the components of the MSP and by combining Proposition~\ref{all_resources} with the fact the component basis of $\sigma^{2^*}$ is $\att^{max}$, we obtain:
\begin{align*}
\smsc\gamma^{\prime} &= \sum_{e \in \att^{max}}\sum_{\{\att \in \mathcal{A}_2 \, | \, e \in \att\}} \sigma^{2^*}_{\att} =  \sum_{e \in \att^{max}}\sum_{\att \in \mathcal{A}_2} \sigma^{2^*}_{\att}\mathds{1}_{\{e \in \att\}}=  \sum_{\att \in \mathcal{A}_2}\sigma^{2^*}_{\att}\sum_{e \in \att^{max}} \mathds{1}_{\{e \in \att\}} \overset{\eqref{res2}}{=} b_2\sum_{\att \in \mathcal{A}_2}\sigma^{2^*}_{\att} = b_2.
\end{align*}
Thus, $\gamma^{\prime} = \frac{b_2}{\smsc}$, meaning that in any NE $(\sigma^{1^*},\sigma^{2^*})$ whose component basis is an MSP, the attack probability is equal to $\frac{b_2}{\smsc}$ for all the components of the MSP, which proves the necessary condition on the attack strategy.\hfill \Halmos
\end{enumerate}
%\vspace{-0.5cm}
%
\endproof
\else
\fi

\ifadditional
\tb{We end our analysis of the case $\smsc = \semm$ with a further characterization of the support of the NE of $\Gamma$. In particular, using the MSCs and the MSPs, we derive necessary conditions that are satisfied by every NE.}
\begin{proposition}\label{necessary_conditions}
If $b_1 <\smsc$, $b_2 < \semm$, and $\smsc = \semm$, then the set of NE has the following properties:
\begin{enumerate}
\item  In any NE, a node receives a sensor with positive probability only if it monitors exactly one component of any MSP:
%
%\tb{or}
%
%\tb{In any NE, a node is in the node basis only if it monitors one component of any MSP:}
%\begin{align*}
%\forall (\sigma^{1^*},\sigma^{2^*}) \in \nash, \ \forall \Def \in \supp(\sigma^{1^*}), \ \forall i \in \Def, \ \forall \att^{max} \in \emm, \ \valdet{i}{\att^{max}} = 1.
%\end{align*}
%\tb{or
\begin{align*}
\forall (\sigma^{1^*},\sigma^{2^*}) \in \nash, \ \forall i \in \nbasis{\sigma^{1^*}}, \ \forall \att^{max} \in \emm, \ \valdet{i}{\att^{max}} = 1.
\end{align*}
Furthermore, in any NE, a sensor placement is chosen with positive probability only if each of its sensors monitors a different component of any MSP:
\begin{align*}
\forall (\sigma^{1^*},\sigma^{2^*}) \in \nash, \ \forall \Def \in \supp(\sigma^{1^*}), \ \forall \att^{max} \in \emm, \ \forall e \in \att^{max}, \ \valdet{\Def}{e} = \sum_{i \in \Def}\valdet{i}{e}.
\end{align*}


%\tb{or equivalently} In any NE, a sensor placement is chosen with positive probability only if it monitors $b_1$ components of any MSP.
%\begin{align*}
%\forall \sigma^* \in \nash, \ \forall \att^{max} \in \emm, \ \Expone[*]{\valdet{\Def}{\att^{max}}} = b_1
%\end{align*}
\item In any NE, a component is targeted with positive probability only if it is monitored by a unique node of any MSC:
%
%\tb{or} 
%
%\tb{In any NE, an component is in the component basis only if it is monitored by a unique node of any MSC.}
%\begin{align*}
%\forall (\sigma^{1^*},\sigma^{2^*}) \in \nash, \ \forall \att \in \supp(\sigma^{2^*}), \ \forall e \in \att, \ \forall \Def^{min} \in \msc, \ \exists \, !\, i \in \Def^{min} \ | \ \valdet{i}{e} = 1.
%\end{align*}
%\tb{or
\begin{align*}
\forall (\sigma^{1^*},\sigma^{2^*}) \in \nash, \ \forall e \in \ebasis{\sigma^{2^*}}, \ \forall \Def^{min} \in \msc, \ \exists \, !\, i \in \Def^{min} \ | \ \valdet{i}{e} = 1.
\end{align*}
\end{enumerate}
\end{proposition}



In other words, if there exists at least one MSP, $\att^{max}$, such that a node $i \in \nodes$ does not monitor any component in $\att^{max}$, then $i$ will never receive a sensor in equilibrium. Besides, Proposition~\ref{necessary_conditions} tells us that if there exists a component $e \in \edges$ that is part of an MSP and such that at least two sensors in a sensor placement $\Def$ monitor $e$, then $\Def$ will never be chosen in equilibrium; since \attacker targets components that are spread across the network, \defender must allocate her sensing resources to avoid redundant detections.

Similarly, if there exists at least one MSC, $\Def^{min}$, such that a component $e$ is monitored by at least two nodes in $\Def^{min}$, then $e$ will never be targeted in equilibrium.


\proof{Proof of Proposition~\ref{necessary_conditions}.}
Let $\sigma^* = (\sigma^{1^*},\sigma^{2^*}) \in \nash$. Consider an MSC $\Def^{min} \in \msc$, an MSP $\att^{max} \in \emm$, and $(\sold{\Def^{min}}{b_1}{},\sola{\att^{max}}{b_2}{})$ constructed in Lemma~\ref{algebra2}.

\begin{enumerate}
\item
Thanks to Lemma~\ref{strategic_eq}, we know that the NE of $\Gamma$ are interchangeable. Proposition~\ref{necessary_conditions} implies that $(\sold{\Def^{min}}{b_1}{},\sola{\att^{max}}{b_2}{})$ defined in \eqref{sigma^S}-\eqref{sigma^T} is a NE. Therefore, $(\sigma^{1^*},\sola{\att^{max}}{b_2}{})$ is also a NE, and we obtain:
\begin{align*}
\frac{b_1b_2}{\smsc} &\overset{\eqref{eq_payoff}}{=} U_1(\sigma^{1^*},\sola{\att^{max}}{b_2}{}) \overset{\eqref{payoff1}}{=} \sum_{\Def \in \mathcal{A}_1}\sum_{\att \in \mathcal{A}_2}\sigma^{1^*}_{\Def}\sola{\att^{max}}{b_2}{\att} \valdet{\Def}{\att} \\
&= \sum_{\Def \in \mathcal{A}_1}\sum_{l=1}^{\order{\smsc}{b_2}}\sigma^{1^*}_{\Def}\sola{\att^{max}}{b_2}{\att^l} \valdet{\Def}{\att^l}   \overset{\eqref{sigma^T}}{=}   \sum_{\Def \in \mathcal{A}_1}\sum_{l=1}^{\order{\smsc}{b_2}}\sigma^{1^*}_{\Def}\frac{1}{\order{\smsc}{b_2}} \valdet{\Def}{\att^l}\\
&  \overset{\eqref{detection_disruptions}}{=}\sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def} \frac{1}{\order{\smsc}{b_2}}\sum_{l=1}^{\order{\smsc}{b_2}}\sum_{e \in \att^l} \valdet{\Def}{e} = \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def} \frac{1}{\order{\smsc}{b_2}}\sum_{e \in \edges} \valdet{\Def}{e}\sum_{l=1}^{\order{\smsc}{b_2}}\mathds{1}_{\{e \in \att^l\}}\\
& = \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def} \frac{1}{\order{\smsc}{b_2}}\sum_{e \in \att^{max}} \valdet{\Def}{e}\sum_{l=1}^{\order{\smsc}{b_2}}\mathds{1}_{\{e \in \att^l\}}\\
& \overset{\eqref{q1}}{=}   \sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def} \frac{1}{\order{\smsc}{b_2}}\sum_{e \in \att^{max}} \valdet{\Def}{e}\antiorder{\smsc}{b_2} \overset{\eqref{detection_disruptions},\eqref{arithmetic equality}}{=}  \frac{b_2}{\smsc}\sum_{\Def \in \mathcal{A}_1}\sigma^{1^*}_{\Def}\valdet{\Def}{\att^{max}}\\
& = \frac{b_2}{\smsc}\Expone[*]{\valdet{\Def}{\att^{max}}}.
\end{align*}
%where we used the fact that each component of $\att^{max}$ is targeted by $\antiorder{\smsc}{b_2}$ attacks in $\sola{\att^{max}}{b_2}{}$ (see Lemma~\ref{algebra2}).

Therefore, we obtain:
\begin{align}
\forall \sigma^* \in \nash, \ \forall \att^{max} \in \emm, \ \Expone[*]{\valdet{\Def}{\att^{max}}} = b_1.\label{I lost count}
\end{align}

We can deduce further results from this equation. Consider  $\sigma^* \in \nash, \ \att^{max} \in \emm$, then:
\begin{align*}
b_1 & \overset{\eqref{I lost count}}{=} \Expone[*]{\valdet{\Def}{\att^{max}}}  \overset{\eqref{detection_disruptions}}{=} \Expone[*]{\sum_{e \in \att^{max}}\valdet{\Def}{e}}  \overset{\eqref{redundant_nodes}}{\leq} \Expone[*]{\sum_{i \in \Def}\sum_{e \in \att^{max}}\valdet{i}{e}} \\
&\overset{\eqref{detection_disruptions}}{=}  \Expone[*]{\sum_{i \in \Def}\valdet{i}{\att^{max}}}  \overset{\eqref{def_extended_matching}}{\leq} \Expone[*]{\sum_{i \in \Def}1} = \Expone[*]{|\Def|} \overset{\eqref{res1}}{=} b_1.
\end{align*}

Therefore, all the previous inequalities become equalities. The first one implies that:
\begin{align*}
\forall \Def \in \supp(\sigma^{1^*}), \ \forall e \in \att^{max}, \ \valdet{\Def}{e} = \sum_{i \in \Def} \valdet{i}{e}.
\end{align*}


The second induced equality implies that:
\begin{align*}
\forall i \in \nbasis{\sigma^{1^*}}, \ \forall \att^{max} \in \emm, \ \valdet{i}{\att^{max}} = 1.
\end{align*}


%The third induced equality implies:
%\begin{align*}
%\forall \Def \in \supp(\sigma^{1^*}), \ |\Def| = b_1
%\end{align*}
%which means that every defense in the support of a NE uses all the resources of \defender.



\item Similarly, by interchangeability $(\sold{\Def^{min}}{b_1}{},\sigma^{2^*}) \in \nash$. Then:
\begin{align*}
\frac{b_1b_2}{\smsc}  &\overset{\eqref{eq_payoff}}{=} U_1(\sold{\Def^{min}}{b_1}{},\sigma^{2^*})  \overset{\eqref{payoff1}}{=}    \sum_{k=1}^{\order{\smsc}{b_1}}\sum_{\att \in \mathcal{A}_2}\sold{\Def^{min}}{b_1}{\Def^k}\sigma^{2^*}_{\att} \valdet{\Def^k}{\att} \\
&\overset{\eqref{sigma^S}}{=}   \sum_{k=1}^{\order{\smsc}{b_1}}\sum_{\att \in \mathcal{A}_2}\frac{1}{\order{\smsc}{b_1}}\sigma^{2^*}_{\att} \valdet{\Def^k}{\att} \overset{\eqref{detection_disruptions}}{=} \frac{1}{\order{\smsc}{b_1}}\sum_{\att \in \mathcal{A}_2}\sigma^{2^*}_{\att}  \sum_{e \in \att} \sum_{k=1}^{\order{\smsc}{b_1}}\valdet{\Def^k}{e}.
\end{align*}

Since $\Def^{min} \in \msc$, then $\forall e \in \edges, \ \exists \,i_e \in \Def^{min} \ | \ \valdet{i_e}{e} = 1$. Therefore:
\begin{align*}
\forall e \in \edges, \  \sum_{k=1}^{\order{\smsc}{b_1}}\valdet{\Def^k}{e} &=  \sum_{\{k\in \llbracket1,\order{\smsc}{b_1} \rrbracket \, | \, i_e \in \Def^k\}}1 + \sum_{\{k\in \llbracket1,\order{\smsc}{b_1} \rrbracket \, | \, i_e \notin \Def^k\}} \underset{\geq 0 }{\underbrace{\valdet{\Def^k}{e}}} \\
&\geq |\{k\in \llbracket1,\order{\smsc}{b_1} \rrbracket \, | \, i_e \in \Def^k\}| \overset{\eqref{q1}}{=} \antiorder{\smsc}{b_1}.
\end{align*}

Thus, by plugging it in the previous equation, we obtain:
\begin{align*}
\frac{b_1b_2}{\smsc}&\geq   \frac{1}{\order{\smsc}{b_1}}\sum_{\att \in \mathcal{A}_2}\sigma^{2^*}_{\att} \sum_{e \in \att} \antiorder{\smsc}{b_1}= \frac{\antiorder{\smsc}{b_1}}{\order{\smsc}{b_1}} \sum_{\att \in \mathcal{A}_2}\sigma^{2^*}_{\att} |\att| \overset{\eqref{arithmetic equality}}{=} \frac{b_1}{\smsc} \mathbb{E}_{\sigma^{2^*}}[|\att|]  \overset{\eqref{res2}}{=} \frac{b_1}{\smsc}b_2.
\end{align*}
%where we used the fact that $\order{\smsc}{b_1} b_1 = \antiorder{\smsc}{b_1} \smsc$.

Therefore, we obtain the following equality:
\begin{align}
\forall \att \in \supp(\sigma^{2^*}), \ \forall e \in \att, \ \forall  k\in \llbracket1,\order{\smsc}{b_1} \rrbracket \, | \, i_e \notin \Def^k, \ \valdet{\Def^k}{e} = 0.\label{cannot_detect}
\end{align}
%From the second induced equality, we obtain:
%\begin{align*}
%\forall \att \in \supp(\sigma^{2^*}), \ |\att| = b_2
%\end{align*}
%which means that every attack in the support of a NE uses all the resources of \attacker.

%With a bit of work, from the induced equality, we can show that:
%\begin{align*}
%\forall \att \in \supp(\sigma^{2^*}), \ \forall e \in \att, \ \forall \Def^{min} \in \msc, \ \exists \, !\, i \in \Def^{min} \ | \ \valdet{i}{e} = 1 
%\end{align*}

Now, consider $\att \in \supp(\sigma^{2^*})$, $e \in \att$, and let $i_e \in \Def^{min}$ be a node that satisfies $\valdet{i_e}{e} = 1$. Note that \eqref{cannot_detect} can be derived starting from any initial ordering of the node indices in $\Def^{min}$. Consider $i^\prime \in \Def^{min} \ | \ i^{\prime} \neq i_e$. Since $b_1 < \smsc$, then we can find an ordering of the node indices in $\Def^{min}$ such that there is a sensor placement $\Def^k$ in the support of $\sold{\Def^{min}}{b_1}{}$  that satisfies $i^{\prime} \in \Def^k$ and $i_e \notin \Def^k$. From \eqref{cannot_detect}, we deduce that $0 \leq \valdet{i^{\prime}}{e} \overset{\eqref{monotonicity_detection}}{\leq} \valdet{\Def^k}{e} \overset{\eqref{cannot_detect}}{=} 0$. Therefore, for any $i^{\prime} \in \Def^{min}$ such that $i^{\prime}\neq i_e$, $i^{\prime}$ does not monitor $e$, which implies that $e$ is only monitored by $i_e$ in $\Def^{min}$. Thus:
\begin{align*}
\forall e \in \ebasis{\sigma^{2^*}}, \ \forall \Def^{min} \in \msc, \ \exists \, !\, i \in \Def^{min} \ | \ \valdet{i}{e} = 1.
\end{align*}
\end{enumerate}
\hfill \Halmos
\endproof

\else
\fi
%\section{Proof of Statements B}


\ifadditional
\subsection{Proof of Section~\ref{sec:Answer}}

%\subsection{Main Case of Interest: $b_2<\smsc$}

%\ifadditional
\begin{proposition}\label{Cor2}
Consider a network $\mathcal{G}$ and sensing model $\{\set{i}, \ i \in \nodes \}$ that satisfy $\smsc = \semm$, a target detection rate $\alpha \in [0,1]$, and \attacker's resources $b_2<\semm$. Then, for any MSC $\Def^{\text{min}} \in \mathcal{S}$ and any MSP $\att^{\text{max}} \in \mathcal{M}$, an optimal solution of \ECOP is given by $\lceil \alpha \smsc \rceil$, $(\sold{\Def^{\text{min}}}{\lceil \alpha \smsc \rceil}{},\sola{\att^{\text{max}}}{b_2}{})$.
\end{proposition}

\proof{Proof of Proposition~\ref{Cor2}.}

When $\smsc = \semm$, we know from Cor.~\ref{Cor1} that $\forall \sigma^* \in \nash, \ r(\sigma^*) = \frac{b_1}{\smsc}$. Therefore, \ECOP can be rewritten as follows:
\begingroup
\addtolength{\jot}{\spacingalign}
\begin{align*}
\underset{b_1,\, \sigma^\dag}{\text{minimize}}& \quad b_1\nonumber\\
\text{subject to}& \quad \frac{b_1}{\smsc} \geq \alpha, \\
& \quad \sigma^\dag \in \nash(b_1,b_2),\\
& \quad b_1 \in \mathbb{N}.\nonumber
\end{align*}
\endgroup
Then, the optimal value of \ECOP in that case is $b_1^\dag = \lceil \alpha \smsc \rceil$. 

Now, consider an MSC $\Def^{min} \in \msc$ and an MSP $\att^{max} \in \emm$. From Lemma~\ref{algebra1} and Proposition~\ref{necessary_conditions}, we know that $(\sold{\Def^{min}}{b_1^\dag}{},\sola{\att^{max}}{b_2}{})\in \nash(b_1^\dag,b_2)$, i.e., is a NE of the game induced by  $b_1^\dag$ and $b_2$. Therefore, $\lceil \alpha \smsc \rceil, (\sold{\Def^{min}}{b_1^\dag}{},\sola{\att^{max}}{b_2}{})$ is an optimal solution of \ECOP.
\hfill \Halmos
\endproof



\proof{Proof of Proposition~\ref{Prop_interim}}
Recall that in the general case $\semm \leq \smsc$, we admit a relaxation of \ECOP and consider instead the following mathematical program with equilibrium constraints:
\begingroup
\addtolength{\jot}{\spacingalign}
\begin{align}
(\mathcal{P}_{\epsilon}): \quad \underset{b_1,\, \sigma^\dag}{\text{minimize}}& \quad b_1\nonumber\\
\text{subject to}& \quad \sdet{*} \geq \alpha, \quad \quad \forall \sigma^* \in \nash(b_1,b_2) \label{all_NE_epsilon}\\
& \quad \sigma^\dag \in \nash_\epsilon(b_1,b_2)\nonumber\\
& \quad b_1 \in \mathbb{N},\nonumber
\end{align}
\endgroup
for some $\epsilon\geq 0$.

In this case, we know from the lower bound in Thm.~\ref{bounds_game} that $\forall b_1 < \smsc, \forall \sigma^* \in \nash(b_1,b_2), \quad  \dfrac{b_1}{\smsc} \leq\sdet{*}.$ Therefore, constraint \eqref{all_NE_epsilon} is satisfied if $b_1 \geq b_1^\prime := \lceil \alpha \smsc\rceil$. Now, consider an MSC $\Def^{min} \in \msc$ and an MSP $\att^{max} \in \emm$.  We know from Thm.~\ref{MSC-MSP-eNE} that $(\sold{\Def^{min}}{b_1^\prime}{},\sola{\att^{max}}{b_2}{}) \in \nash_{\epsilon}(b_1^\prime,b_2)$, where $\epsilon = b_1^\prime b_2\left( \frac{1}{\max\{b_1^\prime,\semm\}} - \frac{1}{\smsc}\right)$. Therefore, $b_1^\prime, (\sold{\Def^{min}}{b_1^\prime}{},\sola{\att^{max}}{b_2}{})$ is a feasible solution of $(\mathcal{P}_{\epsilon})$ (with the same $\epsilon$), and the corresponding objective value is $b_1^\prime$.

Finally, from the upper bound in Thm.~\ref{bounds_game}, we know that $\forall b_1 < \smsc, \forall \sigma^* \in \nash(b_1,b_2), \quad  \sdet{*} \leq \min\left\{\frac{b_1}{\semm},1\right\}$. Therefore, constraint \eqref{all_NE_epsilon} cannot be satisfied if $b_1 < \lceil \alpha \semm \rceil$. This implies that an optimality gap associated with $b_1^\prime, (\sold{\Def^{min}}{b_1^\prime}{},\sola{\att^{max}}{b_2}{})$ is given by $\lceil \alpha \smsc \rceil - \lceil \alpha \semm \rceil$.


\hfill \Halmos
\endproof
\else
\fi

\section{Proofs of Section~\ref{conclusions}} \label{Main Proofs 6}





\begin{lemma}\label{Big Support}
Given $b_2 < \semm$, let $\rho \in  [0,1]^{|\edges|}$ that satisfies $\sum_{e \in \edges} \rho_e = b_2$. Then, there exists an attack strategy $\sigma^2 \in \Delta(\mathcal{A}_2)$ that satisfies $\forall e \in \edges, \ \rho_{\sigma^2}(e) = \rho_e.$ %\tr{Actually, such a strategy can be constructed so that its support is of size at most $m$.}
\end{lemma}

\proof{Proof of Lemma~\ref{Big Support}.}

Given $b_2 < \semm$, let $\bs{A}$ be the $|\edges| \times {|\edges| \choose b_2}$ binary matrix whose rows (resp. columns) are indexed by the components (resp. the size-$b_2$ subsets) of $\edges$, and which satisfies $\forall (e,\att) \in \edges \times \overline{\mathcal{A}_2}, \ a_{e,\att} = \mathds{1}_{\{e \in \att\}}$. Then, given $\rho \in [0,1]^{|\edges|}$ that satisfies $\sum_{e \in \edges}\rho_e = b_2$, we must show that the following system of equations has a feasible solution:
\vspace{-0.3cm}
%\begin{align*}
%d_{e\att} = \begin{cases} 1 \text{ if component } e \text{ is in subset } \att \\
%0 \text{ otherwise}.
%\end{cases}
%\end{align*}
%
%Then, we must show that there exists a probability distribution $\sigma^2$ on $R$ such that $D\sigma^2 = \rho$ (check for the sets). It suffices to show that there always exists a solution to:
\begin{align*}
&\bs{A}\sigma^2 = \rho\\[-0.2cm]
&\boldsymbol{1}^T_{|\overline{\mathcal{A}_2}|}\sigma^2 = 1\\[-0.2cm]
&\sigma^2 \geq \bs{0}_{|\overline{\mathcal{A}_2}|}.
\end{align*}

%where $\bs{1}_{|\overline{\mathcal{A}_2}|}$ represents the vector of length $|\overline{\mathcal{A}_2}|$ filled with ones. 
%\vspace{-0.3cm}

Since each $\att \in \overline{\mathcal{A}_2}$ is of size $b_2$, it is easy to see that $\frac{1}{b_2}\bs{1}_{|\edges|}^T \bs{A} = \bs{1}_{|\overline{\mathcal{A}_2}|}^T$. Furthermore, since $\frac{1}{b_2}\bs{1}_{|\edges|}^T \rho = 1$, it implies that if $\sigma^2$ satisfies $\bs{A}\sigma^2 = \rho$, it also satisfies $\bs{1}_{|\overline{\mathcal{A}_2}|}^T \sigma^2 = 1$. Therefore, we only need to show that there exists $\sigma^2 \geq \bs{0}_{|\overline{\mathcal{A}_2}|}$ such that $\bs{A}\sigma^2 = \rho$.
%\begin{align*}
%\bs{1}_{|\att^\prime|}^T D = \sum_{e \in \att^\prime} \mathds{1}_{e \in \att}
%\end{align*}
%\begin{align*}
%b_2 = \sum_{e \in \att^\prime} \rho \sum_{e \in \att^\prime} (D\sigma^2)_e = 
%\end{align*}
%Summing the constraints of $D\sigma^2= \rho$ and dividing by $b_2$ gives $\boldsymbol{1}^T\sigma^2 = 1$, so the latter constraint is redundant. Given that $\boldsymbol{1}^T\sigma^2 = 1$ and $\sigma^2 \geq0$, the constraints $\sigma^2 \leq 1$ are also redundant. Thus, we only need to show that there is a solution to:
%\begin{align*}
%&D\sigma^2 = \rho\\
%&0 \leq \sigma^2.
%\end{align*}
By Farkas' lemma, such a solution exists if and only if there does not exist $w \in \mathbb{R}^{|\edges|}$ such that $w^T\bs{A} \leq \bs{0}_{|\overline{\mathcal{A}_2}|}^T$ and $w^T\rho >0$. 

%Let $w \in \mathbb{R}^{|\edges|}$ that satisfies $w^TA \leq 0$, and assume, without loss of generality, that $w_1 \geq \dots \geq w_{|\edges|}$. Note that since $\att^1 = \{e_1,\dots,e_{b_2}\} \in \overline{\mathcal{A}_2}$, we have $\sum_{k=1}^{b_2} w_k = (w^TA)_{\att^1} \leq 0$. Then, we obtain:
%\begin{align*}
%w^T\rho &= \sum_{k=1}^m w_k \rho_k = \sum_{k=1}^{b_2} w_k \rho_k + \sum_{k=b_2+1}^{m} w_k \rho_k + \sum_{k=1}^{b_2} w_k (1-\rho_k) - \sum_{k=1}^{b_2} w_k (1-\rho_k)\\
%& = \underset{\leq 0}{\underbrace{\sum_{k=1}^{b_2} w_k}} + \sum_{k=b_2+1}^{m} \underset{\leq w_{b_2}}{\underbrace{w_k}} \underset{\geq 0}{\underbrace{\rho_k}} - \sum_{k=1}^{b_2} \underset{\geq w_{b_2}}{\underbrace{w_k}} \underset{\leq 0}{\underbrace{(1-\rho_k)}} \leq  w_{b_2}\left(\sum_{k=b_2+1}^{m} \rho_k - \sum_{k=1}^{b_2}  (1-\rho_k)\right) \\
%& =  w_{b_2} \left(\sum_{k=1}^{m} \rho_k - b_2\right) = 0.
%\end{align*}
Let $w \in \mathbb{R}^{|\edges|}$ that satisfies $w^T\bs{A} \leq \bs{0}_{|\overline{\mathcal{A}_2}|}^T$, and let us order the components in $\edges$ so that $w_{e_1} \geq \dots \geq w_{e_{|\edges|}}$. For notational simplicity, let $w_k \coloneqq w_{e_k}$ and $\rho_k \coloneqq \rho_{e_k}$, $\forall k \in \llbracket 1,|\edges|\rrbracket$. Note that since $\att^1 = \{e_1,\dots,e_{b_2}\} \in \overline{\mathcal{A}_2}$, we have $\sum_{k=1}^{b_2} w_k = (w^T\bs{A})_{\att^1} \leq 0$. Then, we obtain:
\begin{align*}
w^T\rho &= \sum_{k=1}^m w_k \rho_k = \underset{\leq 0}{\underbrace{\sum_{k=1}^{b_2} w_k}} + \sum_{k=b_2+1}^{m} \underset{\leq w_{b_2}}{\underbrace{w_k}} \underset{\geq 0}{\underbrace{\rho_k}} - \sum_{k=1}^{b_2} \underset{\geq w_{b_2}}{\underbrace{w_k}} \underset{\leq 0}{\underbrace{(1-\rho_k)}} \leq   w_{b_2} \left(\sum_{k=1}^{m} \rho_k - b_2\right) = 0.
\end{align*}
Therefore, there does not exist $w \in \mathbb{R}^{|\edges|}$ such that $w^T\bs{A} \leq \bs{0}_{|\overline{\mathcal{A}_2}|}^T$ and $w^T\rho >0$, which, by Farkas' lemma, implies that there exists an attack strategy $\sigma^2 \in \Delta(\mathcal{A}_2)$ such that $\forall e \in \edges, \ \rho_{\sigma^2}(e) = \rho_e$.
%$\sum_{k=1}^{b_2} w_k \geq w^T \rho$ because $0 \leq \rho \leq 1$, and $1^T\rho = b_2$. But one of the constraints of $w^TD \leq 0$ is $\sum_{k=1}^{b_2}w_k \leq 0$, so $w^T\rho \leq 0$.
%Do the special cases first.
%\begin{align*}
%\forall \att \subset \att^\prime \, | \, |\att|=b_2, \ \sigma^2_{\att} = \frac{1}{{m-2 \choose b_2-1}}\sum_{\{l \in \llbracket 1,m\rrbracket \, | \, e_l \in \att\}}\rho_l - \frac{b_2-1}{{m-1 \choose b_2}}
%\end{align*}
%
%First, let us show that $\sigma^2 \in \Delta(\mathcal{A}_2)$, i.e., that $\sigma^2$ is a probability distribution.
%\begin{align*}
%\forall \att \subset \att^\prime \ | \ |\att| = b_2, \ \sigma^2_\att &= \frac{1}{{m-2 \choose b_2-1}}\sum_{\{l \in \llbracket 1,m\rrbracket \, | \, e_l \in \att\}}\rho_l - \frac{b_2-1}{{m-1 \choose b_2}}\\
%& = \frac{1}{{m-2 \choose b_2-1}}\left(\sum_{\{l \in \llbracket 1,m\rrbracket \, | \, e_l \in \att\}}\rho_l - \frac{b_2(b_2-1)}{m-1}\right)
%\end{align*} 
\hfill
\Halmos
\endproof



\proof{Proof of Theorem~\ref{Constant}.}

Consider \defender's amount of resources $b_1$. If $b_1 \geq \smsc$, then it is easy to see that $\forall b_2 < \semm$, $\forall \sigma^* \in \nash(b_1,b_2)$, $r(\sigma^*) = 1$. Henceforth, we assume that $b_1 < \smsc$. Recall from Proposition~\ref{all_resources} that the NE of $\Gamma$ can be obtained by solving \lpob and \lptb. 

\begin{enumerate}
\item
First, we show  that for $b_2 = 1$, there exists an optimal solution of \lptp, $\sigma^{2^*} \in \Delta(\overline{\mathcal{A}_2})$, that satisfies $
\forall e \in \edges, \ \rho_{\sigma^{2^*}}(e) \leq \frac{1}{\semm}.$ Since $b_2 = 1$, then $\overline{\mathcal{A}_2} = \edges$, and $\forall \sigma^2 \in \Delta(\edges), \ \forall e \in \edges, \ \sigma^2_e = \rho_{\sigma^2}(e)$.

\begin{enumitemize}
\item[--] Consider an optimal solution of \lptp, $\sigma^{2^*} \in \Delta(\edges)$, and assume on the contrary that $\exists \, e^\prime \in \edges, \  \exists \, \varepsilon >0 \ | \ \rho_{\sigma^{2^*}}(e^\prime) = \frac{1}{\semm} + \varepsilon.$ Let $\Def^* \in \argmax_{\Def \in \overline{\mathcal{A}_1}} U_1(\Def,\sigma^{2^*})$. 
%We show the following result by induction: For any $b_2 <\semm$, there exists an optimal solution of \lpt, $\sigma^{2^*} \in \Delta(\mathcal{A}_2)$, that satisfies:
%\begin{align*}
%\forall e \in \edges, \ \rho_{\sigma^{2^*}}(e) \leq \frac{b_2}{\semm}
%\end{align*}
From Prop.~\ref{best_set_cover}, we know that: 
\vspace{-0.0cm}
\begin{align}
U_1(\Def^*,\sigma^{2^*}) \overset{\eqref{transform1}}{=} - U_2(\Def^*,\sigma^{2^*}) + 1 \leq -\max\{ 1 - \frac{b_1}{\semm},0\} + 1 = \min\{\frac{b_1}{\semm},1\}\leq \frac{b_1}{\semm}.\label{One of the very last}
\end{align}

%From Eq.~\eqref{nice_detection_inequality}, we can  the sensing function $\detect$ satisfies:
%\begin{align}
%\forall \Def \in \overline{\mathcal{A}_1}, \ \forall e \in \edges, \ \valdet{\Def}{e} \leq \frac{1}{b_1 -1} \sum_{i \in \Def} \valdet{\Def\backslash\{i\}}{e}. \label{For Later}
%\end{align}
\vspace{-0.0cm}

Therefore, we can show that $\exists \, i^\prime \in \Def^* \ | \ U_1(\Def^*,\sigma^{2^*}) - U_1(\Def^*\backslash\{i^\prime\},\sigma^{2^*}) \leq \frac{1}{\semm}$. Indeed, if $\forall i \in \Def^*, \ U_1(\Def^*,\sigma^{2^*}) - U_1(\Def^*\backslash\{i^\prime\},\sigma^{2^*}) > \frac{1}{\semm}$, then we obtain the following contradiction:
\vspace{-0.0cm}
\begin{align*}
&(b_1  -1)U_1(\Def^*,\sigma^{2^*}) \overset{\eqref{payoff1},\eqref{nice_detection_inequality}}{\leq}\sum_{i \in \Def^*} U_1(\Def^*\backslash\{i^\prime\},\sigma^{2^*}) <b_1 U_1(\Def^*,\sigma^{2^*}) - \frac{b_1}{\semm} \overset{\eqref{One of the very last}}{\leq} (b_1 - 1) U_1(\Def^*,\sigma^{2^*}).
\end{align*}

\vspace{-0.0cm}

\item[--] This implies that $e^\prime \in \set{\Def^*}$: If  $e^\prime \notin \set{\Def^*}$ instead, then repositioning the detector on node $i^\prime$ to a node that can monitor $e^\prime$ improves \defender's payoff by at least $\varepsilon$ and contradicts the definition of $\Def^*$. %$U_1(\Def^*\backslash\{i^\prime\}\cup\{i^*\},\sigma^{2^*})  \geq \varepsilon+ U_1(\Def^*,\sigma^{2^*}) > U_1(\Def^*,\sigma^{2^*}).$
%\begin{align*}
%U_1(\Def^*\backslash\{i^\prime\}\cup\{i^*\},\sigma^{2^*}) &= \sum_{e \in \edges}\sigma^{2^*}_e \valdet{\Def^*\backslash\{i^\prime\}\cup\{i^*\}}{e} = \sigma^{2^*}_{e^\prime} + \sum_{e \in \edges\backslash\{e^\prime\}}\sigma^{2^*}_e \valdet{\Def^*\backslash\{i^\prime\}\cup\{i^*\}}{e}\\
%&\geq \sigma^{2^*}_{e^\prime} + \sum_{e \in \edges\backslash\{e^\prime\}}\sigma^{2^*}_e \valdet{\Def^*\backslash\{i^\prime\}}{e}\\
%& = \sigma^{2^*}_{e^\prime} + \sum_{e \in \edges}\sigma^{2^*}_e \valdet{\Def^*\backslash\{i^\prime\}}{e}\\
%& = \frac{1}{\semm}+ \varepsilon + U_1(\Def^*\backslash\{i^\prime\},\sigma^{2^*}) - U_1(\Def^*,\sigma^{2^*}) + U_1(\Def^*,\sigma^{2^*})\\
%& \geq \frac{1}{\semm}+ \varepsilon - \frac{1}{\semm} + U_1(\Def^*,\sigma^{2^*})\\
%& > U_1(\Def^*,\sigma^{2^*}) = \max_{\Def \in \overline{\mathcal{A}_1}}U_1(\Def,\sigma^{2^*})
%\end{align*}
%\begin{align*}
%U_1(\Def^*\backslash\{i^\prime\}\cup\{i^*\},\sigma^{2^*}) &\overset{\eqref{payoff1}}{=} \sum_{e \in \edges}\sigma^{2^*}_e \valdet{\Def^*\backslash\{i^\prime\}\cup\{i^*\}}{e} = \sigma^{2^*}_{e^\prime} + \sum_{e \in \edges\backslash\{e^\prime\}}\sigma^{2^*}_e \valdet{\Def^*\backslash\{i^\prime\}\cup\{i^*\}}{e}\\
%&\overset{\eqref{monotonicity_detection}}{\geq} \sigma^{2^*}_{e^\prime}+ \sum_{e \in \edges\backslash\{e^\prime\}}\sigma^{2^*}_e \valdet{\Def^*\backslash\{i^\prime\}}{e}  = \sigma^{2^*}_{e^\prime} + \sum_{e \in \edges}\sigma^{2^*}_e \valdet{\Def^*\backslash\{i^\prime\}}{e}\\
%& \overset{\eqref{payoff1}}{=} \frac{1}{\semm}+ \varepsilon + U_1(\Def^*\backslash\{i^\prime\},\sigma^{2^*}) - U_1(\Def^*,\sigma^{2^*}) + U_1(\Def^*,\sigma^{2^*})\\
%& \geq \frac{1}{\semm}+ \underset{>0}{\underbrace{\varepsilon}} - \frac{1}{\semm} + U_1(\Def^*,\sigma^{2^*}) > U_1(\Def^*,\sigma^{2^*}) = \max_{\Def \in \overline{\mathcal{A}_1}}U_1(\Def,\sigma^{2^*}).
%\end{align*}

%Thus, $e^\prime \in \mathcal{C}_{\Def^*}$. 

\item[--] Then, we show that at least $b_1$ components are monitored by $\Def^*$. 
%
%
%Let $\widehat{\sigma}^2 \in \Delta(\edges)$ denote the uniform probability over the set of components $\edges$, and let $\widehat{\Def} \in \argmax_{\Def \in \overline{\mathcal{A}_1}} U_1(\Def,\widehat{\sigma}^2)$. Since $b_1 < \smsc$, $\exists \, \widehat{e} \in \edges \ | \ \valdet{\widehat{\Def}}{\widehat{e}} = 0$. Then, we obtain:
%\begin{align}
%&U_1(\Def^*,\sigma^{2^*}) = \min_{\sigma^2 \in \Delta(\edges)}\max_{\Def \in \overline{\mathcal{A}_1}} U_1(\Def,\sigma^2) \leq  U_1(\widehat{\Def},\widehat{\sigma}^2) \overset{\eqref{payoff1}}{=} \sum_{e \in \edges} \widehat{\sigma}^2_e \valdet{\widehat{\Def}}{e}\nonumber \\
%& = \underset{=0}{\underbrace{\widehat{\sigma}^2_{\widehat{e}} \valdet{\widehat{\Def}}{\widehat{e}}}} +  \sum_{e \in \edges\backslash\{\widehat{e}\}} \widehat{\sigma}^2_e \underset{\leq 1}{\underbrace{\valdet{\widehat{\Def}}{e}}} \leq \sum_{e \in \edges} \widehat{\sigma}^2_e - \widehat{\sigma}^2_{\widehat{e}}= 1 -  \widehat{\sigma}^2_{\widehat{e}} < 1. \label{Incomplete Monitoring}
%\end{align}
%
If we assume that $|\set{\Def^*}| < b_1$, then at least one detector in $\Def^*$ can be removed without changing \defender's payoff. Let $i_0 \in \Def^*$ denote the location of that detector. Now, we can show that $\exists \, e \in \edges\backslash\{\set{\Def^*}\} \ | \ \sigma_e^{2^*} >0$: if on the contrary, we had $\forall e \in \edges\backslash\{\set{\Def^*}\}, \ \sigma_e^{2^*} =0$, then we would obtain $U_1(\Def^*,\sigma^{2^*}) = 1$, which is contradiction: Since $b_1 < \smsc$, \defender's payoff in equilibrium must be strictly smaller than 1. Let $e \in \edges\backslash\{\set{\Def^*}\} \ | \ \sigma_e^{2^*} >0$ and let $i \in \nodes \ | \ \valdet{i}{e}=1$. Repositioning the detector from node $i_0$ to node $i$ will increase \defender's payoff by at least $\sigma_e^{2^*}$, which contradicts the definition of $\Def^*$. Thus, $|\set{\Def^*}| \geq b_1$.




\item[--] Now, we show that we can construct $\sigma^{2^\prime}$ which is the same probability distribution as $\sigma^{2^*}$ except that it reallocates $\varepsilon$ probability from $e^\prime$ to a subset of components $\att^1$ monitored by $\Def^*$ while ensuring that the  attack probability of each component in $\att^1$ is not above $\frac{1}{\semm}$. Let us split $\mathcal{C}_{\Def^*}$ into $\{e^\prime\}$, $\att^1 = \{e \in \mathcal{C}_{\Def^*} \backslash\{e^\prime\} \ | \ \sigma^{2^*}_e <\frac{1}{\semm}\}$, and  $\att^2 = \{e \in \mathcal{C}_{\Def^*} \backslash\{e^\prime\} \ | \ \sigma^{2^*}_e \geq\frac{1}{\semm}\}$.
%Note that $\att^1 \neq \emptyset$, otherwise we would have $|\mathcal{C}_{\Def^*}| = |\att^2| +1$ and:
%\begin{align*}
%\sum_{e \in \mathcal{C}_{\Def^*}}\sigma^{2^*}_e = \sigma^{2^*}_{e^\prime} + \sum_{e \in \att^2} \sigma^{2^*}_e \geq \frac{|\att^2| +1}{\semm} + \varepsilon = \frac{|\mathcal{C}_{\Def^*}|}{\semm} + \varepsilon \geq \frac{b_1}{\semm} + \varepsilon > \frac{b_1}{\semm},
%\end{align*}
%which would contradict \eqref{One of the very last}.
%
Now, we have:
\begin{align*}
\varepsilon\overset{\eqref{payoff1}}{=}  U_1(\Def^*,\sigma^{2^*})  - \sum_{\mathclap{e \in \att^1\cup \att^2}}\sigma^{2^*}_e - \frac{1}{\semm}\overset{\eqref{One of the very last}}{\leq}   \frac{|\set{\Def^*}| - |\att^2| - 1}{\semm}  - \sum_{e \in \att^1}\sigma^{2^*}_e = \sum_{e \in \att^1} (\frac{1}{\semm} - \sigma^{2^*}_e),
\end{align*}
%
%
%\begin{align*}
%\frac{|\mathcal{C}_{\Def^*}|}{\semm}\geq\frac{b_1}{\semm} \overset{\eqref{One of the very last}}{\geq} U_1(\Def^*,\sigma^{2^*}) \overset{\eqref{payoff1}}{=} \sum_{e \in \mathcal{C}_{\Def^*}} \sigma^{2^*}_e  = \sigma^{2^*}_{e^\prime} + \sum_{e \in \att^1}\sigma^{2^*}_e + \sum_{e \in \att^2}\sigma^{2^*}_e \geq \frac{|\att^2| +1}{\semm} + \varepsilon + \sum_{e \in \att^1}\sigma^{2^*}_e,
%\end{align*}
%which is equivalent to:
%\begin{align}
%0 < \varepsilon \leq \frac{|\mathcal{C}_{\Def^*}| - |\att^2| - 1}{\semm} - \sum_{e \in \att^1}\sigma^{2^*}_e = \frac{|\att^1|}{\semm} - \sum_{e \in \att^1}\sigma^{2^*}_e = \sum_{e \in \att^1} (\frac{1}{\semm} - \sigma^{2^*}_e). \label{Enough Transfer}
%\end{align}
which implies that $\att^1 \neq \emptyset$, and that it is possible to allocate $\varepsilon$ additional probability to components in $\att^1$ so that the attack probability of each component in $\att^1$ is not above $\frac{1}{\semm}$. Thus, $\sigma^{2^\prime}$ can be constructed. It satisfies $\forall e \in \edges \backslash \{\att^1 \cup\{e^\prime\}\}, \ \sigma^{2^\prime}_e = \sigma^{2^*}_e$, $\sigma^{2^\prime}_{e^\prime} = \sigma^{2^*}_{e^\prime} - \varepsilon$, and $\sum_{e \in \att^1} (\sigma^{2^\prime}_e - \sigma^{2^*}_e) = \varepsilon$.

%This equation implies that it is possible to allocate $\varepsilon$ to components in $\att^1$ (which is nonempty) in a way that each attack probability is not above $\frac{1}{\semm}$.

\item[--] Now, consider $\Def^\prime \in \argmax_{\Def \in \overline{\mathcal{A}_1}} U_1(\Def,\sigma^{2^\prime})$. The goal of this step is to show (by contradiction) that $e^\prime \in \mathcal{C}_{\Def^\prime}$. First, we derive the following calculations:
%
%
%Then we show (by contradiction) that necessarily, $e^\prime \in \mathcal{C}_{\Def^\prime}$.
%
%\begin{itemize}
%\item[-] Case 1: If $e^\prime \in \mathcal{C}_{\Def^\prime}$, then necessarily, $\att^1 \in \mathcal{C}_{\Def^\prime}$ and the optimal value is the same.
%Indeed:
\begin{align}
&U_1(\Def^\prime,\sigma^{2^\prime}) \overset{\eqref{payoff1}}{=} (\sigma^{2^*}_{e^\prime} - \varepsilon)\valdet{\Def^\prime}{e^\prime} +\sum_{\mathclap{e \in \edges\backslash\{\att^1\cup\{e^\prime\}\}}}\sigma^{2^*}_e  \valdet{\Def^\prime}{e} +\sum_{e \in \att^1}\underset{\geq 0}{\underbrace{(\sigma^{2^\prime}_e - \sigma^{2^*}_e)}}\underset{\leq 1}{\underbrace{\valdet{\Def^\prime}{e}}} + \sum_{e \in \att^1}\sigma^{2^*}_e \valdet{\Def^\prime}{e}\nonumber\\
& \leq \sum_{e \in \edges}\sigma^{2^*}_e  \valdet{\Def^\prime}{e} +\sum_{e \in \att^1}(\sigma^{2^\prime}_e - \sigma^{2^*}_e)  -\varepsilon\valdet{\Def^\prime}{e^\prime}  \overset{\eqref{payoff1}}{=} U_1(\Def^\prime,\sigma^{2^*}) + \varepsilon(1 - \valdet{\Def^\prime}{e^\prime}).\label{Good epsilon}
\end{align}

Thus, if $e^\prime \notin \mathcal{C}_{\Def^\prime}$, then $U_1(\Def^\prime,\sigma^{2^\prime}) \leq U_1(\Def^\prime,\sigma^{2^*})+ \varepsilon$. Let  $i^* \in \nodes \backslash\Def^\prime \ | \  e^\prime \in \mathcal{C}_{i^*}$. Then, we have:
\vspace{-0.0cm}
\begin{align}
\forall i \in \Def^\prime, \ U_1(\Def^*,\sigma^{2^*})  \geq U_1(\{i^*\} \cup \Def^\prime\backslash\{i\},\sigma^{2^*}) \overset{\eqref{payoff1},\eqref{monotonicity_detection}}{\geq}\frac{1}{\semm} + \varepsilon + U_1(\Def^\prime\backslash\{i\},\sigma^{2^*}).\label{Almost...}
\end{align}
%
%
%\begin{align}
%&\forall i \in \Def^\prime, \ U_1(\Def^*,\sigma^{2^*}) = \max_{\Def \in \overline{\mathcal{A}_1}}U_1(\Def,\sigma^{2^*}) \geq U_1(\{i^*\} \cup \Def^\prime\backslash\{i\},\sigma^{2^*})  \overset{\eqref{payoff1}}{=} \sum_{e \in \edges}\sigma^{2^*}_e \valdet{\{i^*\} \cup \Def^\prime\backslash\{i\}}{e}\nonumber\\
%& = \sigma^{2^*}_{e^\prime} \underset{=1}{\underbrace{\valdet{\{i^*\} \cup \Def^\prime\backslash\{i\}}{e^\prime}}} + \sum_{e \in \edges\backslash\{e^\prime\}}\sigma^{2^*}_e \valdet{\{i^*\} \cup \Def^\prime\backslash\{i\}}{e}  \overset{\eqref{monotonicity_detection}}{\geq} \frac{1}{\semm} + \varepsilon +  \sum_{e \in \edges\backslash\{e^\prime\}}\sigma^{2^*}_e \valdet{\Def^\prime\backslash\{i\}}{e}\nonumber\\
%& = \frac{1}{\semm} + \varepsilon +  \sigma^{2^*}_{e^\prime}\underset{=0}{\underbrace{\valdet{\Def^\prime\backslash\{i\}}{e^\prime}}}+\sum_{e \in \edges\backslash\{e^\prime\}}\sigma^{2^*}_e \valdet{\Def^\prime\backslash\{i\}}{e}  \overset{\eqref{payoff1}}{=} \frac{1}{\semm} + \varepsilon + U_1(\Def^\prime\backslash\{i\},\sigma^{2^*}).\label{Almost...}
%\end{align}

%Thus, we have:
% and construct the sensor placement $(\Def^\prime \backslash\{i_k\})\cup\{i^*\}$, $\forall k \in \llbracket 1,b_1\rrbracket$. Then we have:
%\begin{align*}
%\forall k \in \llbracket 1,b_1\rrbracket, \ U_1(\Def^*,\sigma^{2^*}) \geq U_1((\Def^\prime \backslash\{i_k\})\cup\{i^*\},\sigma^{2^*}) \geq \frac{1}{\semm} + \varepsilon + U_1(\Def^\prime\backslash\{i_k\},\sigma^{2^*}).
%\end{align*}
%
%Thus, we have:
%\begin{align*}
%\sum_{i \in \Def^\prime} U_1(\Def^\prime\backslash\{i\},\sigma^{2^*})\leq b_1U_1(\Def^*,\sigma^{2^*}) - \frac{b_1}{\semm} - b_1 \varepsilon
%\end{align*}
\vspace{-0.0cm}

Next, we can derive the following calculations:
%
%Then:
\vspace{-0.0cm}
\begin{align}
&U_1(\Def^\prime,\sigma^{2^*})\overset{\eqref{payoff1},\eqref{nice_detection_inequality}}{\leq} \frac{1}{b_1-1}\sum_{i \in \Def^\prime}U_1(\Def^\prime\backslash\{i\},\sigma^{2^*}) \overset{\eqref{Almost...},\eqref{One of the very last}}{\leq} U_1(\Def^*,\sigma^{2^*}) - \frac{b_1}{b_1-1}\varepsilon. \label{Out of ideas}
\end{align}
%\end{itemize}

\vspace{-0.0cm}

Combining everything together, we obtain the following contradiction:
\vspace{-0.0cm}
\begin{align*}
\max_{\Def \in \overline{\mathcal{A}_1}}U_1(\Def,\sigma^{2^\prime}) \overset{\eqref{Good epsilon},\eqref{Out of ideas}}{\leq} U_1(\Def^*,\sigma^{2^*}) - \frac{1}{b_1-1}\varepsilon  <  U_1(\Def^*,\sigma^{2^*}) =  \min_{\sigma^2 \in \Delta(\edges)} \max_{\Def \in \overline{\mathcal{A}_1}}U_1(\Def,\sigma^{2}).
\end{align*}
%\begin{align*}
%\max_{\Def \in \overline{\mathcal{A}_1}}U_1(\Def,\sigma^{2^\prime}) &= U_1(\Def^\prime,\sigma^{2^\prime}) \overset{\eqref{Good epsilon}}{\leq} U_1(\Def^\prime,\sigma^{2^*}) + \varepsilon(1 - \underset{=0}{\underbrace{\valdet{\Def^\prime}{e^\prime}}}) \overset{\eqref{Out of ideas}}{\leq} U_1(\Def^*,\sigma^{2^*}) - \frac{b_1}{b_1-1}\varepsilon + \varepsilon \\
%&= U_1(\Def^*,\sigma^{2^*}) - \frac{1}{b_1-1}\varepsilon  <  U_1(\Def^*,\sigma^{2^*}) = \max_{\Def \in \overline{\mathcal{A}_1}}U_1(\Def,\sigma^{2^*}) = \min_{\sigma^2 \in \Delta(\edges)} \max_{\Def \in \overline{\mathcal{A}_1}}U_1(\Def,\sigma^{2}).
%\end{align*}
%Which is a contradiction since $\sigma^{2^*}$ is an optimal solution of \lptp.

\vspace{-0.0cm}

\item[--] Therefore, we showed that $e^\prime \in \mathcal{C}_{\Def^\prime}$. This implies that $\varepsilon(1-\valdet{\Def^\prime}{e^\prime}) =0$, and we obtain: $\max_{\Def \in \overline{\mathcal{A}_1}}U_1(\Def,\sigma^{2^\prime})  \overset{\eqref{Good epsilon}}{\leq} U_1(\Def^\prime,\sigma^{2^*})  \leq  \max_{\Def \in \overline{\mathcal{A}_1}} U_1(\Def,\sigma^{2^*})  = \min_{\sigma^2 \in \Delta(\edges)} \max_{\Def \in \overline{\mathcal{A}_1}} U_1(\Def,\sigma^2).$
%\begin{align*}
%\max_{\Def \in \overline{\mathcal{A}_1}}U_1(\Def,\sigma^{2^\prime}) = U_1(\Def^\prime,\sigma^{2^\prime}) \overset{\eqref{Good epsilon}}{\leq} U_1(\Def^\prime,\sigma^{2^*})  \leq \max_{\Def \in \overline{\mathcal{A}_1}} U_1(\Def,\sigma^{2^*}) = \min_{\sigma^2 \in \Delta(\edges)} \max_{\Def \in \overline{\mathcal{A}_1}} U_1(\Def,\sigma^2).
%\end{align*}
%\begin{align*}
%U_1(\Def^\prime,\sigma^{2^\prime}) &\overset{\eqref{payoff1}}{=} \sigma^{2^\prime}_{e^\prime} \underset{=1}{\underbrace{\valdet{\Def^\prime}{e^\prime}}} + \sum_{e \in \att^1}\sigma^{2^\prime}_e \valdet{\Def^\prime}{e} + \sum_{e \in \edges \backslash\{\att^1 \cup \{e^\prime\}\}}\sigma^{2^\prime}_e \valdet{\Def^\prime}{e}\\
%& = \sigma^{2^*}_{e^\prime} - \varepsilon +\sum_{e \in \att^1}(\sigma^{2^\prime}_e - \sigma^{2^*}_e+ \sigma^{2^*}_e)\valdet{\Def^\prime}{e} + \sum_{e \in \edges\backslash\{\att^1\cup\{e^\prime\}\}}\sigma^{2^\prime}_e  \valdet{\Def^\prime}{e} \\
%& = \sigma^{2^*}_{e^\prime} - \varepsilon +\sum_{e \in \att^1}(\sigma^{2^\prime}_e - \sigma^{2^*}_e)\underset{\leq 1}{\underbrace{\valdet{\Def^\prime}{e}}} + \sum_{e \in \att^1}\sigma^{2^*}_e \valdet{\Def^\prime}{e} + \sum_{e \in \edges\backslash\{\att^1\cup\{e^\prime\}\}}\sigma^{2^*}_e  \valdet{\Def^\prime}{e} \\
%& \leq \sigma^{2^*}_{e^\prime}\underset{=1}{\underbrace{\valdet{\Def^\prime}{e^\prime}}} - \varepsilon + \varepsilon + \sum_{e \in \edges\backslash\{e^\prime\}}\sigma^{2^*}_e  \valdet{\Def^\prime}{e} \overset{\eqref{payoff1}}{=} U_1(\Def^\prime,\sigma^{2^*})  \leq \max_{\Def \in \overline{\mathcal{A}_1}} U_1(\Def,\sigma^{2^*}).
%\end{align*}
%Thus, $\max_{\Def \in \overline{\mathcal{A}_1}} U_1(\Def,\sigma^{2^\prime}) \leq \max_{\Def \in \overline{\mathcal{A}_1}} U_1(\Def,\sigma^{2^*}) = \min_{\sigma^2 \in \Delta(\overline{\mathcal{A}_2})} \max_{\Def \in \overline{\mathcal{A}_1}} U_1(\Def,\sigma^2)$. 
Thus, $\sigma^{2^\prime}$ is also an optimal solution of \lptp. Therefore, if  an optimal solution of \lptp is such that at least one component is targeted with probability more than $\frac{1}{\semm}$, we can construct another optimal solution of \lptb with one less component targeted with probability more than $\frac{1}{\semm}$. We can then repeat this process until all attack probabilities are no more than $\frac{1}{\semm}$. %Therefore, given $b_1 < \smsc$, and $b_2 = 1$, there exists an optimal solution of \lptp, denoted $\widetilde{\sigma}^{2} \in \Delta(\mathcal{A}_2)$, that satisfies $\rho_{\widetilde{\sigma}^{2}}(e) \leq \frac{1}{\semm}$, $\forall e \in \edges$. 
\end{enumitemize}

\item Given $b_1 < \smsc$, let $z^*(b_2)$ denote the optimal value of \lptb for any $b_2 <\semm$. Now, consider $b_2 < \semm$, and let $\sigma^{2^*} \in \Delta(\mathcal{A}_2)$ be an optimal solution of \lptp. Since $\sum_{e \in \edges}\frac{\rho_{\sigma^{2^*}(e)}}{b_2} =1$, we can construct an attack strategy $\sigma^{2^\prime} \in \Delta(\edges)$  such that $\forall e \in \edges, \ \sigma^{2^\prime}_e = \rho_{\sigma^{2^\prime}}(e) =  \frac{\rho_{\sigma^{2^*}}(e)}{b_2}$. Then, the additivity of $\detect$ gives us: $z^*(b_2) = \max_{\Def \in \overline{\mathcal{A}_1}} \sum_{e \in \edges} \valdet{\Def}{e}\rho_{\sigma^{2^*}}(e) = b_2\max_{\Def \in \overline{\mathcal{A}_1}}U_1(\Def,\sigma^{2^\prime}) \geq b_2 z^*(1).$ 
%\begin{align}
%z^*(b_2) & \overset{\eqref{payoff1},\eqref{rho_sigma2},\eqref{detection_disruptions}}{=}\max_{\Def \in \overline{\mathcal{A}_1}} \sum_{e \in \edges} \valdet{\Def}{e}\rho_{\sigma^{2^*}}(e) \overset{\eqref{payoff1}}{=}b_2\max_{\Def \in \overline{\mathcal{A}_1}}U_1(\Def,\sigma^{2^\prime}) \geq b_2 z^*(1). \label{ONE}
%\end{align}

Now, consider $\widetilde{\sigma}^2 \in \Delta(\edges)$ which is an optimal solution of \lptp (where the number of attack resources is 1) with the additional property that $\forall e \in \edges, \ \rho_{\widetilde{\sigma}^2}(e) \leq \frac{1}{\semm}$. Then, given $b_2 <\semm$, since $\forall e \in \edges, \ b_2\rho_{\widetilde{\sigma}^2}(e) \leq 1$ and $\sum_{e \in \edges} b_2\rho_{\widetilde{\sigma}^2}(e) = b_2$, there exists a probability distribution $\widehat{\sigma}^{2} \in \Delta(\mathcal{A}_2)$, that satisfies $\rho_{\widehat{\sigma}^{2}}(e) = b_2  \rho_{\widetilde{\sigma}^2}(e), \ \forall e \in \edges$ (Lemma~\ref{Big Support}). Then, by additivity of $\detect$,  we obtain: $z^*(1) =\max_{\Def \in \overline{\mathcal{A}_1}} \sum_{e \in \edges} \valdet{\Def}{e}\rho_{\widetilde{\sigma}^{2}}(e) = \max_{\Def \in \overline{\mathcal{A}_1}}\frac{1}{b_2} \sum_{e \in \edges} \valdet{\Def}{e}\rho_{\widehat{\sigma}^{2}}(e) \geq \frac{1}{b_2} z^*(b_2).$
%
%Similarly, 
%\begin{align}
%z^*(1) &= \max_{\Def \in \overline{\mathcal{A}_1}}U_1(\Def,\widetilde{\sigma}^{2}) \overset{\eqref{payoff1}}{=}\max_{\Def \in \overline{\mathcal{A}_1}} \sum_{e \in \edges} \valdet{\Def}{e}\rho_{\widetilde{\sigma}^{2}}(e) = \max_{\Def \in \overline{\mathcal{A}_1}}\frac{1}{b_2} \sum_{e \in \edges} \valdet{\Def}{e}\rho_{\widehat{\sigma}^{2}}(e) \nonumber\\
%&\overset{\eqref{payoff1},\eqref{rho_sigma2},\eqref{detection_disruptions}}{=}\frac{1}{b_2}\max_{\Def \in \overline{\mathcal{A}_1}}U_1(\Def,\widehat{\sigma}^{2}) \geq \frac{1}{b_2} \min_{\sigma^2 \in \Delta(\overline{\mathcal{A}_2})}\max_{\Def \in \overline{\mathcal{A}_1}}U_1(\Def,\sigma^{2}) = \frac{1}{b_2} z^*(b_2). \label{TWO}
%\end{align}

Thus, $\forall b_2 < \semm, \ z^*(b_2) = b_2z^*(1).$ Therefore, we conclude that $\forall \sigma^* \in \nash(b_1,b_2), \ r(\sigma^*) \overset{\eqref{res2}}{=} \frac{U_1(\sigma^*)}{b_2} = \frac{z^*(b_2)}{b_2} = z^*(1) \eqqcolon r^*_{b_1},$ which does not depend on $b_2$.\hfill
\Halmos
%
%\vspace{-0.3cm}
%\hfill 
%\Halmos
%\endproof
\end{enumerate}
%\vspace{-0.3cm}

\endproof



\begin{proposition}\label{Identical strategies}
Given \defender's number of detectors $b_1 < \smsc$, inspection strategies in equilibrium of the game $\Gamma(b_1,1)$ are also inspection strategies in equilibrium of any game $\Gamma(b_1,b_2)$ with $b_2 < \semm$.
\end{proposition}
\proof{Proof of Proposition~\ref{Identical strategies}.}

Given \defender's resources $b_1 < \smsc$, let $\sigma^{1^*} \in \Delta(\overline{\mathcal{A}_1})$ be an inspection strategy in equilibrium of the game $\Gamma(b_1,1)$. From Proposition~\ref{all_resources}, we know that $\sigma^{1^*}$ is an optimal solution of \lpob for $b_2 = 1$. Now, consider $b_2 < \semm$. We can derive the following inequality:
%$\sigma^{1^*},\sigma^{2^*}) \in \nash(b_1,1)$. From Proposition~\ref{all_resources}, we know that $\sigma^{1^*}$ is an optimal solution of \lpo.
\begin{align*}
\forall \att \in \overline{\mathcal{A}_2}, \ U_1(\sigma^{1^*},\att) \overset{\eqref{detection_disruptions}}{=} \sum_{e \in \att}U_1(\sigma^{1^*},e) \geq  \sum_{e \in \att} \underset{= r^*_{b_1}}{\underbrace{\min_{e^\prime \in \edges} U_1(\sigma^{1^*},e^\prime)}} =  b_2r^*_{b_1}\overset{\eqref{General_Formulation}}{=}\max_{\sigma^{1} \in \Delta(\overline{\mathcal{A}_1})} \min_{\att^\prime \in \overline{\mathcal{A}_2}}U_1(\sigma^{1},\att^\prime).
\end{align*}
Since this inequality is valid for any $\att \in \overline{\mathcal{A}_2}$, we deduce that $\min_{\att \in \overline{\mathcal{A}_2}} U_1(\sigma^{1^*},\att) \geq \max_{\sigma^{1} \in \Delta(\overline{\mathcal{A}_1})} \min_{\att \in \overline{\mathcal{A}_2}}U_1(\sigma^{1},\att)$. Therefore, $\sigma^{1^*}$ is an optimal solution of \lpob (when the number of attack resources is $b_2$), and is an inspection strategy in equilibrium of the game $\Gamma(b_1,b_2)$.
%\begin{align*}
%\min_{\att \in \overline{\mathcal{A}_2}} U_1(\sigma^{1^*},\att)  \geq b_2r^*_{b_1}
%\end{align*}
%\vspace{-0.3cm}
\hfill
\Halmos
\endproof







%For scenario \textit{(b)}, monitoring sets are constructed through simulations using a hydraulic network solver \citep{epanet:2002} that tracks the advection and reaction dynamics from a contaminant intrusion event \citep{ostfeld2008battle,doi:10.1021/es3014024}.  Fig.~\ref{fig:net1_layout} illustrates the region of a network from where the signal resulting from a pipe break (left) and a contaminant intrusion (right) can be detected. Note that in both scenarios, the network topology plays a key role in the propagation of the signal resulting from a failure event. In particular, the signal generated from a break event propagates in all directions of the network, whereas the signal from a contaminant intrusion heavily depends on the direction of the flow.

%\begin{figure}[htbp]
%        \centering
%        \begin{subfigure}[b]{0.45\textwidth} \centering
%               \includegraphics[trim = 40mm 70mm 10mm 70mm, clip,scale = 0.4]{or_fig1b.pdf}       
%		\caption{Pipeline break event}    \label{fig:net1_burst} 
%        \end{subfigure}
%        ~ 
%        \begin{subfigure}[b]{0.45\textwidth} \centering
%               \includegraphics[trim = 40mm 70mm 10mm 70mm, clip,scale = 0.4]{or_fig1q.pdf}       
%		\caption{Contaminant intrusion event}   \label{fig:net1_contamination}  
%        \end{subfigure}
%       \caption{Sensing model for the Apulian water network. The colored regions indicate the set of network locations from where the signal generated by the failure events can be detected.}   \label{fig:net1_layout}
%\end{figure}

%Now, we consider the problem \ECOP for scenario \textit{(a)}, where the operator faces an adversary with $b_2 = 2$ number of attack resources (i.e., up to two pipes can be targeted), and wants to ensure an expected detection rate of $\alpha = 0.75$. Due to the small size of the problem, we can directly solve  the two linear programs \lpo and \lpt to compute the NE of $\Gamma(b_1,b_2)$, and obtain  the expected detection rate in any equilibrium for each $b_1 \in \mathbb{N}$.  Fig.~\ref{fig:net1_15} shows the expected detection rate in equilibrium, for each $b_1$. From this figure, we can conclude that the optimal value of (\hyperlink{(P)}{$\mathcal{P}$}) is $b_1^\dag = 3$, i.e., with  $3$ sensors, \defender is capable of detecting $\frac{5}{6} \geq \alpha$ of the failure events in equilibrium. As mentioned in Section~\ref{sec:Formal problem}, this brute-force approach  does not extend to larger networks, as it requires solving large \lpo and \lpt for each $b_1 \in \mathbb{N}$ and checking if the constraint on the expected detection rate in equilibrium \eqref{all_NE} is met. However, it is instructive to benchmark our solution approach with the brute-force approach for this small-sized network.
%
%
%\pgfplotsset{figureStyle/.style={%
%  %width=0.57\linewidth,
% % thick,
%  font=\small,
%  xmin=0,
%  xmax=4,
%  ymin=0,
%  ymax=1,
%  xtick={0,1,2,3,4},
%% ytick={0,0.2, alpha},
%  legend pos=south east,
%	legend cell align={left},
%  legend style={draw=none, font = \tiny},
%%  legend style={draw=none, legend columns=-1},
%}}
%
%\begin{figure}[htbp]
%\centering
%
%\begin{tikzpicture}
%\begin{axis}[
%  figureStyle,
%  grid=major, % Display a grid
%  grid style={dashed,gray!30}, % Set the style
%  xlabel=$b_1$ ,
%  ylabel=$\sdet{*}$,
%]
%
%\addplot[dashdotted, color = red,very thick] table[x=b1, y=ub, col sep=comma, comment chars={\%}] {Evaluation_2.csv};
%\addplot[solid, color = black,very thick,mark=*] table[x=b1, y=ne, col sep=comma, comment chars={\%}] {Evaluation_2.csv};
% \addplot[dashed, color = blue,very thick] table[x=b1, y=lb, col sep=comma, comment chars={\%}] {Evaluation_2.csv};
%\legend{Upper Bound, NE, Lower Bound}
%
% \addplot[dotted, color = green!0!black,thick] table[x=b1, y=alpha, col sep=comma, comment chars={\%}] {Evaluation_2.csv};
% 
%
% 
%\end{axis}
% \node at (-0.3,4.27) {$\alpha$};
%\end{tikzpicture}
%\\
%%\footnotesize (a) Water network 1 %&
%%\hspace{0.1in}
%\caption{Detection rate for the Apulian network with respect to the number of sensing resources $b_1$.}    \label{fig:net1_15} 
%
%\end{figure}
%--------------------------------- Figure -------------------------------



%Let us apply our solution approach to obtain an approximate solution of \ECOP. First, using the monitoring sets $\set{i}, \ i \in \nodes$, we solve (\hyperlink{(MSC)}{$\mathcal{I}_{\text{MSC}}$}) to compute an MSC $\Def^{min} \in \msc$. The results show that for scenario \textit{(a)}, the size of $\Def^{min}$ is $\smsc  = 4$. Then, from Thm.~\ref{bounds_game},  we know that, for any $b_1 < \smsc$, the expected detection rate in any equilibrium of the game $\Gamma(b_1,b_2)$ is constant and lower bounded by $\frac{b_1}{\smsc}$. Thus, with $b_1^\prime=\lceil \alpha \smsc \rceil = 3$ sensors, the expected detection rate in any equilibrium is at least $\alpha$. 
%
%Secondly, by solving (\hyperlink{(MSP)}{$\mathcal{I}_{\text{MSP}}$}), we compute an MSP $\att^{max} \in \emm$ which is of size $\semm = 3$. Then, from Proposition~\ref{Prop_interim}, we know that the optimality gap associated with $b_1^\prime$ is given by $\lceil \alpha \smsc\rceil - \lceil \alpha \semm \rceil = \lceil 3\rceil - \lceil 2.25 \rceil = 0$. Therefore, by solving (\hyperlink{(MSC)}{$\mathcal{I}_{\text{MSC}}$}) and (\hyperlink{(MSP)}{$\mathcal{I}_{\text{MSP}}$}), we can estimate the number of sensing resources to ensure that the equilibrium constraints in \ECOP are satisfied; furthermore, we can verify that this number is optimal for this scenario, i.e., $b_1^\prime = b_1^\dag = 3$.
%
%Thirdly, given $b_1^\prime=3$ and $b_2 =2$, we can use $\Def^{min}$ and $\att^{max}$ to construct an approximate NE. Using Lemma~\ref{algebra1}, we construct the strategy profile ${\sigma} = (\sold{\Def^{min}}{b_1^\prime}{},\sola{\att^{max}}{b_2}{})$. As shown in Theorem~\ref{MSC-MSP-eNE}, this strategy profile is an $\epsilon-$NE, and provides each player a payoff that is $\epsilon-$close to their equilibrium payoff, with $\epsilon=  b_1^\prime b_2\left( \frac{1}{\max\{b_1^\prime,\semm\}} - \frac{1}{\smsc}\right) = \frac{1}{2}$. Indeed, by solving \lpo and \lpt, we can deduce that \defender and \attacker's equilibrium payoffs in the game $\Gamma(b_1^\prime,b_2)$ are $\frac{5}{3}$ and $\frac{1}{3}$ respectively, while the strategy profile $\sigma$  we constructed provides the players with the respective expected payoffs $\frac{3}{2}$ and $\frac{1}{2}$. One can easily check that $\sigma$ gives each player a payoff that is $\frac{1}{6} \ (\leq \epsilon)$ close to their equilibrium payoff. %\tb{In Section~\ref{conclusions}, we discuss how $\sigma$ can be iteratively improved and become a NE.}
%
%
%
%Finally, we give an upper bound on the loss in detection performance by choosing our sensing strategy $\sold{\Def^{min}}{b_1^\prime}{}$ instead of choosing an equilibrium strategy for \defender.
%%Indeed, we showed in Thm.~\ref{Prop_interim} that an equilibrium sensing strategy maximinimizes the expected detection rate. 
%From Theorem~\ref{MSC-MSP-eNE}, we know that $\sold{\Def^{min}}{b_1^\prime}{}$ detects at least $\frac{3}{4}$ of the failures regardless of \attacker's strategy, while in equilibrium $\frac{5}{6}$ of the failures are detected (Fig.~\ref{fig:net1_15}). Thus,  the relative loss in detection performance is $10\,\%$. This exact calculation is possible only because, for this network, we can solve \lpo and \lpt and compute the value of the expected detection rate in equilibrium. In contrast,  Theorem~\ref{MSC-MSP-eNE} provides  an upper bound on the  loss in detection performance \emph{without} solving \lpo and \lpt, but instead by computing $\smsc$ and $\semm$ from (\hyperlink{(MSC)}{$\mathcal{I}_{\text{MSC}}$}) and  (\hyperlink{(MSP)}{$\mathcal{I}_{\text{MSP}}$}). This upper bound is given  by $1 - \frac{\max\{b_1^\prime,\semm\}}{\smsc} = 25\,\%$. To summarize, for scenario \textit{(a)}, our solution approach provides the optimum number of sensing resources required to achieve the target detection rate $\alpha$, and gives a sensing strategy that only faces 10\,\% of loss in detection performance with respect to an optimal strategy.
%
%
%
%
%
%
%We now consider the problem \ECOP using the monitoring sets computed for the contaminant intrusion scenario \textit{(b)} on the benchmark network. In this scenario, we notice that the optimal solutions $\Def^{min}$ of (\hyperlink{(MSC)}{$\mathcal{I}_{\text{MSC}}$}) and $\att^{max}$ of (\hyperlink{(MSP)}{$\mathcal{I}_{\text{MSP}}$}) satisfy $|\Def^{min}| = \smsc = \semm = |\att^{max}| = 4$. Therefore, from Proposition~\ref{Prop_interim}, we know that, given $\alpha \in [0,1]$ and $b_2 <\semm$, $\lceil \alpha \smsc \rceil$, $(\sold{\Def^{min}}{\lceil \alpha \smsc \rceil}{},\sola{\att^{max}}{b_2}{})$ is an optimal solution of the network monitoring problem. In particular, for this scenario, our solution approach provides the optimal number of sensing resources, and their allocation in equilibrium.

%\color{black}

%, while for the contamination scenario $\smsc  = \semm = 4$,
%
%In the contaminant intrusion scenario, $\smsc =\semm$, thus our approximate NE gives the optimal solution of \ECOP (Prop.~\ref{Cor2}). %In case $\smsc = \semm$, the upper and lower bounds will coincide and give the actual value of the payoffs for the two players. %Additionally, as expected, as the budget of the defender increases, it's payoff increases and the attacker's payoff decreases.
%In summary, using Theorem \ref{bounds_game} we can compute the sensing budget and the strategy profile that guarantee the desired detection rate, $\sdet{*}$. %Furthermore, the strategy profile is supported over an MSC such that the node sensing probability of each node in the MSC is $\frac{b_1}{\smsc}$. 
%The MSC problem and the $\smsc$ can be solved to optimality within seconds even for very large networks using modern optimization solvers, as we demonstrate in the next section.



%% Table generated by Excel2LaTeX from sheet 'Sheet1'
%\begin{table}[htbp]\footnotesize
%  \centering
%  \caption{Payoff bounds for the Apulian network.}
%\tabcolsep=0.18cm
%\renewcommand{\arraystretch}{1.3} 
%    \begin{tabular}{|c|c|c|}
%\hline
%%\rowcolor{gray!30}   
%\boldmath{$b_1,b_2$}& \boldmath{$\underline{u_1},u_1,\overline{u_1}$}& \boldmath{$\underline{u_2},u_2,\overline{u_2}$} \\
%\hline
%    1,1   & $(0.250,0.286,0.333)$ & $(0.667,0.714,0.750)$  \\
%    1,2   & $(0.500,0.571,0.667)$ & $(1.333,1.429,1.500)$  \\
%    2,1   & $(0.500,0.571,0.667)$ &$(0.333,0.429,0.500) $ \\
%    2,2   & $(1.000,1.143,1.333)$ &$(0.667,0.857,1.000) $ \\
%    3,1   & $(0.750,0.833,1.000)$ &$ (0.000,0.167,0.250)$  \\
%    3,2   & $(1.500,1.667,2.000)$ & $(0.000,0.333,0.500)$  \\
%\hline
%    \end{tabular}%
% \label{tab:3}
%\end{table}%







%\textit{Monitoring problem.} %For presentation purposes, in the remaining of the paper we focus on pipe burst events. We assume that the origin of the event occurs in the center of each pipe and approximate the detectability of an event based on the length of the shortest path from the origin to the node, i.e. before it dissipates in the system \citep{deshpande2013optimal,sensors:autom}. The typical distance for detection in urban water networks is $1000[m]$ \citep{visenti}. 
%We formulate the attacker-defender game, $\Gamma :=\langle\{\defender,\attacker\},(\mathcal{A}_1,\mathcal{A}_2),(u_1,u_2)\rangle$, considering that the defender and the attacker have an available budget of $b_1 = 2, b_2 = 2$, i.e. each time the defender can sense any two nodes and the attacker -- attack any two links simultaneously. In this example,  there are $|\mathcal{A}_1| = \displaystyle \sum_{k=0}^2\dbinom{23}{k}=277$ for \defender and $|\mathcal{A}_2| = \displaystyle \sum_{k=0}^3\dbinom{43}{k}=596$ actions for \attacker. 



\section{Solution Refinement}\label{Sec:Important}

%\subsection{Degenerate Example}
%\rem{As stated in Section~\ref{conclusions}, we can construct a peculiar example for which the performance guarantees provided by our solution approach can be arbitrarily bad. 
%\begin{example}
%Consider a graph $G = (N,A)$, where $N = \llbracket 1,n\rrbracket$, and $A = \{(i,j) \in N^2 \ | \ i \neq j\}\backslash\{(1,2)\}$. Let the sensing model be such that $\nodes = A$, $\edges = N$, and $\forall i = (u,v) \in A, \ \set{i} = \{u,v\}$. Then, in this case, an MSC is a minimum edge cover of $G$, which is of size $\lceil \frac{n}{2}\rceil$, and an MSP is a maximum independent set of $G$, which is only of size 2. Let $b_2 = 1$ and $\alpha \in [0,1]$. Then, as the size of the graph $n$ increases, the upper bound on the optimality gap of our solution given in Proposition~\ref{Prop_interim} is equal to $\lceil \alpha \lceil \frac{n}{2}\rceil \rceil - \lceil 2\alpha \rceil \underset{n \to +\infty}{\longrightarrow} +\infty $. Furthermore, for $b_1 = b_2 = 1$, the relative loss of performance of our MSC-based sensing strategy, derived from Theorem~\ref{MSC-MSP-eNE},  is equal to $1 - \frac{2}{\lceil n/2\rceil} \underset{n \to +\infty}{\longrightarrow} 100\,\%$.
%%
%%Give the formulas..
%\hfill $\triangle$
%\end{example}}




In order to refine our MSC/MSP-based solution and improve its performance guarantees, we presented in Section~\ref{conclusions} a column generation algorithm. Given $b_1 < \smsc$, we showed in Proposition~\ref{Identical strategies} that inspection strategies in equilibrium of any game $\Gamma(b_1,b_2)$ with $b_2 < \semm$ can be obtained by solving \lpob for $b_2 = 1$.  
%, which can be formulated as follows:
%\begin{align*}
%\begin{array}{clc}
%\text{maximize} & \displaystyle z&\\
%\text{subject to} & z \leq \displaystyle\sum_{\Def \in \overline{\mathcal{A}_1}}\valdet{\Def}{e}\sigma^{1}_{\Def}, & \forall e \in \edges\\
%&  \displaystyle\sum_{\Def \in \overline{\mathcal{A}_1}} \sigma^{1}_\Def = 1&\\
%& \sigma^1_{\Def} \geq 0, & \forall \Def \in \overline{\mathcal{A}_1}.
%\end{array}
%\end{align*}
Given a subset $\mathcal{I} \subseteq \overline{\mathcal{A}_1}$ of indices, the master problem of the column generation algorithm applied to \lpob is given by:\hypertarget{Pcg}{}
\begin{align}
\begin{array}{cclc}
(P_{\text{CG}}): \quad & \text{maximize} & \displaystyle z&\mcr
&\text{subject to} & z \leq \displaystyle\sum_{\Def \in\mathcal{I}}\valdet{\Def}{e}\sigma^{1}_{\Def}, & \forall e \in \edges\\
&&  \displaystyle\sum_{\Def \in \mathcal{I}} \sigma^{1}_\Def = 1&\\
&& \sigma^1_{\Def} \geq 0, & \forall \Def \in \mathcal{I}.
\end{array} \label{Master Problem}
\end{align}

Let $\sigma^{1^*}, \ z^*$ (resp. $\rho_e^*, \ (e \in \edges)$, $ z^{\prime^*}$) denote the optimal primal (resp. dual) solution of \pcg. The reduced cost associated with each $\Def \in \overline{\mathcal{A}_1}$ is given by $\sum_{e \in \edges}\valdet{\Def}{e}\rho_e^* - z^{\prime^*}$. Therefore, the detector positioning with the highest reduced cost can be obtained by solving a maximum weighted covering set problem, which can be formulated as the following integer program:\hypertarget{Dcg}{}
%(note that the variable $z$ is always 
\begin{align*}
\begin{array}{cclc}
(D_{\text{CG}}): \quad &\text{maximize} & \displaystyle \sum_{e \in \edges} \rho_e^* y_e&\\
&\text{subject to} & y_e \leq \displaystyle \sum_{\{i \in \nodes \, | \, e \in \set{i}\}} x_i, & \forall e \in \edges\\
&&  \displaystyle\sum_{i \in \nodes} x_i = b_1&\\
&& x_i, y_e \in \{0,1\}, & \forall i \in \nodes, \ \forall e \in \edges.
\end{array}
%\label{Subproblem}
\end{align*}

If the optimal value of \dcg is no more than $z^{\prime^*}$, then this proves that the optimal primal solution of \pcg, $(\sigma^{1^*}, z^*)$,  is also an optimal solution of \lpob. However, if the optimal value of \dcg is more than $z^{\prime^*}$, then we add the detector positioning corresponding to the optimal solution of  \dcg to the set of indices $\mathcal{I}$.  \pcg is then solved with the new set of indices $\mathcal{I}$.

This algorithm can be initiated by considering $\mathcal{I} = \supp(\sold{\Def^{min}}{b_1}{})$, and can be repeated until an optimal solution of \lpob is found. In that case, the optimal dual variables $\rho_e^*, \ \forall e \in \edges$, give the probabilities with which each component can be targeted in equilibrium of the game $\Gamma(b_1,1)$. In the proof of Theorem~\ref{Constant}, we show how to reallocate these probabilities to create an attack strategy in equilibrium of $\Gamma(b_1,1)$ with the additional property that each component is not targeted with probability more than $\frac{1}{\semm}$. Then, from Lemma~\ref{Big Support}, given $b_2 < \semm$, we can obtain an attack strategy in equilibrium of $\Gamma(b_1,b_2)$, denoted $\sigma^2 \in \Delta(\overline{\mathcal{A}_2})$, by solving the linear program: $\bs{A}\sigma^2 = b_2\rho^*$, and $\sigma^2\geq\bs{0}_{|\overline{\mathcal{A}_2}|}$. This can be done by considering the following auxiliary problem:
\begin{align*}
\begin{array}{clc}
\text{minimize} & \displaystyle \bs{1}_{|\edges|}^Ts&\mcr
\text{subject to} & \bs{A}\sigma^2 + s = b_2\rho^*  &\mcr
& \sigma^2 \geq \bs{0}_{|\overline{\mathcal{A}_2}|}, \ s \geq \bs{0}_{|\edges|}. & \end{array}
\label{CG Feasible}
\end{align*}

This auxiliary problem can also be solved using column generation, with $(\sigma^2,s) = (\bs{0}_{|\overline{\mathcal{A}_2}|},b_2\rho^*)$ as initial feasible solution. Given the current master problem generated by the column generation algorithm, let $\beta^* \in \mathbb{R}^{|\edges|}$ denote its optimal dual variables. Then, the index ${\att^*}$ with lowest reduced cost is given by $\att^* \in \argmax_{\att \in \overline{\mathcal{A}_2}}\sum_{e \in \att} \beta^*_e$, i.e., $\att^*$ targets the components with highest values $\beta_{e}^*$.
%
%is the attack (of size $b_2$) that 
%
From Lemma~\ref{Big Support}, we know that at optimality, the objective value is 0 (i.e., $s = \bs{0}_{|\edges|}$) and $\sigma^2$ is an equilibrium attack strategy. In summary, given $b_1 < \smsc$ and $b_2 <\semm$, two column generation algorithms can be run in order to obtain an \emph{exact} NE of game $\Gamma(b_1,b_2)$. 


%
%Note that if one is interested in \attacker's strategy in equilibrium, then it can be obtained as follows. By solving \lptb for $b_2 = 1$, one obtains a strategy $\widetilde{\sigma}^{2}$ for \attacker. In the proof of Thm.~\ref{Constant}, we provide a transformation to $\widetilde{\sigma}^{2}$  to make sure that each component is not targeted with probability more than $\frac{1}{\semm}$. 

%
%\section{Proof of Theorem \ref{marg-butt-th}.}
%A general heading for the whole e-companion should be provided here as in the example above this paragraph.
%
%
%To avoid confusion, theorems that we repeat for readers' convenience
%will have the same appearance as when they were mentioned for the first
%time. However, here they should be coded by \verb+repeattheorem+ instead
%of \verb+theorem+ to keep labels/pointers uniquely resolvable. Other predefined theorem-like
%environments work similarly if they need to be repeated in what becomes the \mbox{e-companion.}
%
%
%\begin{repeattheorem}[Theorem 1.]
%%\label{marg-butt-th}
%In a reverse dictionary, $(\mbox{\bi marg}\succ\mbox{\bi butt\/}\; \land\;  
%\mbox{\bi arine}\succ\mbox{\bi er})$.
%Moreover, continuous reading of a compact subset of the dictionary
%attains the minimum of patience at the moment of giving up.
%\end{repeattheorem}
%
%\subsection{Preparatory Material}
%
%\begin{lemma}
%\label{aux-lem1}
%In a reverse dictionary, $\mbox{\bi g}\succ\mbox{\bi t\/}$.
%\end{lemma}
%
%\begin{lemma}
%\label{aux-lem2}
%In a reverse dictionary, $\mbox{\bi e}\succ\mbox{\bi r\/}$.
%\end{lemma}
%
%\proof{Proof of Lemmas \ref{aux-lem1} and \ref{aux-lem2}.} See the alphabet and the tebahpla.\Halmos
%\endproof
%
%\begin{remark} 
%Note that the title of the proof should be keyed
%explicitly in each case. Authors can hardly agree on what would be the
%default proof title, so there is no default. Even \verb+\proof{Proof.}+ should be keyed out. 
%\end{remark}
%
%
%\subsection{Proof of the Main Result}
%
%\proof{Proof of Theorem 1.} The first statement is a conseqence of
%Lemmas~\ref{aux-lem1} and \ref{aux-lem2}. The rest relies on the fact that the continuous
%image of a compact set into the reals is a closed interval, thus having
%a minimum point.\Halmos 
%\endproof

%\begin{figure}[t]
%\begin{center}
%\includegraphics[height=1.5in]{Sample-Figure}
%\caption{Production Possibilities Frontier Again.} \label{ECfrontier}
%\end{center}
%\end{figure}









\section{Case when $b_2 \geq \semm$}\label{Other Case}

As argued in Section~\ref{general}, the network inspection problem \ECOP when $b_2 \geq \semm$ is of limited practical interest. However, for the sake of completeness, we now briefly discuss this case. First, recall from Section~\ref{general} that the optimal value of \ECOP is no more than $\smsc$, since \defender can achieve any target detection rate when she has at least $\smsc$ detectors; thus, we will continue to restrict our attention to the game $\Gamma(b_1,b_2)$ when $b_1 < \smsc$.

To evaluate the equilibrium constraints \eqref{all_NE}-\eqref{one_NE}, we derived in Section~\ref{general} equilibrium properties of the game $\Gamma(b_1,b_2)$ that hold when $b_1 < \smsc$ and $b_2 < \semm$. Note that all these properties, except Prop.~\ref{all_edges}, also hold when $b_1 < \smsc$ and $b_2 = \semm$. This implies that Prop.~\ref{Prop_interim}, i.e., our (approximate) solution for the network inspection problem \ECOP, and Theorem~\ref{Constant}, are still valid when $b_2 = \semm$.  

However, most of these properties are not satisfied by the NE of $\Gamma(b_1,b_2)$ when $b_1 < \smsc$ and $b_2 > \semm$, as discussed in the following example:
%
%For Proposition~\ref{best_set_cover}, we can only conclude that given any minimal set cover $\Def^\prime$, the optimal value of \rlpo{\Def^{\prime}} is \emph{at least} $b_2\left(\frac{b_1}{|\Def^\prime|} - 1\right)$. Furthermore, set packings cannot be used anymore since their sizes are less than $b_2$. \rem{We can also find a counterexample (see example \ref{example_other_case}) that violates \eqref{res2} in Proposition~\ref{all_resources}. Proposition~\ref{all_edges} does not hold, even when $b_2 = \semm$: in example~\ref{example_other_case}, we find a \emph{pure} NE whose node basis is not a set cover. Theorem~\ref{bounds_game} is not valid anymore: we can find NE with different payoffs for \defender, and different expected detection rates. This directly implies that Theorem~\ref{Constant} does not hold anymore.} Furthermore, the bounds on the players' equilibrium payoffs, and the upper bound on the equilibrium expected detection rates, do not hold anymore.  Theorem~\ref{MSC-MSP-eNE} does not hold either: we cannot construct a ``good'' $\epsilon-$NE from an MSC and an MSP, and the worst expected detection rate when choosing $\sold{\Def^{min}}{b_1}{}$ may be arbitrarily far from an expected detection rate in equilibrium.  
%
%Next, we present an illustrative example to discuss the equilibrium properties of the game $\Gamma(b_1,b_2)$  when $b_1 < \smsc$ and $b_2 > \semm$. 
%
%
%
\begin{example}\label{example_other_case}

Consider the detection model $\mathcal{G} = (\nodes,\edges,\{\set{i}, \ i \in \nodes)$ defined as follows. Let $\nodes = \{i_1,\dots,i_{2n}\}$, with $n \in \mathbb{N}$, and let $\edges = \edges_1 \cup \{e_1,\dots,e_n\}$, where $\edges_1$ is a discrete set. Then, the monitoring sets are defined by: $\forall k \in \llbracket 1,n\rrbracket, \ \set{i_k} = \edges_1 \cup \{e_k\}$ and $\set{i_{n+k}} = \{e_k\}$.

%Consider the network represented in Fig.~\ref{Fail1}. Detectors can be placed on the nodes of the network, and can monitor the network edges.
%\begin{figure}[ht]
%%\small
%\centering
%\begin{tikzpicture}[-,auto,x=1.4cm, y=0.6cm,
%  thick,main node/.style={circle,draw,inner sep = 0.14cm,black},main node2/.style={circle,draw,inner sep = 0.04cm,black},main node3/.style={circle,draw,inner sep = 0.1cm,black},flow_a/.style ={gray!100}]
%\tikzstyle{edge} = [draw,thick,-,black]
%\tikzstyle{cut} = [draw,very thick,-]
%\tikzstyle{match} = [draw,very thick,black,-, dashed]
%\tikzstyle{flow} = [draw,line width = 1.5pt,->,gray!100]
%\small
%%\begin{scope}[yshift=0, xshift =-110]
%	\node[main node] (1) at (0,2.5) {$i_1$};
%%	\node[main node] (2) at (0,1.75) {$i_2$};
%	\node[main node] (3) at (0,0+0.5) {$i_{n}$};
%	\node[main node2] (4) at (2.5,2.5) {$i_{n+1}$};
%%	\node[main node2] (5) at (2.5,1.75) {$i_{n+2}$};
%	\node[main node3] (6) at (2.5,0+0.5) {$i_{2n}$};
%
%	%\node[main node, draw=white] (7) at (3.5,-0.5) {\textbf{a}};
%	
%	\path[edge]	
%	%(2) edge (5)
%	%(1) edge  (2)
%	(1) edge node{$e_1$} (4)
%%	(2) edge node {$e_2$} (5)
%	(3) edge  node {$e_n$} (6);
%%\end{scope}
%
%%\draw[dashed,very thick,black] (0.75,0.5) -- (0.75,1.2);
%
%\draw[dashed,thick,black] (0,0.4+0.5) -- (0,1.35);
%
%\draw[dashed,thick,black] (2.5,0.4+0.5) -- (2.5,1.35);
%
%%\draw[dashed,black] (-1,1.25+0.25) ellipse (3.1cm and 2.0cm);
%
%%\draw[dashed,black] (-4.5,-0.5) -- (-0.5,-0.5) -- (-0.5,3) -- (-4.5,3) -- (-4.5,-0.5);
%
%\node[black] (99) at (-3.1,2.75) {$(\nodes_1,\edges_1)$};
%\node[black] (100) at (-2,2.5) {\ };
%%\node[black] (101) at (-2,1.75) {\ };
%\node[black] (102) at (-2,0+0.5) {\ };
%
%%\draw[thick,dashed,black] (-2,1.25) circle (2.3cm);
%
%	\path[edge]
%	(1) edge (100)
%%	(2) edge (101)
%	(3) edge (102);
%\end{tikzpicture}
%
%\caption{Network which violates some of the equilibrium properties derived in Section~\ref{general}.} 
%\label{Fail1}
%\end{figure}
%This network is composed of a subnetwork $G_1 = (\nodes_1,\edges_1)$, and $n$ extra nodes $i_{n+1},\dots, i_{2n}$ and extra edges $e_1,\dots,e_n$ that are connected  according to Fig.~\ref{Fail1}. Note that $i_{n+1},\dots, i_{2n} \notin \nodes_1$ and $e_1,\dots,e_n \notin \edges_1$. We suppose the detection model is given by: $\forall i \in \nodes_1 \backslash\{i_1,\dots,i_n\}, \ \set{i} \subseteq \edges_1$, $\forall k \in \llbracket 1,n\rrbracket, \ \set{i_k} = \edges_1 \cup \{e_k\}$ and $\set{i_{n+k}} = \{e_k\}$.

%Assume that the detection model is such that a detector positioned at any node of $\nodes_1$ except $i_1,i_2,\dots,i_n$ cannot monitor any of the edges $e_1,\dots,e_n$. Then, we assume that a detector positioned at $i_k$ (for $k \in \llbracket 1,n \rrbracket$) can monitor $e_k$ and \emph{all} the edges of $G_1$. Finally, we assume that a detector positioned at $i_{n+k}$ (for $k \in \llbracket 1,n \rrbracket$) can monitor $e_k$. More formally, we have $\forall i \in \nodes_1 \backslash\{i_1,\dots,i_n\}, \ \set{i} \subseteq \edges_1$, $\forall k \in \llbracket 1,n\rrbracket, \ \set{i_k} = \edges_1 \cup \{e_k\}$ and $\set{i_{n+k}} = \{e_k\}$.
%\begin{align*}
%\forall i \in \nodes_1 \backslash\{i_1,\dots,i_n\}, \ &\set{i} \subseteq \edges_1,\\
% \forall k \in \llbracket 1,n\rrbracket, \ &\set{i_k} = \edges_1 \cup \{e_k\},\\
% \forall k \in \llbracket 1,n\rrbracket, \ &\set{i_{n+k}} = \{e_k\}.
%\end{align*}

In this example, $\Def^{min} = \{i_1,\dots,i_n\}$ is an MSC, and  $\att^{max} = \{e_1,\dots,e_n\}$ is an MSP; so $\smsc = \semm = n$. Given any $b_1 < n$ and any $b_2 \in \llbracket n, |\edges_1| + n\rrbracket$, one can check that $\forall \att \in \mathcal{A}_2 \ | \ \att^{max} \subseteq \att, \ (\{i_1,\dots,i_{b_1}\},\att)$ is a pure NE, whose node basis is not a set cover. Therefore, Prop.~\ref{all_edges} does not hold anymore.

Now, if we consider $b_2 = |\edges_1| + n$, we just showed that we could construct NE where \attacker can use $n,n+1,\dots$, or $n+|\edges_1| = b_2$ resources. Thus, \eqref{res2} in Prop.~\ref{all_resources} does not hold anymore. This also implies that \defender's payoff and the expected detection rate are not constant in equilibrium anymore: We found equilibria where \defender's payoff is equal to $b_1,b_1+1,\dots,b_1 + |\edges_1|$. This corresponds to equilibrium detection rates equal to $\frac{b_1}{n},\frac{b_1+1}{n+1},\dots,\frac{b_1+|\edges_1|}{n+|\edges_1|}$, which violates Thm.~\ref{Constant}. Since $\frac{b_1+|\edges_1|}{n+|\edges_1|} \underset{|\edges_1| \to +\infty}{\longrightarrow} 1$, the upper bound on the expected detection rates given by Thm.~\ref{bounds_game} is violated. Furthermore, the bound derived in Thm.~\ref{MSC-MSP-eNE} is not valid anymore. By choosing $\sold{\Def^{min}}{b_1}{}$, the expected detection rate may be arbitrarily far from an equilibrium expected detection rate: we can only trivially bound the difference with $1 - \frac{b_1}{\smsc}$.
%
%\vspace{-0.3cm}
\hfill $\triangle$
% Still, in this example, if \defender chooses $\lceil \alpha \smsc \rceil$ sensors, then the expected detection rates in equilibrium will be at least $\alpha$. Furthermore, given an MSC, $\Def^{min}$, if \defender allocates these  $\lceil \alpha \smsc \rceil$ sensors according to the sensing strategy $\sold{\Def^{min}}{\lceil\alpha\smsc\rceil}{}$, the expected detection rate will also be at least $\alpha$, regardless of which strategy \attacker chooses.

%This example also shows that even though the previous results are intuitive, they do not hold in general and may require extensive proofs that rely on $b_2 < \semm$, thus stressing the importance of MSPs in our analysis.

\end{example}

%\tr{Therefore, when $b_2 > \semm$, we lose the optimality guarantee that the MSPs provided us with.} 

Still, some results remain valid when $b_1 < \smsc$ and $b_2 > \semm$: In Proposition~\ref{all_resources}, \eqref{res1} still holds. In Theorem~\ref{bounds_game}, the lower bound on the equilibrium expected detection rates is still valid. In Theorem~\ref{MSC-MSP-eNE}, when choosing $\sold{\Def^{min}}{b_1}{}$, the expected detection rate is still guaranteed to be at least $\frac{b_1}{\smsc}$, regardless of \attacker's strategy.
From these remaining results, we can show that $b_1^\prime = \lceil \alpha \smsc \rceil$ is still a sufficient condition for the expected detection rates in equilibrium to be at least $\alpha$, and provides an upper bound on the optimal value $b_1^\dag$ of \ECOP. %However, the optimality gap associated with it is not valid anymore; see Section~\ref{example_other_case}.
 Furthermore, given an MSC, $\Def^{min}$, if \defender positions these  $b_1^\prime$ detectors according to the inspecting strategy $\sold{\Def^{min}}{b_1^\prime}{}$, she is still guaranteed to detect a fraction $\alpha$ of the attacks in expectation, regardless of which strategy \attacker chooses.
% 
%Furthermore, although we cannot provide a good $\epsilon-$NE from an MSC and an MSP anymore, \defender is still guaranteed to detect a fraction $\alpha$ of the failures in expectation by operating $b_1^\prime$ sensors according to the strategy $\sold{\Def^{min}}{b_1^\prime}{}$.


%\subsection{Network Monitoring Problem}

%Implications for the network monitoring problem:

%Results still hold when $b_2 = \semm$, but not when $b_2 > \semm$.

%The positive result is that $b_1^\prime = \lceil \alpha \smsc \rceil$ remains a sufficient condition for the expected detection rates in equilibrium to be at least $\alpha$, and provides an upper bound on the optimal value $b_1^*$ of \ECOP. However, the optimality gap associated with it is not valid anymore; see Section~\ref{example_other_case}. Moreover, by operating $b_1^\prime$ sensors according to the strategy $\sold{\Def^{min}}{b_1^\prime}{}$, \defender is still guaranteed to detect $\alpha$ of the failure events in expectation, regardless of what \attacker does. 


%\section{Contaminant}
%\tb{
%Our setup can be applied to pipe failures and contamination intrusions scenarios in water networks.  
%Similarly, early detection of contamination event can be achieved by monitoring water quality parameters (e.g., turbidity, conductivity) \citep{EPA:quality}. The constituent injected into the system moves with the flow and reacts with its environment. Its signal diminishes with the distance from the source due to decay and dilution governed by network dynamics. Contamination event can be simulated using steady state hydraulic and water quality analysis of the system and is available in commercial and public software, e.g. EPANET \citep{epanet:2002}. Contamination events and their detectability have been widely studied by the water research community \citep{ostfeld2008battle,doi:10.1021/es3014024}. Using these softwares, the network operator can determine the nodes that can monitor each failure event, or equivalently, the monitoring sets.}




%\subsection{A Simple Example V17}\label{example_detection_sensing}
%
%%\begin{example}%[MSC and MCS]
%Consider the network shown in Fig.~\ref{Example1}. Assume a sensing model in which a sensor placed at any node can monitor components at one-hop vertically, and at two hops horizontally. Thus, $\set{i_1} = \{e_1,e_2,e_3\}$, $\set{i_2} = \{e_1,e_2,e_4\}$, $\set{i_3} = \{e_1,e_2,e_5\}$, $\set{i_4} = \{e_4,e_6,e_7\}$, $\set{i_5} = \{e_5,e_6,e_8\}$, $\set{i_6} = \{e_3,e_9,e_{10}\}$, $\set{i_7} = \{e_7,e_9,e_{10}\}$, $\set{i_8} = \{e_8,e_9,e_{10}\}$.
%
%%%%---------------------------------------------------------------------------------------------------
%\def \sizefig {1.4cm}
%\def \scalefig {\small}
%\def \innersepfig {0.07cm}
%%%%---------------------------------------------------------------------------------------------------
%
%\begin{figure}[ht]
%\centering
%{\scalefig
%\begin{tikzpicture}[-,auto,x=\sizefig, y=\sizefig,
%  thick,main node/.style={circle,draw,inner sep = \innersepfig,black},main node2/.style={circle,black,draw,fill=blue!60,inner sep = \innersepfig},flow_a/.style ={gray!100}]
%\tikzstyle{edge} = [draw,thick,-,black]
%\tikzstyle{cut} = [draw,very thick,-]
%\tikzstyle{match} = [draw,very thick,black,-, dashed]
%\tikzstyle{flow} = [draw,line width = 1.5pt,->,gray!100]
%
%%\begin{scope}[yshift=0, xshift =-110]
%	\node[main node] (1) at (0,2) {$i_1$};
%	\node[main node] (2) at (1,2) {$i_2$};
%	\node[main node2] (3) at (2,2) {$i_3$};
%	\node[main node] (4) at (1,1) {$i_4$};
%	\node[main node] (5) at (2,1) {$i_5$};
%	\node[main node] (6) at (0,0) {$i_6$};
%	\node[main node] (7) at (1,0) {$i_7$};
%	\node[main node] (8) at (2,0) {$i_8$};
%	%\node[main node, draw=white] (7) at (3.5,-0.5) {\textbf{a}};
%	
%	\path[edge]	
%	%(2) edge (5)
%	%(1) edge  (2)
%	(1) edge node[left]{$e_3$} (6)
%	(4) edge node {$e_6$} (5)
%	(2) edge[double,blue!80]  node {$e_2$} (3)
%	(2) edge node[left] {$e_4$} (4)
%	(6) edge node[below] {$e_9$} (7)
%	(7) edge node[below] {$e_{10}$} (8)
%	%(3) edge  (5)	
%	%(4) edge  (6)
%	(5) edge node {$e_8$} (8);
%
%	\path[edge]
%	(1) edge[double,blue!80] node {$e_1$} (2)
%	(3) edge[double,blue!80] node {$e_5$} (5)
%	(4) edge node[left] {$e_7$} (7);
%%\end{scope}
%
%\end{tikzpicture}}
%
%\caption{Example network. The monitoring set $\set{i_3} = \{e_1,e_2,e_5\}$ is represented by the double blue edges.} \label{Example1}
%\end{figure}
%
%
%
%Consider the problem \ECOP with the target expected detection rate $\alpha = 0.75$ and the number of attack resources $b_2 = 2$. For this small-sized problem, we can solve  \lpo and \lpt to compute the NE of $\Gamma$, and obtain  the expected detection rate in any NE for each $b_1 \in \mathbb{N}$; see Table~\ref{r_sigma_example}.
%\begin{table}[htbp]
%\centering
%\caption{Expected detection rate in equilibrium for every $b_1 \in \mathbb{N}$.}
%\def\arraystretch{\spacingtable}
%\begin{tabular}{|c|c|c|c|c|c|}\hline $b_1$ & 0 & 1 & 2 & 3 & $\geq 4$ \\\hline $\sdet{*}$ & 0 & $\frac{2}{7}$ & $\frac{4}{7}$ & $\frac{6}{7}$ & 1 \\\hline \end{tabular}
%\label{r_sigma_example}
%\end{table}
%
%Notice that for a given $b_1$, the expected detection rate is the same in any NE; this property is shown in Thm.~\ref{bounds_game}. From Table~\ref{r_sigma_example}, we conclude that the optimal value of (\hyperlink{(P)}{$\mathcal{P}$}) is $b_1^\dag = 3$, i.e., with  $3$ sensors, \defender is capable of detecting $\frac{6}{7} \geq \alpha$ of the failure events in equilibrium. However, as mentioned in Section~\ref{sec:Formal problem}, this method does not extend to larger networks, as it requires solving large \lpo and \lpt for each $b_1 \in \mathbb{N}$ and checking if the constraint on the expected detection rate in any equilibrium \eqref{all_NE} is met.
%
%
%
%%\tb{For the network in Fig.~\ref{Example1} and its sensing model, a solution of (\hyperlink{(MSC)}{MSC}) is given by $\{i_3,i_4,i_6,i_8\} \in \msc$ and a solution of (\hyperlink{(MSP)}{MSP}) is $\{e_3,e_4,e_8\} \in \emm$. Thus, $\smsc = 4$ and $\semm = 3$. }
%
%
%%We now propose the following approach: First, we solve (\hyperlink{(MSC)}{MSC}); an optimal solution is given by  $\Def^{min} = \{i_3,i_6,i_4,i_8\}$. Second, given $b_1$ sensors between $0$ and $|\Def^{min}|$, we randomize the placement of these $b_1$ sensors over subsets of $\Def^{min}$ such that each node in $\Def^{min}$ is sensed with an identical probability. Then, as we will show in Section~\ref{general}, such a sensing strategy guarantees that regardless of which strategy \attacker chooses, the expected detection rate will be at least $\frac{b_1}{|\Def^{min}|}$. Thus, by choosing 3 sensors, our sensing strategy ensures that $0.75\geq \alpha$ of the failure events be detected. Thm.~\ref{bounds_game} implies that, in this example, with 3 sensors, the expected detection rate in \emph{any} equilibrium of the resulting game is at least $\alpha$. Therefore, for this example, our method provides a feasible solution of \ECOP which turned out to be the optimal one ($b_1^* = 3$). 
%
%We now propose the following approach: First, by solving \eqref{IP1}, we obtain an MSC given by  $\Def^{min} = \{i_3,i_4,i_6,i_8\}$; thus $\smsc = 4$. Then, from Thm.~\ref{bounds_game}, we know that the expected detection rate in any equilibrium is lower bounded by $\frac{b_1}{\smsc}$. Thus, with $b_1^\prime:=\lceil \alpha \smsc \rceil = 3$ sensors, the expected detection rate in any equilibrium is at least $\alpha$.
%
%Secondly, by solving \eqref{IP2}, we obtain an MSP given by $\att^{max} = \{e_3,e_4,e_8\}$; thus $\semm = 3$. Again, from Thm.~\ref{bounds_game}, we know that the expected detection rate in any equilibrium is upper bounded by $\frac{b_1}{\semm}$, which implies that if $b_1< \lceil \alpha \semm \rceil$, the equilibrium constraints \eqref{all_NE} are not satisfied. Then, we deduce that an optimality gap associated with $b_1^\prime$ is given by $\lceil \alpha \smsc\rceil - \lceil \alpha \semm \rceil = \lceil 3\rceil - \lceil 2.25 \rceil = 0$ (Prop.~\ref{Prop_interim}). Therefore, by solving (\hyperlink{(MSC)}{MSC}) and (\hyperlink{(MSP)}{MSP}), we can estimate the number of sensing resources to ensure that the equilibrium constraints in \ECOP are satisfied; furthermore, we can verify that this number is optimal for this example, i.e., $b_1^\prime = b_1^\dag = 3$.
%
%Thirdly, given $b_1^\prime=3$ and $b_2 =2$, we can use $\Def^{min}$ and $\att^{max}$ to construct an approximate NE. Using Lemma~\ref{algebra2}, we construct a strategy profile ${\sigma} = (\sigma^1,{\sigma}^2)$, where ${\sigma}^1_{\{i_3,i_4,i_6\}} = {\sigma}^1_{\{i_8,i_3,i_4\}}  =  {\sigma}^1_{\{i_6, i_8,i_3\}}  = {\sigma}^1_{\{i_4,i_6,i_8\}}  = \frac{1}{4}$, and ${\sigma}^2_{\{e_3,e_4\}} = {\sigma}^2_{\{e_8,e_3\}} = {\sigma}^2_{\{e_4,e_8\}}  =  \frac{1}{3}$; see Fig.~\ref{Strategies} for an illustration.  From Thm.~\ref{MSC-MSP-eNE}, we obtain that the above-constructed strategy profile ${\sigma}$ is an $\epsilon-$NE, and provides each player a payoff that is $\epsilon-$close to their equilibrium payoff, with $\epsilon=  b_1^\prime b_2\left( \frac{1}{\max\{b_1^\prime,\semm\}} - \frac{1}{\smsc}\right) = \frac{1}{2}$. Indeed, from Table~\ref{r_sigma_example} and Prop.~\ref{all_resources}, we deduce that \defender and \attacker's equilibrium payoffs are $\frac{12}{7}$ and $\frac{2}{7}$ respectively, while our strategy profile $\sigma$ provides them with the respective payoffs $\frac{3}{2}$ and $\frac{1}{2}$. One can easily check that $\sigma$ gives each player a payoff that is $\frac{3}{14} \ (\leq \epsilon)$ close to their equilibrium payoff.
%
%% and the influence matrix can be written as follows:
%%\begin{align*}
%%\boldsymbol{F} = {\arraycolsep=3.5pt
%%	\kbordermatrix{&\mbox{$e_1$}&\mbox{$e_2$}&\mbox{$e_3$}&\mbox{$e_4$}&\mbox{$e_5$} &\mbox{$e_6$} & \mbox{$e_7$} & \mbox{$e_8$}\\
%%\mbox{$i_1$}&1 & 1 & 0 & 1 & 1 & 0 &0 &0 \\
%%	\mbox{$i_2$}&1 & 0 & 1 & 1 & 0 & 0&0 &0  \\
%%	\mbox{$i_3$}&0 & 1 & 1 & 0 & 1 & 0 &0 &0\\
%%	\mbox{$i_4$}&0 & 0 & 0 & 1 & 0 & 1 &1 &0\\
%%	\mbox{$i_5$}&0 & 0 & 0 & 0 & 1 & 1 &0 &1 \\
%%	\mbox{$i_6$}&0 & 0 & 0 & 0 & 0 & 0&1 &1
%%}}.
%%\end{align*}
%\begin{figure}[ht]
%\centering
%\begin{subfigure}[b]{0.23\textwidth}
%\centering
%{\scalefig
%\begin{tikzpicture}[-,auto,x=\sizefig, y=\sizefig,
%  thick,main node/.style={circle,draw,inner sep = \innersepfig,black},main node2/.style={circle,black,draw,fill=blue!60,inner sep = \innersepfig},flow_a/.style ={gray!100}]
%\tikzstyle{edge} = [draw,thick,-,black]
%\tikzstyle{cut} = [draw,very thick,-]
%\tikzstyle{match} = [draw,very thick,black,-, dashed]
%\tikzstyle{flow} = [draw,line width = 1.5pt,->,gray!100]
%
%%\begin{scope}[yshift=0, xshift =-110]
%	\node[main node] (1) at (0,2) {$i_1$};
%	\node[main node] (2) at (1,2) {$i_2$};
%	\node[main node2] (3) at (2,2) {$i_3$};
%	\node[main node2] (4) at (1,1) {$i_4$};
%	\node[main node] (5) at (2,1) {$i_5$};
%	\node[main node2] (6) at (0,0) {$i_6$};
%	\node[main node] (7) at (1,0) {$i_7$};
%	\node[main node] (8) at (2,0) {$i_8$};
%	%\node[main node, draw=white] (7) at (3.5,-0.5) {\textbf{a}};
%	
%	\path[edge]	
%	%(2) edge (5)
%	%(1) edge  (2)
%	(1) edge node[left]{$e_3$} (6)
%	(4) edge node {$e_6$} (5)
%	(2) edge  node {$e_2$} (3)
%	(2) edge node[left] {$e_4$} (4)
%	(6) edge node[below] {$e_9$} (7)
%	(7) edge node[below] {$e_{10}$} (8)
%	%(3) edge  (5)	
%	%(4) edge  (6)
%	(5) edge node {$e_8$} (8);
%
%	\path[edge]
%	(1) edge node {$e_1$} (2)
%	(3) edge node {$e_5$} (5)
%	(4) edge node[left] {$e_7$} (7);
%%\end{scope}
%
%\end{tikzpicture}}
%
%\caption{${\sigma}^1_{\{i_3,i_4,i_6\}} = \frac{1}{4}$.} 
%\end{subfigure}
%~
%\begin{subfigure}[b]{0.23\textwidth}
%\centering
%{\scalefig
%\begin{tikzpicture}[-,auto,x=\sizefig, y=\sizefig,
%  thick,main node/.style={circle,draw,inner sep = \innersepfig,black},main node2/.style={circle,black,draw,fill=blue!60,inner sep = \innersepfig},flow_a/.style ={gray!100}]
%\tikzstyle{edge} = [draw,thick,-,black]
%\tikzstyle{cut} = [draw,very thick,-]
%\tikzstyle{match} = [draw,very thick,black,-, dashed]
%\tikzstyle{flow} = [draw,line width = 1.5pt,->,gray!100]
%
%%\begin{scope}[yshift=0, xshift =-110]
%	\node[main node] (1) at (0,2) {$i_1$};
%	\node[main node] (2) at (1,2) {$i_2$};
%	\node[main node2] (3) at (2,2) {$i_3$};
%	\node[main node2] (4) at (1,1) {$i_4$};
%	\node[main node] (5) at (2,1) {$i_5$};
%	\node[main node] (6) at (0,0) {$i_6$};
%	\node[main node] (7) at (1,0) {$i_7$};
%	\node[main node2] (8) at (2,0) {$i_8$};
%	%\node[main node, draw=white] (7) at (3.5,-0.5) {\textbf{a}};
%	
%	\path[edge]	
%	%(2) edge (5)
%	%(1) edge  (2)
%	(1) edge node[left]{$e_3$} (6)
%	(4) edge node {$e_6$} (5)
%	(2) edge  node {$e_2$} (3)
%	(2) edge node[left] {$e_4$} (4)
%	(6) edge node[below] {$e_9$} (7)
%	(7) edge node[below] {$e_{10}$} (8)
%	%(3) edge  (5)	
%	%(4) edge  (6)
%	(5) edge node {$e_8$} (8);
%
%	\path[edge]
%	(1) edge node {$e_1$} (2)
%	(3) edge node {$e_5$} (5)
%	(4) edge node[left] {$e_7$} (7);
%%\end{scope}
%
%\end{tikzpicture}}
%
%\caption{${\sigma}^1_{\{i_8,i_3,i_4\}} = \frac{1}{4}$.} 
%\end{subfigure}
%~
%\begin{subfigure}[b]{0.23\textwidth}
%\centering
%{\scalefig
%\begin{tikzpicture}[-,auto,x=\sizefig, y=\sizefig,
%  thick,main node/.style={circle,draw,inner sep = \innersepfig,black},main node2/.style={circle,black,draw,fill=blue!60,inner sep = \innersepfig},flow_a/.style ={gray!100}]
%\tikzstyle{edge} = [draw,thick,-,black]
%\tikzstyle{cut} = [draw,very thick,-]
%\tikzstyle{match} = [draw,very thick,black,-, dashed]
%\tikzstyle{flow} = [draw,line width = 1.5pt,->,gray!100]
%
%%\begin{scope}[yshift=0, xshift =-110]
%	\node[main node] (1) at (0,2) {$i_1$};
%	\node[main node] (2) at (1,2) {$i_2$};
%	\node[main node2] (3) at (2,2) {$i_3$};
%	\node[main node] (4) at (1,1) {$i_4$};
%	\node[main node] (5) at (2,1) {$i_5$};
%	\node[main node2] (6) at (0,0) {$i_6$};
%	\node[main node] (7) at (1,0) {$i_7$};
%	\node[main node2] (8) at (2,0) {$i_8$};
%	%\node[main node, draw=white] (7) at (3.5,-0.5) {\textbf{a}};
%	
%	\path[edge]	
%	%(2) edge (5)
%	%(1) edge  (2)
%	(1) edge node[left]{$e_3$} (6)
%	(4) edge node {$e_6$} (5)
%	(2) edge  node {$e_2$} (3)
%	(2) edge node[left] {$e_4$} (4)
%	(6) edge node[below] {$e_9$} (7)
%	(7) edge node[below] {$e_{10}$} (8)
%	%(3) edge  (5)	
%	%(4) edge  (6)
%	(5) edge node {$e_8$} (8);
%
%	\path[edge]
%	(1) edge node {$e_1$} (2)
%	(3) edge node {$e_5$} (5)
%	(4) edge node[left] {$e_7$} (7);
%%\end{scope}
%
%\end{tikzpicture}}
%
%\caption{${\sigma}^1_{\{i_6,i_8,i_3\}} = \frac{1}{4}$.} 
%\end{subfigure}
%~
%\begin{subfigure}[b]{0.23\textwidth}
%\centering
%{\scalefig
%\begin{tikzpicture}[-,auto,x=\sizefig, y=\sizefig,
%  thick,main node/.style={circle,draw,inner sep = \innersepfig,black},main node2/.style={circle,black,draw,fill=blue!60,inner sep = \innersepfig},flow_a/.style ={gray!100}]
%\tikzstyle{edge} = [draw,thick,-,black]
%\tikzstyle{cut} = [draw,very thick,-]
%\tikzstyle{match} = [draw,very thick,black,-, dashed]
%\tikzstyle{flow} = [draw,line width = 1.5pt,->,gray!100]
%
%%\begin{scope}[yshift=0, xshift =-110]
%	\node[main node] (1) at (0,2) {$i_1$};
%	\node[main node] (2) at (1,2) {$i_2$};
%	\node[main node] (3) at (2,2) {$i_3$};
%	\node[main node2] (4) at (1,1) {$i_4$};
%	\node[main node] (5) at (2,1) {$i_5$};
%	\node[main node2] (6) at (0,0) {$i_6$};
%	\node[main node] (7) at (1,0) {$i_7$};
%	\node[main node2] (8) at (2,0) {$i_8$};
%	%\node[main node, draw=white] (7) at (3.5,-0.5) {\textbf{a}};
%	
%	\path[edge]	
%	%(2) component (5)
%	%(1) edge  (2)
%	(1) edge node[left]{$e_3$} (6)
%	(4) edge node {$e_6$} (5)
%	(2) edge  node {$e_2$} (3)
%	(2) edge node[left] {$e_4$} (4)
%	(6) edge node[below] {$e_9$} (7)
%	(7) edge node[below] {$e_{10}$} (8)
%	%(3) edge  (5)	
%	%(4) edge  (6)
%	(5) edge node {$e_8$} (8);
%
%	\path[edge]
%	(1) edge node {$e_1$} (2)
%	(3) edge node {$e_5$} (5)
%	(4) edge node[left] {$e_7$} (7);
%%\end{scope}
%
%\end{tikzpicture}}
%
%\caption{${\sigma}^1_{\{i_4,i_6,i_8\}} = \frac{1}{4}$.} 
%\end{subfigure}
%
%\medskip
%
%\begin{subfigure}[b]{0.3\textwidth}
%\centering
%{\scalefig
%\begin{tikzpicture}[-,auto,x=\sizefig, y=\sizefig,
%  thick,main node/.style={circle,draw,inner sep = \innersepfig,black},main node2/.style={circle,black,draw,fill=Green,inner sep = 0.08cm},flow_a/.style ={gray!100}]
%\tikzstyle{edge} = [draw,thick,-,black]
%\tikzstyle{cut} = [draw,very thick,-]
%\tikzstyle{match} = [draw,very thick,black,-, dashed]
%\tikzstyle{flow} = [draw,line width = 1.5pt,->,gray!100]
%
%%\begin{scope}[yshift=0, xshift =-110]
%	\node[main node] (1) at (0,2) {$i_1$};
%	\node[main node] (2) at (1,2) {$i_2$};
%	\node[main node] (3) at (2,2) {$i_3$};
%	\node[main node] (4) at (1,1) {$i_4$};
%	\node[main node] (5) at (2,1) {$i_5$};
%	\node[main node] (6) at (0,0) {$i_6$};
%	\node[main node] (7) at (1,0) {$i_7$};
%	\node[main node] (8) at (2,0) {$i_8$};
%	%\node[main node, draw=white] (7) at (3.5,-0.5) {\textbf{a}};
%	
%	\path[edge]	
%	%(2) edge (5)
%	%(1) edge  (2)
%	(1) edge node[left = 0.1cm]{$e_3$} (6)
%	(4) edge node {$e_6$} (5)
%	(2) edge  node {$e_2$} (3)
%	(2) edge node[left = 0.1cm] {$e_4$} (4)
%	(6) edge node[below] {$e_9$} (7)
%	(7) edge node[below] {$e_{10}$} (8)
%	%(3) edge  (5)	
%	%(4) edge  (6)
%	(5) edge node {$e_8$} (8);
%
%	\path[edge]
%	(1) edge node {$e_1$} (2)
%	(3) edge node {$e_5$} (5)
%	(4) edge node[left] {$e_7$} (7);
%%\end{scope}
%
%	\node(12) at (0,1) {\textcolor{Red}{\Huge{\Cross}}};
%	\node(13) at (1,1.5) {\textcolor{Red}{\Huge{\Cross}}};
%
%\end{tikzpicture}}
%
%\caption{${\sigma}^2_{\{e_3,e_4\}} = \frac{1}{3}$.}
%\end{subfigure}
%~
%\begin{subfigure}[b]{0.3\textwidth}
%\centering
%{\scalefig
%\begin{tikzpicture}[-,auto,x=\sizefig, y=\sizefig,
%  thick,main node/.style={circle,draw,inner sep = \innersepfig,black},main node2/.style={circle,black,draw,fill=Green,inner sep = 0.08cm},flow_a/.style ={gray!100}]
%\tikzstyle{edge} = [draw,thick,-,black]
%\tikzstyle{cut} = [draw,very thick,-]
%\tikzstyle{match} = [draw,very thick,black,-, dashed]
%\tikzstyle{flow} = [draw,line width = 1.5pt,->,gray!100]
%
%%\begin{scope}[yshift=0, xshift =-110]
%	\node[main node] (1) at (0,2) {$i_1$};
%	\node[main node] (2) at (1,2) {$i_2$};
%	\node[main node] (3) at (2,2) {$i_3$};
%	\node[main node] (4) at (1,1) {$i_4$};
%	\node[main node] (5) at (2,1) {$i_5$};
%	\node[main node] (6) at (0,0) {$i_6$};
%	\node[main node] (7) at (1,0) {$i_7$};
%	\node[main node] (8) at (2,0) {$i_8$};
%	%\node[main node, draw=white] (7) at (3.5,-0.5) {\textbf{a}};
%	
%	\path[edge]	
%	%(2) edge (5)
%	%(1) edge  (2)
%	(1) edge node[left = 0.1cm]{$e_3$} (6)
%	(4) edge node {$e_6$} (5)
%	(2) edge  node {$e_2$} (3)
%	(2) edge node[left] {$e_4$} (4)
%	(6) edge node[below] {$e_9$} (7)
%	(7) edge node[below] {$e_{10}$} (8)
%	%(3) edge  (5)	
%	%(4) edge  (6)
%	(5) edge node[right = 0.1cm] {$e_8$} (8);
%
%	\path[edge]
%	(1) edge node {$e_1$} (2)
%	(3) edge node {$e_5$} (5)
%	(4) edge node[left] {$e_7$} (7);
%%\end{scope}
%\node(12) at (0,1) {\textcolor{Red}{\Huge{\Cross}}};
%	\node(13) at (2,0.5) {\textcolor{Red}{\Huge{\Cross}}};
%\end{tikzpicture}}
%
%\caption{${\sigma}^2_{\{e_8,e_3\}} = \frac{1}{3}$.} 
%\end{subfigure}
%~
%\begin{subfigure}[b]{0.3\textwidth}
%\centering
%{\scalefig
%\begin{tikzpicture}[-,auto,x=\sizefig, y=\sizefig,
%  thick,main node/.style={circle,draw,inner sep = \innersepfig,black},main node2/.style={circle,black,draw,fill=Green,inner sep = 0.08cm},flow_a/.style ={gray!100}]
%\tikzstyle{edge} = [draw,thick,-,black]
%\tikzstyle{cut} = [draw,very thick,-]
%\tikzstyle{match} = [draw,very thick,black,-, dashed]
%\tikzstyle{flow} = [draw,line width = 1.5pt,->,gray!100]
%
%%\begin{scope}[yshift=0, xshift =-110]
%	\node[main node] (1) at (0,2) {$i_1$};
%	\node[main node] (2) at (1,2) {$i_2$};
%	\node[main node] (3) at (2,2) {$i_3$};
%	\node[main node] (4) at (1,1) {$i_4$};
%	\node[main node] (5) at (2,1) {$i_5$};
%	\node[main node] (6) at (0,0) {$i_6$};
%	\node[main node] (7) at (1,0) {$i_7$};
%	\node[main node] (8) at (2,0) {$i_8$};
%	%\node[main node, draw=white] (7) at (3.5,-0.5) {\textbf{a}};
%	
%	\path[edge]	
%	%(2) edge (5)
%	%(1) edge  (2)
%	(1) edge node[left]{$e_3$} (6)
%	(4) edge node {$e_6$} (5)
%	(2) edge  node {$e_2$} (3)
%	(2) edge node[left = 0.1cm] {$e_4$} (4)
%	(6) edge node[below] {$e_9$} (7)
%	(7) edge node[below] {$e_{10}$} (8)
%	%(3) edge  (5)	
%	%(4) edge  (6)
%	(5) edge node[right = 0.1cm] {$e_8$} (8);
%
%	\path[edge]
%	(1) edge node {$e_1$} (2)
%	(3) edge node {$e_5$} (5)
%	(4) edge node[left] {$e_7$} (7);
%%\end{scope}
%\node(12) at (2,0.5) {\textcolor{Red}{\Huge{\Cross}}};
%	\node(13) at (1,1.5) {\textcolor{Red}{\Huge{\Cross}}};
%\end{tikzpicture}}
%
%\caption{${\sigma}^2_{\{e_4,e_8\}} = \frac{1}{3}$.}
%\end{subfigure}
%
%
%
%
%\caption{\defender's sensing strategy ${\sigma}^1$ (top) and \attacker's attack strategy ${\sigma}^2$ (bottom) for the example network in Fig.~\ref{Example1}.} \label{Strategies}
%\end{figure}
%
%
%
%Finally, we give an upper bound on the loss in detection performance by choosing our sensing strategy $\sigma^1$ (see Fig.~\ref{Strategies} (top)), instead of choosing an equilibrium strategy for \defender.
%%Indeed, we showed in Thm.~\ref{Prop_interim} that an equilibrium sensing strategy maximinimizes the expected detection rate. 
%It turns out that, with 3 sensors, $\sigma^1$ detects at least $\frac{3}{4}$ of the failures, regardless of \attacker's strategy (Prop.~\ref{robust_r}), while in equilibrium $\frac{6}{7}$ of the failures are detected (Table~\ref{r_sigma_example}). Thus,  the loss in detection performance is $12.5\,\%$. This exact calculation is possible only because, for this simple example, we can solve \lpo and \lpt and compute the expected detection rate in equilibrium. In contrast, Prop.~\ref{robust_r} provides  an upper bound on the loss in detection performance without solving \lpo and \lpt, but instead by computing $\smsc$ and $\semm$ from \eqref{IP1} and \eqref{IP2}. This upper bound is given  by $1 - \frac{\max\{b_1^\prime,\semm\}}{\smsc} = 25\,\%$. In the next two sections, we formalize these results.
%
%
%

\ifadditional
\section{A Simple Example}\label{example_detection_sensing}

%\begin{example}%[MSC and MCS]


%%%---------------------------------------------------------------------------------------------------
\def \sizefig {1.4cm}
\def \scalefig {\small}
\def \innersepfig {0.07cm}
%%%---------------------------------------------------------------------------------------------------

%\begin{figure}[ht]
%\centering
%{\scalefig
%\begin{tikzpicture}[-,auto,x=\sizefig, y=\sizefig,
%  thick,main node/.style={circle,draw,inner sep = \innersepfig,black},main node2/.style={circle,black,draw,fill=blue!60,inner sep = \innersepfig},flow_a/.style ={gray!100}]
%\tikzstyle{edge} = [draw,thick,-,black]
%\tikzstyle{cut} = [draw,very thick,-]
%\tikzstyle{match} = [draw,very thick,black,-, dashed]
%\tikzstyle{flow} = [draw,line width = 1.5pt,->,gray!100]
%
%%\begin{scope}[yshift=0, xshift =-110]
%	\node[main node] (1) at (0,2) {$i_1$};
%	\node[main node] (2) at (1,2) {$i_2$};
%	\node[main node2] (3) at (2,2) {$i_3$};
%	\node[main node] (4) at (1,1) {$i_4$};
%	\node[main node] (5) at (2,1) {$i_5$};
%	\node[main node] (6) at (0,0) {$i_6$};
%	\node[main node] (7) at (1,0) {$i_7$};
%	\node[main node] (8) at (2,0) {$i_8$};
%	%\node[main node, draw=white] (7) at (3.5,-0.5) {\textbf{a}};
%	
%	\path[edge]	
%	%(2) edge (5)
%	%(1) edge  (2)
%	(1) edge node[left]{$e_3$} (6)
%	(4) edge node {$e_6$} (5)
%	(2) edge[double,blue!80]  node {$e_2$} (3)
%	(2) edge node[left] {$e_4$} (4)
%	(6) edge node[below] {$e_9$} (7)
%	(7) edge node[below] {$e_{10}$} (8)
%	%(3) edge  (5)	
%	%(4) edge  (6)
%	(5) edge node {$e_8$} (8);
%
%	\path[edge]
%	(1) edge[double,blue!80] node {$e_1$} (2)
%	(3) edge[double,blue!80] node {$e_5$} (5)
%	(4) edge node[left] {$e_7$} (7);
%%\end{scope}
%
%\end{tikzpicture}}
%
%\caption{Example network. The monitoring set $\set{i_3} = \{e_1,e_2,e_5\}$ is represented by the double blue edges.} \label{Example1}
%\end{figure}



Consider the problem \ECOP with the target expected detection rate $\alpha = 0.75$ and the number of attack resources $b_2 = 2$. For this small-sized problem, we can solve  \lpo and \lpt to compute the NE of $\Gamma$, and obtain  the expected detection rate in any NE for each $b_1 \in \mathbb{N}$; see Table~\ref{r_sigma_example}. Notice that for a given $b_1$, the expected detection rate is the same in any NE; this property is shown in Thm.~\ref{bounds_game}.
\begin{table}[htbp]
\centering
\caption{Expected detection rate in equilibrium for every $b_1 \in \mathbb{N}$.}
\def\arraystretch{\spacingtable}
\begin{tabular}{|c|c|c|c|c|c|}\hline $b_1$ & 0 & 1 & 2 & 3 & $\geq 4$ \\\hline $\sdet{*}$ & 0 & $\frac{2}{7}$ & $\frac{4}{7}$ & $\frac{6}{7}$ & 1 \\\hline \end{tabular}
\label{r_sigma_example}
\end{table}

From Table~\ref{r_sigma_example}, we conclude that the optimal value of (\hyperlink{(P)}{$\mathcal{P}$}) is $b_1^\dag = 3$, i.e., with  $3$ sensors, \defender is capable of detecting $\frac{6}{7} \geq \alpha$ of the failure events in equilibrium. However, as mentioned in Section~\ref{sec:Formal problem}, this method does not extend to larger networks, as it requires solving large \lpo and \lpt for each $b_1 \in \mathbb{N}$ and checking if the constraint on the expected detection rate in any equilibrium \eqref{all_NE} is met.



%\tb{For the network in Fig.~\ref{Example1} and its sensing model, a solution of (\hyperlink{(MSC)}{MSC}) is given by $\{i_3,i_4,i_6,i_8\} \in \msc$ and a solution of (\hyperlink{(MSP)}{MSP}) is $\{e_3,e_4,e_8\} \in \emm$. Thus, $\smsc = 4$ and $\semm = 3$. }


%We now propose the following approach: First, we solve (\hyperlink{(MSC)}{MSC}); an optimal solution is given by  $\Def^{min} = \{i_3,i_6,i_4,i_8\}$. Second, given $b_1$ sensors between $0$ and $|\Def^{min}|$, we randomize the placement of these $b_1$ sensors over subsets of $\Def^{min}$ such that each node in $\Def^{min}$ is sensed with an identical probability. Then, as we will show in Section~\ref{general}, such a sensing strategy guarantees that regardless of which strategy \attacker chooses, the expected detection rate will be at least $\frac{b_1}{|\Def^{min}|}$. Thus, by choosing 3 sensors, our sensing strategy ensures that $0.75\geq \alpha$ of the failure events be detected. Thm.~\ref{bounds_game} implies that, in this example, with 3 sensors, the expected detection rate in \emph{any} equilibrium of the resulting game is at least $\alpha$. Therefore, for this example, our method provides a feasible solution of \ECOP which turned out to be the optimal one ($b_1^* = 3$). 

Now consider another approach that is based on our results in Sections~\ref{general} and \ref{sec:Answer}: First, by solving (\hyperlink{(MSC)}{$\mathcal{I}_{\text{MSC}}$}), we obtain an MSC given by  $\Def^{min} = \{i_3,i_4,i_6,i_8\}$; thus $\smsc = 4$. Then, from Thm.~\ref{bounds_game},  we know that the expected detection rate in any equilibrium is lower bounded by $\frac{b_1}{\smsc}$. Thus, with $b_1^\prime:=\lceil \alpha \smsc \rceil = 3$ sensors, the expected detection rate in any equilibrium is at least $\alpha$.

Secondly, by solving (\hyperlink{(MSP)}{$\mathcal{I}_{\text{MSP}}$}), we obtain an MSP given by $\att^{max} = \{e_3,e_4,e_8\}$; thus $\semm = 3$. Then, from Thm.~\ref{bounds_game}, we know that the expected detection rate in any equilibrium is upper bounded by $\frac{b_1}{\semm}$, which implies that if $b_1< \lceil \alpha \semm \rceil$, the equilibrium constraints \eqref{all_NE} are not satisfied. This enables us  to deduce that an optimality gap associated with $b_1^\prime$ is given by $\lceil \alpha \smsc\rceil - \lceil \alpha \semm \rceil$ (Proposition~\ref{Prop_interim}). In fact, for this example, we obtain that the optimality gap is $\lceil 3\rceil - \lceil 2.25 \rceil = 0$. Therefore, by solving (\hyperlink{(MSC)}{$\mathcal{I}_{\text{MSC}}$}) and (\hyperlink{(MSP)}{$\mathcal{I}_{\text{MSP}}$}), we can estimate the number of sensing resources to ensure that the equilibrium constraints in \ECOP are satisfied; furthermore, we can verify that this number is optimal for this example, i.e., $b_1^\prime = b_1^\dag = 3$.

Thirdly, given $b_1^\prime=3$ and $b_2 =2$, we can use $\Def^{min}$ and $\att^{max}$ to construct an approximate NE. Using Lemma~\ref{algebra2}, we construct a strategy profile ${\sigma} = (\sigma^1,{\sigma}^2)$, where ${\sigma}^1_{\{i_3,i_4,i_6\}} = {\sigma}^1_{\{i_8,i_3,i_4\}}  =  {\sigma}^1_{\{i_6, i_8,i_3\}}  = {\sigma}^1_{\{i_4,i_6,i_8\}}  = \frac{1}{4}$, and ${\sigma}^2_{\{e_3,e_4\}} = {\sigma}^2_{\{e_8,e_3\}} = {\sigma}^2_{\{e_4,e_8\}}  =  \frac{1}{3}$; $\sigma$ is illustrated in Fig.~\ref{Strategies}. From Thm.~\ref{MSC-MSP-eNE}, we obtain that the above-constructed strategy profile ${\sigma}$ is an $\epsilon-$NE, and provides each player a payoff that is $\epsilon-$close to their equilibrium payoff, with $\epsilon=  b_1^\prime b_2\left( \frac{1}{\max\{b_1^\prime,\semm\}} - \frac{1}{\smsc}\right) = \frac{1}{2}$. Indeed, from \lpo and \lpt, we can deduce that \defender and \attacker's equilibrium payoffs in the game $\Gamma$ are $\frac{12}{7}$ and $\frac{2}{7}$ respectively, while our strategy profile $\sigma$ provides them with the respective payoffs $\frac{3}{2}$ and $\frac{1}{2}$. One can easily check that $\sigma$ gives each player a payoff that is $\frac{3}{14} \ (\leq \epsilon)$ close to their equilibrium payoff.

% and the influence matrix can be written as follows:
%\begin{align*}
%\boldsymbol{F} = {\arraycolsep=3.5pt
%	\kbordermatrix{&\mbox{$e_1$}&\mbox{$e_2$}&\mbox{$e_3$}&\mbox{$e_4$}&\mbox{$e_5$} &\mbox{$e_6$} & \mbox{$e_7$} & \mbox{$e_8$}\\
%\mbox{$i_1$}&1 & 1 & 0 & 1 & 1 & 0 &0 &0 \\
%	\mbox{$i_2$}&1 & 0 & 1 & 1 & 0 & 0&0 &0  \\
%	\mbox{$i_3$}&0 & 1 & 1 & 0 & 1 & 0 &0 &0\\
%	\mbox{$i_4$}&0 & 0 & 0 & 1 & 0 & 1 &1 &0\\
%	\mbox{$i_5$}&0 & 0 & 0 & 0 & 1 & 1 &0 &1 \\
%	\mbox{$i_6$}&0 & 0 & 0 & 0 & 0 & 0&1 &1
%}}.
%\end{align*}
\begin{figure}[ht]
\centering
\begin{subfigure}[b]{0.23\textwidth}
\centering
{\scalefig
\begin{tikzpicture}[-,auto,x=\sizefig, y=\sizefig,
  thick,main node/.style={circle,draw,inner sep = \innersepfig,black},main node2/.style={circle,black,draw,fill=blue!60,inner sep = \innersepfig},flow_a/.style ={gray!100}]
\tikzstyle{edge} = [draw,thick,-,black]
\tikzstyle{cut} = [draw,very thick,-]
\tikzstyle{match} = [draw,very thick,black,-, dashed]
\tikzstyle{flow} = [draw,line width = 1.5pt,->,gray!100]

%\begin{scope}[yshift=0, xshift =-110]
	\node[main node] (1) at (0,2) {$i_1$};
	\node[main node] (2) at (1,2) {$i_2$};
	\node[main node2] (3) at (2,2) {$i_3$};
	\node[main node2] (4) at (1,1) {$i_4$};
	\node[main node] (5) at (2,1) {$i_5$};
	\node[main node2] (6) at (0,0) {$i_6$};
	\node[main node] (7) at (1,0) {$i_7$};
	\node[main node] (8) at (2,0) {$i_8$};
	%\node[main node, draw=white] (7) at (3.5,-0.5) {\textbf{a}};
	
	\path[edge]	
	%(2) edge (5)
	%(1) edge  (2)
	(1) edge node[left]{$e_3$} (6)
	(4) edge node {$e_6$} (5)
	(2) edge  node {$e_2$} (3)
	(2) edge node[left] {$e_4$} (4)
	(6) edge node[below] {$e_9$} (7)
	(7) edge node[below] {$e_{10}$} (8)
	%(3) edge  (5)	
	%(4) edge  (6)
	(5) edge node {$e_8$} (8);

	\path[edge]
	(1) edge node {$e_1$} (2)
	(3) edge node {$e_5$} (5)
	(4) edge node[left] {$e_7$} (7);
%\end{scope}

\end{tikzpicture}}

\caption{${\sigma}^1_{\{i_3,i_4,i_6\}} = \frac{1}{4}$.} 
\end{subfigure}
~
\begin{subfigure}[b]{0.23\textwidth}
\centering
{\scalefig
\begin{tikzpicture}[-,auto,x=\sizefig, y=\sizefig,
  thick,main node/.style={circle,draw,inner sep = \innersepfig,black},main node2/.style={circle,black,draw,fill=blue!60,inner sep = \innersepfig},flow_a/.style ={gray!100}]
\tikzstyle{edge} = [draw,thick,-,black]
\tikzstyle{cut} = [draw,very thick,-]
\tikzstyle{match} = [draw,very thick,black,-, dashed]
\tikzstyle{flow} = [draw,line width = 1.5pt,->,gray!100]

%\begin{scope}[yshift=0, xshift =-110]
	\node[main node] (1) at (0,2) {$i_1$};
	\node[main node] (2) at (1,2) {$i_2$};
	\node[main node2] (3) at (2,2) {$i_3$};
	\node[main node2] (4) at (1,1) {$i_4$};
	\node[main node] (5) at (2,1) {$i_5$};
	\node[main node] (6) at (0,0) {$i_6$};
	\node[main node] (7) at (1,0) {$i_7$};
	\node[main node2] (8) at (2,0) {$i_8$};
	%\node[main node, draw=white] (7) at (3.5,-0.5) {\textbf{a}};
	
	\path[edge]	
	%(2) edge (5)
	%(1) edge  (2)
	(1) edge node[left]{$e_3$} (6)
	(4) edge node {$e_6$} (5)
	(2) edge  node {$e_2$} (3)
	(2) edge node[left] {$e_4$} (4)
	(6) edge node[below] {$e_9$} (7)
	(7) edge node[below] {$e_{10}$} (8)
	%(3) edge  (5)	
	%(4) edge  (6)
	(5) edge node {$e_8$} (8);

	\path[edge]
	(1) edge node {$e_1$} (2)
	(3) edge node {$e_5$} (5)
	(4) edge node[left] {$e_7$} (7);
%\end{scope}

\end{tikzpicture}}

\caption{${\sigma}^1_{\{i_8,i_3,i_4\}} = \frac{1}{4}$.} 
\end{subfigure}
~
\begin{subfigure}[b]{0.23\textwidth}
\centering
{\scalefig
\begin{tikzpicture}[-,auto,x=\sizefig, y=\sizefig,
  thick,main node/.style={circle,draw,inner sep = \innersepfig,black},main node2/.style={circle,black,draw,fill=blue!60,inner sep = \innersepfig},flow_a/.style ={gray!100}]
\tikzstyle{edge} = [draw,thick,-,black]
\tikzstyle{cut} = [draw,very thick,-]
\tikzstyle{match} = [draw,very thick,black,-, dashed]
\tikzstyle{flow} = [draw,line width = 1.5pt,->,gray!100]

%\begin{scope}[yshift=0, xshift =-110]
	\node[main node] (1) at (0,2) {$i_1$};
	\node[main node] (2) at (1,2) {$i_2$};
	\node[main node2] (3) at (2,2) {$i_3$};
	\node[main node] (4) at (1,1) {$i_4$};
	\node[main node] (5) at (2,1) {$i_5$};
	\node[main node2] (6) at (0,0) {$i_6$};
	\node[main node] (7) at (1,0) {$i_7$};
	\node[main node2] (8) at (2,0) {$i_8$};
	%\node[main node, draw=white] (7) at (3.5,-0.5) {\textbf{a}};
	
	\path[edge]	
	%(2) edge (5)
	%(1) edge  (2)
	(1) edge node[left]{$e_3$} (6)
	(4) edge node {$e_6$} (5)
	(2) edge  node {$e_2$} (3)
	(2) edge node[left] {$e_4$} (4)
	(6) edge node[below] {$e_9$} (7)
	(7) edge node[below] {$e_{10}$} (8)
	%(3) edge  (5)	
	%(4) edge  (6)
	(5) edge node {$e_8$} (8);

	\path[edge]
	(1) edge node {$e_1$} (2)
	(3) edge node {$e_5$} (5)
	(4) edge node[left] {$e_7$} (7);
%\end{scope}

\end{tikzpicture}}

\caption{${\sigma}^1_{\{i_6,i_8,i_3\}} = \frac{1}{4}$.} 
\end{subfigure}
~
\begin{subfigure}[b]{0.23\textwidth}
\centering
{\scalefig
\begin{tikzpicture}[-,auto,x=\sizefig, y=\sizefig,
  thick,main node/.style={circle,draw,inner sep = \innersepfig,black},main node2/.style={circle,black,draw,fill=blue!60,inner sep = \innersepfig},flow_a/.style ={gray!100}]
\tikzstyle{edge} = [draw,thick,-,black]
\tikzstyle{cut} = [draw,very thick,-]
\tikzstyle{match} = [draw,very thick,black,-, dashed]
\tikzstyle{flow} = [draw,line width = 1.5pt,->,gray!100]

%\begin{scope}[yshift=0, xshift =-110]
	\node[main node] (1) at (0,2) {$i_1$};
	\node[main node] (2) at (1,2) {$i_2$};
	\node[main node] (3) at (2,2) {$i_3$};
	\node[main node2] (4) at (1,1) {$i_4$};
	\node[main node] (5) at (2,1) {$i_5$};
	\node[main node2] (6) at (0,0) {$i_6$};
	\node[main node] (7) at (1,0) {$i_7$};
	\node[main node2] (8) at (2,0) {$i_8$};
	%\node[main node, draw=white] (7) at (3.5,-0.5) {\textbf{a}};
	
	\path[edge]	
	%(2) edge (5)
	%(1) edge  (2)
	(1) edge node[left]{$e_3$} (6)
	(4) edge node {$e_6$} (5)
	(2) edge  node {$e_2$} (3)
	(2) edge node[left] {$e_4$} (4)
	(6) edge node[below] {$e_9$} (7)
	(7) edge node[below] {$e_{10}$} (8)
	%(3) edge  (5)	
	%(4) edge  (6)
	(5) edge node {$e_8$} (8);

	\path[edge]
	(1) edge node {$e_1$} (2)
	(3) edge node {$e_5$} (5)
	(4) edge node[left] {$e_7$} (7);
%\end{scope}

\end{tikzpicture}}

\caption{${\sigma}^1_{\{i_4,i_6,i_8\}} = \frac{1}{4}$.} 
\end{subfigure}

\medskip

\begin{subfigure}[b]{0.3\textwidth}
\centering
{\scalefig
\begin{tikzpicture}[-,auto,x=\sizefig, y=\sizefig,
  thick,main node/.style={circle,draw,inner sep = \innersepfig,black},main node2/.style={circle,black,draw,fill=Green,inner sep = 0.08cm},flow_a/.style ={gray!100}]
\tikzstyle{edge} = [draw,thick,-,black]
\tikzstyle{cut} = [draw,very thick,-]
\tikzstyle{match} = [draw,very thick,black,-, dashed]
\tikzstyle{flow} = [draw,line width = 1.5pt,->,gray!100]

%\begin{scope}[yshift=0, xshift =-110]
	\node[main node] (1) at (0,2) {$i_1$};
	\node[main node] (2) at (1,2) {$i_2$};
	\node[main node] (3) at (2,2) {$i_3$};
	\node[main node] (4) at (1,1) {$i_4$};
	\node[main node] (5) at (2,1) {$i_5$};
	\node[main node] (6) at (0,0) {$i_6$};
	\node[main node] (7) at (1,0) {$i_7$};
	\node[main node] (8) at (2,0) {$i_8$};
	%\node[main node, draw=white] (7) at (3.5,-0.5) {\textbf{a}};
	
	\path[edge]	
	%(2) edge (5)
	%(1) edge  (2)
	(1) edge node[left = 0.1cm]{$e_3$} (6)
	(4) edge node {$e_6$} (5)
	(2) edge  node {$e_2$} (3)
	(2) edge node[left = 0.1cm] {$e_4$} (4)
	(6) edge node[below] {$e_9$} (7)
	(7) edge node[below] {$e_{10}$} (8)
	%(3) edge  (5)	
	%(4) edge  (6)
	(5) edge node {$e_8$} (8);

	\path[edge]
	(1) edge node {$e_1$} (2)
	(3) edge node {$e_5$} (5)
	(4) edge node[left] {$e_7$} (7);
%\end{scope}

	\node(12) at (0,1) {\textcolor{Red}{\Huge{\Cross}}};
	\node(13) at (1,1.5) {\textcolor{Red}{\Huge{\Cross}}};

\end{tikzpicture}}

\caption{${\sigma}^2_{\{e_3,e_4\}} = \frac{1}{3}$.}
\end{subfigure}
~
\begin{subfigure}[b]{0.3\textwidth}
\centering
{\scalefig
\begin{tikzpicture}[-,auto,x=\sizefig, y=\sizefig,
  thick,main node/.style={circle,draw,inner sep = \innersepfig,black},main node2/.style={circle,black,draw,fill=Green,inner sep = 0.08cm},flow_a/.style ={gray!100}]
\tikzstyle{edge} = [draw,thick,-,black]
\tikzstyle{cut} = [draw,very thick,-]
\tikzstyle{match} = [draw,very thick,black,-, dashed]
\tikzstyle{flow} = [draw,line width = 1.5pt,->,gray!100]

%\begin{scope}[yshift=0, xshift =-110]
	\node[main node] (1) at (0,2) {$i_1$};
	\node[main node] (2) at (1,2) {$i_2$};
	\node[main node] (3) at (2,2) {$i_3$};
	\node[main node] (4) at (1,1) {$i_4$};
	\node[main node] (5) at (2,1) {$i_5$};
	\node[main node] (6) at (0,0) {$i_6$};
	\node[main node] (7) at (1,0) {$i_7$};
	\node[main node] (8) at (2,0) {$i_8$};
	%\node[main node, draw=white] (7) at (3.5,-0.5) {\textbf{a}};
	
	\path[edge]	
	%(2) edge (5)
	%(1) edge  (2)
	(1) edge node[left = 0.1cm]{$e_3$} (6)
	(4) edge node {$e_6$} (5)
	(2) edge  node {$e_2$} (3)
	(2) edge node[left] {$e_4$} (4)
	(6) edge node[below] {$e_9$} (7)
	(7) edge node[below] {$e_{10}$} (8)
	%(3) edge  (5)	
	%(4) edge  (6)
	(5) edge node[right = 0.1cm] {$e_8$} (8);

	\path[edge]
	(1) edge node {$e_1$} (2)
	(3) edge node {$e_5$} (5)
	(4) edge node[left] {$e_7$} (7);
%\end{scope}
\node(12) at (0,1) {\textcolor{Red}{\Huge{\Cross}}};
	\node(13) at (2,0.5) {\textcolor{Red}{\Huge{\Cross}}};
\end{tikzpicture}}

\caption{${\sigma}^2_{\{e_8,e_3\}} = \frac{1}{3}$.} 
\end{subfigure}
~
\begin{subfigure}[b]{0.3\textwidth}
\centering
{\scalefig
\begin{tikzpicture}[-,auto,x=\sizefig, y=\sizefig,
  thick,main node/.style={circle,draw,inner sep = \innersepfig,black},main node2/.style={circle,black,draw,fill=Green,inner sep = 0.08cm},flow_a/.style ={gray!100}]
\tikzstyle{edge} = [draw,thick,-,black]
\tikzstyle{cut} = [draw,very thick,-]
\tikzstyle{match} = [draw,very thick,black,-, dashed]
\tikzstyle{flow} = [draw,line width = 1.5pt,->,gray!100]

%\begin{scope}[yshift=0, xshift =-110]
	\node[main node] (1) at (0,2) {$i_1$};
	\node[main node] (2) at (1,2) {$i_2$};
	\node[main node] (3) at (2,2) {$i_3$};
	\node[main node] (4) at (1,1) {$i_4$};
	\node[main node] (5) at (2,1) {$i_5$};
	\node[main node] (6) at (0,0) {$i_6$};
	\node[main node] (7) at (1,0) {$i_7$};
	\node[main node] (8) at (2,0) {$i_8$};
	%\node[main node, draw=white] (7) at (3.5,-0.5) {\textbf{a}};
	
	\path[edge]	
	%(2) edge (5)
	%(1) edge  (2)
	(1) edge node[left]{$e_3$} (6)
	(4) edge node {$e_6$} (5)
	(2) edge  node {$e_2$} (3)
	(2) edge node[left = 0.1cm] {$e_4$} (4)
	(6) edge node[below] {$e_9$} (7)
	(7) edge node[below] {$e_{10}$} (8)
	%(3) edge  (5)	
	%(4) edge  (6)
	(5) edge node[right = 0.1cm] {$e_8$} (8);

	\path[edge]
	(1) edge node {$e_1$} (2)
	(3) edge node {$e_5$} (5)
	(4) edge node[left] {$e_7$} (7);
%\end{scope}
\node(12) at (2,0.5) {\textcolor{Red}{\Huge{\Cross}}};
	\node(13) at (1,1.5) {\textcolor{Red}{\Huge{\Cross}}};
\end{tikzpicture}}

\caption{${\sigma}^2_{\{e_4,e_8\}} = \frac{1}{3}$.}
\end{subfigure}




\caption{\defender's sensing strategy ${\sigma}^1$ (top) and \attacker's attack strategy ${\sigma}^2$ (bottom) for the example network in Fig.~\ref{Example1}.} \label{Strategies}
\end{figure}



Finally, we give an upper bound on the loss in detection performance by choosing our sensing strategy $\sigma^1$ (see Fig.~\ref{Strategies} (top)), instead of choosing an equilibrium strategy for \defender.
%Indeed, we showed in Thm.~\ref{Prop_interim} that an equilibrium sensing strategy maximinimizes the expected detection rate. 
It turns out that, with 3 sensors, $\sigma^1$ detects at least $\frac{3}{4}$ of the failures regardless of \attacker's strategy (Proposition~\ref{robust_r}), while in equilibrium $\frac{6}{7}$ of the failures are detected (Table~\ref{r_sigma_example}). Thus,  the loss in detection performance is $12.5\,\%$. This exact calculation is possible only because, for this  example, we can solve \lpo and \lpt and compute the value of the expected detection rate in equilibrium. In contrast,  Proposition~\ref{robust_r} provides  an upper bound on the loss in detection performance \emph{without} solving \lpo and \lpt, but instead by computing $\smsc$ and $\semm$ from \eqref{IP1} and \eqref{IP2}. This upper bound is given  by $1 - \frac{\max\{b_1^\prime,\semm\}}{\smsc} = 25\,\%$. In the next two sections, we formalize these results.

\else
\fi

\ifadditional
\section{Example}

Fig. \ref{fig:net1_msc_emm} shows the location of the $\Def^{min}$ nodes and the $\att^{max}$ pipelines for the break (left) and the contamination (right) scenarios.

%-Table-1 ---------------------------------
\begin{table}[htbp] \footnotesize
  \centering
  \caption{NE solution for the Apulian network with $b_1 = 2, b_2 = 2$.}
%\tabcolsep=0.11cm
%\renewcommand{\arraystretch}{1.1} 
    \begin{tabular}{|ccc|cc|ccc|cc|}
\hline
	%\rowcolor{gray!30}
\multicolumn{5}{|c|}{\textbf{Operator strategy}} &\multicolumn{5}{c|}{\textbf{Attacker strategy}}\\
	\hline
    \multicolumn{2}{|c}{\textbf{Support}} & \textbf{Probability}  & \textbf{Node basis} & \textbf{Probability} & \multicolumn{2}{c}{\textbf{Support}} & \textbf{Probability}  & \textbf{Edge basis} & \textbf{Probability} \\
 \multicolumn{2}{|c}{\boldmath{$\supp(\sigma^1)$}} & \boldmath{$\sigma^1_\Def$}  & \boldmath{$s_{\sigma^1}$} & \boldmath{$\nprob$} &  \multicolumn{2}{c}{\boldmath{$\supp(\sigma^2)$}} & \boldmath{$\sigma^2_\Def$}  & \boldmath{$s_{\sigma^2}$} & \boldmath{$\eprob$}  \\
\hline
    1     & 8         & 0.286   & 1     & 0.286 &   5     	& 34    & 0.143  		&5     	& 0.143\\
    6     & 21         & 0.036  & 6     & 0.071 & 10     & 31   & 0.143 		& 10     & 0.143\\
    6     & 23         & 0.036  & 7     & 0.214 & 13     & 15   & 0.286  		& 13    & 0.286\\
    7     &9        & 0.071  & 8    & 0.286 & 28     & 30 	 & 0.286  	& 15     & 0.286\\
    7     & 11         & 0.071   & 9    & 0.214 & 29    	& 32       & 0.143  	& 28  	& 0.286 \\
    7     & 17        & 0.071   & 10    & 0.107 & &       	&   			& 29    & 0.143 \\
    9     & 23        & 0.143   & 11    & 0.071 & &         	&   			& 30    & 0.286\\
    10     & 17        & 0.107   &  12     &  0.107 & &          &       		& 31    & 0.143 \\
    12     & 17      & 0.107  &  13     &  0.071 & &          &       		& 32    & 0.143\\
    13     & 21        & 0.071  &  17     &  0.286 &  &           &       		& 34    & 0.143 \\
          &       &       &        21     &  0.107 &&&&&\\
          &       &       &       23     &  0.179 &&&&& \\ 
\hline
    \end{tabular}\\
%\scriptsize{NSP - node sensing probability; EAP - edge attack probability}
  \label{tab:1}%
\end{table}%



%-Table-2 ---------------------------------
\begin{table}[htbp] \footnotesize
  \centering
  \caption{Equilibrium properties for the Apulian network with $b_1 = 2, b_2 = 2$.}
%\tabcolsep=0.11cm
%\renewcommand{\arraystretch}{1.1} 
    \begin{tabular}{|ccc|cc|ccc|cc|}
\hline
	%\rowcolor{gray!30} 
\multicolumn{5}{|c|}{\textbf{Operator strategy}} &\multicolumn{5}{c|}{\textbf{Attacker strategy}}\\
	\hline
    \multicolumn{2}{|c}{\textbf{Support}} & \textbf{Probability}  & \textbf{Node basis} & \textbf{Probability} & \multicolumn{2}{c}{\textbf{Support}} & \textbf{Probability}  & \textbf{Link basis} & \textbf{Probability} \\
 \multicolumn{2}{|c}{\boldmath{$\supp(\sigma^1)$}} & \boldmath{$\sigma^1_\Def$}  & \boldmath{$s_{\sigma^1}$} & \boldmath{$\nprob$} &  \multicolumn{2}{c}{\boldmath{$\supp(\sigma^2)$}} & \boldmath{$\sigma^2_\Def$}  & \boldmath{$s_{\sigma^2}$} & \boldmath{$\eprob$}  \\
\hline
     1     & 8         & 0.5   & 1     & 0.5 &   13     	& 30    & 0.333  		&13     	& 0.667\\
    10     & 23         & 0.5  & 8     & 0.5 & 13     & 34   & 0.333 		& 30     & 0.667 \\
    &          &   & 10     & 0.5 & 30     & 34   & 0.333  		& 34   & 0.667\\
    &      &  & 23    & 0.5 &&&&&\\
\hline
    \end{tabular}\\
%\scriptsize{NSP - node sensing probability; EAP - edge attack probability}
  \label{tab:2}%
\end{table}%

\begin{figure}
        \centering
        \begin{subfigure}[b]{0.45\textwidth} \centering
              \includegraphics[trim = 60mm 30mm 50mm 30mm, clip,scale = 0.4]{or_fig35burst.pdf}
       \caption{Pipeline break}  \label{fig:net1_msc_emm_burst}
        \end{subfigure}
        ~ 
        \begin{subfigure}[b]{0.45\textwidth} \centering
               \includegraphics[trim = 60mm 30mm 50mm 30mm, clip,scale = 0.4]{or_fig35contamination.pdf}       
		\caption{Contaminant intrusion}   \label{fig:net1_msc_emm_cont}  
        \end{subfigure}
       \caption{$\Def^{min}$ and $\att^{max}$ for the Apulian water network. The labeled links indicate the links in a $\att^{max}$ and the labeled nodes indicate the nodes in a $\Def^{min}$.}   \label{fig:net1_msc_emm}

\end{figure}

\tr{Hence, to solve \ECOP  we compute a NE of the game $\Gamma$ for each $b_1 \in \mathbb{N}$, and compute the expected detection rate $\sdet{*}$. One NE solution of $\Gamma$ given $b_1 = 2, b_2 = 2$ for the pipeline break scenario is listed in Table \ref{tab:1}. %At equilibrium, the payoff of \defender is equal to 1.43 and of \attacker is equal to 0.857. 
Table \ref{tab:1} lists the supports, the bases, and their corresponding probability for the operator (columns one and two) and for the attacker (columns three and four). Result show that the node basis spans 12 nodes, which implies that the operator will have to shift between 12 different locations in the network.  }



We use the solutions to (\hyperlink{(MSC)}{$\mathcal{I}_{\text{MSC}}$}) and (\hyperlink{(MSP)}{$\mathcal{I}_{\text{MSP}}$}) to derive an approximate solution of \ECOP according to Proposition~\ref{Prop_interim}. In the pipeline break scenario, we have $\smsc  = 4 > \semm = 3$. Restricting support of the operator to $\Def^{min}$ and the support of the attacker to $\att^{max}$, the strategy profile is the solution to the two relaxed linear programs, $LP_{S'}$ and $LP_{T'}$ (Propositions \ref{best_set_cover} and \ref{best_maximum_matching}). The solution of the two linear programs is listed in Table \ref{tab:2}, showing the node and component bases and the corresponding sensing probability. For example, the operator should equally shift between sensing nodes $\{1, 8\}$ and nodes $\{10, 23\}$. The attacker should equally shift between pipelines $\{13,20\}$, $\{13,34\}$, and $\{30,34\}$. Under this strategy, all the nodes in the MSC are monitored with equal probability, $\rho_{\sigma^{\Def}}(i) = \frac{b_1}{n}=\frac{2}{4}=0.5$, as well as all the pipes in MSP are disrupted with equal probability, $\rho_{\sigma^{\att}}(e) = \frac{b_2}{m}=\frac{2}{3}= 0.667$ (see Lemma \ref{algebra1}). %Based on this strategy, the payoffs for the players are $u_1 = 1 \text{ and } u_2 = 0.667$, for $\defender$ and $\attacker$, respectively (Theorem \ref{bounds_game}). %In fact, for 6 out of the 13 networks, the equality $\smsc =\semm$ is satisfied; thus we have an optimal solution of \ECOP for these networks (Proposition~\ref{Cor2}).
Using Theorem \ref{bounds_game}, we evaluate the upper and lower bounds of the expected detection rate as a function of $b_1$ (see Fig. ~\ref{fig:net1_15}) of our approximate NE. Our estimate of the number of sensors required to achieve a targeted detection rate is close to the \textit{optimal} value. 



\else
\fi

==> S1_Introduction_Mathieu.tex <==
%!TEX root = OR Manuscript V23.tex
\section{Introduction}\label{sec:intro}

%\subsection{Network Monitoring Problem}
%\subsection{Motivation}


Inspection systems for monitoring critical infrastructure networks play a crucial role in ensuring the availability and quality of essential services that rely on these networks. These systems are responsible for providing situational awareness to the distribution utilities, who are tasked with maintaining the functional state and service quality of their expansive assets. Reliability issues resulting from the deterioration of age-old infrastructure \citep{Jackson2014}, combined with threats from malicious entities such as fraudulent customers and social miscreants pose significant problems for today's resource-constrained utilities \citep{Physical2016}. Moreover, recent cyber incidents confirm that external hackers and adversarial nation states are capable of sabotaging critical network components in a strategic manner \citep{Dancy2017,Cyber2018}. Such attacks, if successful, can result in prolonged service interruptions, and even pose a direct risk to human lives. Thus, utilities companies and their customers can directly benefit from better information systems designed for detecting a variety of incidents, both random and adversarial.  
%\citep{}

%Security of physical infrastructures such as water distribution, power grids, and gas and oil transmission networks, is crucial for ensuring the availability and quality of the essential services that rely on these networks. However, recent incidents have confirmed that infrastructure networks continue to be attractive targets for adversarial entities, including malicious insiders, external hackers, and even nation states . \maybe{In some situations, these entities can use physical or remote access points to compromise multiple network components   in a strategic manner . Such an attack, if successful, can result in prolonged service interruptions and incur significant economic losses.} Thus, infrastructure operators and utilities face an important task of maintaining adequate situation awareness in the presence of security attacks. 
%Infrastructure networks fortified by sensing technologies has been identified as one of the primary mechanisms towards resilient infrastructure systems. Driven by sensing technologies, monitoring of infrastructure networks has been identified as primary mechanism for securing modern infrastructure.

Consider the inspection problem faced by a utility company (typically a regulated monopoly) who manages a natural gas pipeline network in an urban area. Traditionally, utility personnel conduct inspections of network assets and customer connections at a predetermined frequency (once every 2-3 years), or when an emergency situation is reported \citep{Inspect2015}. Issues such as service interruptions, minor gas leaks, and faulty/illegal line connections are addressed by the utility with varying degrees of response rates, and notifications are filed with the regulator retroactively. However, these traditional inspection systems, based on manual checks and ex-post  reporting, are very limited with regards to three aspects: 

\begin{enumerate}
\item[1)] Minor incidents (leaks) occasionally evolve to become major disruptions. However, the current inspection operations tend to prioritize major components such as main lines and valve stations. As a result, the detection of minor leaks is delayed, often causing significant damages in the future.
%
%Some secondary distribution points are less frequently inspected, which occasionally results in minor leaks evolving to become major disruptions. Thus,
%
% often due to delayed detection and response by utility personnel. Thus, inspecting most often the major components such as main line and valve stations is not adequate, as failures of remote distribution points can also cause substantive damages.

\item[2)] Physical or remote access to critical components can be exploited by malicious entities. These entities may use a combination of physical and digital tampering to bypass safety systems. However, inspection systems typically do not account for strategic and resourceful attackers whose actions are more difficult to detect, in comparison to isolated random failures. 
 
\item[3)] Utility companies are the primary entities responsible for network monitoring and incident response. The regulator has various degrees of oversight on utilities' response to reported incidents, but the guidelines on proactive inspection are relatively sparse. Thus, the existing regulatory framework can benefit from inspection systems that provide better sensing and reporting capabilities. 

%
% and ensuring the quality of service. Typically, the regulators do not have adequate resources to conduct extensive audits and compliance checks. Thus, utilities companies  companies inspection systems should enable filing of timely and specific details about relevant incidents by the utility company to the regulator.


\end{enumerate}




Fortunately, recent advances in sensing technologies have resulted in commercially available smart detector systems, which include a sensor, a detection software, and a communication unit \citep{1219475,Fischer2017}. These detectors can be easily operated by the utility personnel and flexibly positioned in the network to meet target inspection goals. 
By adopting smart detectors in their inspection operations, the utilities can at least partly address the aforementioned limitations \citep{PGE2010}.
Our article is motivated by this technological trend; in particular, the need to enhance the capabilities of traditional inspection systems through the use of smart  detectors, and achieve a target level of detection performance against incidents, including strategic attacks. We consider a game-theoretic formulation of the strategic network inspection problem, and address the question: \emph{How many detectors are required and how to strategically position them in the network to detect multiple adversarial attacks?} Our formulation is also relevant to a range of applications, as listed in Table~\ref{List_app}.



%Fortunately, recent advances in modern sensing technologies provide new capabilities for monitoring network components by way of detecting the physical disturbances that can result from failure events. For example, wireless sensor networks have been successfully used in the monitoring of water networks \citep{Stoianov:2007:PWS:1236360.1236396,allen:smart}. These sensors provide timely and accurate data to enable the detection of possible pipeline breaks and contamination events \citep{PERELMAN20134217}. Sensor networks are also being utilized to monitor oil and natural gas networks \citep{s120100189}.  These sensing technologies often come with flexible scheduling and remote monitoring capabilities, which are important for timely detection of failure events. 

%A particularly interesting feature of these sensing technologies is their ability to be remotely configured, and the ease with which they can be scheduled. Thus, the operator can use them for timely detection of a broad class of failure events.


 
%However, the allocation of these sensing resources is a challenging problem, especially when the failures can arise from strategic attacks. First, a strategic and resourceful attacker can simultaneously target multiple components in a manner which makes their detection more difficult, in comparison to isolated random failure events. Secondly, due to the cost of deploying sensors, the operator is typically constrained to use a small number of sensing resources, which is further limiting due to the large-scale nature of infrastructure networks. Thus, every network component cannot be simultaneously monitored, raising the possibility of attacks that can target components while avoiding detection \citep{Liu:2009:FDI:1653662.1653666,Parfomak2012,6303885}. Despite the recent progress on sensor placement problems, as well as strategic infrastructure defense, we lack a systematic approach to enable the allocation of sensing resources in large-scale networks, with guarantees on detection performance against strategic attacks. In this article, we address the following \emph{network monitoring problem}, which we denote $(\mathcal{P})$:  \emph{How many sensors are required and how to strategically place them in the infrastructure network to detect adversarial attacks?}



%This article is driven by the  


%cannot directly be applied to address this question, requiring new modeling and analysis techniques need to be developed, which we present in this article.


%to infrastructure network monitoring, as they do not account for any sensing model.

\subsection{Our Contributions}


In Section \ref{sec:form}, we introduce a generic detection model, which captures the key features of modern inspection systems with respect to sensing technology for event detection and flexibility of positioning. Mathematically, the model is represented by a monotone submodular detection function. We use this detection model to define a game-theoretic model of strategic interaction between a defender (inspection agency) and an attacker. The defender chooses where to position her detectors, and the attacker chooses to target one or more network components. Each player is resource-constrained. The defender's objective is to maximize the number of detected attacks, whereas the attacker's objective is to maximize the number of undetected attacks. We adopt mixed strategy Nash equilibrium as the solution concept of this game. 
%For any mixed strategy profile, we consider the expected detection rate of attacks as the metric of defender's performance against the attacker. 
We then formulate our inspection problem, denoted  $(\mathcal{P})$, as a mathematical program with equilibrium constraints. In this problem, the defender seeks to minimize the number of detectors such that the expected detection rate of attacks (i.e., detection performance)  in \emph{any} Nash equilibrium is above a pre-specified threshold. 

%
%
%
%In Section 2, we introduce a generic detection model to define the players? payoffs in a strategic game between a defender and an attacker. The defender chooses where to position her detectors, and the attacker chooses to target one or more network components. Each player is resource-constrained in that the defender (resp. the attacker) cannot position more detectors (resp. cannot target more network components) than her available resources. The defender?s objective is to maximize the number of attacks that are detected by her inspection strategy, represented by a monotone submodular detection function. The attacker?s objective is to maximize the number of attacks that remain undetected. The equilibrium concept of this game is mixed strategy Nash equilibrium. We then formulate our inspection problem, denoted (\P), as a mathematical program with equilibrium constraints. In this problem, the defender seeks to minimize the number of detectors such that the expected attack detection performance is above a pre-specified threshold in any equilibrium of the defender-attacker game. 



%\tr{In this article, we  adopt a generic detection model following, in which the ability of any detector to detect an attack depends on the sensor's technological features (e.g., sensing range), type of failures (e.g., pipe bursts versus contamination events), and network topology (e.g., pipe length and connectivity).}  We use this model to define, in Section \ref{sec:form}, the players' payoffs in a strategic game between a defender who chooses where to position her detectors, and an attacker who chooses to target one or more network components. Each player is resource-constrained in that the operator (resp. the attacker) cannot place more sensors (resp. cannot target more network components) than her available resources. The operator's objective is to maximize the number of failure events that are detected by her sensing strategy, represented by a monotone submodular sensing function, while the attacker's objective is to maximize the number of failure events that remain undetected. The outcome of this game is evaluated using the concept of mixed strategy Nash equilibrium. We then  formulate the problem $(\mathcal{P})$ as a mathematical program with equilibrium constraints. In this problem, the network operator wants to minimize the number of sensors such that the expected rate of detection of adversarial failures (i.e., detection performance) is above a pre-specified threshold in \emph{any} Nash equilibrium of the induced operator-attacker game. 

Essentially, solving the problem $(\mathcal{P})$ involves computing the equilibria of the defender-attacker game. However, the sets of players' actions grow combinatorially with the size of the network, which makes the equilibrium computation challenging. For large-scale networks, the number of available pure strategies for each player $n$ can easily reach $10^{60}$. Well-known algorithms such as \cite{Lipton:2003:PLG:779928.779933}'s $n^{O(\ln n/\epsilon^2)}$ time algorithm for computing an $\epsilon-$Nash equilibrium are practically inapplicable for this setting. Instead, in this article, we develop a new solution approach based on the properties of minimum set cover (MSC) and maximum set packing (MSP) problems. This approach enables us to solve the problem $(\mathcal{P})$ in a scalable manner and also provide performance guarantees.

%Instead, we derive a solution approach based on the properties of a minimum set cover (MSC) problem and maximum set packing (MSP) problem  \citep{Vazirani:2001}. 

%
%
%Essentially, solving the problem $(\mathcal{P})$ relies on solving the operator-attacker game. However, the sets of actions of both players grow combinatorially with the size of the network, which makes the equilibrium computation challenging. In particular, commonly known algorithms \citep{Nisan:2007:AGT:1296179,Porter2008642} cannot be used to compute exact or approximate equilibrium player strategies in a scalable manner. Indeed, for the problem sizes considered in our article, the number of available pure strategies for each player $n$ can easily reach $10^{60}$, which even makes \cite{Lipton:2003:PLG:779928.779933}'s $n^{O(\ln n/\epsilon^2)}$ time algorithm for computing an $\epsilon-$Nash equilibrium  practically inapplicable for our setting. Instead, in this article, we derive a solution approach based on the properties of two combinatorial optimization problems, which we formulate as a minimum set cover (MSC) problem and maximum set packing (MSP) problem \citep{Vazirani:2001}. 




%Although both MSC and MSP problems are known to be NP-hard, we find that modern integer programming solvers can solve them even for large-scale networks. Importantly, unlike classical approximation algorithms for solving large games which randomly select actions to consider in the support of their strategy profile, we provide a direct construction of an approximate Nash equilibrium of this large game. A main advantage of this construction is that it naturally leads to a solution with a small support, which is easy to implement in practice thanks to the current technological capabilities for implementing randomized sensing schemes.

%\tb{From the recent technological advances that allow for flexible on/off schedules and simultaneous collection of measurements at desired network locations, randomized sensing has become practically feasible in the context of infrastructure defense, making the resulting mixed sensing strategy in equilibrium easily implementable by the network operator. }

Our equilibrium analysis in Section \ref{general} consists of first studying useful structural properties that are satisfied by all Nash equilibria of the defender-attacker game. We present these properties for the most conservative case when the attacker has the ability to spread her attacks across the network. In particular, we show that in any equilibrium, both players must randomize their actions and use all available resources, and every network component must be monitored with positive probability (Propositions \ref{all_resources}-\ref{all_edges}). Importantly, while these are game-theoretic results, their proofs also rely on the properties of the detection function, as well as MSCs and MSPs which respectively capture the ``coverage'' and ``spread'' of the network.

%Interestingly, showing these results relies on the properties of the detection function, as well as the coverage and the spread of the network, captured by MSCs and MSPs, respectively. 

These properties enable us to derive lower and upper bounds on the expected detection rate in equilibrium in terms of both players' available resources, and the optimal values of the MSC and MSP problems (Theorem \ref{bounds_game}). A preliminary and specialized version of this result was presented in \cite{7852316}. Moreover, using solutions of MSC and MSP problems, we construct a strategy profile that not only is an $\epsilon-$Nash equilibrium, but also provides each player a payoff that is $\epsilon-$close to the payoff they would get in any Nash equilibrium (Theorem \ref{MSC-MSP-eNE}). 
%
%
%Our analysis consists in first studying structural properties that are satisfied by all Nash equilibria of the operator-attacker game. We present the results for the case when the size of the network is large in that the attacker has the ability to spread her attacks across the network. This case captures the situations in which it is most challenging for the operator to detect failures induced by the attacker. In Section~\ref{general}, we show that in any equilibrium, both players must randomize their actions and use all available resources, and every network component must be monitored with positive probability (Propositions~\ref{all_resources}-\ref{all_edges}). Interestingly, showing these game-theoretic results relies on the submodularity of the sensing function, as well as the coverage and the spread of the network, captured by MSCs and MSPs respectively. Since these results represent necessary conditions satisfied by all Nash equilibria, this enables us to derive lower and upper bounds on the expected detection rate in equilibrium in terms of  both players' available resources, and the optimal values of our MSC and MSP problems (Theorem~\ref{bounds_game}). An initial version of this result (without proof) was presented in \cite{7852316}. Using  solutions of the MSC and MSP problems, we construct a strategy profile that not only is an $\epsilon-$Nash equilibrium, but also provides each player a payoff that is $\epsilon-$close to the payoff they would get in any Nash equilibrium (Theorem~\ref{MSC-MSP-eNE}).  
Theorems \ref{bounds_game} and \ref{MSC-MSP-eNE} are then used to derive an approximate solution to the problem $(\mathcal{P})$,  with guarantees on the detection performance and the corresponding optimality gap (Proposition~\ref{Prop_interim} in Section~\ref{sec:Answer}). It turns out that our solution is optimal for the special case when the MSCs and MSPs are of same size.
%\tr{, i.e., we provide an analytical expression of the optimum number of sensors, and an equilibrium strategy profile. Importantly, our equilibrium characterization for this special case generalizes some of the classical results on hide-and-seek games \citep{karlin2016game} and security games \citep{garnaev2000search,mavronicolas}. [it will be said in Sec 1.2]]}
% In Section \ref{sec:app}, we show that our approach to solve problem $(\mathcal{P})$ is scalable to large-sized benchmark distribution networks in the water sector, and provides good performance guarantees for detecting adversarial disruptions.

Although our approach to solve problem $(\mathcal{P})$ relies on the MSC and MSP problems which are known to be NP-hard, we find that modern integer programming solvers can solve large instances of these problems. In particular, in Section \ref{sec:app}, we show that our solution approach is scalable to large-sized benchmark distribution networks, and provides good performance guarantees.

%we find that they can be solved using modern integer programming solvers, even for large-scale networks.} \tr{Importantly, unlike classical approximation algorithms for solving large-scale games which randomly select actions to consider in the support of their strategy profile, we provide a direct construction of an approximate Nash equilibrium of this large game.} \tb{Importantly.} The main advantage of this construction is that it naturally leads to a solution with a small support, which is easy to implement in practice thanks to the current technological capabilities for implementing randomized inspection strategies. 

%we instantiate our model for scenarios involving two practically relevant types of pipes disruptions. In particular, we show that our approach provides a scalable solution to problem $(\mathcal{P})$ with good performance guarantees, for large-sized benchmark  water networks. 

Finally, in Section \ref{conclusions}, we prove  that the expected detection rate and the inspection strategies in equilibrium do not depend on the attacker's number of resources if they are smaller than the size of MSPs (Theorem \ref{Constant}). This important and rather surprising structural property  is a consequence of the attacker's ability to spread her attacks in the network, and the submodularity of the detection model. From the defender's perspective, this implies that she does not need to know precisely the amount of attack resources. Another implication is that Nash equilibria can be obtained by solving a linear program with a large number of variables but a small number of constraints. Therefore, column generation can be used to iteratively improve our MSC/MSP-based solution to optimality.


%Although our approach to $(\mathcal{P})$ provides a solution with good approximation guarantees in practice, the operator might still prefer to improve that solution. For that purpose, we prove in Section \ref{conclusions} that the expected detection rate and the sensing strategies in equilibrium do not depend on the attacker's number of resources, if they are smaller than the size of MSPs (Theorem~\ref{Constant}). This structural result is a consequence of the attacker's ability to spread her attacks in the network, and the submodularity of the operator's payoff function. A direct implication is that Nash equilibria can be obtained by solving a linear program with a large number of variables but a small number of constraints. Therefore, one can use a column generation procedure to iteratively improve our MSC/MSP-based solution. Each iteration provides stronger performance guarantees until it reaches optimality, where the primal and dual solutions give the players strategies in equilibrium. However, the downside is that it can result in a sensing strategy with a large support, which may not be desirable from an implementation perspective. Therefore, a compromise can be reached by running iterations of the refinement procedure until a tradeoff between the performance and simplicity of the solution is achieved. 


The complete proofs of our results are provided in the electronic companion of this article.



\subsection{Related Work}

Our detection model is inspired by modern sensing technology used in detecting leaks and other failure events in pipeline networks for distribution of natural gas \citep{PHILLIPS20131}, and water \citep{Ost1415211920040901,sensors:autom}. A classical problem in sensing of these infrastructure networks is to optimally place sensors for maximizing the detection of leaks and burst events. Robust formulations of the sensor placement problem have received interest in the literature; for example, 
 \cite{krause+al:jmlr08} proposed an efficient approximation algorithm to maximize the worst-case detection performance against a set of possible failure scenarios. More recently, \cite{Orlin2016} and \cite{8263844} designed approximation algorithms to find a sensor placement that is robust against a subset of sensors' failures. The main feature of this line of work is \emph{fixed sensing}, i.e., continuous operation of sensors placed at fixed locations in the network. On the other hand, our setting is inspired by inspection operations based on smart detectors that can be flexibly positioned in various parts of the network to detect and report incidents.  
% strategies that are typically adopted by utility companies (and regulators) to find evidence of unauthorized tapping by fraudulent customers or malicious tampering by adversarial entities such as social miscreants and external hackers.
In such settings, it is well-known that \emph{randomized strategies} can significantly improve the defender's performance  against worst-case or  adversarial failure events \citep{doi:10.1287/opre.43.2.243,Pita:2008:DAP:1402795.1402819,BERTSIMAS2016114}.%; indeed, this is a key feature of our formulation.


%In the network sensing literature, the dominant approach is to consider an optimal resource allocation problem to maximize a metric of detection performance \citep{berry,Krause:2008:NSP:1390681.1390689,SELA201855}. Some of these formulations can be solved using mixed-integer programming methods, while others exhibit properties of submodular optimization -- derived from the sensing model -- leading to the application of greedy algorithms with approximation guarantees. Robust formulations of the sensor placement problem have also received interest. In particular, \cite{krause+al:jmlr08}  propose an efficient approximation algorithm to maximize the worst-case detection performance against a set of possible failure scenarios. Similarly, \cite{Orlin2016} and \cite{8263844}
%%, and \cite{DBLP:journals/corr/abs-1710-04740} 
%design approximation algorithms to find a sensor placement that is robust against a subset of sensors' failures. The main feature of this line of work is \emph{fixed} sensing, i.e., continuous operation of sensors placed at fixed locations in the network. However, it is well known that in many adversarial situations, \emph{randomized} strategies can significantly improve the operator's performance \citep{doi:10.1287/opre.43.2.243,Pita:2008:DAP:1402795.1402819,BERTSIMAS2016114}.

Our game-theoretic model is more general than the classical Hide-and-Seek game first introduced by \cite{von1953certain}, and further discussed in Ch. 3.2 of \cite{karlin2016game}. In this zero-sum game, a robber hides in one of a set of ``safe-houses'' located at roads intersections, and a police unit simultaneously chooses to travel along one road to find the robber. The roads are restricted to be vertical avenues and horizontal streets. Our solution approach can be applied to solve the generalized hide-and-seek game which involves multiple police units patrolling in a complex street network to find multiple robbers. This is possible because our approach can account for multiple player resources, and more realistic monitoring capabilities of the patrolling units.
%
%
%of the modeling flexibility of our detection model and the multiple player resources that our formulation accounts for.
%
%and game-theoretic analysis can be adopted to solve a more complex and realistic hide-and-seek game involving multiple robbers and multiple police units due to the fact our model considers multiple resources for both players.
%Thanks to the generality of our detection model, we can extend their setting to a more complex and realistic example of urban transportation network. Additionally, since our setting considers multiple resources for both players, we can apply our results to the search of multiple robbers, by dispatching multiple police units. 
Our game similarly generalizes the Infiltration Game with a Cable, as defined in Ch. 2.1 of \cite{garnaev2000search}.%; see Table~\ref{List_games} for full comparison.

%Both these problems can be modeled with our formulation, thanks to the generality of our detection model. More importantly, our analysis generalizes their  equilibrium analysis results since we consider that both players have multiple resources, whereas the above-mentioned literature assumed that each of the two players has a unit resource.

Finally, related to our setting is the work by \cite{mavronicolas}, who consider a security game on an information network in which the nodes (servers) are vulnerable to multiple attacks and the defender can install a firewall to protect a subnetwork. The defender's goal is to maximize the number of attack detections by randomizing the placement of her firewall. Simultaneously, the attacker's goal is to minimize the number of attacks detected by the firewall. While the authors made the restricting assumption that each subnetwork contains exactly two servers, our detection model can accommodate attack detections within subnetworks of heterogeneous sizes. In fact, our solution approach can be used to derive a defense strategy based on the installation of multiple firewalls to secure the network against multiple simultaneous attacks.
%Additionally, our equilibrium characterization generalizes their results to the case where the defender has multiple resources. Specifically, our results now provide the defender a strategy concerning the installation of multiple firewalls to secure an information network against multiple attacks.
%For this application, this implies that the def\
%
% enables the defender to 
%
%
%Again, our model subsumes [word check] their game, and generalizes their results to the case where the defender has multiple resources, which is a significant improvement when considering securing an information network. 
%From a theoretical viewpoint, increasing the number of resources is more challenging because of the inherent submodularity of the detection model. One of our main contributions is to address this difficulty using both game-theoretic and combinatorial arguments. I don?t understand the this.

A comparison of these security games is given in Table~\ref{List_games}.


%In the context of network security, several models have been recently proposed for the strategic allocation of defense resources \citep{mavronicolas,BaykalGursoy2014469,Goyal:2014aa}. Applications of these models include search  games \citep{von1953certain,Gal20140062}, infiltration games \citep{Garnaev1997}, patrolling games \citep{patrolling}, and inspection problems \citep{doi:10.1287/opre.43.2.243,doi:10.1287/opre.46.2.184,smith2008algorithms}. However, these formulations cannot be applied to solve problem $(\mathcal{P})$, as they do not account for the sensing models that arise in network monitoring applications.


%\subsection{Additional}
%\rem{In general, the choice of a mixed strategy by a player entails a decision to introduce randomness in her behavior. Consider, for example, the problem of sensing an urban water network to detect adversary-induced events on pipes. In this problem, a mixed strategy of \defender can be viewed as ``random scheduling'' of a subset of fixed sensors that are installed in some locations of the network, with the constraint that only up to $b_1$ of these sensors can be used simultaneously.  A mixed strategy of \attacker, constrained by the parameter $b_2$, can be similarly interpreted.} 
%
%
%We argued in Section~\ref{2 Comb Pbs} that the size of MSPs $\semm$ is no more than the size of MSCs $\smsc$ for any given network and \tb{detection} model $\mathcal{G}$. However, in some situations, MSCs and MSPs are of same size. For example, consider a bipartite graph where \tb{sensors can be placed on the vertices to monitor adjacent edges (i.e., one-hop sensing model).???} In this setting, MSCs and MSPs respectively become minimum vertex covers and maximum matchings, and are of the same size \citep{Konig}. 
%
%A more realistic example is that of a security game between an attacker who chooses up to $b_2$ paths in a transportation network to route illegal goods, and the operator who can interdict up to $b_1$ edges. We can model this game in our setup by viewing $\nodes$ (resp. $\edges$) as the set of edges (resp. paths) in the network, and the monitoring set for each edge in $\nodes$ as the set of paths which contain that edge. Now one can see that an MSC is a minimum cardinality cut set, and an MSP is a set of maximum edge-disjoint paths. Using the max-flow min-cut theorem, we obtain that the sizes of MSCs and MSPs satisfy $\smsc = \semm$.
%
%
% for the classical Hide-and-Seek game (see Ch. 3.2 of \cite{karlin2016game}) based on minimum line-covers and maximum matchings; and also for the computer network security game studied by \cite{mavronicolas} based on minimum edge covers and maximum independent sets. Finally, our result also generalizes the NE derivation for the Infiltration Game with a Cable, as defined in Ch. 2.1 of \cite{garnaev2000search}. 
 





==> S1_intro_LS.tex <==
%!TEX root = OR Manuscript V23.tex
\section{Introduction}\label{sec:intro}
%\rev{[a few notes: (1) need to add more references, (2) need to reconcile terminology]}

%\subsection{Network Monitoring Problem}
%\subsection{Motivation}
\rev{Securing critical infrastructure systems including water, gas, and power distribution systems is crucial for societal welfare and prosperity. These critical infrastructures, spanning huge geographical distances, are inherently vulnerable to intentional and unintentional threats (cite). Public utilities and municipalities are the primary entities responsible for ensuring infrastructure integrity and service quality, and employ various degrees of oversight to manage and respond to hazardous events. A growing number of policies, regulations, and laws addressing  infrastructure vulnerability are emerging, charging municipalities and public utilities with recognizing and reducing risks to urban infrastructure (cite). Continuous research efforts are being conducted to guide and support local municipalities and public utilities in emergency management activities, including threat assessment, mitigation, and preparedness as well as response, and recovery activities~\citep{Lindell2007IntroductionManagement,MONROE201837}. %This emergency management framework was adopted by many government and state agencies including the Government Accountability Office (GAO), the Federal Emergency Management Agency (FEMA), and the Environmental Protection Agency (EPA) (cite). %  and has been applied to wide range of disasters including floods, hurricanes, and wildfires. 
%Among the five thrusts of emergency management, the majority of research efforts for urban infrastructure focuses on post-disaster management, i.e., response and recovery activities, of unintentional threats such as hurricanes and tornadoes causing severe floods, power outages, and population shifts~\citep{MONROE201837}. 
Disaster mitigation and preparedness activities involve allocating countermeasures to limit and reduce the occurrence of unintentional, as well as discourage intentional threats. Regardless of the emergency management activities, advanced sensing technologies have been recognized as primary mechanism for securing urban infrastructure systems.} 

\rev{In this research, we propose utilizing \textit{advances in sensing technology to design inspection strategies for networked infrastructure to limit and discourage intentional threats}. Our modeling framework applies to flow networks such as water, oil, and gas [MD: I am having a hard time balancing between application and generality...], which allow for the application of sensing technologies, including flow meters and pressure sensors, capable of continuously collecting and transmitting measurements at fine temporal resolution~\citep{PHILLIPS20131,XING2019291}. These sensing technologies facilitate an accurate and timely estimation of the network state and operating conditions, and through advanced data analytics, enable the identification of possible pipeline faults and leakages. We demonstrate our proposed approach by, firstly, presenting the theoretical foundation for the inspection strategy under strategic attacks for general flow networks [MD: again, should we restrict to flow networks.], and secondly, evaluating the proposed strategy using a set of realistic, large-scale water distribution networks.} %The physical network is abstracted into a network-theoretical representation. Physical attacks causing hydraulic failures.  both defender and attacker use hydraulic information about the network to select locations. nodes represent access points that can be seen by the public and can be attacked, for example, by inducing backflow at hydrants, sabotaging valves, or accessing pipes through manholes. These mechanical failures causing hydraulic faults can be detected using various detection mechanisms (e.g. fault detection matrix).


%In recent years, the public utility sector has seen a huge uptake in deployment of advanced sensing technologies, which in addition to the monitoring benefits, can be partially attributed to the small size, ease of installation, low cost of the sensors, and non-interference with routine operation of the pipelines.

\rev{In the context of unintentional threats, the dominant paradigm is to cast the network monitoring problem [MD: okay if we mention network inspection problem?] as the optimal sensor placement problem, in which a budget-constrained utility aims to allocate a limited number of sensors in the system to, for example, maximize the number of detected events~\citep{4729806,berry,Krause:2008:NSP:1390681.1390689}. [MD: These papers consider more complicated metrics of performance than number of detected events...] 
In large-scale networks, it is impractical to monitor every component, inevitably leaving some parts of the network unmonitored. In an adversarial situation, a strategic and resourceful attacker will target these unmonitored parts to avoid or make their detection more difficult. It follows that a \textit{fixed sensing strategy} can face a significant loss of detection performance and, in turn, serious lapses in integrity of the infrastructure system. Importantly, a strategic attacker can target multiple network components simultaneously~\citep{kroll2006securing}. In adversarial settings, it is well-known that \emph{randomized strategies} can significantly improve the defender's performance against adversarial failure events \citep{doi:10.1287/opre.43.2.243,Pita:2008:DAP:1402795.1402819,BERTSIMAS2016114}.
%and a key challenge for the utility is how to select a small subset of network components to monitor that will provide the most network-wide information gain to ensure a desired level of performance. In allocating sensors, a small number of critical sites are selected among hundreds or thousands of potential locations, which are identified based on integrating network dynamics, sensing, and threat detection models. Various optimization approaches, including mixed-integer optimization, greedy approximation, heuristic, and evolutionary algorithms have been proposed to solve the sensor placement in networked infrastructure systems~ \citep{krause+al:jmlr08, Orlin2016, 8263844}. %For example,  \cite{krause+al:jmlr08} proposed an efficient approximation algorithm to maximize the worst-case detection performance against a set of possible failure scenarios. More recently, \cite{Orlin2016} and \cite{8263844} designed approximation algorithms to find a sensor placement that is robust against a subset of sensors' failures.%Several solution approaches have been suggested to address the sensor placement problem, some of which involve mixed-integer programming methods \citep{} \textcolor{red}{cite}, while others exhibit properties of submodular optimization leading to the application of greedy algorithms with approximation guarantees \citep{} \textcolor{red}{cite}. 
%Regardless of the performance metric or the optimization method, previous approaches are characterized by two salient features: (1) unintentional threats are typically modeled as \textit{random} failure events, and (2) the utility is allocating a given number of sensing devices at \textit{fixed}  locations in the network, i.e., employing a \textit{fixed sensing} strategy. Under these two assumptions, a budget-constrained utility will place the fixed sensing devices at critical locations, thus inevitably leaving some parts of the network unmonitored. In an adversarial situation, a strategic and resourceful attacker will target these unmonitored parts to avoid or make their detection more difficult. It follows, that in an adversarial setting, a fixed sensing strategy can face a significant loss of detection performance and, in turn, serious lapses in integrity of the infrastructure system. Importantly, a strategic attacker can target multiple network components simultaneously~\citep{kroll2006securing}. In such settings, it is well-known that \emph{randomized strategies} can significantly improve the defender's performance against adversarial failure events \citep{doi:10.1287/opre.43.2.243,Pita:2008:DAP:1402795.1402819,BERTSIMAS2016114}.
%%It follows that a strategic attacker mandates a counterpart defense strategy for allocating sensing resources shifting from traditional fixed sensor placement paradigm.
In light of the above, this work is inspired by recent defense strategies employing randomized inspection for network security against strategic attacker~\citep{BaykalGursoy2014469}.
For example,~\cite{Pita:2008:DAP:1402795.1402819} use randomized strategies for the scheduling of checkpoints and for generating patrolling schedules for canine units to assist the police at the Los Angeles International Airport. \cite{Hochbaum2011} investigate the allocation of mobile sensors to detect transported nuclear weapons based on related radiological dispersion devices.} 

\rev{To address the problem of network defense against a strategic attacker, we propose a \textit{bilevel optimization formulation} of the strategic network inspection problem. [MD: I don't agree with the next sentence] The physical network is abstracted into a network-theoretical representation, in which links represent system components that can be accessed and attacked and network nodes represent access points in which the utility can deploy sensing devices. %, for example, inducing backflow at fire hydrants, sabotaging valves, or accessing pipes through manholes (cite). Network nodes represent access points in which the utility can deploy sensing devices to monitor and detect mechanical and process failures using various detection mechanisms, e.g., pipe bursts and leaks (cite). 
%In our setting, both the defender and the attacker use information about the flow-network to select the defense/attack locations, respectively. 
The objective of the utility is to minimize the number of resources required to achieve a performance target (e.g., detection rate), while the attacker is interested in avoiding or minimizing detection. This problem allows the utility to deploy randomized sensing strategy, thus shifting from traditional fixed sensor placement paradigm. In the context of infrastructure defense, randomized sensing implies mobilizing sensing devices in the network and enabling synchronous collection of measurements at desired network locations. Although, randomized sensing technology are not yet widely used and are limited in their capability, they are constantly under development and their deployment can provide insights which are not available using fixed sensing technologies. In addition to flow networks, our strategic game is also relevant to a range of applications, such as listed in Table~\ref{List_app}.}

\OneAndAHalfSpacedXI
\begin{table}[h]\footnotesize
\centering
\caption{List of applications of \rev{the} network inspection problem.}
\begin{tabular}{|l|l|l|l|}
\hline Inspection setting & Network & Type of detector & Type of attacks  \\\hline%\hhline{|-||=|=|=|}
\hline Urban patrolling & city streets  & police unit & robbery \\
\hline Network security & information network & firewall & cyberattack on server \\
\hline Sensing of gas and water networks & gas and water pipelines & leak/pressure sensor & pipe disruption \\
%\hline Sensing of water networks & urban water network & contaminant sensor & contaminant  injection\\
\hline Interdiction of illegal goods & transportation network & police officer & drug trafficking  \\
\hline Infiltration game & water channel & electric cable & malicious infiltration \\\hline
\end{tabular}
\label{List_app}
\end{table}


\ifarXiv
\OneAndAHalfSpacedXI
\else
\DoubleSpacedXI
\fi

%, and address the question: \emph{How many detectors are required and how to strategically position them in the network to detect multiple adversarial attacks?} 

\rev{
In the context of strategic games, several game-theoretic models have been proposed recently for strategic allocation of defense resources in network security scenarios \citep{BaykalGursoy2014469}. 
Such games have been extensively studied in various forms such as search \citep{Gal20140062}, inspection \citep{Avenhaus20021947}, infiltration \citep{Garnaev1997}, and patrolling games \citep{patrolling}. 
%Our setting generalizes two well-known search games. The first one is the Hide-and-Seek game defined in Ch. 3.2 of \cite{karlin2016game} and first introduced by \cite{von1953certain}. In this zero-sum game, a robber hides in one of a set of ``safe-houses'' located at roads intersections, and a cop simultaneously chooses to travel along one road to find the robber. The second is the Infiltration Game with a Cable, as defined in Ch. 2.1 of \cite{garnaev2000search}. In this problem, an infiltrator wants to cross a (discretized) channel and a guard uses an electric cable to detect the infiltrator. Both these problems can be modeled with our game by restricting our sensing model and by giving each player only one unit of resources. Our formulation is also relevant to a range of applications, as listed in Table~\ref{List_app}.
Our game-theoretic model is more general than the classical \textit{hide-and-seek} game first introduced by \cite{von1953certain}, and further discussed in Ch. 3.2 of \cite{karlin2016game}. In this zero-sum game, a robber hides in one of a set of ``safe-houses'' located at roads' intersections, and a police unit simultaneously chooses to travel along one road to find the robber. The roads are restricted to be vertical avenues and horizontal streets. Our solution approach can be applied to solve the generalized hide-and-seek game, which involves multiple police units patrolling in a complex street network to find multiple robbers. This is possible because our approach can account for multiple player resources, and more realistic monitoring capabilities of the patrolling units. Our game similarly generalizes the Infiltration Game with a Cable, as defined in Ch. 2.1 of \cite{garnaev2000search}. %; see Table~\ref{List_games} for full comparison.
Finally, related to our setting is the work by \cite{mavronicolas}, who consider a security game on an information network in which the nodes (servers) are vulnerable to multiple attacks and the defender can install a firewall to protect a subnetwork. The defender's goal is to maximize the number of attack detections by randomizing the placement of her firewall. Simultaneously, the attacker's goal is to minimize the number of attacks detected by the firewall. While the authors made the restricting assumption that each subnetwork contains exactly two servers, our detection model can accommodate attack detections within subnetworks of heterogeneous sizes. In fact, our solution approach can be used to derive a defense strategy based on the installation of multiple firewalls to secure the network against multiple simultaneous attacks.}


%Randomized sensing has become practically feasible in the context of infrastructure defense, driven by the recent technological advances that allow for flexible and simultaneous collection of measurements at desired network locations.  For example, \cite{Pita:2008:DAP:1402795.1402819} use randomized strategies for the scheduling of checkpoints and for generating patrolling schedules for canine units to assist the police at the Los Angeles International Airport. \cite{Hochbaum2011} investigate the allocation of mobile sensors to detect transported nuclear weapons based on related radiological dispersion devices. In the urban water sector, recent deployments \citep{allen:smart, infrasense} enable the implementation of mobile sensing strategies to detect pipe failures and the presence of contaminants \citep{6779697,PERELMAN20134217}. 








%One approach to address the above-mentioned issue is to consider the problem of robust sensor placement, which aims to maximize the worst-case detection performance against a set of possible failure scenarios.  \cite{krause+al:jmlr08} study a robust network sensing problem where the possible failure scenarios are modeled as normalized monotone submodular functions. The authors propose an efficient approximation algorithm to solve this problem and provide applications in outbreak detection and robustness against sensor failures. \cite{Orlin2016}, motivated by the latter application, provide a constant factor approximation algorithm to find a sensor placement that is robust against a subset of sensors' failures. \textcolor{red}{add another reference water quality.}

%Advanced sensing, monitoring, and inspection technologies have been recognized as key mechanism for securing urban infrastructure by providing situational awareness to the distribution utilities, who are tasked with maintaining the functional state and service quality of their expansive assets. In response to the rapid advances in sensing and monitoring technologies, The majority of research for emergency management focuses on developing secondary lines of defense, which include early warning systems and response actions. First line of defense includes includes a set of countermeasures to discourage, limit, or deny physical access to vulnerable points and reduce the occurrence of deliberate sabotage. 





%Security of physical infrastructures such as water distribution, power grids, and gas and oil transmission networks, is crucial for ensuring the availability and quality of the essential services that rely on these networks. However, recent incidents have confirmed that infrastructure networks continue to be attractive targets for adversarial entities, including malicious insiders, external hackers, and even nation states . \maybe{In some situations, these entities can use physical or remote access points to compromise multiple network components   in a strategic manner . Such an attack, if successful, can result in prolonged service interruptions and incur significant economic losses.} Thus, infrastructure operators and utilities face an important task of maintaining adequate situation awareness in the presence of security attacks. 

% Consider the inspection problem faced by a utility company (typically a regulated monopoly) who manages a natural gas pipeline network in an urban area. Traditionally, utility personnel conduct inspections of network assets and customer connections at a predetermined frequency (once every 2-3 years), or when an emergency situation is reported \citep{Inspect2015}. Issues such as service interruptions, minor gas leaks, and faulty/illegal line connections are addressed by the utility with varying degrees of response rates, and notifications are filed with the regulator retroactively. However, these traditional inspection systems, based on manual checks and ex-post  reporting, are very limited with regards to three aspects: 

% \begin{enumerate}
% \item[1)] Minor incidents (leaks) occasionally evolve to become major disruptions. However, the current inspection operations tend to prioritize major components such as main lines and valve stations. As a result, the detection of minor leaks is delayed, often causing significant damages in the future.
% %
% %Some secondary distribution points are less frequently inspected, which occasionally results in minor leaks evolving to become major disruptions. Thus,
% %
% % often due to delayed detection and response by utility personnel. Thus, inspecting most often the major components such as main line and valve stations is not adequate, as failures of remote distribution points can also cause substantive damages.

% \item[2)] Physical or remote access to critical components can be exploited by malicious entities. These entities may use a combination of physical and digital tampering to bypass safety systems. However, inspection systems typically do not account for strategic and resourceful attackers whose actions are more difficult to detect, in comparison to isolated random failures. 
 
% \item[3)] Utility companies are the primary entities responsible for network monitoring and incident response. The regulator has various degrees of oversight on utilities' response to reported incidents, but the guidelines on proactive inspection are relatively sparse. Thus, the existing regulatory framework can benefit from inspection systems that provide better sensing and reporting capabilities. 

% %
% % and ensuring the quality of service. Typically, the regulators do not have adequate resources to conduct extensive audits and compliance checks. Thus, utilities companies  companies inspection systems should enable filing of timely and specific details about relevant incidents by the utility company to the regulator.


% \end{enumerate}




% Fortunately, recent advances in sensing technologies have resulted in commercially available smart detector systems, which include a sensor, a detection software, and a communication unit \citep{1219475,Fischer2017}. These detectors can be easily operated by the utility personnel and flexibly positioned in the network to meet target inspection goals. 
% By adopting smart detectors in their inspection operations, the utilities can at least partly address the aforementioned limitations \citep{PGE2010}.



%Fortunately, recent advances in modern sensing technologies provide new capabilities for monitoring network components by way of detecting the physical disturbances that can result from failure events. For example, wireless sensor networks have been successfully used in the monitoring of water networks \citep{Stoianov:2007:PWS:1236360.1236396,allen:smart}. These sensors provide timely and accurate data to enable the detection of possible pipeline breaks and contamination events \citep{PERELMAN20134217}. Sensor networks are also being utilized to monitor oil and natural gas networks \citep{s120100189}.  These sensing technologies often come with flexible scheduling and remote monitoring capabilities, which are important for timely detection of failure events. 

%A particularly interesting feature of these sensing technologies is their ability to be remotely configured, and the ease with which they can be scheduled. Thus, the operator can use them for timely detection of a broad class of failure events.


 
%However, the allocation of these sensing resources is a challenging problem, especially when the failures can arise from strategic attacks. First, a strategic and resourceful attacker can simultaneously target multiple components in a manner which makes their detection more difficult, in comparison to isolated random failure events. Secondly, due to the cost of deploying sensors, the operator is typically constrained to use a small number of sensing resources, which is further limiting due to the large-scale nature of infrastructure networks. Thus, every network component cannot be simultaneously monitored, raising the possibility of attacks that can target components while avoiding detection \citep{Liu:2009:FDI:1653662.1653666,Parfomak2012,6303885}. Despite the recent progress on sensor placement problems, as well as strategic infrastructure defense, we lack a systematic approach to enable the allocation of sensing resources in large-scale networks, with guarantees on detection performance against strategic attacks. In this article, we address the following \emph{network monitoring problem}, which we denote $(\mathcal{P})$:  \emph{How many sensors are required and how to strategically place them in the infrastructure network to detect adversarial attacks?}



%This article is driven by the  


%cannot directly be applied to address this question, requiring new modeling and analysis techniques need to be developed, which we present in this article.


%to infrastructure network monitoring, as they do not account for any sensing model.


\subsection{\rev{Main} Contributions}


In Section \ref{sec:form}, we introduce a generic detection model, which captures the key features of modern inspection systems with respect to sensing technology for event detection and flexibility of positioning. \rem{Mathematically, the model is represented by a monotone submodular detection function.} We use this detection model to define a \rev{bilevel optimization problem, denoted  $(\mathcal{P})$, that models the strategic interactions
% game-theoretic model of strategic interaction 
between a defender (inspection agency) and an attacker. The defender first selects a randomized positioning of detectors to detect attacks. Then, the attacker targets multiple network components so as to maximize the number of undetected attacks. The defender's objective is to determine the minimum number of detectors required to ensure the expected detection rate of worst-case attacks (i.e., detection performance) is above a pre-specified threshold.}

%inspects the network with minimum number of detectors 
%
%chooses how many detectors 
%
%the minimum number of detectors
%
%determines how many detectors to 


%The defender chooses where to position her detectors, and the attacker chooses to target one or more network components. Each player is resource-constrained. The defender's objective is to maximize the number of detected attacks, whereas the attacker's objective is to maximize the number of undetected attacks. We adopt mixed strategy Nash equilibrium as the solution concept of this game. 
%For any mixed strategy profile, we consider the expected detection rate of attacks as the metric of defender's performance against the attacker. 
%We then formulate our inspection problem, denoted  $(\mathcal{P})$, as a mathematical program with equilibrium constraints. In this problem, the defender seeks to minimize the number of detectors such that the expected detection rate of attacks (i.e., detection performance)  in \emph{any} Nash equilibrium is above a pre-specified threshold. 

%
%
%
%In Section 2, we introduce a generic detection model to define the players? payoffs in a strategic game between a defender and an attacker. The defender chooses where to position her detectors, and the attacker chooses to target one or more network components. Each player is resource-constrained in that the defender (resp. the attacker) cannot position more detectors (resp. cannot target more network components) than her available resources. The defender?s objective is to maximize the number of attacks that are detected by her inspection strategy, represented by a monotone submodular detection function. The attacker?s objective is to maximize the number of attacks that remain undetected. The equilibrium concept of this game is mixed strategy Nash equilibrium. We then formulate our inspection problem, denoted (\P), as a mathematical program with equilibrium constraints. In this problem, the defender seeks to minimize the number of detectors such that the expected attack detection performance is above a pre-specified threshold in any equilibrium of the defender-attacker game. 



%\tr{In this article, we  adopt a generic detection model following, in which the ability of any detector to detect an attack depends on the sensor's technological features (e.g., sensing range), type of failures (e.g., pipe bursts versus contamination events), and network topology (e.g., pipe length and connectivity).}  We use this model to define, in Section \ref{sec:form}, the players' payoffs in a strategic game between a defender who chooses where to position her detectors, and an attacker who chooses to target one or more network components. Each player is resource-constrained in that the operator (resp. the attacker) cannot place more sensors (resp. cannot target more network components) than her available resources. The operator's objective is to maximize the number of failure events that are detected by her sensing strategy, represented by a monotone submodular sensing function, while the attacker's objective is to maximize the number of failure eventfs that remain undetected. The outcome of this game is evaluated using the concept of mixed strategy Nash equilibrium. We then  formulate the problem $(\mathcal{P})$ as a mathematical program with equilibrium constraints. In this problem, the network operator wants to minimize the number of sensors such that the expected rate of detection of adversarial failures (i.e., detection performance) is above a pre-specified threshold in \emph{any} Nash equilibrium of the induced operator-attacker game. 

Essentially, \rev{we show that} solving the problem $(\mathcal{P})$ involves computing \rev{Nash equilibria of a zero-sum game, where the sets of players' actions grow combinatorially with the size of the network.
To overcome the inherent computational challenge, we analyze the equilibria of the zero-sum game.} Our equilibrium analysis in Section \ref{general} consists of first studying structural properties that are satisfied by all Nash equilibria. We present these properties for the most conservative case when the attacker has the ability to spread her attacks across the network. In particular, we show that in any equilibrium, both players must randomize their actions and use all available resources, and every network component must be monitored with positive probability (\rev{Theorem \ref{all_resources} and Proposition \ref{all_edges}}). Importantly, while these are game-theoretic results, their proofs also rely on the properties of the detection function, as well as \rev{the minimum set cover (MSC) and maximum set packing (MSP) problems, which respectively capture the ``coverage'' and ``spread'' of the network.
}

%equilibrium properties of the game's Nash eq 
%
%develop a novel approach to

%However, the sets of players' actions grow combinatorially with the size of the network, which makes the equilibrium computation challenging. \rem{For large-scale networks, the number of available pure strategies for each player $n$ can easily reach $10^{60}$. Well-known algorithms such as \cite{Lipton:2003:PLG:779928.779933}'s $n^{O(\ln n/\epsilon^2)}$ time algorithm for computing an $\epsilon-$Nash equilibrium are practically inapplicable for this setting.} Instead, in this article, we develop a new solution approach based on the properties of minimum set cover (MSC) and maximum set packing (MSP) problems. This approach enables us to solve the problem $(\mathcal{P})$ in a scalable manner and also provide performance guarantees.

%Instead, we derive a solution approach based on the properties of a minimum set cover (MSC) problem and maximum set packing (MSP) problem  \citep{Vazirani:2001}. 

%
%
%Essentially, solving the problem $(\mathcal{P})$ relies on solving the operator-attacker game. However, the sets of actions of both players grow combinatorially with the size of the network, which makes the equilibrium computation challenging. In particular, commonly known algorithms \citep{Nisan:2007:AGT:1296179,Porter2008642} cannot be used to compute exact or approximate equilibrium player strategies in a scalable manner. Indeed, for the problem sizes considered in our article, the number of available pure strategies for each player $n$ can easily reach $10^{60}$, which even makes \cite{Lipton:2003:PLG:779928.779933}'s $n^{O(\ln n/\epsilon^2)}$ time algorithm for computing an $\epsilon-$Nash equilibrium  practically inapplicable for our setting. Instead, in this article, we derive a solution approach based on the properties of two combinatorial optimization problems, which we formulate as a minimum set cover (MSC) problem and maximum set packing (MSP) problem \citep{Vazirani:2001}. 




%Although both MSC and MSP problems are known to be NP-hard, we find that modern integer programming solvers can solve them even for large-scale networks. Importantly, unlike classical approximation algorithms for solving large games which randomly select actions to consider in the support of their strategy profile, we provide a direct construction of an approximate Nash equilibrium of this large game. A main advantage of this construction is that it naturally leads to a solution with a small support, which is easy to implement in practice thanks to the current technological capabilities for implementing randomized sensing schemes.

%\tb{From the recent technological advances that allow for flexible on/off schedules and simultaneous collection of measurements at desired network locations, randomized sensing has become practically feasible in the context of infrastructure defense, making the resulting mixed sensing strategy in equilibrium easily implementable by the network operator. }


%Interestingly, showing these results relies on the properties of the detection function, as well as the coverage and the spread of the network, captured by MSCs and MSPs, respectively. 

These properties enable us to derive lower and upper bounds on the expected detection rate in equilibrium in terms of both players' available resources, and the optimal values of the MSC and MSP problems (Theorem \ref{bounds_game}). A preliminary and specialized version of this result was presented in \cite{7852316}. 
%Moreover, using solutions of MSC and MSP problems, we construct a strategy profile that not only is an $\epsilon-$Nash equilibrium, but also provides each player a payoff that is $\epsilon-$close to the payoff they would get in any Nash equilibrium (Theorem \ref{MSC-MSP-eNE}). 
%
%
%Our analysis consists in first studying structural properties that are satisfied by all Nash equilibria of the operator-attacker game. We present the results for the case when the size of the network is large in that the attacker has the ability to spread her attacks across the network. This case captures the situations in which it is most challenging for the operator to detect failures induced by the attacker. In Section~\ref{general}, we show that in any equilibrium, both players must randomize their actions and use all available resources, and every network component must be monitored with positive probability (Propositions~\ref{all_resources}-\ref{all_edges}). Interestingly, showing these game-theoretic results relies on the submodularity of the sensing function, as well as the coverage and the spread of the network, captured by MSCs and MSPs respectively. Since these results represent necessary conditions satisfied by all Nash equilibria, this enables us to derive lower and upper bounds on the expected detection rate in equilibrium in terms of  both players' available resources, and the optimal values of our MSC and MSP problems (Theorem~\ref{bounds_game}). An initial version of this result (without proof) was presented in \cite{7852316}. Using  solutions of the MSC and MSP problems, we construct a strategy profile that not only is an $\epsilon-$Nash equilibrium, but also provides each player a payoff that is $\epsilon-$close to the payoff they would get in any Nash equilibrium (Theorem~\ref{MSC-MSP-eNE}).  
Theorems \ref{bounds_game} and \ref{MSC-MSP-eNE} are then used to derive an approximate solution to the problem $(\mathcal{P})$,  with guarantees on the detection performance and the corresponding optimality gap (Section~\ref{sec:Answer}). It turns out that our solution is optimal for the special case when the MSCs and MSPs are of same size.
%\tr{, i.e., we provide an analytical expression of the optimum number of sensors, and an equilibrium strategy profile. Importantly, our equilibrium characterization for this special case generalizes some of the classical results on hide-and-seek games \citep{karlin2016game} and security games \citep{garnaev2000search,mavronicolas}. [it will be said in Sec 1.2]]}
% In Section \ref{sec:app}, we show that our approach to solve problem $(\mathcal{P})$ is scalable to large-sized benchmark distribution networks in the water sector, and provides good performance guarantees for detecting adversarial disruptions.

Finally, in Section \ref{conclusions}, we prove  that the expected detection rate and the inspection strategies in equilibrium do not depend on the attacker's number of resources if they are smaller than the size of MSPs (Theorem \ref{Constant}). This important and rather surprising structural property  is a consequence of the attacker's ability to spread her attacks in the network, and the submodularity of the detection model. From the defender's perspective, this implies that she does not need to know precisely the amount of attack resources. Another implication is that Nash equilibria can be obtained by solving a linear program with a large number of variables but a small number of constraints. Therefore, column generation can be used to iteratively improve our MSC/MSP-based solution to optimality.

Although our approach to solve problem $(\mathcal{P})$ relies on the MSC and MSP problems which are known to be NP-hard, we find that modern integer programming solvers can solve large instances of these problems. In particular, in Section \ref{sec:app}, we show that our solution approach is scalable to large-sized benchmark distribution networks, and provides good performance guarantees.

%we find that they can be solved using modern integer programming solvers, even for large-scale networks.} \tr{Importantly, unlike classical approximation algorithms for solving large-scale games which randomly select actions to consider in the support of their strategy profile, we provide a direct construction of an approximate Nash equilibrium of this large game.} \tb{Importantly.} The main advantage of this construction is that it naturally leads to a solution with a small support, which is easy to implement in practice thanks to the current technological capabilities for implementing randomized inspection strategies. 

%we instantiate our model for scenarios involving two practically relevant types of pipes disruptions. In particular, we show that our approach provides a scalable solution to problem $(\mathcal{P})$ with good performance guarantees, for large-sized benchmark  water networks. 




%Although our approach to $(\mathcal{P})$ provides a solution with good approximation guarantees in practice, the operator might still prefer to improve that solution. For that purpose, we prove in Section \ref{conclusions} that the expected detection rate and the sensing strategies in equilibrium do not depend on the attacker's number of resources, if they are smaller than the size of MSPs (Theorem~\ref{Constant}). This structural result is a consequence of the attacker's ability to spread her attacks in the network, and the submodularity of the operator's payoff function. A direct implication is that Nash equilibria can be obtained by solving a linear program with a large number of variables but a small number of constraints. Therefore, one can use a column generation procedure to iteratively improve our MSC/MSP-based solution. Each iteration provides stronger performance guarantees until it reaches optimality, where the primal and dual solutions give the players strategies in equilibrium. However, the downside is that it can result in a sensing strategy with a large support, which may not be desirable from an implementation perspective. Therefore, a compromise can be reached by running iterations of the refinement procedure until a tradeoff between the performance and simplicity of the solution is achieved. 


The complete proofs of our results are provided in the electronic companion of this article.



% \subsection{Related Work}

% Our detection model is inspired by modern sensing technology used in detecting leaks and other failure events in pipeline networks for distribution of natural gas \citep{PHILLIPS20131}, and water \citep{Ost1415211920040901,sensors:autom}. A classical problem in sensing of these infrastructure networks is to optimally place sensors for maximizing the detection of leaks and burst events. Robust formulations of the sensor placement problem have received interest in the literature; for example, 
%  \cite{krause+al:jmlr08} proposed an efficient approximation algorithm to maximize the worst-case detection performance against a set of possible failure scenarios. More recently, \cite{Orlin2016} and \cite{8263844} designed approximation algorithms to find a sensor placement that is robust against a subset of sensors' failures. The main feature of this line of work is \emph{fixed sensing}, i.e., continuous operation of sensors placed at fixed locations in the network. On the other hand, our setting is inspired by inspection operations based on smart detectors that can be flexibly positioned in various parts of the network to detect and report incidents.  
% % strategies that are typically adopted by utility companies (and regulators) to find evidence of unauthorized tapping by fraudulent customers or malicious tampering by adversarial entities such as social miscreants and external hackers.
% In such settings, it is well-known that \emph{randomized strategies} can significantly improve the defender's performance  against worst-case or  adversarial failure events \citep{doi:10.1287/opre.43.2.243,Pita:2008:DAP:1402795.1402819,BERTSIMAS2016114}.%; indeed, this is a key feature of our formulation.


%In the network sensing literature, the dominant approach is to consider an optimal resource allocation problem to maximize a metric of detection performance \citep{berry,Krause:2008:NSP:1390681.1390689,SELA201855}. Some of these formulations can be solved using mixed-integer programming methods, while others exhibit properties of submodular optimization -- derived from the sensing model -- leading to the application of greedy algorithms with approximation guarantees. Robust formulations of the sensor placement problem have also received interest. In particular, \cite{krause+al:jmlr08}  propose an efficient approximation algorithm to maximize the worst-case detection performance against a set of possible failure scenarios. Similarly, \cite{Orlin2016} and \cite{8263844}
%%, and \cite{DBLP:journals/corr/abs-1710-04740} 
%design approximation algorithms to find a sensor placement that is robust against a subset of sensors' failures. The main feature of this line of work is \emph{fixed} sensing, i.e., continuous operation of sensors placed at fixed locations in the network. However, it is well known that in many adversarial situations, \emph{randomized} strategies can significantly improve the operator's performance \citep{doi:10.1287/opre.43.2.243,Pita:2008:DAP:1402795.1402819,BERTSIMAS2016114}.


%In the context of network security, several models have been recently proposed for the strategic allocation of defense resources \citep{mavronicolas,BaykalGursoy2014469,Goyal:2014aa}. Applications of these models include search  games \citep{von1953certain,Gal20140062}, infiltration games \citep{Garnaev1997}, patrolling games \citep{patrolling}, and inspection problems \citep{doi:10.1287/opre.43.2.243,doi:10.1287/opre.46.2.184,smith2008algorithms}. However, these formulations cannot be applied to solve problem $(\mathcal{P})$, as they do not account for the sensing models that arise in network monitoring applications.


%\subsection{Additional}
%\rem{In general, the choice of a mixed strategy by a player entails a decision to introduce randomness in her behavior. Consider, for example, the problem of sensing an urban water network to detect adversary-induced events on pipes. In this problem, a mixed strategy of \defender can be viewed as ``random scheduling'' of a subset of fixed sensors that are installed in some locations of the network, with the constraint that only up to $b_1$ of these sensors can be used simultaneously.  A mixed strategy of \attacker, constrained by the parameter $b_2$, can be similarly interpreted.} 
%
%
%We argued in Section~\ref{2 Comb Pbs} that the size of MSPs $\semm$ is no more than the size of MSCs $\smsc$ for any given network and \tb{detection} model $\mathcal{G}$. However, in some situations, MSCs and MSPs are of same size. For example, consider a bipartite graph where \tb{sensors can be placed on the vertices to monitor adjacent edges (i.e., one-hop sensing model).???} In this setting, MSCs and MSPs respectively become minimum vertex covers and maximum matchings, and are of the same size \citep{Konig}. 
%
%A more realistic example is that of a security game between an attacker who chooses up to $b_2$ paths in a transportation network to route illegal goods, and the operator who can interdict up to $b_1$ edges. We can model this game in our setup by viewing $\nodes$ (resp. $\edges$) as the set of edges (resp. paths) in the network, and the monitoring set for each edge in $\nodes$ as the set of paths which contain that edge. Now one can see that an MSC is a minimum cardinality cut set, and an MSP is a set of maximum edge-disjoint paths. Using the max-flow min-cut theorem, we obtain that the sizes of MSCs and MSPs satisfy $\smsc = \semm$.
%
%
% for the classical Hide-and-Seek game (see Ch. 3.2 of \cite{karlin2016game}) based on minimum line-covers and maximum matchings; and also for the computer network security game studied by \cite{mavronicolas} based on minimum edge covers and maximum independent sets. Finally, our result also generalizes the NE derivation for the Infiltration Game with a Cable, as defined in Ch. 2.1 of \cite{garnaev2000search}. 
 



% $\bullet$ Two-stage sequential game. Defender chooses a randomized detection strategy. The attacker knows defender's strategy (but not the realizations). The defender wants to minimize the number of countermeasures allocated in the network, while maintaining a targeted performance.Attacker is interested in minimizing the number of detected attacks.

% $\bullet$ the psychical system is abstracted into network-theoretical representation. Physical attacks causing hydraulic failures.  both defender and attacker use hydraulic information about the network to select locations. nodes represent access points that can be seen by the public and can be attacked, for example, by inducing backflow at hydrants, sabotaging valves, or accessing pipes through manholes. These mechanical failures causing hydraulic faults can be detected using various detection mechanisms (e.g. fault detection matrix).

% $\bullet$ defense strategies: random defense strategy (randomly patrol the distribution system for defensive cover); critical node defense strategy; hardening strategies (place security equipment, e.g. cameras, guards).


% $\bullet$ in allocating countermeasures, a small number of nodes should be selected among hundreds or thousands to be hardened. Critical nodes can be identified based on consequences using simulations. Critical nodes which generate high consequences.

% $\bullet$ budget-constrained utility cannot cover the entire system, hence inevitable blind spots.

%$\bullet$ Critical infrastructure, power, gas, and water networks. Spanning large geographical distances are vulnerable to intentional and unintentional threats, including physical and cyber failures. 





%Each failure event, e.g. leak, pipe break, and contaminant intrusion, generates a fault signature. This fault signature is based on system dynamics and can be estimated empirically or theoretically. Depending on the features of interest (e.g. flow, pressure, and quality) and types of failures (e.g. leak, pipeline break and contamination event), the fault event can be identified by comparing the observed residuals against the expected values at the sensing locations. Regardless of the type of failure and the features of interest, the physical phenomena is significantly mediated by the network topology. A failure event in pipeline network, such as pipe break, causes a disturbance in the local flow conditions and results in a pressure drop. The pressure signal spreads from the break point in all directions of the pipeline and dissipates as it travels through the pipelines due to friction and attenuation [cite]. The pipe break can be detected by detecting the change in the pressure conditions based on the signal recorded by a pressure sensor. In the event of contaminant intrusion, the contaminant spread is mediated by the network topology and flow conditions. The contaminant moves with the flow and reacts with its environment. Its signal decreases with the distance from the source due to decay and dilution governed by system dynamics [cite]. Based on the signal received from a sensor, the rate of change of the measured feature can be estimated and the potential fault can be identified.
 
 \subsection{\rem{To possibly reassign}}

\rem{In this section, we introduce a generic formulation of a strategic network inspection problem based on a game-theoretic model of defender-attacker interaction on a networked-infrastructure. In the network inspection problem, a strategic attacker is interested in damaging the components of the network while avoiding detection as much as possible, and the utility is interested in minimizing the number resources required to achieve a performance benchmark, defined here as the detection rate. The outcome of the solution of the network inspection problem is a defense strategy for the utility that prescribes the allocation of countermeasures (i.e., the number, locations, and randomization of sensing devices) in the network. Next, we describe the foundations for the game-theoretic model for general flow-networks, and in Section~\ref{sec:app}, we demonstrate and evaluate the proposed defense strategy using large-scale water distribution networks.} 




\textcolor{magenta}{In the context of infrastructure defense, this implies mobilizing sensing devices in the network by utility personnel and enabling synchronous collection of measurements at desired network locations.}


\textcolor{magenta}{This probability can be translated to scheduling visits to the specific locations in the network. Similar scheduling assignments are often performed by utilities for infrastructure inspection and maintenance.}


 \textcolor{magenta}{This random scheduling is performed daily by various utilities for routine activities, such as inspection and maintenance, where utility personnel visit different sites based on some defined schedule. For example, water utilities routinely sample water quality in random locations in the distribution system to comply with safety standards the Safe Drinking Water Act (SDWA) rules~\cite{tiemann2014safe}}. 
 

==> S2_problem.tex <==
%!TEX root = OR Manuscript V23.tex

%------------------------------------------------------------------------------------------------

\section{Problem Description}\label{sec:form}


\rev{In this section, we introduce a generic formulation of a strategic network inspection problem based on a game-theoretic model of defender-attacker interaction on the network with multiple resources.} \rev{Our formulation is a sequential game with constraints on the resulting detection performance.
[Can remove the second sentence]}



\rev{ALTERNATIVE: In this section, we introduce a generic formulation of a strategic network inspection problem. Our formulation is a defender-attacker sequential game with constraints on the detection performance resulting from the defender-attacker[/players'] interaction on the network.}


% Our formulation is a sequential game between a defender and an attacker with multiple resources. The game is defined with constraints on the detection performance resulting from the defender-attacker interaction on the network.}

% Our formulation considers a generic detection model,
% In this section, we formulate a strategic network inspection problem using a game-theoretic model of defender-attacker interaction on the network with mul
% Our formulation is a defender-attacker sequential game  
% In this section, we introduce a generic formulation of strategic network inspection problem.


% with constraints on the defender's resulting detection performance based on a generic detection model.
% }
% Our formulation is a mathematical program with constraints defined in terms of the Nash equilibria of this game.
%
%\tb{In this section, we define a model of strategic network interdiction, between a defender and attacker. We first introduce the objectives and capabilities of these players, and model their interaction as a strategic game.} Then, we formulate the network inspection problem as a mathematical program with equilibrium constraints. We also discuss the main assumptions of our formulation and highlight its practical relevance. 


%In this section, we first introduce a generic detection model and define a strategic game to model the interaction between an inspector and an attacker. Then, we formulate the network inspection problem under strategic attacks as a mathematical program with equilibrium constraints, and discuss the main features of the model.




%-----------------------------------------------------------------------------------------------------
\subsection{Defender and Attacker Models} \label{sec:detect}
%-----------------------------------------------------------------------------------------------------


Consider the setting where a defender (inspection agency) is concerned with positioning a set of smart detectors in a given network to monitor a predefined set of components, denoted $\edges$. The set of locations (or nodes) where a detector can be positioned is also predefined, and is denoted $\nodes$. 
%  \rem{All components in the set $\edges$ are ``critical'' in that they are prone to targeted attacks by an attacker (malicious entity).  The attacker can simultaneously attack multiple components, and compromise their functionality or quality of service. The attacker wishes to avoid being detected (i.e., maximize the number of undetected attacks), so as to reduce the overall functionality of the network. The defender seeks to inspect the network in order to maximize the number of detected attacks. On the other hand, the attacker wishes to avoid being detected (i.e., maximize the number of undetected attacks), so as to reduce the overall functionality of the network.} 
\rev{
All components in the set $\edges$ are ``critical'' in that they are prone to targeted attacks by an attacker (malicious entity) who wants to compromise their functionality or quality of service. First, the defender seeks to inspect the network with a minimum number of detectors while meeting a target detection performance against attacks. After observing the defender's inspection strategy, the attacker aims to simultaneously attack multiple components and avoid being detected, so as to reduce the overall functionality of the network.}

% The goal of the defender is to meet a target detection performance using a minimum-resource inspection strategy.
% The attacker aims to  simultaneously attack multiple components and avoid being detected, so as to reduce the overall functionality of the network. On the other hand, the defender seeks to inspect the network to minimize the number of undetected attacks in the worst-case scenario.

% \rev{

% }
% (i.e., minimize the maximum number of undetected attacks)
% (i.e., maximize the number of undetected attacks)
%\tg{}

%In this article, we adopt a sensing model following \cite{Ost1415211920040901} and \cite{sensors:autom} in which the detection of a failure event by a sensor is binary and only depends on the location of the sensor and the network component that is targeted. This  sensing model is, in practice, constructed based on the sensors' technological features (e.g., sensing range), type of failures (e.g., pipe bursts versus contamination events), and network topology. %In \cite{Ost1415211920040901}, the authors consider a network sensing problem where the operator places fixed sensors on the network to maximize the number of possible failure events that would be detected if realized.
%We use this  model to define the players' payoff functions in the simultaneous operator-attacker game. \tb{[repetition?]}

For our purpose, each \emph{detector} can be viewed as an integrated system comprised of a sensor, a detection software, a communication unit, and a human operator (utility employee) \citep{1219475}. When a detector is positioned at node $i\in\nodes$, the following steps are executed: Firstly, the sensor collects relevant state measurements from node $i$. These measurements capture the operational state of a subset of components $\set{i} \in 2^\edges$. Secondly, the detection software processes these measurements and generates a diagnostic signal indicating the number of attacks present within the component set $\set{i}$. Thirdly, the communication unit transmits the diagnostic signal to the defender. Finally, the human operator coordinates all these steps, and also ensures that the detector system is positioned in the network as intended by the defender. The cost of data collection, processing, and transmission is negligible in comparison to the cost of procuring the detector (which includes the cost of purchasing the equipment and the cost of employing the operator). \rev{[Should we make the previous text more specific and more ``public-sector oriented"?]}
For a detector positioned at node $i\in\nodes$, we refer to the set $\set{i}$ as a \emph{monitoring set}, because under the aforementioned assumptions, an attack to any component $e\in\edges$ can be detected if and only if $e\in\set{i}$. The tuple $\mathcal{G}\coloneqq(\nodes, \edges, \{\set{i}, \ i \in\nodes\})$ represents the \emph{detection model} of the network. Without loss of generality, we assume that each component in $\edges$ can be monitored from at least one node in $\nodes$.%\endnote{Indeed, if a set $\att^\prime$ of $k$ components cannot be monitored from any node in the network, then \attacker's incentive is to always target those components, and then allocate her remaining resources (if any) to target other components. We can remove those $k$ components from $\edges$, and solve the resulting game where \attacker has now $b_2 - k$ resources that she can allocate on the resulting subnetwork (where each component is now monitored from at least one node); we just need to increase her payoff by $k$ to account for the components already targeted and never detected by \defender.}

We assume that the defender has access to only a limited number of detectors for network inspection. This limitation results from the economic and operational constraints of the defender. For simplicity, we \rev{suppose} that all detectors are homogeneous in terms of their monitoring and detection capabilities, and cost. Let $b_1\in\mathbb{N}$ be the number of available detectors that can be simultaneously positioned on distinct nodes in $\nodes$. We denote a \emph{detector positioning} by a set $\Def\in 2^\nodes$ of nodes that receive detectors. The set of feasible detector positionings is then defined by $\mathcal{A}_1\coloneqq \{\Def\in 2^\nodes \ | \  |\Def|\leq b_1\}$. For a given detector positioning $\Def\in \mathcal{A}_1$, let $\set{\Def}\coloneqq \cup_{i\in \Def}\, \set{i}$ denote the set of components that are monitored by at least one detector in $\Def$. 



%Consider the setting where an inspection agency is concerned with positioning a set of detectors to monitor the critical components of a network that can be targeted by an attacker. For a given network, let $\nodes$ be the set of locations (or nodes) where a detector can be positioned, and let $\edges$ be the set of components that the inspector is interested in monitoring using available detectors.

%We adopt a detection model in which the detection of an attack by a detector is binary, i.e., each component is either monitored or not by a detector.
%Thus, for each node $i \in \nodes$, the set of components monitored by a detector positioned at node $i$ can be represented as a \emph{monitoring set} $\set{i} \in 2^\edges$. Equivalently, we say that the attack of a component $e \in \edges$ is detected by a detector positioned at node $i$ if and only if $e \in \set{i}$.  For our purpose, the \emph{detection model}, represented by the tuple $\mathcal{G} := (\nodes,\edges,\{\set{i}, \ i \in \nodes\})$, is assumed to be known.
%We assume that the set of \change{edge events that are detected by any sensor}{edges that a sensor can monitor} depends on its location on the network, and on the type of \annote{events of interest}{failure events (of interest?)} (bursts versus contaminant propagation). For every node $i \in \nodes$, we denote $\set{i} \in 2^{\edges}$ the set of components that a sensor placed in node $i$ can \change{detect}{monitor}. We assume that the operator knows $\set{i}$ for each node $i \in \nodes$.
%Next, we extend the notion of monitoring set $\set{i}$ for a single detector at node $i$ to the set of components that can collectively be monitored by a set of detectors. We denote a \emph{detector positioning} by a set $\Def \in 2^\nodes$ of nodes that receive detectors. For a given detector positioning $\Def$, let $\set{\Def}:= \bigcup_{i \in \Def }\, \set{i}$ denote the set of components that are monitored by at least one detector in $\Def$.
%We define a configuration of sensors (i.e. a \emph{sensor placement}) by a set $\Def \in 2^{\nodes}$ of nodes with \annote{sensors that are simultaneously active in}{active sensors that are simultaneously} monitoring the network. For a sensor placement $\Def$, the set of components that are \change{detected}{monitored} by $\Def$ is given by:
%\begin{align*}
%\set{\Def} := \bigcup_{i \in \Def }\, \set{i}.
%\end{align*}

To count the number of components in any given subset of components of $\edges$ that can be monitored using an arbitrary detector positioning, we define a \emph{detection function} $\detect: 2^{\nodes} \times 2^{\edges} \longrightarrow \mathbb{N}$. Specifically, for a detector positioning $\Def \in 2^\nodes$ and a subset of components $\att \in 2^\edges$, the value of $\detect(\Def,\att)$ is the number of components of $\att$ that are monitored by at least one detector positioned in $\Def$, i.e.:
%For a given sensor placement $\Def \in 2^\nodes$ and a subset of components $\att \in 2^\edges$, we define a \emph{detection function} $\detect: 2^{\nodes} \times 2^{\edges} \longrightarrow \mathbb{N}$ which determines the number of elements of $\att$ that are \change{detected}{monitored} by at least one sensor placed in $\Def$ 
\begin{align}
\forall (\Def,\att) \in 2^{\nodes} \times 2^{\edges},  \quad \valdet{\Def}{\att}  \coloneqq  |\set{\Def} \cap \att| \rem{= \sum_{e\in\att}\mathds{1}_{\{e \in \set{\Def}\}}}.\label{detect_sets}
\end{align}

The detection function has two natural properties: %We call $(\mathcal{G},\{\set{i}\})$ the sensing model of our network monitoring problem.

%\begin{lemma}\label{Submodularity}
%The sensing function $\detect$ satisfies the following properties:

\begin{enumerate}
\item For any subset of components $\att \in 2^\edges$, $\valdet{\cdot}{\att}$ is submodular and monotone:
\begin{align*}
\forall \att \in 2^\edges, \ \forall (\Def,\Def^\prime) \in (2^\nodes)^2, \quad \left\{\begin{array}{l}
\valdet{\Def \cup \Def^\prime}{\att} + \valdet{\Def \cap \Def^\prime}{\att} \leq \valdet{\Def}{\att} + \valdet{\Def^\prime}{\att},\mcr
\Def \subseteq \Def^\prime \ \Longrightarrow\ \valdet{\Def }{\att} \leq \valdet{\Def^\prime}{\att}.\end{array}\right.
\end{align*}
%\begin{align*}
%\forall \att \in 2^\edges, \ \forall (\Def,\Def^\prime) \in (2^\nodes)^2 \ | \ 
%\end{align*}
That is, adding a detector to a smaller detector positioning increases the number of monitored components in $\att$ by at least as many as when adding that detector to a larger detector positioning.

\item For any detector positioning $\Def \in 2^\nodes$, $\valdet{\Def}{\cdot}$ is finitely additive (a direct consequence of \eqref{detect_sets}):
\begin{align*}
\forall \Def \in 2^\nodes,\ \forall (\att,\att^\prime) \in (2^\edges)^2 \ | \ \att \cap \att^\prime = \emptyset, \quad \valdet{\Def}{\att \cup \att^\prime} = \valdet{\Def}{\att} + \valdet{\Def}{\att^\prime}.
\end{align*}
%\item Since $\detect$ is nonnegative, then we can also deduce that $\valdet{\cdot}{\att}$ is fractionally subadditive:
%\begin{align*}
%\forall \att \in 2^\edges, \ 
%\end{align*}
\end{enumerate}
%\color{black}
%\end{lemma}

Similar to the defender, the attacker is also resource-constrained, in that she can attack a subset of components $\att\in 2^\edges$ of the network of size no larger than $b_2\in\mathbb{N}$; we refer to such a subset as an \emph{attack plan}. This limitation arises from the attacker's constraints in gaining an unauthorized access to network components and compromising their functionality. However, the attacker has the flexibility to spread her attacks throughout the network. The set of all attack plans is given by $\mathcal{A}_2\coloneqq \{\att\in 2^\edges \ | \ |\att|\leq b_2\}$.  



\subsection{Network Inspection Problem}



% \rem{We model the simplest form of strategic interaction in which both players make individual decisions to maximize their objectives. Particularly, for a detector positioning $S\in\mathcal{A}_1$ and an attack plan $T\in\mathcal{A}_2$, the payoff of the defender (resp. attacker) is $\valdet{\Def}{\att}$ (resp. $\natt{\att} - \valdet{\Def}{\att}$).} 

In our model, the defender (resp. attacker) inspects (resp. attacks) the network using a detector positioning $\Def$ (resp. an attack plan $\att$) realized from a chosen probability distribution on the set $\mathcal{A}_1$ (resp. $\mathcal{A}_2$). 
%\tg{The defender (resp. attacker) inspects (resp. attacks) the network using a detector positioning $\Def$ (resp. an attack plan $\att$) realized from her own probability distribution on the set $\mathcal{A}_1$ (resp. $\mathcal{A}_2$).}
Specifically, the defender and attacker respectively choose a mixed inspection strategy $\sigma^1 \in 
\Delta(\mathcal{A}_1)$ and a mixed attack strategy $\sigma^2 \in  \Delta(\mathcal{A}_2)$, where 
$\Delta(\mathcal{A}_1)\coloneqq\{\sigma^1 \in [0,1]^{|\mathcal{A}_1|}\ | \ \sum_{{\Def} \in \mathcal{A}_1} \sigma^1_\Def = 1 \}$ and $\Delta(\mathcal{A}_2) \coloneqq \{\sigma^2 \in [0,1]^{|\mathcal{A}_2|}\ | \ \sum_{{\att} \in \mathcal{A}_2} \sigma^2_{\att} = 1 \}$ denote the strategy sets. Here, $\sigma^1_\Def$ (resp. $\sigma^2_\att$) represents the probability assigned to the detector positioning $\Def$ (resp. attack plan $\att$) by the defender's strategy $\sigma^1$ (resp. the attacker's strategy $\sigma^2$).  \rev{This model provides both players with the flexibility of changing their actions from one subset to another. For the defender, this means that her detectors can be repositioned from one subset of nodes to another. Practically, changes in detector positioning are executed by the utility personnel who use manual or automated means to shift detectors.}

% We are now in the position to introduce our network inspection problem, which we define as a mathematical program with equilibrium constraints.

\rev{We are now in the position to introduce our network inspection problem, which we define as a sequential game. In this problem, the defender (referred to as player 1 or \defender) is the leader and selects an inspection strategy $\sigma^1 \in \Delta(\mathcal{A}_1)$. The attacker (referred to as player 2 or \attacker) is the follower and selects an attack strategy $\sigma^2 \in \Delta(\mathcal{A}_2)$ after observing $\sigma^1$. Note that the attacker does not observe the realization of $\sigma^1$. We consider that the model parameters $(\mathcal{G}, b_1, b_2)$ are common knowledge. }



% We also assume that the attacker knows the defender's inspection strategy $\sigma^1 \in \Delta(\mathcal{A}_1)$, but does not know the realization of $\sigma^1$ [Justification]. 
\rev{
\emph{Second stage:} Given an inspection strategy $\sigma^1 \in \Delta(\mathcal{A}_1)$, the attacker aims to find an attack strategy $\sigma^2 \in \Delta(\mathcal{A}_2)$ that maximizes the expected number of undetected attacks: 
\begin{align}
U(\sigma^1,\sigma^2)\coloneqq \mathbb{E}_{(\sigma^1,\sigma^2)}[|\att| - \valdet{\Def}{\att}].\label{payoff2}
\end{align} 
We denote $B_2(\sigma^1,b_2)\coloneqq \argmax_{\sigma^2 \in \Delta(\mathcal{A}_2)}U(\sigma^1,\sigma^2)$ the set of attack strategies that are best responses to $\sigma^1$.

\emph{First stage:} The defender is interested in protecting the network against attacks with minimum resources. To evaluate the level of protection of the network, we define the following metric of detection performance against attacks: 
For a given a strategy profile $\sigma \in \Delta(\mathcal{A}_1) \times \Delta(\mathcal{A}_2)$, the \emph{expected detection rate}, denoted $\sdet{}$, is the expectation (under $\sigma$) of the ratio between the number of attacks that are detected and the total number of attacks:
\begin{align}
\sdet{} := \Expboth{}{}{\dfrac{\valdet{\Def}{\att}}{|\att|}}. \label{Exp_detection_rate}
\end{align}
Then, given the attacker’s resources $b_2$, the defender seeks to determine a minimum-resource inspection strategy (i.e., to minimize the number of detectors $b_1$ and strategically position them in the network), while ensuring that the expected detection rate is no less than a pre-specified threshold level $\alpha\in [0,1]$ \rev{for any best response strategy of the attacker}. 

[In the definition of the game in this section, should I use ``\defender'' and ``\attacker'' instead of ``defender'' and ``attacker''?]

The network inspection problem can be formulated as the following bilevel optimization problem:\hypertarget{(P)}{}
%\vspace{-0.3cm}
%Finally, we present the  network inspection problem, where we use the expected detection rate in equilibrium of the game $\Gamma$ as metric of strategic inspection performance.
%Consider the problem in which \defender is concerned with inspecting the network, while facing a strategic adversary \attacker whose attack capability is constrained by $b_2$. In this  problem, \defender aims to minimize the number of detectors, $b_1$, and strategically position them to ensure that the expected detection rate in any equilibrium of the induced game $\Gamma(b_1,b_2)$ does not fall below a pre-specified threshold. Formally, the network inspection problem can be posed as follows:\hypertarget{(P)}{}
% \begingroup
% \addtolength{\jot}{\spacingalign}
\begin{align}
(\mathcal{P}): \quad \underset{b_1,\, \sigma^{1}}{\text{minimize}}& \quad b_1\nonumber\\
\text{subject to}& \quad r(\sigma^{1},\sigma^{2}) \geq \alpha,  \quad \forall \sigma^{2} \in B_2(\sigma^{1},b_2) \label{all_NE}\\
& \quad \sigma^1 \in \Delta(\mathcal{A}_1)\nonumber \\
& \quad b_1 \in \mathbb{N}.\nonumber
\end{align}
% \endgroup


Constraints \eqref{all_NE} ensure that, given the number of attack resources $b_2$, the expected detection rate induced by the chosen number of detectors $b_1$ and their positioning $\sigma^1$ is at least $\alpha$ whenever the attacker plays a best response to $\sigma^1$. The optimal value of \ECOP, denoted $b_1^*$, is the minimum number of detectors for which constraints \eqref{all_NE} are satisfied. 
% Thus, $(b_1^\dag,\sigma^\dag)$ with $\sigma^\dag\in\nash(b_1^\dag,b_2)$ is an optimal solution of \ECOP, where the inspection strategy in $\sigma^\dag$ specifies a randomized positioning of $b_1^\dag$ detectors.
The target detection rate $\alpha$ reflects the performance requirement that the defender seeks to achieve against the attacker's strategy, besides seeking a minimum-resource inspection strategy.

}


% use the notations $U(\Def,\att) = U(\mathds{1}_{\{\Def\}},\mathds{1}_{\{\att\}})$ and $r(\Def,\att) = r(\mathds{1}_{\{\Def\}},\mathds{1}_{\{\att\}})$.}


For ease of exposition, we denote $\valdet{i}{e} := \valdet{\{i\}}{\{e\}}, \ \forall (i,e) \in \nodes \times \edges$.  \rev{We will also refer to the degenerate mixed-strategies $\mathds{1}_{\{\Def\}} \in \Delta(\mathcal{A}_1)$ and  $\mathds{1}_{\{\att\}} \in \Delta(\mathcal{A}_2)$ as $S$ and $T$.}  The \emph{support} of $\sigma^1 \in \Delta(\mathcal{A}_1)$ (resp. $\sigma^2 \in \Delta(\mathcal{A}_2)$) is defined as $\supp(\sigma^1) = \{\Def \in \mathcal{A}_1 \ | \ \sigma^1_{\Def} >0 \}$ (resp. $\supp(\sigma^2) = \{\att \in \mathcal{A}_2 \ | \ \sigma^2_{\att} >0 \}$). The \emph{node basis} of a strategy $\sigma^1 \in \Delta(\mathcal{A}_1)$, denoted  $\nbasis{\sigma^1}:= \{i \in \nodes \ | \ \mathbb{P}_{\sigma^1} (i \in \Def)>0\}$, is the set of nodes that are inspected with non-zero probability. Analogously, the \emph{component basis} of a strategy $\sigma^2 \in \Delta(\mathcal{A}_2)$, denoted $\ebasis{\sigma^2}:=\{e \in \edges \ | \ \mathbb{P}_{\sigma^2}(e \in \att) >0\}$, is the set of components that are targeted with positive probability.  %Finally, we refer to defender and attacker as \defender and \attacker, respectively. 
%\tb{[This is said when the game is defined, but you chose not to use P1/P2 in the discussion that followed]}

\rev{[$\uparrow$ These two paragraphs may be swapped $\downarrow$]}

% Despite its simplicity, the game $\Gamma(b_1,b_2)$
\rev{The problem \ECOP} captures some of the key features of network inspection in strategic settings; see Table~\ref{List_app} for a comparison of various applications. Firstly, the underlying detection model $\mathcal{G}$ is generic in that it represents the detection capability of the defender, without making further modeling assumptions about how the monitoring sets $\set{i}$, $i\in\nodes$, depend on specific aspects such as sensing technology employed by the detectors, the different means that the attacker may use in targeting a component, and the network's topological structure. Secondly, it considers multiple resources on the part of both defender and attacker. This is a particularly desirable feature for strategic inspection settings, in which the attacker can simultaneously attack multiple components across the network, and the defender's inspection involves positioning multiple detectors \rev{[Still trying to propose the idea of coordination: ``the defender's inspection involves coordinating the positioning of multiple detectors'']} in order to monitor a large number of critical components.
%This feature is characteristic of situations in which the defender (resp. attacker) has the capability to simultaneously inspect (resp. attack) multiple nodes (resp. components) across the network.  \tg{Thirdly, our game is large-scale in that both players have combinatorial action sets. Indeed, in inspecting networks with a large number of critical components that can be arbitrarily targeted by a resource-constrained attacker, the defender faces the issue of choosing subsets of detector positionings and the corresponding inspection probabilities.}
%
In contrast, the previously studied security games typically assume that one or both players are constrained to using only a single resource; see Table~\ref{List_games}. \rev{[Although the mentioned security games are simultaneous games and are not exactly like our new sequential game (for now), I believe that comparative sentence still works.]}



% the set of $\epsilon-$NE of the game $\Gamma(b_1,b_2)$. When there is no confusion, we will refer to $\Gamma(b_1,b_2)$, $\nash(b_1,b_2)$, and $\nash_{\epsilon}(b_1,b_2)$ simply as $\Gamma$, $\nash$, and $\nash_{\epsilon}$.%\endnote{From a game-theoretic viewpoint, a NE in mixed strategies describes the behavior of \defender and \attacker who play the game $\Gamma$ repeatedly against each other and ignore any strategic relationship in-between plays. Thus, NE in mixed strategies can be viewed as a stochastic steady state of the repeated interaction between players. By extension, we view $\epsilon-$NE as strategy profiles in which the players are almost at a stochastic steady state, i.e., no player has more than an incentive of $\epsilon$ to change her mixed strategy.} 

%Given the parameters $b_1$ and $b_2$, we denote $\nash(b_1,b_2)$ the set of NE of the game $\Gamma(b_1,b_2)$\rem{, which is nonempty since $\Gamma(b_1,b_2)$ is a finite game}.

%\begin{align}
%\forall i \in \{1,2\}, \ \forall \sigma^i \in \Delta(\mathcal{A}_i), \ U_i(\sigma^{i^\prime},\sigma^{-i^\prime}) \geq U_i(\sigma^i,\sigma^{-i^\prime}) - \epsilon. 
%\label{best_epsilon}
%\end{align}

%\section{General Case}




%\note{For now, I am vague... If you want, we can formally rewrite the monitoring problem here. For example, it could be to determine  $b_1$ and $\sigma^1$ such that (i) for any $\sigma^2$, $r_{\sigma} \geq \alpha$, or (ii) in equilibrium $r_{\sigma} \geq \alpha$.}


%\begin{example}[Water Contamination Scenario]
%Consider the network shown in Fig.~\ref{Example1}. Assume a sensing model in which a sensor placed at any node can monitor components at one-hop vertically, and at two hops horizontally. Thus, $\set{i_1} = \{e_1,e_2,e_3\}$, $\set{i_2} = \{e_1,e_2,e_4\}$, $\set{i_3} = \{e_1,e_2,e_5\}$, $\set{i_4} = \{e_4,e_6,e_7\}$, $\set{i_5} = \{e_5,e_6,e_8\}$, $\set{i_6} = \{e_3,e_9,e_{10}\}$, $\set{i_7} = \{e_7,e_9,e_{10}\}$, $\set{i_8} = \{e_8,e_9,e_{10}\}$.
%
%%%%---------------------------------------------------------------------------------------------------
%\def \sizefig {1.4cm}
%\def \scalefig {\small}
%\def \innersepfig {0.07cm}
%%%%---------------------------------------------------------------------------------------------------
%
%\begin{figure}[ht]
%\centering
%{\scalefig
%\begin{tikzpicture}[-,auto,x=\sizefig, y=\sizefig,
%  thick,main node/.style={circle,draw,inner sep = \innersepfig,black},main node2/.style={circle,black,draw,fill=blue!60,inner sep = \innersepfig},flow_a/.style ={gray!100}]
%\tikzstyle{edge} = [draw,thick,-,black]
%\tikzstyle{cut} = [draw,very thick,-]
%\tikzstyle{match} = [draw,very thick,black,-, dashed]
%\tikzstyle{flow} = [draw,line width = 1.5pt,->,gray!100]
%
%%\begin{scope}[yshift=0, xshift =-110]
%	\node[main node] (1) at (0,2) {$i_1$};
%	\node[main node] (2) at (1,2) {$i_2$};
%	\node[main node2] (3) at (2,2) {$i_3$};
%	\node[main node] (4) at (1,1) {$i_4$};
%	\node[main node] (5) at (2,1) {$i_5$};
%	\node[main node] (6) at (0,0) {$i_6$};
%	\node[main node] (7) at (1,0) {$i_7$};
%	\node[main node] (8) at (2,0) {$i_8$};
%	%\node[main node, draw=white] (7) at (3.5,-0.5) {\textbf{a}};
%	
%	\path[edge]	
%	%(2) component (5)
%	%(1) component  (2)
%	(1) component node[left]{$e_3$} (6)
%	(4) component node {$e_6$} (5)
%	(2) component[double,blue!80]  node {$e_2$} (3)
%	(2) component node[left] {$e_4$} (4)
%	(6) component node[below] {$e_9$} (7)
%	(7) component node[below] {$e_{10}$} (8)
%	%(3) component  (5)	
%	%(4) component  (6)
%	(5) component node {$e_8$} (8);
%
%	\path[edge]
%	(1) component[double,blue!80] node {$e_1$} (2)
%	(3) component[double,blue!80] node {$e_5$} (5)
%	(4) component node[left] {$e_7$} (7);
%%\end{scope}
%
%\end{tikzpicture}}
%
%\caption{Example network. The monitoring set $\set{i_3} = \{e_1,e_2,e_5\}$ is represented by the double blue components.} \label{Example1}
%\end{figure}
%


%Consider the problem \ECOP with the target expected detection rate $\alpha = 0.75$ and the number of attack resources $b_2 = 2$. For this small-sized problem, we can solve  \lpo and \lpt to compute the NE of $\Gamma$, and obtain  the expected detection rate in any NE for each $b_1 \in \mathbb{N}$; see Table~\ref{r_sigma_example}. Notice that for a given $b_1$, the expected detection rate is the same in any NE.
%\begin{table}[htbp]
%\centering
%\caption{Expected detection rate in equilibrium for every $b_1 \in \mathbb{N}$.}
%\def\arraystretch{\spacingtable}
%\begin{tabular}{|c|c|c|c|c|c|}\hline $b_1$ & 0 & 1 & 2 & 3 & $\geq 4$ \\\hline $\sdet{*}$ & 0 & $\frac{2}{7}$ & $\frac{4}{7}$ & $\frac{6}{7}$ & 1 \\\hline \end{tabular}
%\label{r_sigma_example}
%\end{table}
%
%From Table~\ref{r_sigma_example}, we conclude that the optimal value of (\hyperlink{(P)}{$\mathcal{P}$}) is $b_1^\dag = 3$, i.e., with  $3$ sensors, \defender is capable of detecting $\frac{6}{7} \geq \alpha$ of the failure events in equilibrium. However, as mentioned in Section~\ref{sec:Formal problem}, this method does not extend to larger networks, as it requires solving large \lpo and \lpt for each $b_1 \in \mathbb{N}$ and checking if the constraint on the expected detection rate in any equilibrium \eqref{all_NE} is met.

%\end{example}

%\subsection{Network Monitoring Problem}\label{sec:Formal problem}
%\tb{[Do we need an introductory sentence?]}
%

% More importantly, any strategy profile \rev{[Can we talk about strategy profiles in optimization problems?]} \rem{of the game $\Gamma(b_1,b_2)$} can be associated with a metric of detection performance against attacks. For a given strategy profile $\sigma \in \Delta(\mathcal{A}_1) \times \Delta(\mathcal{A}_2)$, we define this metric as the \emph{expected detection rate}, $\sdet{}$, which is the expectation (under $\sigma$) of the ratio between the number of attacks that are detected and the total number of attacks:
% \begin{align}
% \sdet{} := \Expboth{}{}{\dfrac{\valdet{\Def}{\att}}{|\att|}}. \label{Exp_detection_rate}
% \end{align}
% %\end{definition}

% We are now in the position to introduce our network inspection problem, which we define as a mathematical program with equilibrium constraints. In this problem, given the attacker's resources $b_2$, the defender seeks to determine a minimum-resource inspection strategy (i.e., to minimize the number of detectors $b_1$ and strategically position them in the network), while ensuring that the expected detection rate \rem{in any equilibrium of the game $\Gamma(b_1,b_2)$} is no less than a pre-specified threshold level $\alpha\in [0,1]$ \rev{for any \attacker's best response strategy}:\hypertarget{(P)}{}
% %\vspace{-0.3cm}
% %Finally, we present the  network inspection problem, where we use the expected detection rate in equilibrium of the game $\Gamma$ as metric of strategic inspection performance.
% %Consider the problem in which \defender is concerned with inspecting the network, while facing a strategic adversary \attacker whose attack capability is constrained by $b_2$. In this  problem, \defender aims to minimize the number of detectors, $b_1$, and strategically position them to ensure that the expected detection rate in any equilibrium of the induced game $\Gamma(b_1,b_2)$ does not fall below a pre-specified threshold. Formally, the network inspection problem can be posed as follows:\hypertarget{(P)}{}
% \begingroup
% \addtolength{\jot}{\spacingalign}
% \rem{\begin{align}
% (\mathcal{P}): \quad \underset{b_1,\, \sigma^\dag}{\text{minimize}}& \quad b_1\nonumber\\
% \text{subject to}& \quad \sdet{*} \geq \alpha, \quad \quad \forall \sigma^* \in \nash(b_1,b_2) \label{all_NE}\\
% & \quad \sigma^\dag \in \nash(b_1,b_2) \label{one_NE}\\
% & \quad b_1 \in \mathbb{N}.\nonumber
% \end{align}}
% \endgroup

% \begingroup
% \addtolength{\jot}{\spacingalign}
% \rev{\begin{align}
% (\mathcal{P}): \quad \underset{b_1,\, \sigma^{1^*}}{\text{minimize}}& \quad b_1\nonumber\\
% \text{subject to}& \quad r(\sigma^{1^*},\sigma^{2^*}) \geq \alpha, \quad \quad \forall \sigma^{2^*} \in B(\sigma^{1^*},b_2) \label{all_NE}\\
% & \quad b_1 \in \mathbb{N}.\nonumber
% \end{align}}
% \endgroup

% \begin{align}
% (\mathcal{P}): \quad \underset{b_1,\, \sigma^{1^*}}{\text{minimize}}& \quad b_1\nonumber\\
% \text{subject to}& \quad r(\sigma^{1^*},\sigma^{2^*}) \geq \alpha\\
% & \sigma^{2^*} \in \argmax U(\sigma^{1^*},b_2)\label{all_NE}\\
% & \quad b_1 \in \mathbb{N}.\nonumber
% \end{align}

% $$r =  -U + 1$$
% \rev{[Few questions: nothing guarantees me right now that the optimal detector positioning for $\mathcal{P}$ and the maximin problem (former game) are the same. Yet, $(\mathcal{P})$ needs the problem $\Gamma$ first, for the definition of best responses...]}
% \tb{New version that does not work:}
% \begin{align}
% (\mathcal{P}): \quad \underset{b_1,\, \sigma^1}{\text{minimize}}& \quad b_1\nonumber\\
% \text{subject to}& \quad r(\sigma^1,\sigma^2) \geq \alpha, \quad \quad \forall \sigma^2 \in \argmax |T| - F(S,T) \label{all_NE}\\
% & \quad \sigma^1 \in \Delta(\mathcal{A}_1) \label{one_NE}\\
% & \quad b_1 \in \mathbb{N}.\nonumber
% \end{align}

% \tb{New version that does not work:}
% \begin{align}
% (\mathcal{P}): \quad \underset{b_1,\, \sigma^1}{\text{minimize}}& \quad b_1\nonumber\\
% \text{subject to}& \quad \mathbb{E}_\sigma[|T| - F(S<T)] \leq (1-\alpha) \mathbb{E}_\sigma[|T|], \quad \quad \forall \sigma^2 \in \argmax |T| - F(S,T) \label{all_NE}\\
% & \quad \sigma^1 \in \Delta(\mathcal{A}_1) \label{one_NE}\\
% & \quad b_1 \in \mathbb{N}.\nonumber
% \end{align}

%\begin{align*}
%%\fbox{$
%\begin{array}{lrclcl}(\mathcal{P}): &\underset{b_1 \in \mathbb{N}, \sigma^\dag \in \Delta(\mathcal{A}_1)\times \Delta(\mathcal{A}_2) }{\text{minimize}} & &b_1 &&\\
%&\text{subject to} &&\sdet{*} \geq \alpha,&& \forall \sigma^* \in \nash(b_1,b_2)\\
%&&& \sigma^\dag \in \nash(b_1,b_2)\end{array}
%%$}
%\end{align*}

%\vspace{-0.3cm}


%where $\alpha \in [0,1]$ denotes the target detection performance that \defender must achieve (for e.g., to meet the operational requirements on limiting network losses due to attacks).Thus, $(b_1^\dag,\sigma^\dag)$ with $\sigma^\dag \in \nash(b_1^\dag,b_2)$ is an optimal solution of \ECOP, where the inspection strategy in $\sigma^\dag$ specifies a positioning of the $b_1^\dag$ detectors in equilibrium such that the target detection performance $\alpha$ is met. 


%\subsection*{?}


%Given a detector positioning $\Def\in 2^{\nodes}$ and a network component $e \in \edges$, $\valdet{\Def}{e}=\mathds{1}_{\{e \in \set{\Def}\}}$ determines whether or not $e$ is monitored by at least one detector positioned in $\Def$.



%\subsection{Model Discussion}

%Cite Tambe








%The definition of the detection model $\mathcal{G} = (\nodes,\edges,\{\set{i}, \ i \in \nodes\})$, along with the detection function $\detect$, enable us to model a variety of settings. Indeed, since no assumption is made on the nature of $\nodes$ and $\edges$, these sets can represent single locations in a network, as well as more complex combinatorial objects such as network paths. Additionally, no assumption is made on the monitoring sets $\set{i}$, for $i \in \nodes$. Thus, we can apply the detection model to different applications. The first example could be a ``physical'' detection, where the attacker targets pipes in a network, and the defender is an inspection agency that sends inspection teams to identify the resulting failures. If they do not have any sensing technology, then they need to manually inspect a pipe in order to detect a failure. In that case, $\nodes = \edges$, and $\forall i \in \nodes, \ \set{i} = \{i\}$, which is related to search games.

%However, the advantage of the monitoring sets is that they can model more complex physical settings, where a detector is again an agent (police officer) who patrols roads in order to find a hiding robber. In the setting where the agent can only find the robber if they hide in a safe-house along the road patrolled by the agent, then our model becomes can be applied, and is such that a ``node'' $i \in \nodes$ is a road taken by the agent, and $e \in \edges$ is a safe-house. Similarly, $\set{i}$ is the set of safe-houses along the road $i$.

%Baykal-Gursoy, Mavronicolas, Pita et al
%
%All of these works are subsumed by our model.
%
%Finally, our model also applies to settings where an inspector possesses a sensing technology to detect attacks occurring in her vicinity. For example, in the context of water networks, a failure event such as pipe burst or contamination event generates a signal which propagates through the network.  Depending on the sensors' technological features, and their locations in the network, the signal can then be identified for failure detection before it dissipates in the network. 
%\cite{Ost1415211920040901} and \cite{sensors:autom} argue that such a binary detection model can be considered.  This detection model is typically obtained based on the outcome of a threshold-based rule that determines the detectors' capability to monitor different types of attacks from each location \citep{allen:smart,doi:10.1061/(ASCE)WR.1943-5452.0000339,sensors:autom}. 
%
%
%Regarding the strategic game, one of the main generalization is the fact that we allowed both players to have multiple resources.

%While some works allow the attacker to have multiple resources, very few consider multiple resources for the inspector, as it increases the difficulty in solving the problem. We address this issue by deriving some structural results, based on game-theoretic and combinatorial arguments. In particular we exploit properties of the detection model, such as the submodularity of the detection function $\detect$. This enabled us to derive a rigorous solution approach.



%1) key features:
%important aspects of security games (check slides).
%
%
%
%Strategic defender-attacker game, with a generic sensing model.


%We emphasize the generality of our model. 
%First, no assumption on $\nodes$ and $\edges$.

%Practical settings where the detection function is relevant


%This was possible because we chose to make this abstraction of the detection model, and did not model the specific details, such as false alarm and misdetections.
%Additionally, we stress that the game is played on the critical components of the network, while there may be others that are not critical, hence not attractive targets to the attacker. However, we do not distinguish different levels of criticality among them.
%Note that criticality is not relevant to (patrolling) settings where the defender is an inspector who wants to catch a malicious person. 



%Aspect of erroneous detections. False alarm misdetections

%Criticality.

%It does not take into account for the heterogeneous criticality of components

%Nevertheless, since we deal with strategic aspects and not operational aspect of sensor scheduling, we do not account for specific modeling features such as errors in detections and communication bandwidth etc.





==> S2_problem_LS.tex <==
%!TEX root = OR Manuscript V23.tex

%------------------------------------------------------------------------------------------------

\section{Problem Description}\label{sec:form}
In this section, we introduce a generic formulation of a strategic network inspection problem based on a game-theoretic model of defender-attacker interaction on a networked-infrastructure. In the network inspection problem, a strategic attacker is interested in damaging the components of the network while avoiding detection as much as possible, and the utility is interested in minimizing the number resources required to achieve a performance benchmark, defined here as the detection rate. The outcome of the solution of the network inspection problem is a defense strategy for the utility that prescribes the allocation of countermeasures (i.e., the number, locations, and randomization of sensing devices) in the network. Next, we describe the foundations for the game-theoretic model for general flow-networks, and in Section~\ref{sec:app}, we demonstrate and evaluate the proposed defense strategy using large-scale water distribution networks. 


%To address the problem of network defense against a strategic attacker, we propose a \textit{game-theoretic formulation} of the strategic network monitoring problem. The physical network is abstracted into a network-theoretical representation, in which links represent system components that can be accessed and attacked, for example, inducing backflow at fire hydrants, sabotaging valves, or accessing pipes through manholes (cite). Network nodes represent access points in which the utility can deploy sensing devices to monitor and detect mechanical and process failures using various detection mechanisms, e.g., pipe bursts and leaks (cite). In our setting, both the defender and the attacker use information about the flow-network to select the defense/attack locations, respectively.  Our modeling framework applies to flow-networks such as water, oil, and gas, which allow for the application of sensing technologies, including flow meters and pressure sensors, capable of continuously collecting and transmitting measurements at fine temporal resolution~\citep{PHILLIPS20131,XING2019291}. These sensing technologies facilitate in an accurate and timely estimation of the network state and operating conditions, and through advanced data analytics, enable the identification of possible pipeline faults and leakages. We demonstrate our proposed approach by, firstly, presenting the theoretical foundation for the monitoring strategy under strategic attacks for general flow-networks, and secondly, evaluating the proposed strategy using a set of realistic, large-scale water distribution networks. 

%\rev{ALTERNATIVE: In this section, we introduce a generic formulation of a strategic network inspection problem. Our formulation is a defender-attacker sequential game with constraints on the detection performance resulting from the defender-attacker[/players'] interaction on the network.}


% Our formulation is a sequential game between a defender and an attacker with multiple resources. The game is defined with constraints on the detection performance resulting from the defender-attacker interaction on the network.}

% Our formulation considers a generic detection model,
% In this section, we formulate a strategic network inspection problem using a game-theoretic model of defender-attacker interaction on the network with mul
% Our formulation is a defender-attacker sequential game  
% In this section, we introduce a generic formulation of strategic network inspection problem.


% with constraints on the defender's resulting detection performance based on a generic detection model.
% }
% Our formulation is a mathematical program with constraints defined in terms of the Nash equilibria of this game.
%
%\tb{In this section, we define a model of strategic network interdiction, between a defender and attacker. We first introduce the objectives and capabilities of these players, and model their interaction as a strategic game.} Then, we formulate the network inspection problem as a mathematical program with equilibrium constraints. We also discuss the main assumptions of our formulation and highlight its practical relevance. 


%In this section, we first introduce a generic detection model and define a strategic game to model the interaction between an inspector and an attacker. Then, we formulate the network inspection problem under strategic attacks as a mathematical program with equilibrium constraints, and discuss the main features of the model.




%-----------------------------------------------------------------------------------------------------
\subsection{Defender and Attacker Models} \label{sec:detect}
%-----------------------------------------------------------------------------------------------------
The physical flow-network is abstracted into a \textit{network-theoretical} representation, in which a defender (utility) is concerned with positioning a set of smart detectors in a given network to monitor its components, denoted $\edges$ (edges). The set of locations where a detector can be positioned is denoted $\nodes$ (nodes). All components in the set $\edges$ are ``critical'' in the sense that they are prone to targeted attacks by an attacker (malicious entity) that wants to compromise their functionality. In water distribution networks, for example, these attacks could include inducing backflow at fire hydrants, sabotaging valves, or damaging pipes through manholes access (cite). 
%These attacks can compromise system integrity and quality of service (cite). 
These events, in turn,  cause disturbances in the local flow and pressure conditions. These disturbances propagate in the network and can be detected by monitoring and detecting a change in the flow or pressure conditions based on the signal recorded by a sensor. %A wide range of sensing devices can be used to detect and locate various mechanical and physical faults. 
Low-cost flow and pressure sensors are the most ubiquitous sensing devices used for water, oil and gas pipeline monitoring. Flow and pressure sensors can be easily mounted on pipelines through many access points in the network, including manholes, valves, or fire hydrant (cite). Based on the signals received from the sensor and using signal processing and data-mining techniques, the state of the system (e.g., the rate of change of pressure or flow) can be estimated, which in turn could indicate a potential fault (cite). Each failure event generates a fault signature, which is based on system dynamics and can be estimated empirically or theoretically. The fault event can then be identified by comparing the observed residuals against the expected values at the sensing locations. 

Hence, for our purposes, we define a \emph{detector}, which can be viewed as an integrated system comprised of a sensor, a detection software, a communication unit, and a human operator (utility employee) \citep{1219475}. When a detector is positioned at node $i\in\nodes$, the following steps are executed: Firstly, the sensor collects relevant state measurements from node $i$. These measurements capture the operational state of a subset of components $\set{i} \in 2^\edges$. Secondly, the detection software processes these measurements and generates a diagnostic signal indicating the number of attacks present within the component set $\set{i}$. Thirdly, the communication unit transmits the diagnostic signal to the defender. Finally, the human operator coordinates all these steps, and also ensures that the detector system is positioned in the network as intended by the defender. \textcolor{red}{I don't really understand the last step. First, why does a human need to coordinate the previous steps, I think they are automated. And I don't get the second part. Do you mean to say that the defender (operator) can position these detectors anywhere in the network? if yes, then I suggest just say that.}The cost of data collection, processing, and transmission is negligible in comparison to the cost of procuring the detector (which includes the cost of purchasing the equipment and the cost of employing the operator). %\rev{[Should we make the previous text more specific and more ``public-sector oriented"?]}
For a detector positioned at node $i\in\nodes$, we refer to the set $\set{i}$ as a \emph{monitoring set}, because under the aforementioned assumptions, an attack to any component $e\in\edges$ can be detected if and only if $e\in\set{i}$. The tuple $\mathcal{G}\coloneqq(\nodes, \edges, \{\set{i}, \ i \in\nodes\})$ represents the \emph{detection model} of the network. We assume that the utility has knowledge of the network dynamics, sensing hardware and software capabilities and is able to estimate the detection model $\mathcal{G}\coloneqq(\nodes, \edges, \{\set{i}, \ i \in\nodes\})$. Additionally, without loss of generality, we assume that each component in $\edges$ can be monitored from at least one node in $\nodes$.  %\endnote{Indeed, if a set $\att^\prime$ of $k$ components cannot be monitored from any node in the network, then \attacker's incentive is to always target those components, and then allocate her remaining resources (if any) to target other components. We can remove those $k$ components from $\edges$, and solve the resulting game where \attacker has now $b_2 - k$ resources that she can allocate on the resulting subnetwork (where each component is now monitored from at least one node); we just need to increase her payoff by $k$ to account for the components already targeted and never detected by \defender.}

We assume that the defender has access to only a limited number of detectors for network inspection. This limitation results from the economic and operational constraints of the defender. For simplicity, we \rev{suppose} that all detectors are homogeneous in terms of their monitoring and detection capabilities, and cost. Let $b_1\in\mathbb{N}$ be the number of available detectors that can be simultaneously positioned on distinct nodes in $\nodes$. We denote a \emph{detector positioning} by a set $\Def\in 2^\nodes$ of nodes that receive detectors. The set of feasible detector positionings is then defined by $\mathcal{A}_1\coloneqq \{\Def\in 2^\nodes \ | \  |\Def|\leq b_1\}$. For a given detector positioning $\Def\in \mathcal{A}_1$, let $\set{\Def}\coloneqq \cup_{i\in \Def}\, \set{i}$ denote the set of components that are monitored by at least one detector in $\Def$. 



%Consider the setting where an inspection agency is concerned with positioning a set of detectors to monitor the critical components of a network that can be targeted by an attacker. For a given network, let $\nodes$ be the set of locations (or nodes) where a detector can be positioned, and let $\edges$ be the set of components that the inspector is interested in monitoring using available detectors.

%We adopt a detection model in which the detection of an attack by a detector is binary, i.e., each component is either monitored or not by a detector.
%Thus, for each node $i \in \nodes$, the set of components monitored by a detector positioned at node $i$ can be represented as a \emph{monitoring set} $\set{i} \in 2^\edges$. Equivalently, we say that the attack of a component $e \in \edges$ is detected by a detector positioned at node $i$ if and only if $e \in \set{i}$.  For our purpose, the \emph{detection model}, represented by the tuple $\mathcal{G} := (\nodes,\edges,\{\set{i}, \ i \in \nodes\})$, is assumed to be known.
%We assume that the set of \change{edge events that are detected by any sensor}{edges that a sensor can monitor} depends on its location on the network, and on the type of \annote{events of interest}{failure events (of interest?)} (bursts versus contaminant propagation). For every node $i \in \nodes$, we denote $\set{i} \in 2^{\edges}$ the set of components that a sensor placed in node $i$ can \change{detect}{monitor}. We assume that the operator knows $\set{i}$ for each node $i \in \nodes$.
%Next, we extend the notion of monitoring set $\set{i}$ for a single detector at node $i$ to the set of components that can collectively be monitored by a set of detectors. We denote a \emph{detector positioning} by a set $\Def \in 2^\nodes$ of nodes that receive detectors. For a given detector positioning $\Def$, let $\set{\Def}:= \bigcup_{i \in \Def }\, \set{i}$ denote the set of components that are monitored by at least one detector in $\Def$.
%We define a configuration of sensors (i.e. a \emph{sensor placement}) by a set $\Def \in 2^{\nodes}$ of nodes with \annote{sensors that are simultaneously active in}{active sensors that are simultaneously} monitoring the network. For a sensor placement $\Def$, the set of components that are \change{detected}{monitored} by $\Def$ is given by:
%\begin{align*}
%\set{\Def} := \bigcup_{i \in \Def }\, \set{i}.
%\end{align*}

To count the number of components in any given subset of components of $\edges$ that can be monitored using an arbitrary detector positioning, we define a \emph{detection function} $\detect: 2^{\nodes} \times 2^{\edges} \longrightarrow \mathbb{N}$. Specifically, for a detector positioning $\Def \in 2^\nodes$ and a subset of components $\att \in 2^\edges$, the value of $\detect(\Def,\att)$ is the number of components of $\att$ that are monitored by at least one detector positioned in $\Def$, i.e.:
%For a given sensor placement $\Def \in 2^\nodes$ and a subset of components $\att \in 2^\edges$, we define a \emph{detection function} $\detect: 2^{\nodes} \times 2^{\edges} \longrightarrow \mathbb{N}$ which determines the number of elements of $\att$ that are \change{detected}{monitored} by at least one sensor placed in $\Def$ 
\begin{align}
\forall (\Def,\att) \in 2^{\nodes} \times 2^{\edges},  \quad \valdet{\Def}{\att}  \coloneqq  |\set{\Def} \cap \att|.\label{detect_sets}
\end{align}

The detection function has two natural properties: %We call $(\mathcal{G},\{\set{i}\})$ the sensing model of our network monitoring problem.

%\begin{lemma}\label{Submodularity}
%The sensing function $\detect$ satisfies the following properties:

\begin{enumerate}
\item For any subset of components $\att \in 2^\edges$, $\valdet{\cdot}{\att}$ is submodular and monotone:
\begin{align*}
\forall \att \in 2^\edges, \ \forall (\Def,\Def^\prime) \in (2^\nodes)^2, \quad \left\{\begin{array}{l}
\valdet{\Def \cup \Def^\prime}{\att} + \valdet{\Def \cap \Def^\prime}{\att} \leq \valdet{\Def}{\att} + \valdet{\Def^\prime}{\att},\mcr
\Def \subseteq \Def^\prime \ \Longrightarrow\ \valdet{\Def }{\att} \leq \valdet{\Def^\prime}{\att}.\end{array}\right.
\end{align*}
%\begin{align*}
%\forall \att \in 2^\edges, \ \forall (\Def,\Def^\prime) \in (2^\nodes)^2 \ | \ 
%\end{align*}
That is, adding a detector to a smaller detector positioning increases the number of monitored components in $\att$ by at least as many as when adding that detector to a larger detector positioning.

\item For any detector positioning $\Def \in 2^\nodes$, $\valdet{\Def}{\cdot}$ is finitely additive (a direct consequence of \eqref{detect_sets}):
\begin{align*}
\forall \Def \in 2^\nodes,\ \forall (\att,\att^\prime) \in (2^\edges)^2 \ | \ \att \cap \att^\prime = \emptyset, \quad \valdet{\Def}{\att \cup \att^\prime} = \valdet{\Def}{\att} + \valdet{\Def}{\att^\prime}.
\end{align*}
%\item Since $\detect$ is nonnegative, then we can also deduce that $\valdet{\cdot}{\att}$ is fractionally subadditive:
%\begin{align*}
%\forall \att \in 2^\edges, \ 
%\end{align*}
\end{enumerate}
%\color{black}
%\end{lemma}

Similar to the defender, the attacker is also resource-constrained, in that she can attack a subset of components $\att\in 2^\edges$ of the network of size no larger than $b_2\in\mathbb{N}$; we refer to such a subset as an \emph{attack plan}. This limitation arises from the attacker's constraints in gaining an unauthorized access to network components and compromising their functionality. However, the attacker has the flexibility to spread her attacks throughout the network. The set of all attack plans is given by $\mathcal{A}_2\coloneqq \{\att\in 2^\edges \ | \ |\att|\leq b_2\}$.  



\subsection{Network Inspection Problem}



% \rem{We model the simplest form of strategic interaction in which both players make individual decisions to maximize their objectives. Particularly, for a detector positioning $S\in\mathcal{A}_1$ and an attack plan $T\in\mathcal{A}_2$, the payoff of the defender (resp. attacker) is $\valdet{\Def}{\att}$ (resp. $\natt{\att} - \valdet{\Def}{\att}$).} 

In our model, the defender (resp. attacker) inspects (resp. attacks) the network using a detector positioning $\Def$ (resp. an attack plan $\att$) realized from a chosen probability distribution on the set $\mathcal{A}_1$ (resp. $\mathcal{A}_2$). 
\tg{First, the defender seeks to inspect the network with a minimum number of detectors while meeting a target detection performance against attacks. After observing the defender's inspection strategy, the attacker aims to simultaneously attack multiple components and avoid being detected, so as to reduce the overall functionality of the network.}
%\tg{The defender (resp. attacker) inspects (resp. attacks) the network using a detector positioning $\Def$ (resp. an attack plan $\att$) realized from her own probability distribution on the set $\mathcal{A}_1$ (resp. $\mathcal{A}_2$).}
Specifically, the defender and attacker respectively choose a mixed inspection strategy $\sigma^1 \in 
\Delta(\mathcal{A}_1)$ and a mixed attack strategy $\sigma^2 \in  \Delta(\mathcal{A}_2)$, where 
$\Delta(\mathcal{A}_1)\coloneqq\{\sigma^1 \in [0,1]^{|\mathcal{A}_1|}\ | \ \sum_{{\Def} \in \mathcal{A}_1} \sigma^1_\Def = 1 \}$ and $\Delta(\mathcal{A}_2) \coloneqq \{\sigma^2 \in [0,1]^{|\mathcal{A}_2|}\ | \ \sum_{{\att} \in \mathcal{A}_2} \sigma^2_{\att} = 1 \}$ denote the strategy sets. Here, $\sigma^1_\Def$ (resp. $\sigma^2_\att$) represents the probability assigned to the detector positioning $\Def$ (resp. attack plan $\att$) by the defender's strategy $\sigma^1$ (resp. the attacker's strategy $\sigma^2$).  \rev{This model provides both players with the flexibility of changing their actions from one subset to another. For the defender, this means that her detectors can be repositioned from one subset of nodes to another. Practically, changes in detector positioning are executed by the utility personnel who use manual or automated means to shift detectors.}

% We are now in the position to introduce our network inspection problem, which we define as a mathematical program with equilibrium constraints.

\rev{We are now in the position to introduce our network inspection problem, which we define as a sequential game. In this problem, the defender (referred to as player 1 or \defender) is the leader and selects an inspection strategy $\sigma^1 \in \Delta(\mathcal{A}_1)$. The attacker (referred to as player 2 or \attacker) is the follower and selects an attack strategy $\sigma^2 \in \Delta(\mathcal{A}_2)$ after observing $\sigma^1$. Note that the attacker does not observe the realization of $\sigma^1$. We consider that the model parameters $(\mathcal{G}, b_1, b_2)$ are common knowledge. }



% We also assume that the attacker knows the defender's inspection strategy $\sigma^1 \in \Delta(\mathcal{A}_1)$, but does not know the realization of $\sigma^1$ [Justification]. 
\rev{
\emph{Second stage:} Given an inspection strategy $\sigma^1 \in \Delta(\mathcal{A}_1)$, the attacker aims to find an attack strategy $\sigma^2 \in \Delta(\mathcal{A}_2)$ that maximizes the expected number of undetected attacks: 
\begin{align}
U(\sigma^1,\sigma^2)\coloneqq \mathbb{E}_{(\sigma^1,\sigma^2)}[|\att| - \valdet{\Def}{\att}].\label{payoff2}
\end{align} 
We denote $B_2(\sigma^1,b_2)\coloneqq \argmax_{\sigma^2 \in \Delta(\mathcal{A}_2)}U(\sigma^1,\sigma^2)$ the set of attack strategies that are best responses to $\sigma^1$.

\emph{First stage:} The defender is interested in protecting the network against attacks with minimum resources. To evaluate the level of protection of the network, we define the following metric of detection performance against attacks: 
For a given a strategy profile $\sigma \in \Delta(\mathcal{A}_1) \times \Delta(\mathcal{A}_2)$, the \emph{expected detection rate}, denoted $\sdet{}$, is the expectation (under $\sigma$) of the ratio between the number of attacks that are detected and the total number of attacks:
\begin{align}
\sdet{} \coloneqq \Expboth{}{}{\dfrac{\valdet{\Def}{\att}}{|\att|}}. \label{Exp_detection_rate}
\end{align}
Then, given the attacker’s resources $b_2$, the defender seeks to determine a minimum-resource inspection strategy (i.e., to minimize the number of detectors $b_1$ and strategically position them in the network), while ensuring that the expected detection rate is no less than a pre-specified threshold level $\alpha\in [0,1]$ \rev{for any best response strategy of the attacker}. 

[In the definition of the game in this section, should I use ``\defender'' and ``\attacker'' instead of ``defender'' and ``attacker''?]

The network inspection problem can be formulated as the following bilevel optimization problem:\hypertarget{(P)}{}
%\vspace{-0.3cm}
%Finally, we present the  network inspection problem, where we use the expected detection rate in equilibrium of the game $\Gamma$ as metric of strategic inspection performance.
%Consider the problem in which \defender is concerned with inspecting the network, while facing a strategic adversary \attacker whose attack capability is constrained by $b_2$. In this  problem, \defender aims to minimize the number of detectors, $b_1$, and strategically position them to ensure that the expected detection rate in any equilibrium of the induced game $\Gamma(b_1,b_2)$ does not fall below a pre-specified threshold. Formally, the network inspection problem can be posed as follows:\hypertarget{(P)}{}
% \begingroup
% \addtolength{\jot}{\spacingalign}
\begin{align}
(\mathcal{P}): \quad \underset{b_1,\, \sigma^{1}}{\text{minimize}}& \quad b_1\nonumber\\
\text{subject to}& \quad r(\sigma^{1},\sigma^{2^*}) \geq \alpha,  \quad \forall \sigma^{2^*} \in B_2(\sigma^{1},b_2) \label{all_NE}\\
& \quad \sigma^1 \in \Delta(\mathcal{A}_1)\nonumber \\
& \quad b_1 \in \mathbb{N}.\nonumber
\end{align}
% \endgroup


Constraints \eqref{all_NE} ensure that, given the number of attack resources $b_2$, the expected detection rate induced by the chosen number of detectors $b_1$ and their positioning $\sigma^1$ is at least $\alpha$ whenever the attacker plays a best response to $\sigma^1$. The optimal value of \ECOP, denoted $b_1^*$, is the minimum number of detectors for which constraints \eqref{all_NE} are satisfied. 
% Thus, $(b_1^\dag,\sigma^\dag)$ with $\sigma^\dag\in\nash(b_1^\dag,b_2)$ is an optimal solution of \ECOP, where the inspection strategy in $\sigma^\dag$ specifies a randomized positioning of $b_1^\dag$ detectors.
The target detection rate $\alpha$ reflects the performance requirement that the defender seeks to achieve against the attacker's strategy, besides seeking a minimum-resource inspection strategy.

}


% use the notations $U(\Def,\att) = U(\mathds{1}_{\{\Def\}},\mathds{1}_{\{\att\}})$ and $r(\Def,\att) = r(\mathds{1}_{\{\Def\}},\mathds{1}_{\{\att\}})$.}


For ease of exposition, we denote $\valdet{i}{e} \coloneqq \valdet{\{i\}}{\{e\}}$,  \rev{for all} $(i,e) \in \nodes \times \edges$.  \rev{We will also refer to the degenerate mixed-strategies $\mathds{1}_{\{\Def\}} \in \Delta(\mathcal{A}_1)$ and  $\mathds{1}_{\{\att\}} \in \Delta(\mathcal{A}_2)$ as $S$ and $T$.}  The \emph{support} of $\sigma^1 \in \Delta(\mathcal{A}_1)$ (resp. $\sigma^2 \in \Delta(\mathcal{A}_2)$) is defined as $\supp(\sigma^1) = \{\Def \in \mathcal{A}_1 \ | \ \sigma^1_{\Def} >0 \}$ (resp. $\supp(\sigma^2) = \{\att \in \mathcal{A}_2 \ | \ \sigma^2_{\att} >0 \}$). The \emph{node basis} of a strategy $\sigma^1 \in \Delta(\mathcal{A}_1)$, denoted  $\nbasis{\sigma^1}\coloneqq \{i \in \nodes \ | \ \mathbb{P}_{\sigma^1} (i \in \Def)>0\}$, is the set of nodes that are inspected with non-zero probability. Analogously, the \emph{component basis} of a strategy $\sigma^2 \in \Delta(\mathcal{A}_2)$, denoted $\ebasis{\sigma^2}\coloneqq\{e \in \edges \ | \ \mathbb{P}_{\sigma^2}(e \in \att) >0\}$, is the set of components that are targeted with positive probability.  %Finally, we refer to defender and attacker as \defender and \attacker, respectively. 
%\tb{[This is said when the game is defined, but you chose not to use P1/P2 in the discussion that followed]}

\rev{[$\uparrow$ These two paragraphs may be swapped $\downarrow$]}

% Despite its simplicity, the game $\Gamma(b_1,b_2)$
\rev{The problem \ECOP} captures some of the key features of network inspection in strategic settings; see Table~\ref{List_app} for a comparison of various applications. Firstly, the underlying detection model $\mathcal{G}$ is generic in that it represents the detection capability of the defender, without making further modeling assumptions about how the monitoring sets $\set{i}$, $i\in\nodes$, depend on specific aspects such as sensing technology employed by the detectors, the different means that the attacker may use in targeting a component, and the network's topological structure. Secondly, it considers multiple resources on the part of both defender and attacker. This is a particularly desirable feature for strategic inspection settings, in which the attacker can simultaneously attack multiple components across the network, and the defender's inspection involves positioning multiple detectors \rev{[Still trying to propose the idea of coordination: ``the defender's inspection involves coordinating the positioning of multiple detectors'']} in order to monitor a large number of critical components.
%This feature is characteristic of situations in which the defender (resp. attacker) has the capability to simultaneously inspect (resp. attack) multiple nodes (resp. components) across the network.  \tg{Thirdly, our game is large-scale in that both players have combinatorial action sets. Indeed, in inspecting networks with a large number of critical components that can be arbitrarily targeted by a resource-constrained attacker, the defender faces the issue of choosing subsets of detector positionings and the corresponding inspection probabilities.}
%
In contrast, the previously studied security games typically assume that one or both players are constrained to using only a single resource; see Table~\ref{List_games}. \rev{[Although the mentioned security games are simultaneous games and are not exactly like our new sequential game (for now), I believe that comparative sentence still works.]}



% the set of $\epsilon-$NE of the game $\Gamma(b_1,b_2)$. When there is no confusion, we will refer to $\Gamma(b_1,b_2)$, $\nash(b_1,b_2)$, and $\nash_{\epsilon}(b_1,b_2)$ simply as $\Gamma$, $\nash$, and $\nash_{\epsilon}$.%\endnote{From a game-theoretic viewpoint, a NE in mixed strategies describes the behavior of \defender and \attacker who play the game $\Gamma$ repeatedly against each other and ignore any strategic relationship in-between plays. Thus, NE in mixed strategies can be viewed as a stochastic steady state of the repeated interaction between players. By extension, we view $\epsilon-$NE as strategy profiles in which the players are almost at a stochastic steady state, i.e., no player has more than an incentive of $\epsilon$ to change her mixed strategy.} 

%Given the parameters $b_1$ and $b_2$, we denote $\nash(b_1,b_2)$ the set of NE of the game $\Gamma(b_1,b_2)$\rem{, which is nonempty since $\Gamma(b_1,b_2)$ is a finite game}.

%\begin{align}
%\forall i \in \{1,2\}, \ \forall \sigma^i \in \Delta(\mathcal{A}_i), \ U_i(\sigma^{i^\prime},\sigma^{-i^\prime}) \geq U_i(\sigma^i,\sigma^{-i^\prime}) - \epsilon. 
%\label{best_epsilon}
%\end{align}

%\section{General Case}




%\note{For now, I am vague... If you want, we can formally rewrite the monitoring problem here. For example, it could be to determine  $b_1$ and $\sigma^1$ such that (i) for any $\sigma^2$, $r_{\sigma} \geq \alpha$, or (ii) in equilibrium $r_{\sigma} \geq \alpha$.}


%\begin{example}[Water Contamination Scenario]
%Consider the network shown in Fig.~\ref{Example1}. Assume a sensing model in which a sensor placed at any node can monitor components at one-hop vertically, and at two hops horizontally. Thus, $\set{i_1} = \{e_1,e_2,e_3\}$, $\set{i_2} = \{e_1,e_2,e_4\}$, $\set{i_3} = \{e_1,e_2,e_5\}$, $\set{i_4} = \{e_4,e_6,e_7\}$, $\set{i_5} = \{e_5,e_6,e_8\}$, $\set{i_6} = \{e_3,e_9,e_{10}\}$, $\set{i_7} = \{e_7,e_9,e_{10}\}$, $\set{i_8} = \{e_8,e_9,e_{10}\}$.
%
%%%%---------------------------------------------------------------------------------------------------
%\def \sizefig {1.4cm}
%\def \scalefig {\small}
%\def \innersepfig {0.07cm}
%%%%---------------------------------------------------------------------------------------------------
%
%\begin{figure}[ht]
%\centering
%{\scalefig
%\begin{tikzpicture}[-,auto,x=\sizefig, y=\sizefig,
%  thick,main node/.style={circle,draw,inner sep = \innersepfig,black},main node2/.style={circle,black,draw,fill=blue!60,inner sep = \innersepfig},flow_a/.style ={gray!100}]
%\tikzstyle{edge} = [draw,thick,-,black]
%\tikzstyle{cut} = [draw,very thick,-]
%\tikzstyle{match} = [draw,very thick,black,-, dashed]
%\tikzstyle{flow} = [draw,line width = 1.5pt,->,gray!100]
%
%%\begin{scope}[yshift=0, xshift =-110]
%	\node[main node] (1) at (0,2) {$i_1$};
%	\node[main node] (2) at (1,2) {$i_2$};
%	\node[main node2] (3) at (2,2) {$i_3$};
%	\node[main node] (4) at (1,1) {$i_4$};
%	\node[main node] (5) at (2,1) {$i_5$};
%	\node[main node] (6) at (0,0) {$i_6$};
%	\node[main node] (7) at (1,0) {$i_7$};
%	\node[main node] (8) at (2,0) {$i_8$};
%	%\node[main node, draw=white] (7) at (3.5,-0.5) {\textbf{a}};
%	
%	\path[edge]	
%	%(2) component (5)
%	%(1) component  (2)
%	(1) component node[left]{$e_3$} (6)
%	(4) component node {$e_6$} (5)
%	(2) component[double,blue!80]  node {$e_2$} (3)
%	(2) component node[left] {$e_4$} (4)
%	(6) component node[below] {$e_9$} (7)
%	(7) component node[below] {$e_{10}$} (8)
%	%(3) component  (5)	
%	%(4) component  (6)
%	(5) component node {$e_8$} (8);
%
%	\path[edge]
%	(1) component[double,blue!80] node {$e_1$} (2)
%	(3) component[double,blue!80] node {$e_5$} (5)
%	(4) component node[left] {$e_7$} (7);
%%\end{scope}
%
%\end{tikzpicture}}
%
%\caption{Example network. The monitoring set $\set{i_3} = \{e_1,e_2,e_5\}$ is represented by the double blue components.} \label{Example1}
%\end{figure}
%


%Consider the problem \ECOP with the target expected detection rate $\alpha = 0.75$ and the number of attack resources $b_2 = 2$. For this small-sized problem, we can solve  \lpo and \lpt to compute the NE of $\Gamma$, and obtain  the expected detection rate in any NE for each $b_1 \in \mathbb{N}$; see Table~\ref{r_sigma_example}. Notice that for a given $b_1$, the expected detection rate is the same in any NE.
%\begin{table}[htbp]
%\centering
%\caption{Expected detection rate in equilibrium for every $b_1 \in \mathbb{N}$.}
%\def\arraystretch{\spacingtable}
%\begin{tabular}{|c|c|c|c|c|c|}\hline $b_1$ & 0 & 1 & 2 & 3 & $\geq 4$ \\\hline $\sdet{*}$ & 0 & $\frac{2}{7}$ & $\frac{4}{7}$ & $\frac{6}{7}$ & 1 \\\hline \end{tabular}
%\label{r_sigma_example}
%\end{table}
%
%From Table~\ref{r_sigma_example}, we conclude that the optimal value of (\hyperlink{(P)}{$\mathcal{P}$}) is $b_1^\dag = 3$, i.e., with  $3$ sensors, \defender is capable of detecting $\frac{6}{7} \geq \alpha$ of the failure events in equilibrium. However, as mentioned in Section~\ref{sec:Formal problem}, this method does not extend to larger networks, as it requires solving large \lpo and \lpt for each $b_1 \in \mathbb{N}$ and checking if the constraint on the expected detection rate in any equilibrium \eqref{all_NE} is met.

%\end{example}

%\subsection{Network Monitoring Problem}\label{sec:Formal problem}
%\tb{[Do we need an introductory sentence?]}
%

% More importantly, any strategy profile \rev{[Can we talk about strategy profiles in optimization problems?]} \rem{of the game $\Gamma(b_1,b_2)$} can be associated with a metric of detection performance against attacks. For a given strategy profile $\sigma \in \Delta(\mathcal{A}_1) \times \Delta(\mathcal{A}_2)$, we define this metric as the \emph{expected detection rate}, $\sdet{}$, which is the expectation (under $\sigma$) of the ratio between the number of attacks that are detected and the total number of attacks:
% \begin{align}
% \sdet{} := \Expboth{}{}{\dfrac{\valdet{\Def}{\att}}{|\att|}}. \label{Exp_detection_rate}
% \end{align}
% %\end{definition}

% We are now in the position to introduce our network inspection problem, which we define as a mathematical program with equilibrium constraints. In this problem, given the attacker's resources $b_2$, the defender seeks to determine a minimum-resource inspection strategy (i.e., to minimize the number of detectors $b_1$ and strategically position them in the network), while ensuring that the expected detection rate \rem{in any equilibrium of the game $\Gamma(b_1,b_2)$} is no less than a pre-specified threshold level $\alpha\in [0,1]$ \rev{for any \attacker's best response strategy}:\hypertarget{(P)}{}
% %\vspace{-0.3cm}
% %Finally, we present the  network inspection problem, where we use the expected detection rate in equilibrium of the game $\Gamma$ as metric of strategic inspection performance.
% %Consider the problem in which \defender is concerned with inspecting the network, while facing a strategic adversary \attacker whose attack capability is constrained by $b_2$. In this  problem, \defender aims to minimize the number of detectors, $b_1$, and strategically position them to ensure that the expected detection rate in any equilibrium of the induced game $\Gamma(b_1,b_2)$ does not fall below a pre-specified threshold. Formally, the network inspection problem can be posed as follows:\hypertarget{(P)}{}
% \begingroup
% \addtolength{\jot}{\spacingalign}
% \rem{\begin{align}
% (\mathcal{P}): \quad \underset{b_1,\, \sigma^\dag}{\text{minimize}}& \quad b_1\nonumber\\
% \text{subject to}& \quad \sdet{*} \geq \alpha, \quad \quad \forall \sigma^* \in \nash(b_1,b_2) \label{all_NE}\\
% & \quad \sigma^\dag \in \nash(b_1,b_2) \label{one_NE}\\
% & \quad b_1 \in \mathbb{N}.\nonumber
% \end{align}}
% \endgroup

% \begingroup
% \addtolength{\jot}{\spacingalign}
% \rev{\begin{align}
% (\mathcal{P}): \quad \underset{b_1,\, \sigma^{1^*}}{\text{minimize}}& \quad b_1\nonumber\\
% \text{subject to}& \quad r(\sigma^{1^*},\sigma^{2^*}) \geq \alpha, \quad \quad \forall \sigma^{2^*} \in B(\sigma^{1^*},b_2) \label{all_NE}\\
% & \quad b_1 \in \mathbb{N}.\nonumber
% \end{align}}
% \endgroup

% \begin{align}
% (\mathcal{P}): \quad \underset{b_1,\, \sigma^{1^*}}{\text{minimize}}& \quad b_1\nonumber\\
% \text{subject to}& \quad r(\sigma^{1^*},\sigma^{2^*}) \geq \alpha\\
% & \sigma^{2^*} \in \argmax U(\sigma^{1^*},b_2)\label{all_NE}\\
% & \quad b_1 \in \mathbb{N}.\nonumber
% \end{align}

% $$r =  -U + 1$$
% \rev{[Few questions: nothing guarantees me right now that the optimal detector positioning for $\mathcal{P}$ and the maximin problem (former game) are the same. Yet, $(\mathcal{P})$ needs the problem $\Gamma$ first, for the definition of best responses...]}
% \tb{New version that does not work:}
% \begin{align}
% (\mathcal{P}): \quad \underset{b_1,\, \sigma^1}{\text{minimize}}& \quad b_1\nonumber\\
% \text{subject to}& \quad r(\sigma^1,\sigma^2) \geq \alpha, \quad \quad \forall \sigma^2 \in \argmax |T| - F(S,T) \label{all_NE}\\
% & \quad \sigma^1 \in \Delta(\mathcal{A}_1) \label{one_NE}\\
% & \quad b_1 \in \mathbb{N}.\nonumber
% \end{align}

% \tb{New version that does not work:}
% \begin{align}
% (\mathcal{P}): \quad \underset{b_1,\, \sigma^1}{\text{minimize}}& \quad b_1\nonumber\\
% \text{subject to}& \quad \mathbb{E}_\sigma[|T| - F(S<T)] \leq (1-\alpha) \mathbb{E}_\sigma[|T|], \quad \quad \forall \sigma^2 \in \argmax |T| - F(S,T) \label{all_NE}\\
% & \quad \sigma^1 \in \Delta(\mathcal{A}_1) \label{one_NE}\\
% & \quad b_1 \in \mathbb{N}.\nonumber
% \end{align}

%\begin{align*}
%%\fbox{$
%\begin{array}{lrclcl}(\mathcal{P}): &\underset{b_1 \in \mathbb{N}, \sigma^\dag \in \Delta(\mathcal{A}_1)\times \Delta(\mathcal{A}_2) }{\text{minimize}} & &b_1 &&\\
%&\text{subject to} &&\sdet{*} \geq \alpha,&& \forall \sigma^* \in \nash(b_1,b_2)\\
%&&& \sigma^\dag \in \nash(b_1,b_2)\end{array}
%%$}
%\end{align*}

%\vspace{-0.3cm}


%where $\alpha \in [0,1]$ denotes the target detection performance that \defender must achieve (for e.g., to meet the operational requirements on limiting network losses due to attacks).Thus, $(b_1^\dag,\sigma^\dag)$ with $\sigma^\dag \in \nash(b_1^\dag,b_2)$ is an optimal solution of \ECOP, where the inspection strategy in $\sigma^\dag$ specifies a positioning of the $b_1^\dag$ detectors in equilibrium such that the target detection performance $\alpha$ is met. 


%\subsection*{?}


%Given a detector positioning $\Def\in 2^{\nodes}$ and a network component $e \in \edges$, $\valdet{\Def}{e}=\mathds{1}_{\{e \in \set{\Def}\}}$ determines whether or not $e$ is monitored by at least one detector positioned in $\Def$.



%\subsection{Model Discussion}

%Cite Tambe








%The definition of the detection model $\mathcal{G} = (\nodes,\edges,\{\set{i}, \ i \in \nodes\})$, along with the detection function $\detect$, enable us to model a variety of settings. Indeed, since no assumption is made on the nature of $\nodes$ and $\edges$, these sets can represent single locations in a network, as well as more complex combinatorial objects such as network paths. Additionally, no assumption is made on the monitoring sets $\set{i}$, for $i \in \nodes$. Thus, we can apply the detection model to different applications. The first example could be a ``physical'' detection, where the attacker targets pipes in a network, and the defender is an inspection agency that sends inspection teams to identify the resulting failures. If they do not have any sensing technology, then they need to manually inspect a pipe in order to detect a failure. In that case, $\nodes = \edges$, and $\forall i \in \nodes, \ \set{i} = \{i\}$, which is related to search games.

%However, the advantage of the monitoring sets is that they can model more complex physical settings, where a detector is again an agent (police officer) who patrols roads in order to find a hiding robber. In the setting where the agent can only find the robber if they hide in a safe-house along the road patrolled by the agent, then our model becomes can be applied, and is such that a ``node'' $i \in \nodes$ is a road taken by the agent, and $e \in \edges$ is a safe-house. Similarly, $\set{i}$ is the set of safe-houses along the road $i$.

%Baykal-Gursoy, Mavronicolas, Pita et al
%
%All of these works are subsumed by our model.
%
%Finally, our model also applies to settings where an inspector possesses a sensing technology to detect attacks occurring in her vicinity. For example, in the context of water networks, a failure event such as pipe burst or contamination event generates a signal which propagates through the network.  Depending on the sensors' technological features, and their locations in the network, the signal can then be identified for failure detection before it dissipates in the network. 
%\cite{Ost1415211920040901} and \cite{sensors:autom} argue that such a binary detection model can be considered.  This detection model is typically obtained based on the outcome of a threshold-based rule that determines the detectors' capability to monitor different types of attacks from each location \citep{allen:smart,doi:10.1061/(ASCE)WR.1943-5452.0000339,sensors:autom}. 
%
%
%Regarding the strategic game, one of the main generalization is the fact that we allowed both players to have multiple resources.

%While some works allow the attacker to have multiple resources, very few consider multiple resources for the inspector, as it increases the difficulty in solving the problem. We address this issue by deriving some structural results, based on game-theoretic and combinatorial arguments. In particular we exploit properties of the detection model, such as the submodularity of the detection function $\detect$. This enabled us to derive a rigorous solution approach.



%1) key features:
%important aspects of security games (check slides).
%
%
%
%Strategic defender-attacker game, with a generic sensing model.


%We emphasize the generality of our model. 
%First, no assumption on $\nodes$ and $\edges$.

%Practical settings where the detection function is relevant


%This was possible because we chose to make this abstraction of the detection model, and did not model the specific details, such as false alarm and misdetections.
%Additionally, we stress that the game is played on the critical components of the network, while there may be others that are not critical, hence not attractive targets to the attacker. However, we do not distinguish different levels of criticality among them.
%Note that criticality is not relevant to (patrolling) settings where the defender is an inspector who wants to catch a malicious person. 



%Aspect of erroneous detections. False alarm misdetections

%Criticality.

%It does not take into account for the heterogeneous criticality of components

%Nevertheless, since we deal with strategic aspects and not operational aspect of sensor scheduling, we do not account for specific modeling features such as errors in detections and communication bandwidth etc.





==> S7_conclusions.tex <==
%!TEX root = OR Manuscript V23.tex



==> Tables_and_Figures.tex <==
%!TEX root = OR Manuscript V23.tex

%\clearpage

\section*{Tables and Figures}


%\vspace{-0.5cm}

%---------------------------------------------------------------------

%\OneAndAHalfSpacedXI
%%\begin{table}[h]\footnotesize
%%\centering
%%\caption{List of applications of our network inspection problem.}
%%\begin{tabular}{|c|c|c|c|}
%%\hline Inspection setting & Network & Type of detector & Type of attacks  \\\hline%\hhline{|-||=|=|=|}
%%\hline Urban patrolling & city streets  & police unit & robbery \\
%%\hline Network security & information network & firewall & cyberattack on server \\
%%\hline Sensing of gas and water networks & gas and water pipelines & leak/pressure sensor & pipe disruption \\
%%%\hline Sensing of water networks & urban water network & contaminant sensor & contaminant  injection\\
%%\hline Interdiction of illegal goods & transportation network & police officer & drug trafficking  \\
%%\hline Infiltration game & water channel & electric cable & malicious infiltration \\\hline
%%\end{tabular}
%%\label{List_app}
%%\end{table}
%
%\begin{table}[h]\footnotesize
%%\renewcommand{\arraystretch}{\spacingcomput} 
%\centering
%\caption{Model comparisons.}
%\begin{tabular}{C{6em}|c|c|C{7.5em}|C{4.45em}|C{5.2em}|C{6.9em}|}
%\cline{2-7}  & \multicolumn{3}{c|}{Detection model} & Resources  &\multicolumn{2}{c|}{Combinatorial objects used } \\
% & \multicolumn{3}{c|}{(monitoring locations, components, monitoring sets)}&def./att.&\multicolumn{2}{c|}{for equilibrium characterization}\\
%%\hline \multicolumn{1}{|C{6em}|}{\textcolor{red}{Model}}  & $\nodes$ & $\edges$ &$\set{i}, \ i \in \nodes$ & $b_1 \geq 1$ $b_2 \geq 1$ & MSC & MSP\\
%\hline \multicolumn{1}{|C{6em}|}{\cite{karlin2016game}} & street roads & safe-houses &safe-houses located on road $i$ & $b_1 = 1$ $b_2 = 1$ & minimum line cover & maximum matching\\
%%\hline Sensing of gas/water networks & access points & pipes & pipes within detection range & ? & ? & ? \\
%\hline \multicolumn{1}{|C{6em}|}{\cite{Garnaev1997}} & cable locations& channel sections& sections covered from the cable's location $i$ & $b_1 = 1$ $b_2 = 1$ & minimum interval cover & maximum independent infiltration set \\
%\hline \multicolumn{1}{|C{6em}|}{\cite{mavronicolas}} & network edges & network nodes & end nodes of edge $i$  & $b_1 = 1$ $b_2 \geq 1$ & minimum edge cover & maximum independent set\\
%\hline \multicolumn{1}{|C{6em}|}{Network path interdiction} & network edges & network paths & paths containing edge $i$& $b_1 = 1$ $b_2 = 1$ & minimum cardinality cut set & maximum edge-disjoint paths \\
%\hline \multicolumn{1}{|C{6em}|}{\textcolor{red}{our model}} & \textcolor{red}{sensing locations} & \textcolor{red}{network components} & \textcolor{red}{components monitored by sensing node $i$} & \textcolor{red}{$b_1 \geq 1$ $b_2 \geq 1$} & \textcolor{red}{minimum set cover} & \textcolor{red}{maximum set packing } \\\hline
%\end{tabular}
%\label{List_games}
%\end{table}
%
%%
%
%%\vspace{-5cm}
%%
%\ifarXiv
%\OneAndAHalfSpacedXI
%\else
%\DoubleSpacedXI
%\fi

%\DoubleSpacedXI
%
%\begin{table}[h]\footnotesize
%  \centering
%  \caption{Network data and computational results, $\alpha = 0.75$.}
%\tabcolsep=0.09cm
%	\renewcommand{\arraystretch}{\spacingcomput} 
%    \begin{tabular}{|c|ccc|cc|cc|c|c|c|}
%\hline
%   	 \multirow{ 2}{*} {\textbf{Network}} &  \textbf{Total length} &  \textbf{No. of}  &  \textbf{No. of} &  
% \textbf{Running}& \textbf{time} [s]&\multirow{ 2}{*} {$\mathbf{m^*}$}& \multirow{ 2}{*} {$\mathbf{n^*}$}& \multirow{ 2}{*} {$\mathbf{\lceil \alpha \smsc \rceil}$} & \textbf{Optimality} & \textbf{Relative loss}\\
%    &  \textbf{$[km]$} & \textbf{pipes}   & \textbf{nodes}&(\hyperlink{(MSP)}{$\mathcal{I}_{\text{MSP}}$})& (\hyperlink{(MSC)}{$\mathcal{I}_{\text{MSC}}$})&& && \textbf{gap}& \textbf{of performance}\\
%\hline
%   \textbf{bwsn1}   & 37.56 & 168   & 126 &  0.05 & 0.11 & 7 &7 & 6 & 0\,\% & 0\,\% \\
%    \textbf{ky3}  & 91.29 &  366   & 269 &  0.01 & 0.03 & 15 & 15 & 12 & 0\,\% & 0\,\% \\
%    \textbf{ky5}  & 96.58 &  496   & 420 &  0.02 & 0.05 & 18 & 19 & 15& 1 (7.14\,\%)& 5.3\,\% \\
%    \textbf{ky7}  & 137.05 &  603   & 481 &  0.09 & 0.08 & 28 & 28  & 21 & 0\,\% & 0\,\%\\
%    \textbf{ky6}  & 123.20 &644   & 543 &   0.08 & 0.06 & 24 & 24 & 18 & 0\,\% & 0\,\%\\
%    \textbf{ky1}  & 166.60 & 907   & 791 & 0.03 & 0.08 & 31 & 31 & 24 & 0\,\% &  0\,\%\\
%    \textbf{ky13}  & 153.30 & 940   & 778 &  0.06 & 0.08 & 28 & 30 & 23 & 2 (9.52\,\%)& 6.7\,\%\\
%    \textbf{ky2}  & 152.25 & 1124  & 811 &  0.39 & 0.41 & 18 & 19 & 15& 1 (7.14\,\%)& 5.3\,\%\\
%    \textbf{ky4}  & 260.24 & 1156  & 959 & 0.03 & 0.05 & 62 & 64 &  48 & 1 (2.13\,\%) &3.1\,\%\\
%    \textbf{ky8} & 247.34 & 1614  & 1325 &  0.14 & 0.22 & 45 & 45 & 34 & 0\,\% & 0\,\%\\
%    \textbf{dover} & 779.86 &  16000 & 14965  &  4.34 & 8.36 & 119 & 121 & 91 & 1 (1.11\,\%)& 1.7\,\%\\
%    \textbf{bswn2} & 1,844.04 &  14822 & 12523  & 0.77 & 4.06 &  352 & 361 & 271 & 7 (2.65\,\%)& 2.5\,\%\\
%   % \textbf{Net13 (FCPH)} & 341.26 & 19402  & 15622 & \tb{38} & \tb{79} & 91.80 & 107.77 & \tb{bad}\\
%    \textbf{mnsr} & 476.67 &  25484 & 24681  & 58.89 & 68.67 & 50 & 52 & 39 & 1 (2.63\,\%) & 3.8\,\%\\
%% \textbf{Net11} & 760.89 & 3032 & 1891 \\
%% \textbf{Net12}& 1844.04 & 14822  & 12523 \\
%\hline
%    \end{tabular}
%  \label{tab:4}%
%\end{table}%

%\newpage

%\section*{Figures}
 
%\vspace{-10.5cm}
%
%\OneAndAHalfSpacedXI
%
%%\vspace{-1.5cm}
%
%\begin{figure}[h]
%\centering
%%\begin{tikzpicture}[x=0.65cm,y=0.57cm]
%\begin{tikzpicture}[x=0.8cm,y=0.58cm]
%% horizontal axis
%
%\def \FontFig {\small}
%\draw[thick][->] (0,0) -- (12,0) node[anchor=north] {\FontFig$b_1$};
%% labels
%\draw	(0,-0.1) node[anchor=north] {\FontFig$0$}
%		(6,-0.1) node[anchor=north] {\FontFig$n^*$};
%
%\draw[thick] (6,-0.07) -- (6,0.07);	
%		
%% vertical axis
%\draw[thick][->] (0,0) -- (0,5) node[anchor=east] {\FontFig$b_2$};
%
%% labels
%\draw	(-0.1,2.5) node[anchor=east] {\FontFig$m^*$};		
%\draw[thick] (-0.07,2.5) -- (0.07,2.5);	
%
%% lines
%\draw[thick] (6,0) -- (6,5);
%\draw[thick] (6,2.5) -- (0,2.5);
%
%		
%
%%\draw	(2,2.4) node{\small{\textcolor{blue}{$\supp(\sigma^{1^*})=\{\flow^0\}$}}}
%%		(2,1.6) node{\small\textcolor{red}{$\supp(\sigma^{2^*})=\{\att^0\}$}}
%%		(5,1.4) node[anchor=west]{\small\textcolor{blue}{$\supp(\sigma^{1^*})=\{\flow^{\ast}\}$}}
%%		(5,0.6) node[anchor=west]{\small\textcolor{red}{$\supp(\sigma^{2^*})=\{\att^{0}\}$}}
%%		(5,3.4) node[anchor=west]{\small\textcolor{blue}{$\supp(\tilde{\sigma}^1)=\{\flow^0,\flow^{\ast}\}$}}
%%		(5,2.6) node[anchor=west]{\small\textcolor{red}{$\supp(\tilde{\sigma}^2)=\{\att^{0},\att^{min}\}$}};
%%
%%\draw	(3.5,3.5) node {\small\textbf{I}};
%%\draw	(9.5,1.5) node {\small\textbf{II}};
%%\draw	(9.5,3.5) node {\small\textbf{III}};
%%\draw	(11,3) node {\small(mixed NE)};
%%\draw	(11,1) node {\small(pure NE)};
%%\draw	(1.75,3.5) node {\small(pure NE)};
%
%%\draw[rounded corners=5,draw=black,fill=red,opacity=0.2]  (6.05,0.05) rectangle (11.95,4.95);
%%\draw[rounded corners=5,draw=black,fill=blue,opacity=0.2]  (0.05,3.05) rectangle (5.95,4.95);
%\draw[draw=black,fill=gray,opacity=0.2]  (0.02,0.02) rectangle (5.98,2.48);
%
%\draw	(9,2.85) node{\FontFig\textcolor{black}{Complete monitoring}};
%\draw	(9,2.15) node{\FontFig\textcolor{black}{(trivial game)}};
%
%\draw	(3,4.1) node{\FontFig\textcolor{black}{Redundant attacks}};
%\draw	(3,3.4) node{\FontFig\textcolor{black}{(easy detections)}};
%
%\draw	(3,1.6) node{\FontFig\textcolor{black}{Case of interest}};
%\draw	(3,0.9) node{\FontFig\textcolor{black}{(large network)}};
%
%%\draw[red,thick] (3,1.47) ellipse (1.65cm and 0.83cm);
%
%
%
%\end{tikzpicture}
%
%\vspace{-0.2cm}
%
%\caption{Equilibrium regimes with respect to the players' resources $b_1$ and $b_2$.}
%\label{Regimes}
%\end{figure}




%\ifarXiv






